Tight bounds for maximum $\ell_1$-margin classifiers

Popular iterative algorithms such as boosting methods and coordinate descent on linear models converge to the maximum $\ell_1$-margin classifier, a.k.a. sparse hard-margin SVM, in high dimensional regimes where the data is linearly separable. Previous works consistently show that many estimators relying on the $\ell_1$-norm achieve improved statistical rates for hard sparse ground truths. We show that surprisingly, this adaptivity does not apply to the maximum $\ell_1$-margin classifier for a standard discriminative setting. In particular, for the noiseless setting, we prove tight upper and lower bounds for the prediction error that match existing rates of order $\frac{\|w^*\|_1^{2/3}}{n^{1/3}}$ for general ground truths. To complete the picture, we show that when interpolating noisy observations, the error vanishes at a rate of order $\frac{1}{\sqrt{\log(d/n)}}$. We are therefore first to show benign overfitting for the maximum $\ell_1$-margin classifier.

==> sections/abstract.tex <==
\vspace*{3 cm}
\section*{Abstract}
Popular iterative algorithms such as boosting methods and coordinate descent are shown to converge in the linear case to the maximum $\ell_1$-margin classifier, a.k.a. sparse hard-margin SVM. Previous works consistently show that estimators relying on the $\ell_1$-norm adapt to hard sparsity of the ground truth, i.e. their statistical rates improve under this assumption. In this thesis we show that surprisingly, this adaptivity does not apply to the maximum $\ell_1$-margin classifier for a standard discriminative setting. In particular, for the noiseless setting, we prove tight upper and lower bounds for the directional estimation error that match existing  rates of order $\frac{\|\wgt\|_1^{2/3}}{n^{1/3}}$  for general ground truths. To complete the picture, for noisy observations where a constant fraction of the labels are flipped, we show that the error vanishes at a rate of order $\frac{1}{\sqrt{\log(d/n)}}$. Our results therefore complement the literature on ``benign overfitting’' for  maximum $\ell_p$-margin classifiers.

\vspace*{4cm}
\section*{Acknowledgements}
I would like to thank Prof. Fanny Yang for giving me the opportunity to work on this thesis and welcoming me as a part of her research group. I am especially grateful to my supervisor PhD student Konstantin Donhauser for inspiring discussions, valuable insights and continuous support during the last year. At the end, I would like to thank all other people that were part of my program at ETH during my master's studies.

==> sections/acknowledgements.tex <==
\vspace*{6 cm}


==> sections/conclusion.tex <==
% \section{Future Work and Conclusion}

% \subfile{sectionsAISTATS/future_work}
\subfile{sectionsAISTATS/conclusion}

==> sections/introduction.tex <==
% \section{Introduction}
\subfile{sectionsAISTATS/intro}










\paragraph{Organization of the document}
In the next section, we briefly review the main motivating ideas for compressed sensing, with a special focus on $1$-bit compressed sensing. Then, we present max $\ell_1$-margin classifiers and give a quick overview of the known recovery guarantees for this type of classifier. We also discuss their connection to AdaBoost and random hyperplane tesselations. 

Then, in Section 3 we give our two main results - risk bounds for the noiseless and noisy setting, and at the end of the chapter we discuss why our methodology gives tighter bounds compared to the analysis based on random hyperplane tesselations.

In Section 4, we present the proofs of the two main theorems - the first four subsections are common for both proofs, and in subsections 4.5 and 4.6 we separately prove the remaining parts of Theorems 3 and 4.

Finally, in Section 5, we give remarks about the future work and conclusion.

The appendix is reserved for technical results used in the proofs of Theorems 3 and 4.


\newpage
\section{Background}
In this section we give a quick overview and motivation of compressed sensing. In particular, we are interested in the $1$-bit compressed sensing, that aims to recover a signal only based on $1$-bit measurements. Furthermore, since we can consider this $0-1$ measurements as two separate classes, this motivates restating the problem as a classification task, where we aim to recover the underlying decision surface for these two classes. In this thesis, we consider max $\ell_1$-margin classifiers, which we present later in this section. Finally, we give a short introduction to the Gaussian Minimax Theorem (GMT) which is a cornerstone of our further analysis. 
\subsection*{Compressed Sensing}
One of the pillars of signal processing, the Nyquist-Shannon sampling theorem, states that uniform sampling of a continuous, band-limited signal with Nyquist rate is sufficient for perfect signal recovery. 
% A similar recovery result holds for discrete signals where the number of measurements is at least as large as the dimensionality of the signal. 
However, a new sampling and reconstruction method called compressed sensing \cite{donoho2006compressed,candes2006robust,candes2006near} shows that for special types of signals that are compressible on some basis, the signal can be recovered even when sampling below the Nyquist frequency. 

Assume that our ground-truth signal $\wgt\in\RR^d$ is $s$-sparse in a basis, and without loss of generality assume that this is the canonical basis $\{ e_i\}_{i=1}^d$. The signal is sampled using $n$ measurements $\{y_i\}_{i=1}^n$ with some measurement vectors $x_i \in \RR^d$ i.e. $y_i = \langle x_i, \wgt \rangle$. Now, the motivating question of compressed sensing is: what is the minimal number of measurements $n$ necessary to recover the signal and, especially, when is it possible to recover the signal for $n<<d$. Note that for any $n<d$ the problem is equivalent to solving an underdetermined system of linear equations that generally does not have a unique solution.

In general, without any assumption on the structure of $\wgt$, we would require at least $d$ measurements for recovery of $\wgt$. On the other hand, compressed sensing enables recovery of a $s$-sparse signal $\wgt$ with high probability already with $n \asymp s \log(\frac{d}{s})$ measurements \cite{candes2006near}, a much smaller number under the assumption that $s << d$.

The main idea of compressed sensing is to take advantage of the sparsity of the signal, and out of all solutions that interpolate the data, choose the one with the smallest support, i.e. choose:
\begin{align}
    \what = \argmin_w \norm{w}_0 \subjto y_i = \langle x_i, w \rangle,  \quad i=1,2,\dots,n
    \label{eq:l0_norm_opt_problem}
\end{align}
where $\norm{w}_0:=|\supp(w)|$ is the $\ell_0$-pseudonorm. But, solving problem \eqref{eq:l0_norm_opt_problem} is computationally very expensive, since it is considered to be an NP-hard combinatorial problem \cite{candes2008introduction}. However, it has been shown \cite{donoho2006most} that under certain conditions it is possible to recover the signal $\wgt$ even by solving the "convexified" version of problem \eqref{eq:l0_norm_opt_problem} called Basis pursuit \cite{chen_1998} given by:
\begin{align}
    \what = \argmin_w \norm{w}_1 \subjto y_i = \langle x_i, w \rangle, \quad i=1,2,\dots,n
    \label{eq:l1_norm_opt_problem}
\end{align}
where the $\ell_1$ norm is given by $\norm{w}_1 = \sum_{i=1}^d \abs{w_i}$. Note that the problem \eqref{eq:l1_norm_opt_problem} is convex and solvable in polynomial time \cite{candes2008introduction}.

We now illustrate a simple sufficient condition for the signal $\wgt$ to be recovered using \eqref{eq:l1_norm_opt_problem}. Denote by $\SSS$ the set of indices on which $\wgt$ is supported, arrange the vectors $x_i$ as columns of matrix $X\in \RR^{n\times d}$ and note that the constraints of \eqref{eq:l1_norm_opt_problem} can be succinctly written as $y = Xw$ for the measurement vector $y\in\RR^n$. 

To recover $\wgt$ using \eqref{eq:l1_norm_opt_problem}, it is enough to show that $\sum_i |\what_i+v_i| > \sum_i |\what_i|$ for any $v\in\NNN(X)$, where $\NNN(X)$ is the nullspace of matrix $X$. Now, note that this inequality is true if $ \sum_{i\not\in\SSS} |v_i| > \sum_{i\in\SSS} |v_i| $ since:
\begin{align}
    \sum_i |\what_i+v_i| - \sum_i |\what_i| \geq \sum_{i\in\SSS} |\what_i+v_i| + \sum_{i\not\in\SSS} |v_i| - \sum_{i\in\SSS} |\what_i| \geq  \sum_{i\not\in\SSS} |v_i| - \sum_{i\in\SSS} |v_i|  > 0
\end{align}
With that in mind, we define a set $C(\SSS) := \{ v\in \RRR^d: \sum_{i\in \SSS^c} \abs{v_i} \leq \sum_{i\in\SSS} \abs{v_i}\}$. Now it is fairly easy to see that $\wgt$ is recovered using \eqref{eq:l1_norm_opt_problem} if $C(\SSS)\cap \NNN(X) = \{0\}$ i.e. if matrix $X$ satisfies the so-called Restricted Null-Space Property (RNSP). Thus, to recover the signal using \eqref{eq:l1_norm_opt_problem} it is sufficient to show that the matrix $X$ satisfies RNSP. Although simple, this condition is not easily verifiable in practice. However, if $X$ satisfies the so-called restricted isometry property i.e. it satisfies:
\begin{align}
    (1-c_{2s}) \norm{w}_2^2 \leq \norm{Xw}_2^2 \leq (1+c_{2s}) \norm{w}_2^2
\end{align}
for all $2s$-sparse vectors $w$ with constant $0<c_{2s}<\sqrt{2}-1$, then $X$ also satisfies RNSP, and thus, by our previous discussion, \eqref{eq:l1_norm_opt_problem} recovers $\wgt$ perfectly \cite{candes2006stable}.

In the case of random matrices $X$ with i.i.d. Gaussian entries and even more general sub-Gaussian distributions, matrix $X$ satisfies $c_{2s}<\sqrt{2}-1$ provided that $n\gtrsim s\log \left( \frac{d}{s}\right)$ \cite{candes2008introduction}, which is exactly the minimal number of measurements we mentioned at the beginning of this section. Moreover, this result motivates the use of random sensing matrices, which we also exploit in our work later in the thesis.

Furthermore, this result can be generalized to non-$s$-sparse ground-truth signals and is robust to noisy measurements. Namely, let the sensing matrix $X$ be Gaussian and the measurements be given by $y_i = \langle x_i, \wgt \rangle + \xi_i$ for some bounded noise $\xi_i$. Then the stability results \cite{candes2006stable,wojtaszczyk_2010} claim that for $\what$ from \eqref{eq:l1_norm_opt_problem} holds $\norm{\what-\wgt}_2 \lesssim \frac{1}{\sqrt{n}}\norm{\xi}_2 + \frac{1}{\sqrt{s}} \inf_{\norm{w}_0\leq s} \norm{\wgt-w}_2$ under some assumptions on $n,d,s$.
   


\subsection*{1-bit Compressed Sensing}
Robustness of compressed sensing algorithms is crucial for practical implementations, as obtaining perfect measurements is not a valid assumption in most experiments. Modern signal acquisition is based on quantization of the input signal, thus introducing additional error in measurements. This noise can usually be reduced by increasing the number of quantization levels. The trade-off depends on the cost of more quantization levels versus the cost of additional measurements. One way to analyze this trade-off is by considering two extreme cases. The first, in which we have perfect measurements without quantization, can be analyzed using standard tools from compressed sensing, mentioned in the previous section. The second extreme case in which we obtain only one bit of information per measurement is at the heart of 1-bit compressed sensing \cite{boufounos2008}.

What we mean by $1$-bit measurements is that the measurements are given by $y_i = \sign \langle x_i, \wgt \rangle$, using the notation from the previous section. In other words, our quantizer takes the form of the comparator to zero, similar to the efficient Sigma-Delta converters \cite{aziz1996overview}. Besides this efficient hardware implementation, $1$-bit CS has certain advantages when the signal-to-noise ratio (SNR) is low \cite{laska2012regime}.

It has been noted that the use of standard compressed sensing tools for $1$-bit measurements and modeling quantization as noise do not provide a good reconstruction \cite{plan2013one}. Instead, the goal of the recovery method proposed in \cite{boufounos2008} is consistent reconstruction, which means that if the reconstructed signal $\what$ was measured using our system, the measurements obtained would be exactly the same as the ones obtained for the ground truth $\wgt$. In other words, similarly to \eqref{eq:l1_norm_opt_problem} we aim to recover the signal as follows:
\begin{align}
    \what = \argmin_w \norm{w}_1 \subjto y_i = \sign \langle x_i, w \rangle, \quad i=1,2,\dots,n
    \label{eq:1bit_cs_opt_problem}
\end{align}
Note that the constraint can be equivalently written as $\min_{1\leq i\leq n} y_i \langle x_i, w\rangle \geq 0$ and that the norm of the ground truth $\normk{\wgt}_2$ is lost in the measurements, so we should aim to recover $\wgt$ up to scaling. Thus, we will assume without loss of generality that $\norm{\wgt}_2=1$. Furthermore, the optimization problem \eqref{eq:1bit_cs_opt_problem} is not well defined, since $\norm{\what}_1\to 0$ unless we impose an additional constraint on the norm of $\what$. One way to fix this issue is by adding the linear constraint $\norm{Xw}_1=n$ to \eqref{eq:1bit_cs_opt_problem} which can be replaced by a nonconvex constraint $\norm{w}_2=1$ as discussed in \cite{plan2013one}.

We denote by $\delta$ the recovery error defined by $\delta = \norm{\frac{\what}{\norm{\what}_2}-\wgt}_2$. The best achievable rates for exactly $s$-sparse $\wgt$ is $\delta = \Omega(\frac{s}{n})$ \cite{jacques2013robust}, and can be achieved up to logarithmic factors with algorithms proposed in \cite{jacques2013robust,gopi13}.

For the problems of the form~\eqref{eq:1bit_cs_opt_problem}, the majority of results are based on the random hyperplane tessellation arguments \cite{plan2014dimension,dirksen2021non} aiming to give the minimum number of hyperplanes needed to obtain a uniform tessellation of a subset of the Euclidean sphere. We refer reader to \cite{plan2013one} for a more thorough introduction to the topic, and we try to give the main idea behind the method here. Moreover, in Section~\ref{subsec:hyperplane} we compare our method with the ones based on tesselations and discuss why our method is superior in the setting we propose.


As we mentioned previously, we can assume that $\norm{\wgt}_2=1$. Further assume that $\wgt$ is effectively $s$-sparse implying that $\norm{\wgt}_1\leq \sqrt{s}$. Hence, we should be interested in tesselations of the set $\SSS^{d-1}\cap \sqrt{s}B_1^d$, where $\SSS^{d-1}$ is the unitary Euclidean sphere and $B_1^d$ is $\ell_1$-ball. Now, we can derive the minimal number $m$ of random hyperplanes needed for dividing this set into cells of diameter $\delta$ with high probability. In other words, if $\norm{w-\wgt}_2>\delta$ then at least one sign constraint must be different, and $w$ cannot be solution of~\eqref{eq:1bit_cs_opt_problem}. Thus, the number of measurements needed for $\delta$-recovery is equal to the number of random hyperplanes $m$.

Now we give an overview of the known recovery guarantees for problem~\eqref{eq:1bit_cs_opt_problem}. One of the initial tesselation proofs show that in the case of noiseless measurements one requires $n = O(\delta^{-5} s\log^2 \left(\frac{d}{s}\right))$ measurements \cite{plan2013one} to achieve recovery error $\delta$. Subsequent work has focused on regularized estimators and provided guarantees for recovering signal from noisy measurements. Namely, using a simple convex problem, signal recovery is possible both when the noise is random for $n = O(\delta^{-2} s \log d)$ and adversarial $n = O(\delta^{-6} s \log d)$ \cite{plan2012robust}. Similarly, \cite{zhang2014efficient} showed in the noisy setting that sample complexity is $n = O(\delta^{-2} s\log d)$ for exactly $s$-sparse, and $O(\delta^{-4} s\log d)$ for effectively $s$-sparse ground truths. Further bounds have been obtained in \cite{oymak2015near,knudson2016one,awasthi2016learning}, and even extension to heavy-tailed distributions has been considered in \cite{dirksen2021non,chinot_2021}. Another interesting direction of research was using adaptive quantization threshold, where even exponential decay in error rate has been shown \cite{baraniuk2017exponential}.

\subsection*{Max-\texorpdfstring{$\ell_1$}{l1}-margin interpolation}
The Support Vector Machine (SVM) is one of the most well-known and commonly used methods for binary classification in machine learning \cite{vapnik2006estimation, cortes1995support}. Assuming tha the data is linearly separable, the so-called hard-margin SVM solution $\what$ is the one that maximizes the minimum margin achieved on the $n$ training samples i.e. is given by:
\begin{align}
    \what = \argmin_w \norm{w}_1 \subjto \min_{1\leq i\leq n} y_i \langle x_i,w \rangle \geq 1 
    \label{eq:1bit_max_l1_opt_problem},
\end{align}
We denote the max-$\ell_1$-margin as $\Delta$ and define it as follows:
\begin{align}
    \Delta:= \max_{w\neq 0} \min_{1\leq i\leq n} \frac{y_i \langle x_i, w \rangle}{\norm{w}_1}
\end{align}
and for $\Delta>0$ we have that $\Delta = \frac{1}{\norm{\what}}_1$ \cite{chinot_2021}. SVM solution is known to possess good generalization properties when the number of support vectors is small compared to the size of training set $n$. However, recent success of overparametrized neural networks which achieve good generalization properties even when overfitting the noisy training data, is not fully understood by classical theory of classification. Similar phenomenon has been observed and analyzed in linear regression setting with high dimensional features, where it is known as benign overfitting \cite{bartlett2020benign,tsigler_2020}. Moreover, it has been observed in the regression tasks that under certain conditions and $d\asymp n\log n$, every training example becomes a support vector with high probability \cite{muthukumar2021classification,hsu2021proliferation}. This phenomenon called proliferation of support vectors, gives connection between hard-$\ell_2$-margin SVMs and min-$\ell_2$-norm interpolators \cite{hastie2022surprises, mei2022generalization, muthukumar2020harmless}.

Contrary to max-$\ell_1$-margin interpolation, the problem of min-$\ell_1$-norm interpolation (or Basis Pursuit) has been more widely studied in the literature. The upper bounds on the prediction error of the BP estimator from Equation~\eqref{eq:l1_norm_opt_problem} have been shown in \cite{wojtaszczyk_2010,foucart_2014,ju_2020,koehler2021uniform,chinot_2021}. In the case of isotropic Gaussian features and random noise, matching upper and lower bound have been shown in \cite{wang2021tight} using the similar methodology to what we propose in this thesis.

In the case of max-margin classifiers, the majority of the non-asymptotic results considers max-$\ell_2$-margin interpolation with special structure of the covariance matrix \cite{chatterji2021finite,wang2020binary,cao2021risk,muthukumar2021classification}. For the proportional regime in which $d\asymp n$, the asymptotic bounds has been derived for max-$\ell_2$-margin interpolation \cite{montanari2019generalization, deng2022model}, as well as for max-$\ell_1$-margin interpolation and boosting \cite{liang2022precise}. Interestingly, for the max-$\ell_p$-margin interpolation with $p\in(1,2)$, authors of \cite{donhauser2022fast} prove non-asymptotic bounds which are even minimax optimal. Finally, max-$\ell_1$-margin interpolation with adversarial noise is considered in \cite{chinot_2021}, where the authors prove only the upper bounds which are tight up to the logarithmic factors.

Now, we discuss a few open problems on this topic. First, almost all bounds derived are only upper-bounding the risk, and it is needed to show whether lower bounds of the same rate generally hold. Recently, matching bounds have been derived in \cite{wang2021tight} for min-$\ell_1$-norm interpolation, and also lower bounds for min-$\ell_p$-norm and general interpolating classifiers have been proven in \cite{donhauser2022fast}. Another open problem is proving bounds for random (non-adversarial) noise models, needed to complement work on adversarial noise in \cite{chinot_2021}. At the end, we also mention the open question of universality of all these bounds in the sense of underlying distribution of the feature vectors.

\subsubsection*{AdaBoost}
Adaptive Boosting (AdaBoost) is a classification algorithm that combines outputs of a number of weak learners into a weighted sum which is the final output of the classifier \cite{freund1997decision,schapire1998improved}. In each iteration of training, AdaBoost decreases the training error \cite{freund1997decision}, and is actually a variant of mirror-gradient-descent for the exponential loss \cite{breiman1998arcing, friedman2000additive}

Empirically it achieves the best generalization when the model is overparametrized and running long after achieving zero training error \cite{drucker1995boosting}. Moreover, in that setting AdaBoost classifier is known to have $\ell_1$-margin converging to the maximal $\ell_1$-margin \cite{ratsch2001soft, zhang2005boosting, rosset2004boosting}.

Thus, guarantees for max-$\ell_1$-margin classifiers can be used for giving guarantees for AdaBoost (see Corollaries 2.1, 2.2. and 2.3 in \cite{chinot_2021}). Obtaining tighter bounds for max-$\ell_1$-margin classifiers as proposed in this thesis is also useful in better understanding of asymptotic behaviour of AdaBoost.


% \subsubsection*{Comparison to \cite{chinot_2021}}
% We now discuss why methodology developed in \cite{chinot2021adaboost} fails to give optimal risk bounds in our setting. Although theorems  therein hold even for non-Gaussian random variables and for adversarial noise, authors fail to prove vanishing risk bounds as is the case in our Theorem \ref{thm:mainl1_class_noisy}. We show how bounds proposed in \cite{chinot2021adaboost} are not sufficiently tight to be able to claim consistency.


% \begin{theorem}[Theorems 2.1 and 2.2 in \cite{chinot_2021}]
% Assume $p\gtrsim n$ and that $\{X_i\}_{i=1}^n$ are i.i.d. $\NNN(0,I_d)$ random variables. Assume that $\wgt\in S^{d-1}$ is effectively $s$-sparse i.e. that it satisfies $\norm{\wgt}_2=1$ and $\norm{\wgt}_1 \leq \sqrt{s}$. Let $c>0$ be a universal constant and assume that $(\log p)^c (s+|\OOO|)=o(n)$ and $\frac{|\OOO |}{n} \lesssim $. Then with probability $1-c_1 n^{-1}$ we have that:
% \begin{align}
%      \norm{ \frac{\what}{\norm{\what}_2} - \wgt }_2 \lesssim \left( \frac{(\log p)^c (s+|\OOO|)}{n} \right)^{1/3}
% \end{align}
% \label{thm:geoffrey_thm}
% \end{theorem}

% We consider two cases of interest. First when $|\OOO|=0$ bound above scales as $\tO \left(\frac{s}{n}\right)^{1/3}$. Second case of interest is $|\OOO| =\kappa n$ for universal constant $\kappa \in (0,1)$ for which the rate above is $\tO(1)$.

% We now discuss why is proof given in \cite{chinot_2021} not tight. The proof of Theorem~\ref{thm:geoffrey_thm} is based on a result from random hyperplane tesselations which we discuss next. For $a>0$ define $\zeta(a) = c \left( a^2 \frac{(\log p)^2 \log n}{n} \right)^{1/3}$. Now fix $a$ and assume $\zeta(a)\lesssim 1$. Then according to Proposition 4.2 in \cite{chinot_2021} inequality:
% \begin{align}
%     \inf_{w \in a B_1^d \cap \SSS^{d-1} \cap \{ \norm{w-\wgt}_2  \geq \zeta(a) \} } \frac{1}{n} \sum_{i=1}^n \indicator{\sgn(\innerprod{x_i}{w})\neq\sgn(\innerprod{x_i}{\wgt})} \gtrsim \zeta(a)
% \end{align}
% holds with high probability. Then in proof of Theorem 2.1 in \cite{chinot_2021} it is shown that $\what \in a B_1^d \cap \SSS^{d-1}$ with $a$ obtainable from Theorem 2.2 in \cite{chinot_2021}. Then by showing that
% \begin{align}
%     \sum_{i=1}^n \indicator{\sgn(\innerprod{X_i}{w})\neq\sgn(\innerprod{X_i}{\wgt})} = \frac{\card{\OOO}}{n} \lesssim \zeta(a)
% \end{align}
% by contradiction follows that $\norm{w-\wgt}_2 \lesssim \zeta(a)$. Choosing $\zeta(a)=const\in(0,\frac{1}{2})$ implies only constant upper bound on the $\norm{w-\wgt}_2$, implying that used theorem is not tight in this case.





\subsection*{Tight bounds via CGMT}
In this section we discuss how application of Convex Gaussian Minimax Theorem (CGMT) \cite{gordon_1988, thrampoulidis_2015} gives a solid framework for obtaining tight bounds for interpolation \cite{koehler2021uniform,wang2021tight,donhauser2022fast}. The mathematically precise statement of a version of CGMT is given in Lemma~\ref{lemma:CGMT_variant} in Appendix, but for illustration purposes we will only use an application of CGMT from \cite{wang2021tight}.
% Let $X\in \RR^{n\times d}$ be a matrix with i.i.d. $\NNN(0,1)$ entries and let $G\sim\NNN(0,I_n)$, $H\sim\NNN(0,I_d)$ be independent of each other and of $X$. Define
% \begin{align}
%     \Phi(X) := \min_{w}\max_{u} \langle u,Xw \rangle + \psi(w,u)
% \end{align}
% \begin{align}
% \phi(G,H) := \min_{w} \max_{u} \norm{w}_2 \langle G,u \rangle + \norm{u}_2 \langle H,w \rangle + \psi(w,u)    
% \end{align}
% Then, under certain conditions on function $\psi$ and the sets over which we optimize, with high probability holds that $\Phi(X) \approx \phi(G,H)$.
% for any $t\in \RR$ holds that:
% \begin{align}
%     \PP(\Phi(X)<t)\leq 2\PP(\phi(G,H)\leq t) ~~\andtxt~~
%     \PP(\Phi(X)>t) \leq 2\PP(\phi(G,H)\geq t)
% \end{align}

In order to illustrate why is tightness of this theorem needed for obtaining the correct bounds, we will use regression setting from \cite{wang2021tight} which is exactly the one given in Equation~\eqref{eq:l1_norm_opt_problem}. However, we will assume that the measurements are corrupted by i.i.d. noise $\xi_i\sim\NNN(0,\sigma^2)$ and are of the form $y_i = \langle x_i,\wgt\rangle + \xi_i$, or in vector form $y = X w+\xi$.

One of the two main steps used in \cite{wang2021tight} is localization, where we need to estimate the following deterministic upper bound $M(n,d)$:
\begin{align}
    \Phi = \left[ \min_{w} \norm{w}_1 \subjto  X w=\xi \right] \leq M(n,d)
\end{align}
As discussed in \cite{wang2021tight}, $M(n,d)$ can be derived straightforwardly by using the CGMT, where instead of upper bounding $\Phi$, we upper bound an auxiliary optimization problem $\phi$. Let $H\sim\NNN(0,I_d)$ and $\phi$ given by
\begin{align}
\phi = \min_w \norm{w}_1 \subjto \frac{1}{n} \langle w,H\rangle^2 \approx \sigma^2+\norm{w}_2^2.
\label{eq:phi_regression_background}
\end{align}
Then, according to CGMT $\Phi \leq \phi$ with high probability \cite{wang2021tight}. Now, the optimization problem~\eqref{eq:phi_regression_background} is simpler for upper bounding since it is a function of one Gaussian random vector, whereas $\Phi$ depends on a Gaussian matrix. Thus, this way obtaining an upper bound on $\Phi$ gives very precise expression for $M(n,d)$. As discussed in Section 3.1 in \cite{wang2021tight}, choosing just a slightly looser upper bound $\widetilde{M}(n,d)$ would not result in matching upper and lower bound of order $\frac{\sigma^2}{\log(d/n)}$. Namely, they show that:
 \begin{enumerate}
     \item for $\widetilde{M}(n,d) = M(n,d)\left(1 +  \frac{c}{\log(d/n)^2}\right)$ with $c>0$: the risk bound stays the same
     \item for $\widetilde{M}(n,d) = M(n,d)\left(1 +  \frac{c}{\log(d/n)}\right)$ with $c>0$: the upper bound is of the correct order up to a multiplicative universal constant factor 
     \item for $\widetilde{M}(n,d) = M(n,d)\left(1 + c\right)$ with $c>0$:
     the upper bound is of the constant order, same as obtained before in \cite{chinot_2021,wojtaszczyk_2010}.
 \end{enumerate}

It should also be noted that combining the precise expression $M(n,d)$ with previous analysis such as in \cite{chinot_2021,wojtaszczyk_2010,koehler2021uniform} would also result in loose bounds. The other source of looseness addressed in \cite{wang2021tight} is the use of H\"olders inequality $\innerprod{w}{H} \leq \norm{w}_1 \norm{H}_{\infty}$ for upper bounding the term on the LHS of constraint from Equation~\eqref{eq:phi_regression_background}. Thus, as proposed in \cite{wang2021tight} it is needed to use a more refined analysis which better takes into account the relationship between $\innerprod{w}{\Hgaussian}, \|w\|_2$ and $\|w\|_1$, based on localized Gaussian width. For our specific setting, we address the same issue in Section~\ref{subsec:proof_path}.


==> sections/proof_props_loc_unicon.tex <==
\section{Proof of Propositions from Theorems~\ref{thm:mainl1_class_noisy} and \ref{thm:mainl1_class_noiseless}}

\input{sections/subsections_theory/noisy/loc_proof.tex}
\input{sections/subsections_theory/noisy/unicon_proof.tex}
\newpage
\input{sections/subsections_theory/noiseless/loc_proof.tex}
\input{sections/subsections_theory/noiseless/unicon_proof.tex}

==> sections/proof_structure.tex <==
% \section{Preliminary tools}
% We now present the proofs for Theorem~\ref{thm:mainl1_class_noiseless} and Theorem~\ref{thm:mainl1_class_noisy}. Both proofs rely on a standard localization/ uniform convergence proof (see e.g., \red{where}), where we:

% Let $X = \{x_i\}_{i=1}^n$ be the matrix of features
%  and let $\matXpar = \{(\xpar)_i\}_{i=1}^n$  of vectors onto the subspace spanned by $\wgt$ 

% Now, since $\RiskC(\what) = 2 -2\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$, in order to obtain a valid bounds for $\RiskC(\what)$ it is sufficient to bound $\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$. 

% The proof consists of two major parts: 
% \begin{enumerate}
%     \item \emph{Localization.}
%     We derive a  high-probability upper bound on the norm $\loneboundclasg$, which only depends on $\xi$ and $\matXpar$, of the max-$\ell_1$-margin interpolator $\what$ ,
%     by finding $\loneboundclasg>0$ such that
%     \begin{equation} \label{eq:PhiCN} \tag{$P_{\CCC,N}$}
%         \min_{ \forall i:\:y_i \langle \xui, w \rangle \geq 1}  \norm{w}_1
%         ~ =: \PhiCNuni
%         ~ \leq \loneboundclasg.
%     \end{equation}

%     \item \emph{Uniform convergence.}
%     Conditioning on $\xi$ and $\matXpar$, 
%     we derive high-probability uniform bounds on the classification error for all interpolators $w$ with  $\norm{w}_1 \leq \loneboundclasg$.
%     Namely, we find a high-probability lower and upper bound, respectively, for
%     \begin{align} \label{eq:PhiCm} \tag{$P_{\CCC,-}$} 
%         \PhiCmuni:&=\min_{\substack{
%             % \norm{w}_p^p \leq \gennormbound \\ % CONVENTION 1
%             \norm{w}_1 \leq \loneboundclasg \\ % CONVENTION 2
%              \forall i:\:y_i \langle \xui, w \rangle \geq 1
%         }}  \frac{\langle w, \wgt\rangle}{\norm{w}_2}
%         ,\\
%      \label{eq:PhiCp} \tag{$P_{\CCC,+}$} 
%          \PhiCpuni:&=\max_{\substack{
%             % \norm{w}_p^p \leq \gennormbound \\ % CONVENTION 1
%             \norm{w}_1 \leq \loneboundclasg \\ % CONVENTION 2
%              \forall i:\:y_i \langle \xui, w \rangle \geq 1
%         }} \frac{\langle w, \wgt \rangle}{\norm{w}_2} 
%     \end{align}
%     which in turn then gives us a high probability bounds for the classification error using that $\RiskC(\what) = 2 -2\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$. 
% \end{enumerate}


% \input{sections/subsections_theory/step_CGMT.tex}
% \input{sections/subsections_theory/step_path.tex}

% \input{sections/subsections_theory/proof_thm1.tex}
% \input{sections/subsections_theory/noisy/loc_sketch}
% \input{sections/subsections_theory/noisy/unicon_sketch}

% \input{sections/subsections_theory/proof_thm2.tex}
% \input{sections/subsections_theory/noiseless/loc_sketch}
% \input{sections/subsections_theory/noiseless/unicon_sketch}

% \input{sections/subsections_theory/step_tools.tex}

\newpage
\section{Proofs}
\label{sec:proofs_sketch_main}
\label{sec:proofsketch}
\subfile{sectionsAISTATS/cgmt_preliminary}
\input{sections/subsections_theory/step_tools}
\subfile{sectionsAISTATS/proof2_sketch}
\input{sections/subsections_theory/proof_thm2}
\input{sections/subsections_theory/noiseless/sloc_proof}
\input{sections/subsections_theory/noiseless/sunicon_proof}


\input{sections/subsections_theory/proof_thm1}
% \subfile{sectionsAISTATS/proof1_sketch}
\input{sections/subsections_theory/noisy/loc_proof}
\input{sections/subsections_theory/noisy/unicon_proof}


 
 

















==> sections/subsections_theory/intro_theory.tex <==
\subsection{Introduction}

==> sections/subsections_theory/noiseless/loc_proof.tex <==
% \subsection{Proof of Localization Proposition~\ref{prop:localization_noiseless}}
% Recall definition of $\PhiCndn$ from Proposition~\ref{prop:parametrization_class_noiseless}:
% \begin{align}
%     % \tag{$A_{\CCC_0,N}'$}\label{eq:PhiCndn_par}
%     \PhiCndn &= \min_{\nu,b,\alpha} |\nu|  + b \alpha
%     \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasn(\nu,b\|\gamma(\alpha)\|_2)
% \end{align}
% In order to upper bound $\PhiCndn$ it is sufficient to find a feasible point $(\tilde{\nu},\tilde{b},\tilde{\alpha})$ which satisfies the constraint, i.e. to show that:
% \begin{align}
%     % \tag{$A_{\CCC_0,N}'$}\label{eq:PhiCndn_par}
%     \PhiCndn &\leq  \tilde{\nu}  + \tilde{b} \tilde{\alpha}
%     \subjto \frac{1}{n}  \tilde{b}^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasn(\tilde{\nu},\tilde{b}\|\gamma(\tilde{\alpha})\|_2)
%     \label{eq:loc_phi_upp_bound_one_point}
% \end{align}
% holds with high probability for some $\tnu>0$. In order to evaluate $\fnclasn(\tilde{\nu},\tilde{b}\|\gamma(\tilde{\alpha})\|_2)$ we will use Proposition~\ref{prop:uniform_conv_noiseless}, which we repeat here for the sake of completeness. Recall that $\eta = b\norm{\gamma(\alpha)}_2$. 

% We show that $\fnclasn$ concentrates well around a simple algebraic expression in the following proposition: 
% \begin{proposition}
% \label{prop:uniform_conv_noiseless}
% For any $p\in(0,\frac{2}{5})$, $\rho \asymp \sqrt{\frac{\log d}{n}}$, $\epsilon_n \asymp \sqrt{\log\log n}$ and $\epsilon_c \asymp n^{-(1+p)/2} $ the following inequality holds with probability at least $1-c_1n^{-1}$:
% \begin{align}
%     \sup_{\substack{\nu = \Omega(n^p)\\ \eta = \OOO(1)}} \left|\fnclasn(\nu,\eta) 
%     -
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} - \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} \right|
%     =
%     O \left( \frac{\eta^2}{\nu^3}, \rho\eta^2, \frac{\eta^3}{\nu}\epsilon_n^3 \right) 
%     +
%     O \left( \frac{1}{\nu^3}, \epsilon_c \right) 
% \end{align}
% \end{proposition}
% Proof of the proposition is deferred to Section~\ref{sec:uniform_conv_noiseless}.
% Using this proposition we can rewrite constraint from Equation~\eqref{eq:loc_phi_upp_bound_one_point} to a simpler form using the following inequality:
% % Assuming that $\nu = \Omega(n^p),\eta = O(1)$ for $p\in(0,\frac{2}{5})$, $\rho \asymp \sqrt{\frac{\log d}{n}}$, $\epsilon_n \asymp \sqrt{\log\log n}$ and $\epsilon_c \asymp n^{-(1+p)/2} $, we have with probability $\geq 1-c_1 n^{-1}$ that
% % $\geq 1-\exp(-c_1 n^{1-p})-\exp(-c_2 \sqrt{n\log d}) -c_3d^{-1}$ that
% % \begin{align}
% %     \left|\fnclasn(\nu,\eta)     -
% %     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} - \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} \right|
% %     =
% %     O \left( \frac{\eta^2}{\nu^3}, \rho\epsilon_n^2 \eta^2, \frac{\eta^3}{\nu}\epsilon_n^3 \right) 
% %     +
% %     O \left( \frac{1}{\nu^3}, \epsilon_c \right) 
% %     % =: \OOO_{\eta}(\eta,n,\rho) + \OOO_{\nu,c}(\nu,\epsilon) 
% %     =: \OOO_{\eta} + \OOO_c
% %     \label{eq:fn_taylor_approx_localization}
% % \end{align}
% \begin{align}
%     \fnclasn(\nu,\eta)     
%     \leq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} 
%     +
%     % O \left( \frac{\eta^2}{\nu^3}, \rho\epsilon_n^2 \eta^2, \frac{\eta^3}{\nu}\epsilon_n^3 \right) 
%     % +
%     % O \left( \frac{1}{\nu^3}, \epsilon_c \right) 
%     % =: \OOO_{\eta}(\eta,n,\rho) + \OOO_{\nu,c}(\nu,\epsilon) 
%     % =: 
%     \OOO_{\eta} + \OOO_c
%     \label{eq:fn_taylor_approx_localization_proof2}
% \end{align}
% where $\OOO_{\eta}:=O \left( \frac{\eta^2}{\nu^3}, \rho\epsilon_n^2 \eta^2, \frac{\eta^3}{\nu}\epsilon_n^3 \right)$ and $\OOO_c:=O \left( \frac{1}{\nu^3}, \epsilon_c \right)$.

% We claim that for our choice of point $(\tnu,\tb,\talpha)$ we get $\OOO_{\eta} = \frac{\teta^2}{\tnu}O \left( \frac{\epsilon_n^3}{t_m} \right)$ and $\OOO_{c} = \frac{1}{\tnu} O \left( \frac{1}{\sqrt{m}} \right)$, where $\teta = \tb \norm{\gamma (\talpha )}_2$ and $\sopt\asymp (n t_{n^{2/3}})^{2/3}$ as given in the proposition statement. Once we have established inequality~\eqref{eq:fn_taylor_approx_localization_proof2}, claim that the point $(\tnu,\tb,\talpha)$ satisfies constraint from \eqref{eq:loc_phi_upp_bound_one_point} is implied by proving the following inequality:
% \begin{align}
%     \frac{1}{n} \tb^2\norm{\Hgaussian}_{\infty}^2  
%     \geq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\tnu} + \sqrt{\frac{2}{\pi}} \frac{\tb^2\norm{\gamma(\talpha)}_2^2}{\tnu} + \frac{\tb^2 \norm{\gamma(\talpha)}_2^2}{\tnu} O \left( \frac{\epsilon_n^3}{t_m} \right) + \frac{1}{\tnu}O \left( \frac{1}{\sqrt{m}} \right)
%     \label{eq:loc_proof_btilde_ineq_approx}
% \end{align}
% % Defining $\tbealpha = \tb\talpha$, we can rewrite \eqref{eq:PhiCndn_par} as follows:
% % \begin{align}
% %     \PhiCndn 
% %     =
% %     \min_{\nu,\bealpha,\alpha} \nu  + \bealpha
% %     \subjto 
% %     \frac{1}{n}\bealpha^2 \frac{\norm{\Hgaussian}_{\infty}^2}{\alpha^2}  
% %     \geq
% %     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} \left( 1 + O \left( \frac{1}{\sqrt{m}} \right) \right) +  \sqrt{\frac{2}{\pi}} \frac{\bealpha^2}{\nu} \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2} \left( 1 + O \left( \frac{\epsilon_n}{t_m} \right) \right)
% % \end{align}
% Defining $\tbealpha = \tb\talpha$ and rearranging the terms in Equation~\eqref{eq:loc_proof_btilde_ineq_approx} we obtain the following lower bound for $\tbealpha$:
% \begin{align}
%     \tbealpha^2 
%     \geq 
%     \frac{n\talpha^2}{\norm{H}_{\infty}^2} \frac{ \frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\tnu} \left( 1  + O \left(\frac{1}{\sqrt{m}} \right)  \right) }{ 1-\sqrt{\frac{2}{\pi}} \frac{n}{\tnu} \frac{\norm{\gamma(\talpha)}_2^2}{\norm{H}_{\infty}^2} \left( 1 + O \left( \frac{\epsilon_n^3}{t_m} \right) \right)}
% \end{align}
% Using concentration results from Proposition~\ref{prop:concentration_gammas} we get the following result:
% \begin{align}
%     \bealpha^2
%     \geq
%     n\frac{1}{t_s^2}\left( 1-\frac{4}{t_s^2} + O \left( \frac{1}{t_s^4} \right) \right) \frac{\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\tnu}  \left( 1 + O \left( \frac{1}{\sqrt{m}} \right) \right)}{ 1 - \sqrt{\frac{2}{\pi}}\frac{n}{\tnu}\frac{2}{st_s^2}\left( 1+O\left( \frac{1}{t_s^2} \right) \right) \left( 1 + O \left( \frac{\epsilon_n^3}{t_m} \right) \right)}  
% \end{align}
% with probability at least $1-6\exp\left(-\frac{2s}{\log(d/s)^5} \right)$.
% Similarly, as in Remark 1 in \cite{wang2021tight}, we choose $s$, which approximately minimizes the expression above, 
% i.e. such to maximize:
% \begin{align}
%     t_s^2 \left( 1 - \sqrt{\frac{2}{\pi}}\frac{n}{\tnu}\frac{2}{st_s^2} \right) \approx 2\log \left( \frac{d}{s} \right) - 2\sqrt{\frac{2}{\pi}} \frac{n}{\tnu s} 
% \end{align}
% This gives $s=\sopt(\tnu) := \sqrt{\frac{2}{\pi}} \frac{n}{\tnu}$. We claim that for our choice of $\tnu$ we can set $\sopt := 2(\frac{3}{\pi})^{1/3} (n t_{n^{2/3}})^{2/3}$ and for such $s=\sopt$ we have:
% \begin{align}
%     \tbealpha^2 \geq \frac{\sqrt{2}}{3\sqrt{\pi}}\frac{n}{\tnu t_\sopt^2} \left( 1 - \frac{2}{t_\sopt^2} + O \left( \frac{1}{\sqrt{m}} +\frac{\epsilon_n^3}{t_m^3} + \frac{1}{t_\sopt^4}  \right) \right)
% \end{align}
% So we let:
% \begin{align}
%     \tbealpha(\tnu) := \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{n}{\tnu t_\sopt^2} \left( 1 - \frac{2}{t_\sopt^2} + O \left( \frac{\epsilon_n^3}{t_m^3}  \right) \right) }
% \end{align}
% In order to obtain tighter bound on $\PhiCndn$ in Equation~\eqref{eq:loc_phi_upp_bound_one_point} we choose $\tnu$ as follows:
% \begin{align}
%     \tnu := \argmin_{\nu} \nu + \tbealpha(\nu) = \argmin_{\nu} \nu + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{n}{\nu t_{\sopt}^2} \left( 1 - \frac{2}{t_{\sopt}^2} + O \left( \frac{\epsilon_n^3}{t_m^3}   \right) \right) }
% \end{align}
% After minimization, we get that $\tnu$ is given by:
% \begin{align}
%     % \left( \frac{1}{72\pi} \right)^{1/4} &\sqrt{\frac{n}{\nu^3 t_{\sopt}^2}} \left( 1 - \frac{3}{t_{\sopt}^2} + O \left( \frac{1}{t_{\sopt}^4},\frac{\epsilon_n}{t_m^3}  \right) \right) = 1\\
%     % &\implies
%     \tnu = (72\pi)^{-1/6} \left( \frac{n}{t_\sopt^2} \right)^{1/3} \left( 1- \frac{2}{t_\sopt^2} + O \left( \frac{\epsilon_n^3}{t_m^3}  \right) \right)>0
% \end{align}
% Note that $\sopt(\tnu) = \sqrt{\frac{2}{\pi}} \frac{n}{\tnu} = 2(\frac{3}{\pi})^{1/3} (n t_{n^{2/3}})^{2/3}(1+O(\frac{\log\log(d/n^{2/3})}{\log (d/n^{2/3})})) = \sopt (1+O(\frac{\log\log (d/n^{2/3})}{\log (d/n^{2/3})}))$. Returning to $\tbealpha$, we obtain the following:
% \begin{align}
%     \tbealpha := \tbealpha(\tnu) = 2(72\pi)^{-1/6} \left( \frac{n}{t_\sopt^2} \right)^{1/3} \left( 1 + O \left( \frac{\epsilon_n^3}{t_m^3}  \right) \right) 
% \end{align}
% Summing up the two terms, we obtain a bound from the proposition.
% % \begin{align}
% % \PhiCndn \leq M := (72\pi)^{-1/6} \left( \frac{n}{t_s^2} \right)^{1/3} \left( 1+2(72\pi)^{1/12} - \frac{2}{t_s^2} + O \left( \frac{1}{t_s^4}+\frac{1}{ADD3} \right)\right)
% % \end{align}
% Also, note that for $s=m$ we get:
% \begin{align}
%     \teta = \tb\norm{\gamma(\talpha)}_2 = \tb\talpha \frac{\norm{\gamma(\talpha)}_2}{\talpha} = \sqrt{\frac{2}{3}}
%     \frac{1}{t_m} \left( 1 + O \left( \frac{1}{t_m^2} \right) \right)
% \end{align}
% So, we have $O \left( \frac{\teta^2}{\tnu^3}, \rho\teta^2, \frac{\teta^3}{\tnu}\epsilon_\eta \right) = O \left( \frac{\teta^2}{\tnu}\frac{\epsilon_n}{t_m} \right)$ and $O \left( \frac{1}{\tnu^3}, \epsilon_c \right) = O \left( \epsilon_c \right) = O \left(\frac{1}{\tnu \sqrt{m}} \right)$  as we assumed at the beginning of the proof.


==> sections/subsections_theory/noiseless/loc_sketch.tex <==
% \subsubsection{Proof sketch of Localization Proposition~\ref{prop:localization_noiseless}}
% \label{subsubsec:proof_sketch_loc_noiseless}

% Recall definition of $\PhiCndn$ from Proposition~\ref{prop:parametrization_class_noisy}. In order to find an upper bound $\loneboundclasn\geq\PhiCndn$, it is sufficient to find one point $(\tnu,\tb,\talpha)$ which satisfies given constraint i.e. we have the following upper bound:
% \begin{align}
%     \PhiCndn &\leq  \tilde{\nu}  + \tilde{b} \tilde{\alpha}
%     \subjto \frac{1}{n}  \tilde{b}^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasn(\tilde{\nu},\tilde{b}\|\gamma(\tilde{\alpha})\|_2)
%     \label{eq:proof_sketch_loc_phicndn}
% \end{align}
% The rest of the proof considers choice of $(\tnu,\tb,\talpha)$ such that obtained upper bound is tight. We show that for our choice of $(\tnu,\tb,\talpha)$ function $\fnclasn$ concentrates around expectation $\fclasn = \EE[\fnclasn]$ sufficiently well. Moreover, we show that $\fnclasn$ concentrates well around a simple algebraic expression in the following proposition: 
% \begin{proposition}
% \label{prop:uniform_conv_noiseless}
% For any $p\in(0,\frac{2}{5})$, $\rho \asymp \sqrt{\frac{\log d}{n}}$, $\epsilon_n \asymp \sqrt{\log\log n}$ and $\epsilon_c \asymp n^{-(1+p)/2} $ the following inequality holds with probability at least $1-c_1n^{-1}$:
% \begin{align}
%     \sup_{\substack{\nu = \Omega(n^p)\\ \eta = \OOO(1)}} \left|\fnclasn(\nu,\eta) 
%     -
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} - \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} \right|
%     =
%     O \left( \frac{\eta^2}{\nu^3}, \rho\eta^2, \frac{\eta^3}{\nu}\epsilon_n^3 \right) 
%     +
%     O \left( \frac{1}{\nu^3}, \epsilon_c \right) 
% \end{align}
% \end{proposition}
% Proof of the proposition is deferred to Section~\ref{sec:uniform_conv_noiseless}.
% Using this proposition we can rewrite constraint from Equation~\eqref{eq:proof_sketch_loc_phicndn} to a simpler form:
% \begin{align}
%     \frac{1}{n}\tb^2 \norm{H}_{\infty}^2   
%     \geq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\tnu} + \sqrt{\frac{2}{\pi}} \frac{\tb^2\norm{\gamma(\talpha)}_2^2}{\tnu} 
%     +
%     \epsilon
% \end{align}
% where $\epsilon$ are small concentration terms. After a few simple calculations the constraint can be written as:
% \begin{align}
%     (\tb\talpha)^2 
%     \geq 
%     \frac{n\talpha^2}{\norm{H}_{\infty}^2} \frac{ \frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\tnu} \left( 1  + O \left(\frac{1}{\sqrt{m}} \right)  \right) }{ 1-\sqrt{\frac{2}{\pi}} \frac{n}{\tnu} \frac{\norm{\gamma(\talpha)}_2^2}{\norm{H}_{\infty}^2} \left( 1 + O \left( \frac{\epsilon_n^3}{t_m} \right) \right)}
%     \label{eq:proof_loc_sketch_balpha}
% \end{align}

% Now in order to have a tight bound in Equation~\eqref{eq:proof_sketch_loc_phicndn} we need to choose $\tnu + \tb\talpha$ as small as possible. Thus we choose term $\tb\talpha$ which saturates Equality~\eqref{eq:proof_loc_sketch_balpha}. Note that this term depends only on $\tnu$ and $\talpha$. First we choose $\talpha$ which minimizes $\tb\talpha$ i.e. expression on the right hand side of Equation~\eqref{eq:proof_loc_sketch_balpha} and obtain that optimal $\alpha=\alpha_s$ with $s=m$, for $m$ given in the statement of the Proposition~\ref{prop:localization_noiseless}. Now since $\tnu+\tb\talpha(\tnu)$ depends only on $\tnu$ we can optimize over $\tnu$ and choose the minimizer. Thus both $\tnu$ and $\tb\talpha$ are determined and bound $\loneboundclasn$ follows straightforwardly from Equation~\eqref{eq:proof_sketch_loc_phicndn}.

==> sections/subsections_theory/noiseless/sloc_proof_old.tex <==
\subsection{Proof of Localization Proposition~\ref{prop:localization_noiseless_ssparse}}
\label{sec:proof_loc_noiseless}
Recall definition of $\PhiCndn$ from Proposition~\ref{prop:parametrization_class_general} and note that in order to upper bound $\PhiCndn$ it is sufficient to find a feasible point $(\tilde{\nu},\tilde{b},\tilde{\alpha},\tilde{\varsigma})$ which satisfies the constraint, i.e. to show that:
\begin{align}
    % \tag{$A_{\CCC_0,N}'$}\label{eq:PhiCndn_par}
    \PhiCndn &\leq  \tilde{\nu}\norm{\wgt}_1  + \sqrt{s}\tilde{\varsigma} + \tilde{b} \tilde{\alpha}
    \subjto \frac{1}{n} (2\sqrt{s} \tilde{\varsigma}+ \tilde{b}^2\norm{\Hgaussian}_{\infty})^2  \geq  \fnclasn(\tilde{\nu},\tilde{b}\|\gamma(\tilde{\alpha})\|_2, \tilde{\varsigma})
    \label{eq:loc_phi_upp_bound_one_point}
\end{align}
holds with high probability for some $\tnu>0$. We choose $\tilde{\varsigma} = 0$.


Note that random variable $(1-\nu \abs{\Gausswone} - \eta\Gausswtwo)_+^2$ for fixed $(\nu,\eta)$ is a sub-exponential random variable. Furthermore, since $(1-\nu \abs{\Gausswone} - \eta\Gausswtwo)_+^2 \lesssim 1+\eta^2(\Gausswtwo)^2$ we obtain that the sub-exponential norm of this random variable is bounded by a constant for $\eta =const$. We can apply results on concentration of sub-exponential random variables to show that $|\fnclasn(\nu,\eta)-\fclasn(\nu,\eta)|$ 
Thus, using this concentration result and Taylor expansion of function $\fclasn = \EE \fnclasn$ from Equation~\eqref{eq:taylor_fclasn} we obtain
\begin{align}
    \fnclasn(\nu,\eta,0)     
    \leq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} 
    \OOO_t + \OOO_c
    \label{eq:fn_taylor_approx_localization_proof2}
\end{align}
where $\OOO_t:=O \left( \frac{1}{\nu^3},\frac{\eta^4}{\nu^3} \right)$ and $\OOO_c:= O \left( \frac{1}{\nu \tsoptn^4} \right)$.

We claim that for our choice of point $(\tnu,\tb,\talpha)$ we get $\OOO_{\eta} = \frac{\teta^2}{\tnu}O \left( \frac{\epsilon_n^3}{\tsopt} \right)$ and $\OOO_{c} = \frac{1}{\tnu} O \left( \frac{1}{\sqrt{\sopt}} \right)$, where $\teta = \tb \norm{\gamma (\talpha )}_2$ and $\sopt\asymp (n t_{n^{2/3}} \norm{\wgt}_1)^{2/3}$ as given in the proposition statement. Once we have established inequality~\eqref{eq:fn_taylor_approx_localization_proof2}, claim that the point $(\tnu,\tb,\talpha)$ satisfies constraint from \eqref{eq:loc_phi_upp_bound_one_point} is implied by proving the following inequality:
\begin{align}
    \frac{1}{n} \tb^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\tnu} + \sqrt{\frac{2}{\pi}} \frac{\tb^2\norm{\gamma(\talpha)}_2^2}{\tnu} + \frac{\tb^2 \norm{\gamma(\talpha)}_2^2}{\tnu} O \left( \frac{\epsilon_n^3}{\tsopt} \right) + \frac{1}{\tnu}O \left( \frac{1}{\sqrt{\sopt}} \right)
    \label{eq:loc_proof_btilde_ineq_approx}
\end{align}
Defining $\tbealpha = \tb\talpha$ and rearranging the terms in Equation~\eqref{eq:loc_proof_btilde_ineq_approx} we obtain the following lower bound for $\tbealpha$:
\begin{align}
    \tbealpha^2 
    \geq 
    \frac{n\talpha^2}{\norm{H}_{\infty}^2} \frac{ \frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\tnu} \left( 1  + O \left(\frac{1}{\sqrt{\sopt}} \right)  \right) }{ 1-\sqrt{\frac{2}{\pi}} \frac{n}{\tnu} \frac{\norm{\gamma(\talpha)}_2^2}{\norm{H}_{\infty}^2} \left( 1 + O \left( \frac{\epsilon_n^3}{\tsopt} \right) \right)}
\end{align}
Using concentration results from Proposition~\ref{prop:concentration_gammas} we get the following result:
\begin{align}
    \bealpha^2
    \geq
    n\frac{1}{\tm^2}\left( 1-\frac{4}{\tm^2} + O \left( \frac{1}{\tm^4} \right) \right) \frac{\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\tnu}  \left( 1 + O \left( \frac{1}{\sqrt{\sopt}} \right) \right)}{ 1 - \sqrt{\frac{2}{\pi}}\frac{n}{\tnu}\frac{2}{m\tm^2}\left( 1+O\left( \frac{1}{\tm^2} \right) \right) \left( 1 + O \left( \frac{\epsilon_n^3}{\tsopt} \right) \right)}  
\end{align}
with probability at least $1-6\exp\left(-\frac{2m}{\log(d/m)^5} \right)$.
Similarly, as in Remark 1 in \cite{wang2021tight}, we choose $m$, which approximately minimizes the expression above, 
i.e. such to maximize:
\begin{align}
    \tm^2 \left( 1 - \sqrt{\frac{2}{\pi}}\frac{n}{\tnu}\frac{2}{m\tm^2} \right) \approx 2\log \left( \frac{d}{m} \right) - 2\sqrt{\frac{2}{\pi}} \frac{n}{\tnu m} 
\end{align}
This gives $m=\sopt(\tnu) := \sqrt{\frac{2}{\pi}} \frac{n}{\tnu}$. We claim that for our choice of $\tnu$ we can set $\sopt := 2(\frac{3}{\pi})^{1/3} \norm{\wgt}_1^{2/3} (n t_{n^{2/3}})^{2/3}$ and for such $m=\sopt$ we have:
\begin{align}
    \tbealpha^2 \geq \frac{\sqrt{2}}{3\sqrt{\pi}}\frac{n}{\tnu \tsopt^2} \left( 1 - \frac{2}{\tsopt^2} + O \left( \frac{1}{\sqrt{\sopt}} +\frac{\epsilon_n^3}{\tsopt^3} + \frac{1}{\tsopt^4}  \right) \right)
\end{align}
So we let:
\begin{align}
    \tbealpha(\tnu) := \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{n}{\tnu \tsopt^2} \left( 1 - \frac{2}{\tsopt^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3}  \right) \right) }
\end{align}
In order to obtain tighter bound on $\PhiCndn$ in Equation~\eqref{eq:loc_phi_upp_bound_one_point} we choose $\tnu$ as follows:
\begin{align}
    \tnu := \argmin_{\nu>0} \nu \norm{\wgt}_1 + \tbealpha(\nu) = \argmin_{\nu} \nu\norm{\wgt}_1 + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{n}{\nu t_{\sopt}^2} \left( 1 - \frac{2}{\tsopt^2} + O \left( \frac{\epsilon_n^3}{t_m^3}   \right) \right) }
\end{align}
After minimization, we get that $\tnu$ is given by:
\begin{align}
    % \left( \frac{1}{72\pi} \right)^{1/4} &\sqrt{\frac{n}{\nu^3 t_{\sopt}^2}} \left( 1 - \frac{3}{t_{\sopt}^2} + O \left( \frac{1}{t_{\sopt}^4},\frac{\epsilon_n}{t_m^3}  \right) \right) = 1\\
    % &\implies
    \tnu = (72\pi)^{-1/6} \norm{\wgt}_1^{-2/3} \left( \frac{n}{\tsopt^2} \right)^{1/3} \left( 1- \frac{2}{\tsopt^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3}  \right) \right)>0
\end{align}
Note that $\sopt(\tnu) = \sqrt{\frac{2}{\pi}} \frac{n}{\tnu} = 2(\frac{3}{\pi})^{1/3} \norm{\wgt}_1^{2/3} (n t_{n^{2/3}})^{2/3}(1+O(\frac{\log\log(d/n^{2/3})}{\log (d/n^{2/3})})) = \sopt (1+O(\frac{\log\log (d/n^{2/3})}{\log (d/n^{2/3})}))$ \red{not tight enough, needs more terms}. Returning to $\tbealpha$, we obtain the following:
\begin{align}
    \tbealpha := \tbealpha(\tnu) = 2(72\pi)^{-1/6} \norm{\wgt}_1^{1/3} \left( \frac{n}{\tsopt^2} \right)^{1/3} \left( 1 + O \left( \frac{\epsilon_n^3}{\tsopt^3}  \right) \right) 
\end{align}
Summing up the two terms, we obtain a bound from the proposition.
% \begin{align}
% \PhiCndn \leq M := (72\pi)^{-1/6} \left( \frac{n}{t_s^2} \right)^{1/3} \left( 1+2(72\pi)^{1/12} - \frac{2}{t_s^2} + O \left( \frac{1}{t_s^4}+\frac{1}{ADD3} \right)\right)
% \end{align}
Also, note that for $m=\sopt$ we get:
\begin{align}
    \teta = \tb\norm{\gamma(\talpha)}_2 = \tb\talpha \frac{\norm{\gamma(\talpha)}_2}{\talpha} = \sqrt{\frac{2}{3}}
    \frac{1}{\tsopt} \left( 1 + O \left( \frac{1}{\tsopt^2} \right) \right)
\end{align}
So, we have $O \left( \frac{\teta^2}{\tnu^3}, \rho\teta^2, \frac{\teta^3}{\tnu}\epsilon_\eta \right) = O \left( \frac{\teta^2}{\tnu}\frac{\epsilon_n}{\tsopt} \right)$ and $O \left( \frac{1}{\tnu^3}, \epsilon_c \right) = O \left( \epsilon_c \right) = O \left(\frac{1}{\tnu \sqrt{\sopt}} \right)$  as we assumed at the beginning of the proof.


==> sections/subsections_theory/noiseless/sunicon_proof_mid_old.tex <==
% \section{TEMP: s sparse uniform convergence noiseless}
\subsection{Proof of Uniform Convergence Proposition~\ref{prop:BoundGamma0_class_noiseless}}
\label{sec:proof_unicon_noiseless}

\begin{align}
    \setNoiselessZero = \Big\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  (2\sqrt{s}\varsigma + b\normk{H}_{\infty})^2 &\geq  \fnclasn(\nu,b\|\gamma(\alpha)\|_2, \varsigma)\\
    &~~\andtxt~~  \max\left\{ |\nu| \|\wgtp\|_1 - \sqrt{s}\varsigma , \varsigma- |\nu| \|\wgtp\|_1 \right\} + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasn \Big\}
    \label{eq:Gamma0_def_class_noiseless}
\end{align}
As discussed in the proof sketch, proof consists of iterative bounding and approximation steps. The structure of the proof is as follows: for every bound step we use different approximation of $\fnclasn$, and based on it we develop tighter bounds on variables of interest. Thus the statement of the proposition follows from the tightest, last bound i.e. Bound 5. We start with the following bound:
\subsubsection*{Bound 1: \texorpdfstring{$\nu\norm{\wgt}_1 = O(\loneboundclasn), \nu = \Omega(n^{2/15})$}{nuomega}}

\textbf{Step 1.1: Upper bound on $\nu\norm{\wgt}_1$.}
Since $\nu \norm{\wgt}_1 \leq \loneboundclasn+\sqrt{s}\varsigma$ in order to show that $\nu\norm{\wgt}_1 = O(\loneboundclasn)$ it is sufficient to show that $\sqrt{s}\varsigma = O(\loneboundclasn)$. 

Let $s =O( n^{1/5} )$ and $\rho = 1/n^{1/10}$. Assume by contradiction that $\sqrt{s}\varsigma = w(\loneboundclasn)$ Then we have:
\begin{align}
    \varsigma^2 \frac{s}{n} + \frac{1}{n^{2/15}} &\gtrsim \fnclasg(\nu,\eta,\varsigma) = \frac{1}{n} \sum_{i=1}^n ( 1 -  \nu |z_i^{(0)}| - z_i^{(1)} \sqrt{\eta^2 + \varsigma^2} )_+^2\\
    &\gtrsim \frac{1}{n} \sum_{i=1}^n ( 1 -  \nu |z_i^{(0)}| - z_i^{(1)} \sqrt{\eta^2 + \varsigma^2} )_+^2 \indicator{\gausswtwo_i\geq 0}
    \gtrsim
    \frac{1}{n} \sum_{i=1}^n ( -\nu |z_i^{(0)}| + z_i^{(1)} \varsigma )_+^2 \\
    &\gtrsim
    \frac{1}{n} \sum_{i=1}^n ( -(\loneboundclasn+\sqrt{s}\varsigma) |z_i^{(0)}| + z_i^{(1)} \varsigma )_+^2 
    \gtrsim
    \frac{1}{n} \sum_{i=1}^n ( -c_1\sqrt{s}\varsigma |z_i^{(0)}| + z_i^{(1)} \varsigma )_+^2 \indicator{|\gausswone_i| \leq \frac{\rho}{2c_1\sqrt{s}}} \indicator{\gausswtwo_i\geq \rho}\\
    &\gtrsim
    (\frac{\rho}{2}\varsigma)^2 \frac{1}{n} \sum_{i=1}^n \indicator{|\gausswone_i| \leq \frac{\rho}{2c_1\sqrt{s}}} \indicator{\gausswtwo_i\geq \rho}
\end{align}
Now use that $\PP(|\gausswone| \lesssim \frac{\rho}{\sqrt{s}}) \gtrsim \frac{\rho}{\sqrt{s}}$ and $\PP(\gausswtwo \geq \rho) \geq const$ and thus we obtain with probability $\geq 1-\exp(-c_2 \frac{\rho^2}{s}n)$:
\begin{align}
    \varsigma^2 \frac{s}{n} + \frac{1}{n^{2/15}} \gtrsim \varsigma^2 \frac{\rho^3}{\sqrt{s}} 
\end{align}
First note that $\frac{s}{n} \lesssim \frac{\rho^3}{\sqrt{s}}$ since $s\sqrt{s} \lesssim n^{3/10}$ and $n\rho^3 = n^{7/10} \gtrsim n^{3/10}$. Thus in order for constraint to hold we need that $\varsigma^2 \lesssim \frac{\sqrt{s}}{\rho^3n^{2/15}} = O(n^{4/15})$ and thus $\sqrt{s} \varsigma = O(n^{7/30}) = o(\loneboundclasn)$, contradiction.

\textbf{Step 1.2: Lower bound on $\nu$.}

Recall the definition of the set $\setNoiselessZero$ from Equation~\eqref{eq:Gamma0_def_class_noiseless} and that by parametric path approach from Section~\ref{subsec:path_param} we have $\eta = \norm{\wtwo}_2 = b\norm{\gamma(\alpha)}_2$. In order to show the lower bound $\nu = \Omega(n^{2/15})$ we define the following set:
\begin{align}
    % \setNoiselessZero^{\nu,L}
    \Gamma_1^{\nu}
    = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasn (\nu,b\norm{\gamma(\alpha)}_2, \varsigma) 
    ~~\andtxt~~ 
    b\alpha \leq \loneboundclasn 
    \right\}.
    \label{eq:Gamma_1_nu_constant_lower}
\end{align}
in which we relax the second constraint from definition of set $\setNoiselessZero$ and thus $\setNoiselessZero \subset \Gamma_1^{\nu}$. The goal is to show that uniformly over all $\nu\in \Gamma_1^{\nu}$ holds that $\nu=\Omega(n^{2/15})$ implying that this lower bound holds also uniformly over $\setNoiselessZero$.

Note that for $(\nu,b,\alpha)\in \Gamma_1^{\nu}$ we have:
\begin{align}
    \fnclasn (\nu,b\norm{\gamma(\alpha)}_2, \varsigma) 
    \leq
    \max_{b,\alpha} \frac{1}{n}b^2 \norm{H}_{\infty}^2 
    \leq
    \max_{\alpha} \frac{1}{n} \frac{\loneboundclasn^2}{\alpha^2} \norm{H}_{\infty}^2
    =
    \frac{1}{n} \loneboundclasn^2 \norm{H}_{\infty}^2
    \lesssim
    \frac{1}{n} \left( \frac{n}{\tsopt^2} \right)^{2/3} \log d 
    \lesssim
    \left( \frac{1}{n} \right)^{2/15}
\end{align}
with probability $\geq 1-\frac{1}{d}$, where we used $d\lesssim \exp(\kappa n^{1/5})$ and $\alpha\geq 1$. Also, we have:
\begin{align}
    \fnclasn (\nu,b\norm{\gamma(\alpha)}_2)  
    =
    \frac{1}{n} \sum_{i=1}^n \possq{ 1 - \nu \abs{\gausswone_i} - \eta\gausswtwo_i - \sum_{j=2}^s \gausswj_i \varsigma_j} 
    \gtrsim
    \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}}
    \label{eq_etanu_to_nu_fnclansn}
\end{align}
with probability $\geq 1-\exp(-c_1 n)$ for some positive universal constant $c_1$. Now we show that $\nu = \Omega(n^{2/15})$. Assume, in contradiction, that there exists some universal constant $\kappa>0$ such that $\nu \leq \kappa n^{2/15}$ for some $\nu\in\Gamma_1^{\nu}$. From the previous two inequalities, we know that $\nu$ must satisfy with high probability that:
\begin{align}
    \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}} 
    \lesssim
    \left( \frac{1}{n} \right)^{2/15}
    \label{eq:ineq_nu_first_bound_condition}
\end{align}
Define $F_n(\frac{1}{2\nu}) := \frac{1}{n}\sum_{i=1}^n \indicator{|\gausswone_i|\leq \frac{1}{2\nu}}$ and $F(\frac{1}{2\nu}) := \PP( |\Gausswone| \leq \frac{1}{2\nu} )$. Using the same reasoning as in Lemma~\ref{lemma:dkw_number_active_indicators} one can show that from the set of indicators $\{ \indicator{1-\nu\abs{\gausswone_i}}\}_{i=1}^n$ there are at least $k:=nF_n(\frac{1}{2\nu}) \gtrsim n^{1-p}$ indicators activated when $\nu=O(n^p)$, $p\in(0,\frac{2}{5})$. Thus we have
\begin{align}
    \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}} 
    \geq
    \frac{n F_n(\frac{1}{2\nu})}{n} \left(\frac{1}{2} \right)^2
    \gtrsim
    n^{-p}
\end{align}

Thus for any $n\geq c_1$ and $p\leq \frac{2}{15}$ we can always choose constants such that  inequality~\eqref{eq:ineq_nu_first_bound_condition} does not hold. Hence we conclude that $\nu = \Omega(n^{2/15})$.



% Assume that $\nu\norm{\wgt}_1 = w(\loneboundclasn)$. Then also $\norm{\varsigma}_1 = w(\loneboundclasn)$ and thus $\varsigma \geq \frac{1}{\sqrt{s}} \norm{\varsigma}_1 \asymp \nu\norm{\wgt}_1 / \sqrt{s}$. Then
% \begin{align}
%     (\frac{1}{n})^{2/15} &\gtrsim \fnclasn = \frac{1}{n}\sum_{i=1}^n (1-\nu|\gausswone_i| - \eta\gausswtwo_i - \sum_{j=2}^s \varsigma_j \gausswj_i )_+^2\\
%     &\gtrsim
%     \frac{1}{n}\sum_{i=1}^n (1-\nu|\gausswone_i| - \eta\gausswtwo_i - \sum_{j=2}^s \varsigma_j \gausswj_i )_+^2 \indicator{\gausswtwo_i \leq 0, - \sum_{j=2}^s \varsigma_j \gausswj_i \geq \varsigma }\\
%     &\gtrsim
%     \frac{1}{n}\sum_{i=1}^k \indicator{1-\nu\abs{\gausswone_i}} \varsigma^2
%     \gtrsim
%     \frac{\varsigma^2}{\nu}
% \end{align}
% where $k = \inf_{\varsigma} \sum_{i=1}^n \indicator{\gausswtwo_i \leq 0, - \sum_{j=2}^s \varsigma_j \gausswj_i \geq \varsigma } = bla bla \asymp n $.

% \begin{align}
%     (\frac{1}{n})^{2/15} &\gtrsim \fnclasn = \frac{1}{n}\sum_{i=1}^n (1-\nu|\gausswone_i| - \eta\gausswtwo_i - \sum_{j=2}^s \varsigma_j \gausswj_i )_+^2\\
%     &\gtrsim
%     \frac{1}{n}\sum_{i=1}^n (1-\nu|\gausswone_i| - \eta\gausswtwo_i - \sum_{j=2}^s \varsigma_j \gausswj_i )_+^2 \indicator{\gausswtwo_i \leq 0, - \sum_{j=2}^s \varsigma_j \gausswj_i \geq \varsigma }\\
%     &\gtrsim
%     \frac{1}{n}\sum_{i=1}^k \indicator{\varsigma-\nu\abs{\gausswone_i}} (1+\varsigma-\nu\abs{\gausswone_i})^2
%     \\
%     &\gtrsim \frac{1}{n} \sum_{i=1}^k \indicator{1-\frac{\nu}{\varsigma}\abs{\gausswone_i}}
% \end{align}
% and $\frac{\nu}{\varsigma} \leq \sqrt{s}/\norm{\wgt}_1 = o(\sqrt{n})$.


% \subsubsection*{Bound 1': \texorpdfstring{$\norm{\varsigma}_1 = O \left( \frac{n^{1/15}}{\tsopt^{3}} \sqrt{\nu} \norm{\wgt}_1^{1/3} \right)$}{bound1p}}
% Conditioning on the fact that $\nu = \Omega(n^{2/15})$ we can use lower bound from Proposition~\ref{prop:fnoiselessquadraticvarsigma}:
% \begin{align}
%     \fnclasn(\nu,\eta) \gtrsim \frac{\varsigma^2}{\nu} -  \frac{\varsigma^2}{\sqrt{n}}
% \end{align}
% which holds with probability $1-s\exp(-c_1 n)$.

% Define
% \begin{align}
%     % \Gamma_1^{\eta,U} =
%     \Gamma_{1'} =
%     \left\{ (\nu, b, \alpha, \varsigma) 
%     \subjto
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \gtrsim \frac{\varsigma^2}{\nu} - \frac{s}{\sqrt{n}}
%     ~~\andtxt~~ 
%     b\alpha \leq \loneboundclasn 
%     ~~\andtxt~~ 
%     \nu = \Omega(n^{2/15})
%     \right\}.
%     \label{eq:Gamma_1p_eta_def_upp}
% \end{align}
% \begin{align}
%     \frac{\varsigma^2}{\nu} 
%     \lesssim
%     \frac{1}{n}b^2 \norm{H}_{\infty}^2 + \frac{s}{\sqrt{n}}
%     \lesssim
%     \frac{\loneboundclasn^2}{n} \frac{\norm{H}_{\infty}^2}{\alpha^2} + \frac{s}{\sqrt{n}}
%     \lesssim
%     \frac{\norm{\wgt}_1^{2/3}}{n^{2/15}\tsopt^{4/3}}
% \end{align}
% where we used assumption $s\lesssim n^{4/15} \tsopt^{-14/3}$. Using this assumption once again we have $\norm{\varsigma}_1 \leq \sqrt{s} \varsigma \lesssim \frac{n^{1/15}}{\tsopt^{3}} \sqrt{\nu} \norm{\wgt}_1^{1/3}$. 

\subsubsection*{Bound 2: \texorpdfstring{$\eta,\varsigma = O(1),\ \nu\norm{\wgt}_1 \geq \kappa_3 \loneboundclasn$}{bound1} }
Since 
$   \left| \nu\| \wgt\|_1 - \norm{\varsigma}_1 \right| 
    =
    \nu \|\wgt\|_1 \left| 1 - \frac{\norm{\varsigma}_1}{\nu\|\wgt\|_1} \right|
    \leq \loneboundclasn
$
and
$
    \frac{\norm{\varsigma}_1}{\nu\|\wgt\|_1}     \lesssim 
    \frac{n^{1/15}}{\tsopt^3 \sqrt{\nu}\|\wgt\|_1^{2/3}} 
    \lesssim
    \frac{1}{\tsopt^3}
$
this implies that $\nu \|\wgt\|_1 \leq \loneboundclasn (1+\frac{c_1}{\tsopt^3}) =: \loneboundclasnt $. Conditioning on the fact that $\nu = \Omega(n^{2/15})$ and $\nu = O(\loneboundclasnt) = o(\sqrt{n}/\log(n s))$ we can use lower bound from Proposition~\ref{prop:fnoiselessquadratic}:\begin{align}
    \fnclasn (\nu,\eta,\varsigma) \geq \kappa_1 \frac{1}{\nu} + \kappa_2 \frac{\eta^2}{\nu} + \kappa_3 \frac{\varsigma^2}{\nu} 
\end{align}
which holds with probability $1-c_1/(n s)$ for some positive universal constants $\kappa_1,\kappa_2,\kappa_3,c_1$.

Define
\begin{align}
    % \Gamma_1^{\eta,U} =
    \Gamma_2 =
    \left\{ (\nu, b, \alpha,\varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq \kappa_1 \frac{1}{\nu} + \kappa_2 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
    ~~\andtxt~~ 
    b\alpha \leq \loneboundclasnt
    ~~\andtxt~~ 
    \nu \norm{\wgt}_1 \leq \loneboundclasnt
    ~~\andtxt~~ 
    \nu = \Omega(n^{2/15})
    \right\}.
    \label{eq:Gamma_2_eta_def_upp}
\end{align}
Note that constraints in $\Gamma_2$ are relaxations of constraints in definition of $\setNoiselessZero$ and hence $\setNoiselessZero \subset \Gamma_2$ with high probability. By finding bounds on $\nu,\eta$ from $\Gamma_2$ we obtain a valid upper bound in $\setNoiselessZero$ as well.

\textbf{Step 2.1: Upper bound on $\eta$.}
We bound $\nu$ as follows:
\begin{align}
    \eta^2
    &\leq
    \max_{\nu,b,\alpha,\varsigma} \left[ b^2\norm{\gamma(\alpha)}_2^2
    \subjto
    (\nu,b,\alpha,\varsigma)\in \Gamma_2 \right]\\
    &=
    \max_{\nu,b,\alpha} \left[ b^2\norm{\gamma(\alpha)}_2^2 
    \subjto 
    \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n}\nu \norm{H}_{\infty}^2
    ~~\andtxt~~ 
    b\alpha \leq \loneboundclasnt
    ~~\andtxt~~ 
    \nu \norm{\wgt}_1 \leq \loneboundclasnt
    \right]\\
    &=
    \max_{\alpha} \left[ \loneboundclasnt^2\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2} 
    \subjto 
    \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n} \frac{\loneboundclasnt}{\norm{\wgt}_1} \norm{H}_{\infty}^2
    \right]
    \label{eq:eta_upper_bound_step21}
\end{align}
where we used only that $(\nu,b,\alpha,\varsigma)\in \Gamma_2$ satisfy appropriate constraints. As we mentioned in the Section~\ref{subsubsec:prop_gamma_alpha}, function $\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}$ is monotonically decreasing function in $\alpha$, whereas $\norm{\gamma(\alpha)}_2^2$ is a convex function. Thus, similarly as previously discussed in \cite{donhauser2022fast}, it is sufficient to find $\alphauls < \alphasopt$ such that
\begin{align}
     \norm{\gamma(\alphauls)}_2^2 > \frac{1}{\kappa_2 n} \frac{\loneboundclasnt}{\norm{\wgt}_1} \norm{H}_{\infty}^2
\end{align}
to obtain an upper bound on $\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}$. Using concentration results from Section~\ref{subsubsec:prop_gamma_alpha} we can rewrite above inequality as follows:
\begin{align}
    \frac{2}{\ulm \tulm^2} \left( 1+O \left( \frac{1}{\tulm^2} \right) \right) > \frac{1}{\kappa_2 n} \frac{\kappam}{\norm{\wgt}_1^{2/3}} \left( \frac{n}{\tsopt^2} \right)^{1/3} \left( 1 + O \left( \frac{1}{\tsopt^2} \right) \right)
\end{align}
It is straightforward to show that we can choose $\ulm = \lambda \left( \frac{n\norm{\wgt}_1}{\tsopt^2} \right)^{2/3}$ with sufficiently small universal constant $\lambda = \lambda(\kappa_2,\kappam)>0$. We finish this step by substituting this choice of $\ulm$ into the upper bound from Equation~\eqref{eq:eta_upper_bound_step21} to get:
\begin{align}
    \eta^2 
    \leq
    \loneboundclasnt^2 \frac{\norm{\gamma(\alphauls)}_2^2}{\alphauls^2}
    = \kappam^2 \left( \frac{n\norm{\wgt}_1}{\tsopt^2} \right)^{2/3} \left( 1 + O \left( \frac{1}{\tsopt^2} \right) \right) 
    \frac{2}{\ulm} \left( 1 + O \left( \frac{1}{\tulm^2} \right) \right) =: \boundeta^2 = O(1) 
\end{align}\\

\noindent\textbf{Step 2.2: Upper bound on $\varsigma$}.
\begin{align}
    \varsigma^2 
    \lesssim
    \max \nu\frac{1}{n}b^2\norm{H}_{\infty}^2
    \lesssim 
    \frac{\loneboundclasnt}{\norm{\wgt}_1} \frac{1}{n} \loneboundclasnt^2 \frac{\norm{H}_{\infty}^2}{\alphauls^2}
    =: B_{\varsigma}^2 = O(1)
\end{align}
\noindent\textbf{Step 2.3: Lower bound on $\nu$}.
Similarly to Equation~\eqref{eq:eta_upper_bound_step21}, we can bound $\nu$ on the set $\Gamma_2$ as follows:
\begin{align}
    \nu
    &\geq
    \kappa_1 n \left[ \min_{b,\alpha} \frac{1}{b^2\norm{H}_{\infty}^2}  \subjto (\nu,b,\alpha,\varsigma)\in \Gamma_2 \right] \\
    &=
    \frac{\kappa_1 n}{\loneboundclasnt^2} \left[ \min_{\alpha} \frac{\alpha^2}{\norm{H}_{\infty}^2} \subjto \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n} \frac{\loneboundclasnt}{\norm{\wgt}_1} \norm{H}_{\infty}^2 \right]
    \label{eq:nu_lower_bound_step22}
\end{align}
Similarly as above, we obtain that $\alpha\geq \alphauls$ and after substitution of $\ulm$ as defined above, we have:
\begin{align}
    \nu \geq \kappa_1 \frac{n}{\loneboundclasnt^2} \frac{\alphauls^2}{\norm{H}_{\infty}^2} 
    &=
    \frac{\kappa_1}{\kappam^2} \norm{\wgt}_1^{-2/3} \frac{(n \tsopt^4)^{1/3}}{\tulm^2}  (1+O \left( \frac{1}{\tsopt^2}, \frac{1}{\tulm^2} \right) ) \\
    &\geq
    \frac{\kappa_1}{\kappam^2} \norm{\wgt}_1^{-2/3} \left( \frac{n}{\tsopt^2} \right)^{1/3} (1+O \left( \frac{1}{\tsopt^2} \right) ) =:  \kappa_3 \frac{\loneboundclasnt}{\norm{\wgt}_1^{2/3}}
\end{align}
implying that $\nu \norm{\wgt}_1 \in [\kappa_3,1]\loneboundclasnt$. Note that from definition of $\kappam$ and the fact that $\kappa_1$ must be smaller than constant from Taylor expansion of $\fnclasn$ i.e. $\kappa_1 \leq \frac{\sqrt{2}}{3\sqrt{\pi}}$ (see Proposition~\ref{prop:uniform_conv_noiseless}) we get that $\kappa_3$ must satisfy $0 < \kappa_3 < \frac{4}{27}(1+O \left( \frac{1}{\tsopt^2} \right) )$.

\subsubsection*{Bound 3: \texorpdfstring{$\eta = \Omega \left( \frac{1}{\tsopt} \right)$}{bound2} } 
Here we use approximation:
\begin{align}
    \fnclasn(\nu,\eta) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + O\left( \frac{1}{\nu^3} \right)
\end{align}
\begin{align}
    % \Gamma_1^{\alpha,U} \textbf{o}
    \Gamma_3^{\eta} 
    = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \frac{1}{\nu^3} \right)
    ~~\andtxt~~ 
    b\alpha + \nu\norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu\norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    \right\}.
    \label{eq:Gamma_3_eta_lower_def}
\end{align}
Again, we have $\setNoiselessZero \subset \Gamma_3^{\eta}$. Note that for $(\nu,b,\alpha,\varsigma)\in \Gamma_3^{\eta}$ holds:
\begin{align}
    \eta^2 
    &\geq 
    \left[ \min_{\nu, b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \frac{1}{\nu^3} \right)
    ~~\andtxt~~ 
    b\alpha + \nu\norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu\norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    \right]\\
    &\gtrsim
     n \left[ \min_{\nu,\alpha} \frac{1}{\nu} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}  \subjto
    \frac{1}{n} \left( \frac{\loneboundclasnt-\nu\norm{\wgt}_1}{\alpha} \right)^2 \norm{H}_{\infty}^2
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \frac{1}{\nu^3} \right)
    % ~~\andtxt~~ 
    % b\alpha + \nu \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu\norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    \right]\\
    &\gtrsim
    \frac{n}{\loneboundclasnt} \left[
    \min_{\nu,\alpha} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} 
    \subjto
    \frac{\alpha^2}{\norm{H}_{\infty}^2} \leq \frac{3\sqrt{\pi}}{\sqrt{2}}\frac{1}{n}\nu(\loneboundclasnt-\nu\norm{\wgt}_1)^2 + O \left( \frac{1}{\nu^3} \right)
    % ~~\andtxt~~ 
    % b\alpha + \nu \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu \norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    \right]
\end{align}
% Also note that $\alpha$ that satisfies constraints above is upper bounded
% \begin{align}
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} \leq \frac{1}{n} b^2 \norm{H}_{\infty}^2 \leq \frac{1}{n} \left( \frac{\loneboundclasnt-\nu}{\alpha} \right)^2 \norm{H}_{\infty}^2
% \end{align}
Since given that $\nu\norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt$ the function $\nu (\loneboundclasnt -\nu\norm{\wgt}_1)^2$ is maximized for $\nu\norm{\wgt}_1 = \loneboundclasnt/3$ and $1/3\in[\kappa_3,1]$ we can upper bound $\alpha$ as follows:
\begin{align}
    \frac{\alpha^2}{\norm{H}_{\infty}^2} 
    \leq
    \frac{3\sqrt{\pi}}{\sqrt{2}} \frac{1}{n} \nu (\loneboundclasnt -\nu\norm{\wgt}_1)^2 + O\left( \frac{1}{\nu^3} \right) 
    &\leq
    \frac{12\sqrt{\pi}}{27\sqrt{2}} \frac{1}{n} \frac{\loneboundclasnt^3}{\norm{\wgt}_1} + O\left( \frac{1}{\loneboundclasnt^3} \right) \\
    &\leq
    \frac{1}{\tsopt^2}  \left( 1 - \frac{2}{3}\frac{1}{\tsopt^2} + O \left( \frac{\epsilon_n}{\tsopt^3} \right) \right)+ O\left( \frac{\tsopt^2}{n} \right) 
    \label{eq:alpha_ols_bound_nu_loneboundclasn}
\end{align}
where we used definition of $\loneboundclasnt$ from Proposition~\ref{prop:localization_noiseless_ssparse}.

From Section~\ref{subsubsec:prop_gamma_alpha} we have that $\norm{\gamma(\alpha)}_2^2$ is a convex function and it decreases over $[1,\alpha_{d+1/2}]$. 
Hence in order to lower bound $\norm{\gamma(\alpha)}_2^2$, it is sufficient to find a point $\alphaols$ such that $\alphaols \geq \alpha_m$ for which Equation~\eqref{eq:alpha_ols_bound_nu_loneboundclasn} does not hold, i.e. for $\olm$ for which we have:
\begin{align}
    \frac{1}{\tolm^2} \left( 1 - \frac{4}{\tolm^2} + O \left( \frac{1}{\tolm^4} \right)\right) 
    >
    \frac{1}{\tsopt^2} \left( 1 - \frac{2}{3}\frac{1}{\tsopt^2} + O \left( \frac{\epsilon_n}{\tsopt^3} \right) \right)
\end{align}
We can choose $\olm = \lambda \sopt$ for some constant $\lambda>1$ since 
\begin{align}
    \frac{\tsopt^2}{\tolm^2} = 1 + \frac{2\log\lambda}{\tsopt^2} + O \left( \frac{1}{\tsopt^4} \right)
\end{align}
Thus we finally obtain:
\begin{align}
    \eta^2  
    \gtrsim
    \frac{n}{\loneboundclasnt} \frac{\norm{\gamma(\alphaols)}_2^2}{\norm{H}_{\infty}^2}
    \gtrsim
    (n \tsopt)^{2/3} \frac{1}{\olm \tolm^2}
    \gtrsim
    \frac{1}{\tsopt^2}
\end{align}
\subsubsection*{Bound 4: Tight bounds on $\nu$ and $\eta = \Theta(\frac{1}{\tsopt})$}
Now we can apply Proposition~\ref{prop:fnoiselessquadratictighter} and use approximation:
\begin{align}
    \fnclasn(\nu,\eta, \varsigma) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    \kappa_4 \frac{\eta^2}{\nu} - \epstight
\end{align}
with $\epstight \asymp \frac{\log n}{\sqrt{n}}$.
% \begin{align}
%     \fnclasn(\nu,\eta) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
%     \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} + O \left( \right)
% \end{align}
\subsubsection*{Step 4.1: Tight bounds on $\nu$}
Define the following set:
\begin{align}
    % \Gamma_1^{\alpha,L} 
    \Gamma_4^{\nu} 
    = \bigg\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    &\kappa_4 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
    - \epstight
    % + O \left( \frac{1}{n^{2/3}} \right)
    \\
    &~~\andtxt~~ 
    b\alpha + \nu \norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu \norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    ~~\andtxt~~ 
    \alpha \leq \alphaols
     \bigg\}.
    \label{eq:Gamma_4_nu_def}
\end{align}
First note that $\setNoiselessZero \subset \Gamma_4^{\nu} \subset \Gamma_2^{\nu}$ with high probability. Thus bound $\alpha \geq \alphauls$ shown in Step 2.2 holds in $\Gamma_4^{\nu}$ as well, which we make use of in the proof below.

For any $(\nu,b,\alpha, \varsigma)\in\Gamma_4^{\nu}$ holds that:
\begin{align}
    \loneboundclasnt - \nu\norm{\wgt}_1 \geq b\alpha \geq 
    \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}}  \frac{\sqrt{n}}{\norm{H}_{\infty}} \frac{\alpha}{\sqrt{\nu}}
\end{align}
where we used that $b^2 \geq \frac{n}{\norm{H}_{\infty}^2}\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\nu}$ since $\frac{\eta^2}{\nu} = w(\epsilon)$ ($\eta = \Omega(\frac{1}{\tsopt}),\nu = \Theta(\loneboundclasnt))$. Rearranging the terms we obtain that for any $(\nu,b,\alpha,\varsigma)\in \Gamma_4^{\nu}$ must hold that:
\begin{align}
    \nu^{3/2}\norm{\wgt}_1 - \loneboundclasnt \nu^{1/2} + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \sqrt{n} \frac{\alpha}{\norm{H}_{\infty}} \leq 0
\end{align}
Thus uniformly over all $\nu$ such that $(\nu,b,\alpha)$ we the following condition must hold:
\begin{align}
    \nu^{3/2}\norm{\wgt}_1 - \loneboundclasnt \nu^{1/2} + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \sqrt{n} \left[ \min \frac{\alpha}{\norm{H}_{\infty}} \subjto (
    \nu,b,\alpha)\in\Gamma_4^{\nu} \right]\leq 0
    \label{eq:nu_ineq_min_alpha}
\end{align}
Thus in order to upper bound $\nu$ we need to find a lower bound on $\alpha$. Note that we already have $\alpha \geq \alphauls$, but using this bound will not give tight bound on $\nu$. Now we discuss obtaining a tighter lower bound on $\alpha$.

For any $ (\nu,b,\alpha,\varsigma)\in\Gamma_4^{\nu}$ holds:
\begin{align}
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} -\epstight \leq b^2 \left( \frac{\norm{H}_{\infty}^2}{n} - \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\nu} \right) 
    \leq
    \frac{(\loneboundclasnt-\nu\norm{\wgt}_1)^2}{\alpha^2} \left( \frac{\norm{H}_{\infty}^2}{n} - \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\nu} \right)
\end{align}
and then plugging $\nu\norm{\wgt}_1 = \kappa \loneboundclasnt$ for $\kappa \in [\kappaunu,1]$ into the equation above yields:
\begin{align}
\label{eq:lower_bound_alpha_fcn_kappa}
    \sqrt{\frac{2}{\pi}} \norm{\gamma(\alpha)}_2^2 
    \leq
    \frac{\norm{H}_{\infty}^2}{n} \frac{\kappa \loneboundclasnt}{\norm{\wgt}_1} - \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\loneboundclasnt^2 (1-\kappa)^2} + O \left(  \frac{\epstight \alpha^2}{\loneboundclasnt} \right)
\end{align}
Note that only the right hand side depends on $\nu$ (and thus on $\kappa$). Hence maximizing over $\kappa$ the right hand side 
% \begin{align}
%     (1-\kappa)^3 = \frac{2\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n}{\loneboundclasnt^3}
% \end{align}
and substituting this $\kappa$ into \eqref{eq:lower_bound_alpha_fcn_kappa} we get the following inequality:
\begin{align}
    \frac{\alpha^{2/3}}{\norm{H}_{\infty}^{2/3}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{1/3} + n^{2/3} \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} \norm{\wgt}_1^{2/3}
    + O \left( \frac{\epstight n^{2/3} \alpha^2}{\norm{H}_{\infty}^2 \loneboundclasnt} \right)
    \leq
    \frac{1}{n^{1/3}} \frac{\loneboundclasnt}{\norm{\wgt}_1^{1/3}}
\end{align}
Note that until now we did not relax the constraints. Now raise to the third power the previous inequality and relax inequality while keeping the first two terms to get:
\begin{align}
    \frac{\alpha^{2}}{\norm{H}_{\infty}^2} \frac{9\sqrt{2}}{4\sqrt{\pi}}  + 3 \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}\norm{\wgt}_1^{2/3} n^{2/3} \frac{\alpha^{4/3}}{\norm{H}_{\infty}^{4/3}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{2/3}
    \leq
    \frac{1}{n} \frac{\loneboundclasnt^3}{\norm{\wgt}_1}   ( 1 + O\left(\frac{\epstight n}{\loneboundclasnt^2}\frac{\alphaols^2}{\norm{H}_{\infty}^2} \right)  )
\end{align}
We can further relax this constraint by using the previous lower bound $\alphauls$ in the second term as follows:
\begin{align}
    \frac{\alpha^{2}}{\norm{H}_{\infty}^2} \frac{9\sqrt{2}}{4\sqrt{\pi}}  + 3 \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} \norm{\wgt}_1^{2/3} n^{2/3} \frac{\alphauls^{4/3}}{\norm{H}_{\infty}^{4/3}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{2/3}
    \leq
    \frac{1}{n} \frac{\loneboundclasnt^3}{\norm{\wgt}_1}  (1+O\left(\frac{\log n}{n^{1/6}}\right))  
\end{align}
Note that the term on the left hand side is sum of two convex functions in $\alpha$ and thus is convex. Similarly, as before, we look for $\alphauuls < \alpha_m$ such that the previous inequality is not satisfied. Using concentration results, we get:
\begin{align}
    \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{1}{\tuulm^2} \left( 1 - \frac{4}{\tuulm^2} + O \left( \frac{1}{\tuulm^4} \right) \right) + 3\sqrt{\frac{2}{\pi}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{2/3} \norm{\wgt}_1^{2/3} &\frac{2 n^{2/3}}{\uulm \tuulm^2} \left(1+ O \left( \frac{1}{\tuulm^2} \right) \right) \frac{1}{\tulm^{4/3}} \left( 1- \frac{8}{3}\frac{1}{\tulm^2} + O \left( \frac{1}{\tulm^4} \right) \right) \\
    &>
    \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{1}{\tsopt^2} \left( 1- \frac{2}{\tsopt^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right)\left(1+O\left( \frac{\log n}{n^{1/6}} \right)\right)
\end{align}
and we can choose $\uulm = \lambda \sopt$ with $\lambda\in(0,1)$. This gives us a lower bound on $\alpha$ which is tight enough for obtaining bounds on $\nu$ with right multiplicative constant. 
Substituting $\alpha=\alphauuls$ into inequality~\eqref{eq:nu_ineq_min_alpha} and setting $\nu\norm{
\wgt}_1 = \kappa^2\loneboundclasnt$ with $\kappa^2 \in [\kappa_3,1]$ we obtain:
\begin{align}
    \kappa^3 - \kappa + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \frac{\sqrt{n}}{\loneboundclasnt^{3/2}} \frac{\alphauuls}{\norm{H}_{\infty}} \leq 0
\end{align}
Using concentration inequalities we obtain
\begin{align}
    \kappa^3 - \kappa + \frac{2}{3\sqrt{3}} \frac{\tsopt}{\tuulm} \left( 1-\frac{2}{\tuulm^2} + O \left( \frac{1}{\tuulm^3} \right) \right) \left( 1 + \frac{1}{\tsopt^2} + O\left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) \leq 0
\end{align}
and after substituting $\uulm = \lambda \sopt$ with $\lambda<1$ we get the following:
\begin{align}
    \kappa^3 - \kappa + \frac{2}{3\sqrt{3}} + \frac{2}{3\sqrt{3}}\frac{\log\lambda -1}{\tsopt^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \leq 0
\end{align}
Thus, we obtain $\kappa^2 \in \left[ \frac{1}{3}-\frac{\tlambda}{\tsopt^{2/3}}, \frac{1}{3}+\frac{\tlambda}{\tsopt^{2/3}} \right]$ for some positive universal constant $\tlambda$, which we can write as $\nu\norm{\wgt}_1 = \frac{\loneboundclasnt}{3} (1+O(\tsopt^{-2/3}))$.
% $\ulambda,\olambda$.

\subsubsection*{Step 4.2: Upper bound on $\eta$}
Define the following set:
\begin{align}
    % \Gamma_1^{\alpha,L} 
    \Gamma_{4}^{\eta} 
    = \bigg\{ (\nu, b, \alpha, \varsigma)
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    &\kappa_4 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
    - \epstight
    % + O \left( \frac{1}{n^{2/3}} \right)
    \\
    &~~\andtxt~~ 
    b\alpha + \nu \norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \left| \nu\norm{\wgt}_1-\frac{\loneboundclasnt}{3} \right| \leq \frac{\tlambda \loneboundclasnt}{\tsopt^{2/3}}
    ~~\andtxt~~ 
    \alpha \geq \alphauuls
     \bigg\}.
    \label{eq:Gamma_4_eta_def}
\end{align}
\begin{align}
\eta^2 
    \leq
    \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 
    \leq 
    \max_{\nu,\alpha} (\loneboundclasnt-\nu\norm{\wgt}_1)^2 \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}
    \leq
    \loneboundclasnt^2 \left( 1-\frac{1}{3} + \frac{\tlambda}{\tsopt^{2/3}} \right)^2 \frac{2}{\uulm} \left(1+O\left(\frac{1}{\tuulm^2}\right)\right)
    \lesssim \frac{1}{\tsopt^2}
\end{align}
\subsubsection*{Bound 5: Tight bounds on $\eta$}
Now we can apply Proposition~\ref{prop:uniform_conv_noiseless} and use approximation:
\begin{align}
    \left|\fnclasn(\nu,\eta)     -
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} - \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} \right|
    =
    O \left( \frac{\eta^2}{\nu^3}, \rho\eta^2, \frac{\eta^3}{\nu}\epsilon_n \right) + O \left( \frac{1}{\nu^3}, \epsilon_c \right) 
    % =: O_{\eta}(\eta,n,\rho) + O_{\nu,c}(\nu,\epsilon) 
    =: \frac{\eta^2}{\nu} \OOO_f
\end{align}
with $\OOO_f = O\left( \frac{\epsilon_n^3}{\tsopt} \right)$, $\epsilon_n \asymp \sqrt{\log\log n}$.
\begin{align}
    \Gamma_5^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    \sqrt{\frac{2}{\pi}} \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu}  (1+\OOO_f)
    ~~\andtxt~~ 
    b\alpha + \nu\norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \left| \nu\norm{\wgt}_1-\frac{\loneboundclasnt}{3} \right| \leq \frac{\tlambda \loneboundclasnt}{\tsopt^{2/3}}
    % \nu \in\loneboundclasnt\left[ \frac{1}{3}-\frac{\tlambda}{\tsopt^{2/3}}, \frac{1}{3}+\frac{\tlambda }{\tsopt^{2/3}} \right]
    \right\}.
    \label{eq:Gamma_5_eta_def}
\end{align}
Similarly to Equality \eqref{eq:lower_bound_alpha_fcn_kappa} we get:
\begin{align}
    \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt} (1-\kappa)^2 (1+\OOO_f) + \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3} 
    \leq
    \kappa(1-\kappa)^2 \leq \frac{4}{27}
\end{align}
and using our established bound on $\nu\norm{\wgt}_1$ we get $(1-\kappa)^2 \geq (1- \frac{1}{3}-\frac{\tlambda}{\tsopt^{2/3}})^2$ and hence we obtain:
\begin{align}
    3\sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}\frac{n\norm{\wgt}_1}{\loneboundclasnt} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} +  \OOO_f \right) +  \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3} 
    \leq 1
    \label{eq:tight_bound_noisy_alpha_ineq_tight}
\end{align}
Note that the function is convex in $\alpha$. Using concentration, we get:
\begin{align}
    2 \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n \tsopt \norm{\wgt}_1 )^{2/3}}{m \tm^2} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right)  \right) \left(1+O \left( \frac{1}{\tm^2} \right) \right) 
    +
    \frac{\tsopt^2}{\tm^2} \left( 1- \frac{2}{\tm^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    \leq 1
\end{align}
Now we claim that the $\ulmstar,\olmstar$ given in Lemma~\ref{lemma_uls_ols_exp}, respectively, with $\kappa=1/3$ do not satisfy this inequality for the well-chosen universal constant $\mu$ since
\begin{align}
    2& \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n \tsopt \norm{\wgt}_1)^{2/3}}{\ulmstar \tulmstar^2} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} +  O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    +
    \frac{\tsopt^2}{\tulmstar^2} \left( 1- \frac{2}{\tulmstar^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    \\
    &=
    1 - \frac{\mu}{\tsopt^{7/3}} \left(1-\frac{\tsopt^2}{\tulmstar^2} \right)  + \frac{2\mu^2-6\tlambda}{\tulmstar^2\tsopt^{2/3}} + O \left( \frac{(\log\log n)^{3/2}}{\tsopt^3} \right) 
    =
    1 +\frac{2\mu^2-6\tlambda}{\tsopt^{8/3}} + O \left( \frac{(\log\log n)^{3/2}}{\tsopt^3} \right) > 1
\end{align}
for $\mu > \sqrt{3\tlambda}$. Similarly, for $\olmstar$ we get:
\begin{align}
    2& \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n \tsopt \norm{\wgt}_1)^{2/3}}{\olmstar \tolmstar^2} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    +
    \frac{\tsopt^2}{\tolmstar^2} \left( 1- \frac{2}{\tolmstar^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    \\
    &=
    1 + \frac{\mu}{\tsopt^{7/3}} \left(1-\frac{\tsopt^2}{\tolmstar^2} \right)  + \frac{2\mu^2-6\tlambda}{\tolmstar^2\tsopt^{2/3}} + O \left( \frac{(\log\log n)^{3/2}}{\tsopt^{3}} \right) 
    =
    1 +\frac{2\mu^2-6\tlambda}{\tsopt^{8/3}} + O \left( \frac{(\log\log n)^{3/2}}{\tsopt^{3}} \right) > 1
\end{align}
Now we can bound $\eta$ as follows:
\begin{align}
    \eta^2 
    \leq
    \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 
    &\leq 
    \max_{\nu,\alpha} (\loneboundclasnt-\nu\norm{\wgt}_1)^2 \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}
    \leq
    \loneboundclasnt^2 \left( 1-\frac{1}{3} + \frac{\tlambda}{\tsopt^{2/3}} \right)^2 \frac{2}{\ulmstar} \left(1+O\left(\frac{1}{\tulmstar^2}\right)\right)
    \\
    &\leq
    \frac{2}{3} \frac{1}{\tsopt^2} \exp \left( \frac{\mu}{2\tsopt^{1/3}} \right) \left(1+ O \left( \frac{1}{\tsopt^{2/3}} \right) \right)
    = 
    \frac{2}{3} \frac{1}{\tsopt^2} \left( 1 + \frac{\mu}{2\tsopt^{1/3}} + O \left( \frac{1}{\tsopt^{2/3}} \right) \right) =: \overline{\eta}^2
\end{align}
and
\begin{align}
    \eta^2 
    \geq
    \min_{b,\alpha} b^2\norm{\gamma(\alpha)}_2^2 
    &\geq
    \min_{\nu,\alpha} \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{n}{\nu} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{n\norm{\wgt}_1}{\loneboundclasnt \left( \frac{1}{3}+\frac{\tlambda}{\tsopt^{2/3}} \right)} \frac{2}{\olmstar\tolmstar^2} \left( 1 + O \left( \frac{1}{\tolmstar^2} \right) \right)
    \\
    &\geq
    \frac{2}{3} \frac{1}{\tsopt^2} \exp \left( -\frac{\mu}{2\tsopt^{1/3}} \right) \left(1 - O \left( \frac{1}{\tsopt^{2/3}} \right) \right)
    =
    \frac{2}{3} \frac{1}{\tsopt^2} \left( 1 - \frac{\mu}{2\tsopt^{1/3}} - O \left( \frac{1}{\tsopt^{2/3}} \right) \right) =: \underline{\eta}^2
\end{align}

\subsubsection*{Bound 5: Tight upper bound on $\varsigma$}
\begin{align}
    \Gamma_6^{\varsigma} = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    \sqrt{\frac{2}{\pi}} \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} (1+\OOO_f)
    + \kappa_5 \frac{\varsigma^2}{\nu} 
    ~~\andtxt~~ 
    b^2\norm{\gamma(\alpha)}_2^2 \geq ... 
    ~~\andtxt~~ 
    \nu + b\alpha \leq \loneboundclasnt
    ~~\andtxt~~ 
    \left| \nu-\frac{\loneboundclasnt}{3} \right| \leq \frac{\tlambda \loneboundclasnt}{t_m^{2/3}}
    \right\}.
    \label{eq:Gamma_6_varsigma_def}
\end{align}
Similarly to Equation~\eqref{eq:tight_bound_noisy_alpha_ineq_tight}:
\begin{align}
    \kappa_5 \varsigma^2 \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3} \leq 
    1-3\sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}\frac{n\norm{\wgt}_1}{\loneboundclasnt} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} +  \OOO_f \right) -  \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3}
\end{align}
\begin{align}
    \varsigma^2 
    \lesssim 
    \frac{\norm{H}_{\infty}^2}{\alpha_{\ulmstar}^2}
    \frac{\loneboundclasnt^3}{n\norm{\wgt}_1} \left[
    1-3\sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha_{\olmstar} )}_2^2}{\norm{H}_{\infty}^2}\frac{n\norm{\wgt}_1}{\loneboundclasnt} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} +  O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) -  \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{\alpha_{\ulmstar}^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3} \right]
    \lesssim 
    \frac{1}{\tsopt^{7/3}}
\end{align}


==> sections/subsections_theory/noiseless/sunicon_proof_old.tex <==
% \section{TEMP: s sparse uniform convergence noiseless}
\subsection{Proof of Uniform Convergence Proposition~\ref{prop:BoundGamma0_class_noiseless}}
\label{sec:proof_unicon_noiseless}

\begin{align}
    \setNoiselessZero = \left\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasn(\nu,b\|\gamma(\alpha)\|_2, \varsigma) ~~\andtxt~~  \Big| \nu\norm{\wgt}_1 - \norm{\varsigma}_1 \Big| + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasn \right\}.
    \label{eq:Gamma0_def_class_noiseless}
\end{align}
As discussed in the proof sketch, proof consists of iterative bounding and approximation steps. The structure of the proof is as follows: for every bound step we use different approximation of $\fnclasn$, and based on it we develop tighter bounds on variables of interest. Thus the statement of the proposition follows from the tightest, last bound i.e. Bound 5. We start with the following bound:
\subsubsection*{Bound 1: \texorpdfstring{$\nu = \Omega(n^{2/15})$}{nuomega}}
Recall the definition of the set $\setNoiselessZero$ from Equation~\eqref{eq:Gamma0_def_class_noiseless} and that by parametric path approach from Section~\ref{subsec:path_param} we have $\eta = \norm{\wtwo}_2 = b\norm{\gamma(\alpha)}_2$. In order to show the lower bound $\nu = \Omega(n^{2/15})$ we define the following set:
\begin{align}
    % \setNoiselessZero^{\nu,L}
    \Gamma_1^{\nu}
    = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasn (\nu,b\norm{\gamma(\alpha)}_2, \varsigma) 
    ~~\andtxt~~ 
    b\alpha \leq \loneboundclasn 
    \right\}.
    \label{eq:Gamma_1_nu_constant_lower}
\end{align}
in which we relax the second constraint from definition of set $\setNoiselessZero$ and thus $\setNoiselessZero \subset \Gamma_1^{\nu}$. The goal is to show that uniformly over all $\nu\in \Gamma_1^{\nu}$ holds that $\nu=\Omega(n^{2/15})$ implying that this lower bound holds also uniformly over $\setNoiselessZero$.

Note that for $(\nu,b,\alpha)\in \Gamma_1^{\nu}$ we have:
\begin{align}
    \fnclasn (\nu,b\norm{\gamma(\alpha)}_2, \varsigma) 
    \leq
    \max_{b,\alpha} \frac{1}{n}b^2 \norm{H}_{\infty}^2 
    \leq
    \max_{\alpha} \frac{1}{n} \frac{\loneboundclasn^2}{\alpha^2} \norm{H}_{\infty}^2
    =
    \frac{1}{n} \loneboundclasn^2 \norm{H}_{\infty}^2
    \lesssim
    \frac{1}{n} \left( \frac{n}{\tsopt^2} \right)^{2/3} \log d 
    \lesssim
    \left( \frac{1}{n} \right)^{2/15}
\end{align}
with probability $\geq 1-\frac{1}{d}$, where we used $d\lesssim \exp(\kappa n^{1/5})$ and $\alpha\geq 1$. Also, we have:
\begin{align}
    \fnclasn (\nu,b\norm{\gamma(\alpha)}_2)  
    =
    \frac{1}{n} \sum_{i=1}^n \possq{ 1 - \nu \abs{\gausswone_i} - \eta\gausswtwo_i - \sum_{j=2}^s \gausswj_i \varsigma_j} 
    \gtrsim
    \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}}
    \label{eq_etanu_to_nu_fnclansn}
\end{align}
with probability $\geq 1-\exp(-c_1 n)$ for some positive universal constant $c_1$. Now we show that $\nu = \Omega(n^{2/15})$. Assume, in contradiction, that there exists some universal constant $\kappa>0$ such that $\nu \leq \kappa n^{2/15}$ for some $\nu\in\Gamma_1^{\nu}$. From the previous two inequalities, we know that $\nu$ must satisfy with high probability that:
\begin{align}
    \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}} 
    \lesssim
    \left( \frac{1}{n} \right)^{2/15}
    \label{eq:ineq_nu_first_bound_condition}
\end{align}
Define $F_n(\frac{1}{2\nu}) := \frac{1}{n}\sum_{i=1}^n \indicator{|\gausswone_i|\leq \frac{1}{2\nu}}$ and $F(\frac{1}{2\nu}) := \PP( |\Gausswone| \leq \frac{1}{2\nu} )$. Using the same reasoning as in Lemma~\ref{lemma:dkw_number_active_indicators} one can show that from the set of indicators $\{ \indicator{1-\nu\abs{\gausswone_i}}\}_{i=1}^n$ there are at least $k:=nF_n(\frac{1}{2\nu}) \gtrsim n^{1-p}$ indicators activated when $\nu=O(n^p)$, $p\in(0,\frac{2}{5})$. Thus we have
\begin{align}
    \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}} 
    \geq
    \frac{n F_n(\frac{1}{2\nu})}{n} \left(\frac{1}{2} \right)^2
    \gtrsim
    n^{-p}
\end{align}

Thus for any $n\geq c_1$ and $p\leq \frac{2}{15}$ we can always choose constants such that  inequality~\eqref{eq:ineq_nu_first_bound_condition} does not hold. Hence we conclude that $\nu = \Omega(n^{2/15})$.



Assume that $\nu\norm{\wgt}_1 = w(\loneboundclasn)$. Then also $\norm{\varsigma}_1 = w(\loneboundclasn)$ and thus $\norm{\varsigma}_2 \geq \frac{1}{\sqrt{s}} \norm{\varsigma}_1 \asymp \nu\norm{\wgt}_1 / \sqrt{s}$. Then
\begin{align}
    (\frac{1}{n})^{2/15} &\gtrsim \fnclasn = \frac{1}{n}\sum_{i=1}^n (1-\nu|\gausswone_i| - \eta\gausswtwo_i - \sum_{j=2}^s \varsigma_j \gausswj_i )_+^2\\
    &\gtrsim
    \frac{1}{n}\sum_{i=1}^n (1-\nu|\gausswone_i| - \eta\gausswtwo_i - \sum_{j=2}^s \varsigma_j \gausswj_i )_+^2 \indicator{\gausswtwo_i \leq 0, - \sum_{j=2}^s \varsigma_j \gausswj_i \geq \norm{\varsigma}_2 }\\
    &\gtrsim
    \frac{1}{n}\sum_{i=1}^k \indicator{1-\nu\abs{\gausswone_i}} \norm{\varsigma}_2^2
    \gtrsim
    \frac{\norm{\varsigma}_2^2}{\nu}
\end{align}
where $k = \inf_{\varsigma} \sum_{i=1}^n \indicator{\gausswtwo_i \leq 0, - \sum_{j=2}^s \varsigma_j \gausswj_i \geq \norm{\varsigma}_2 } = bla bla \asymp n $.

\begin{align}
    (\frac{1}{n})^{2/15} &\gtrsim \fnclasn = \frac{1}{n}\sum_{i=1}^n (1-\nu|\gausswone_i| - \eta\gausswtwo_i - \sum_{j=2}^s \varsigma_j \gausswj_i )_+^2\\
    &\gtrsim
    \frac{1}{n}\sum_{i=1}^n (1-\nu|\gausswone_i| - \eta\gausswtwo_i - \sum_{j=2}^s \varsigma_j \gausswj_i )_+^2 \indicator{\gausswtwo_i \leq 0, - \sum_{j=2}^s \varsigma_j \gausswj_i \geq \norm{\varsigma}_2 }\\
    &\gtrsim
    \frac{1}{n}\sum_{i=1}^k \indicator{\norm{\varsigma}_2-\nu\abs{\gausswone_i}} (1+\norm{\varsigma}_2-\nu\abs{\gausswone_i})^2
    \\
    &\gtrsim \frac{1}{n} \sum_{i=1}^k \indicator{1-\frac{\nu}{\norm{\varsigma}_2}\abs{\gausswone_i}}
\end{align}
and $\frac{\nu}{\norm{\varsigma}_2} \leq \sqrt{s}/\norm{\wgt}_1 = o(\sqrt{n})$.


\subsubsection*{Bound 1': \texorpdfstring{$\norm{\varsigma}_1 = O \left( \frac{n^{1/15}}{\tsopt^{3}} \sqrt{\nu} \norm{\wgt}_1^{1/3} \right)$}{bound1p}}
Conditioning on the fact that $\nu = \Omega(n^{2/15})$ we can use lower bound from Proposition~\ref{prop:fnoiselessquadraticvarsigma}:
\begin{align}
    \fnclasn(\nu,\eta) \gtrsim \frac{\norm{\varsigma}_2^2}{\nu} -  \frac{\norm{\varsigma}_2^2}{\sqrt{n}}
\end{align}
which holds with probability $1-s\exp(-c_1 n)$.

Define
\begin{align}
    % \Gamma_1^{\eta,U} =
    \Gamma_{1'} =
    \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \gtrsim \frac{\norm{\varsigma}_2^2}{\nu} - \frac{s}{\sqrt{n}}
    ~~\andtxt~~ 
    b\alpha \leq \loneboundclasn 
    ~~\andtxt~~ 
    \nu = \Omega(n^{2/15})
    \right\}.
    \label{eq:Gamma_1p_eta_def_upp}
\end{align}
\begin{align}
    \frac{\norm{\varsigma}_2^2}{\nu} 
    \lesssim
    \frac{1}{n}b^2 \norm{H}_{\infty}^2 + \frac{s}{\sqrt{n}}
    \lesssim
    \frac{\loneboundclasn^2}{n} \frac{\norm{H}_{\infty}^2}{\alpha^2} + \frac{s}{\sqrt{n}}
    \lesssim
    \frac{\norm{\wgt}_1^{2/3}}{n^{2/15}\tsopt^{4/3}}
\end{align}
where we used assumption $s\lesssim n^{4/15} \tsopt^{-14/3}$. Using this assumption once again we have $\norm{\varsigma}_1 \leq \sqrt{s} \norm{\varsigma}_2 \lesssim \frac{n^{1/15}}{\tsopt^{3}} \sqrt{\nu} \norm{\wgt}_1^{1/3}$. 

\subsubsection*{Bound 2: \texorpdfstring{$\eta,\norm{\varsigma}_2 = O(1),\ \nu\norm{\wgt}_1 \geq \kappa_3 \loneboundclasn$}{bound1} }
Since 
$   \left| \nu\| \wgt\|_1 - \norm{\varsigma}_1 \right| 
    =
    \nu \|\wgt\|_1 \left| 1 - \frac{\norm{\varsigma}_1}{\nu\|\wgt\|_1} \right|
    \leq \loneboundclasn
$
and
$
    \frac{\norm{\varsigma}_1}{\nu\|\wgt\|_1}     \lesssim 
    \frac{n^{1/15}}{\tsopt^3 \sqrt{\nu}\|\wgt\|_1^{2/3}} 
    \lesssim
    \frac{1}{\tsopt^3}
$
this implies that $\nu \|\wgt\|_1 \leq \loneboundclasn (1+\frac{c_1}{\tsopt^3}) =: \loneboundclasnt $. Conditioning on the fact that $\nu = \Omega(n^{2/15})$ and $\nu = O(\loneboundclasnt) = o(\sqrt{n}/\log(n s))$ we can use lower bound from Proposition~\ref{prop:fnoiselessquadratic}:\begin{align}
    \fnclasn (\nu,\eta,\varsigma) \geq \kappa_1 \frac{1}{\nu} + \kappa_2 \frac{\eta^2}{\nu} + \kappa_3 \frac{\norm{\varsigma}_2^2}{\nu} 
\end{align}
which holds with probability $1-c_1/(n s)$ for some positive universal constants $\kappa_1,\kappa_2,\kappa_3,c_1$.

Define
\begin{align}
    % \Gamma_1^{\eta,U} =
    \Gamma_2 =
    \left\{ (\nu, b, \alpha,\varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq \kappa_1 \frac{1}{\nu} + \kappa_2 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
    ~~\andtxt~~ 
    b\alpha \leq \loneboundclasnt
    ~~\andtxt~~ 
    \nu \norm{\wgt}_1 \leq \loneboundclasnt
    ~~\andtxt~~ 
    \nu = \Omega(n^{2/15})
    \right\}.
    \label{eq:Gamma_2_eta_def_upp}
\end{align}
Note that constraints in $\Gamma_2$ are relaxations of constraints in definition of $\setNoiselessZero$ and hence $\setNoiselessZero \subset \Gamma_2$ with high probability. By finding bounds on $\nu,\eta$ from $\Gamma_2$ we obtain a valid upper bound in $\setNoiselessZero$ as well.

\textbf{Step 2.1: Upper bound on $\eta$.}
We bound $\nu$ as follows:
\begin{align}
    \eta^2
    &\leq
    \max_{\nu,b,\alpha,\varsigma} \left[ b^2\norm{\gamma(\alpha)}_2^2
    \subjto
    (\nu,b,\alpha,\varsigma)\in \Gamma_2 \right]\\
    &=
    \max_{\nu,b,\alpha} \left[ b^2\norm{\gamma(\alpha)}_2^2 
    \subjto 
    \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n}\nu \norm{H}_{\infty}^2
    ~~\andtxt~~ 
    b\alpha \leq \loneboundclasnt
    ~~\andtxt~~ 
    \nu \norm{\wgt}_1 \leq \loneboundclasnt
    \right]\\
    &=
    \max_{\alpha} \left[ \loneboundclasnt^2\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2} 
    \subjto 
    \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n} \frac{\loneboundclasnt}{\norm{\wgt}_1} \norm{H}_{\infty}^2
    \right]
    \label{eq:eta_upper_bound_step21}
\end{align}
where we used only that $(\nu,b,\alpha,\varsigma)\in \Gamma_2$ satisfy appropriate constraints. As we mentioned in the Section~\ref{subsubsec:prop_gamma_alpha}, function $\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}$ is monotonically decreasing function in $\alpha$, whereas $\norm{\gamma(\alpha)}_2^2$ is a convex function. Thus, similarly as previously discussed in \cite{donhauser2022fast}, it is sufficient to find $\alphauls < \alphasopt$ such that
\begin{align}
     \norm{\gamma(\alphauls)}_2^2 > \frac{1}{\kappa_2 n} \frac{\loneboundclasnt}{\norm{\wgt}_1} \norm{H}_{\infty}^2
\end{align}
to obtain an upper bound on $\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}$. Using concentration results from Section~\ref{subsubsec:prop_gamma_alpha} we can rewrite above inequality as follows:
\begin{align}
    \frac{2}{\ulm \tulm^2} \left( 1+O \left( \frac{1}{\tulm^2} \right) \right) > \frac{1}{\kappa_2 n} \frac{\kappam}{\norm{\wgt}_1^{2/3}} \left( \frac{n}{\tsopt^2} \right)^{1/3} \left( 1 + O \left( \frac{1}{\tsopt^2} \right) \right)
\end{align}
It is straightforward to show that we can choose $\ulm = \lambda \left( \frac{n\norm{\wgt}_1}{\tsopt^2} \right)^{2/3}$ with sufficiently small universal constant $\lambda = \lambda(\kappa_2,\kappam)>0$. We finish this step by substituting this choice of $\ulm$ into the upper bound from Equation~\eqref{eq:eta_upper_bound_step21} to get:
\begin{align}
    \eta^2 
    \leq
    \loneboundclasnt^2 \frac{\norm{\gamma(\alphauls)}_2^2}{\alphauls^2}
    = \kappam^2 \left( \frac{n\norm{\wgt}_1}{\tsopt^2} \right)^{2/3} \left( 1 + O \left( \frac{1}{\tsopt^2} \right) \right) 
    \frac{2}{\ulm} \left( 1 + O \left( \frac{1}{\tulm^2} \right) \right) =: \boundeta^2 = O(1) 
\end{align}\\

\noindent\textbf{Step 2.2: Upper bound on $\norm{\varsigma}_2$}.
\begin{align}
    \norm{\varsigma}_2^2 
    \lesssim
    \max \nu\frac{1}{n}b^2\norm{H}_{\infty}^2
    \lesssim 
    \frac{\loneboundclasnt}{\norm{\wgt}_1} \frac{1}{n} \loneboundclasnt^2 \frac{\norm{H}_{\infty}^2}{\alphauls^2}
    =: B_{\varsigma}^2 = O(1)
\end{align}
\noindent\textbf{Step 2.3: Lower bound on $\nu$}.
Similarly to Equation~\eqref{eq:eta_upper_bound_step21}, we can bound $\nu$ on the set $\Gamma_2$ as follows:
\begin{align}
    \nu
    &\geq
    \kappa_1 n \left[ \min_{b,\alpha} \frac{1}{b^2\norm{H}_{\infty}^2}  \subjto (\nu,b,\alpha,\varsigma)\in \Gamma_2 \right] \\
    &=
    \frac{\kappa_1 n}{\loneboundclasnt^2} \left[ \min_{\alpha} \frac{\alpha^2}{\norm{H}_{\infty}^2} \subjto \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n} \loneboundclasnt \norm{H}_{\infty}^2 \right]
    \label{eq:nu_lower_bound_step22}
\end{align}
Similarly as above, we obtain that $\alpha\geq \alphauls$ and after substitution of $\ulm$ as defined above, we have:
\begin{align}
    \nu \geq \kappa_1 \frac{n}{\loneboundclasnt^2} \frac{\alphauls^2}{\norm{H}_{\infty}^2} 
    &=
    \frac{\kappa_1}{\kappam^2} \norm{\wgt}_1^{-2/3} \frac{(n \tsopt^4)^{1/3}}{\tulm^2}  (1+O \left( \frac{1}{\tsopt^2}, \frac{1}{\tulm^2} \right) ) \\
    &\geq
    \frac{\kappa_1}{\kappam^2} \norm{\wgt}_1^{-2/3} \left( \frac{n}{\tsopt^2} \right)^{1/3} (1+O \left( \frac{1}{\tsopt^2} \right) ) =:  \kappa_3 \frac{\loneboundclasnt}{\norm{\wgt}_1^{2/3}}
\end{align}
implying that $\nu \norm{\wgt}_1 \in [\kappa_3,1]\loneboundclasnt$. Note that from definition of $\kappam$ and the fact that $\kappa_1$ must be smaller than constant from Taylor expansion of $\fnclasn$ i.e. $\kappa_1 \leq \frac{\sqrt{2}}{3\sqrt{\pi}}$ (see Proposition~\ref{prop:uniform_conv_noiseless}) we get that $\kappa_3$ must satisfy $0 < \kappa_3 < \frac{4}{27}(1+O \left( \frac{1}{\tsopt^2} \right) )$.

\subsubsection*{Bound 3: \texorpdfstring{$\eta = \Omega \left( \frac{1}{\tsopt} \right)$}{bound2} } 
Here we use approximation:
\begin{align}
    \fnclasn(\nu,\eta) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + O\left( \frac{1}{\nu^3} \right)
\end{align}
\begin{align}
    % \Gamma_1^{\alpha,U} \textbf{o}
    \Gamma_3^{\eta} 
    = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \frac{1}{\nu^3} \right)
    ~~\andtxt~~ 
    b\alpha + \nu\norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu\norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    \right\}.
    \label{eq:Gamma_3_eta_lower_def}
\end{align}
Again, we have $\setNoiselessZero \subset \Gamma_3^{\eta}$. Note that for $(\nu,b,\alpha,\varsigma)\in \Gamma_3^{\eta}$ holds:
\begin{align}
    \eta^2 
    &\geq 
    \left[ \min_{\nu, b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \frac{1}{\nu^3} \right)
    ~~\andtxt~~ 
    b\alpha + \nu\norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu\norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    \right]\\
    &\gtrsim
     n \left[ \min_{\nu,\alpha} \frac{1}{\nu} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}  \subjto
    \frac{1}{n} \left( \frac{\loneboundclasnt-\nu\norm{\wgt}_1}{\alpha} \right)^2 \norm{H}_{\infty}^2
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \frac{1}{\nu^3} \right)
    % ~~\andtxt~~ 
    % b\alpha + \nu \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu\norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    \right]\\
    &\gtrsim
    \frac{n}{\loneboundclasnt} \left[
    \min_{\nu,\alpha} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} 
    \subjto
    \frac{\alpha^2}{\norm{H}_{\infty}^2} \leq \frac{3\sqrt{\pi}}{\sqrt{2}}\frac{1}{n}\nu(\loneboundclasnt-\nu\norm{\wgt}_1)^2 + O \left( \frac{1}{\nu^3} \right)
    % ~~\andtxt~~ 
    % b\alpha + \nu \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu \norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    \right]
\end{align}
% Also note that $\alpha$ that satisfies constraints above is upper bounded
% \begin{align}
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} \leq \frac{1}{n} b^2 \norm{H}_{\infty}^2 \leq \frac{1}{n} \left( \frac{\loneboundclasnt-\nu}{\alpha} \right)^2 \norm{H}_{\infty}^2
% \end{align}
Since given that $\nu\norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt$ the function $\nu (\loneboundclasnt -\nu\norm{\wgt}_1)^2$ is maximized for $\nu\norm{\wgt}_1 = \loneboundclasnt/3$ and $1/3\in[\kappa_3,1]$ we can upper bound $\alpha$ as follows:
\begin{align}
    \frac{\alpha^2}{\norm{H}_{\infty}^2} 
    \leq
    \frac{3\sqrt{\pi}}{\sqrt{2}} \frac{1}{n} \nu (\loneboundclasnt -\nu\norm{\wgt}_1)^2 + O\left( \frac{1}{\nu^3} \right) 
    &\leq
    \frac{12\sqrt{\pi}}{27\sqrt{2}} \frac{1}{n} \frac{\loneboundclasnt^3}{\norm{\wgt}_1} + O\left( \frac{1}{\loneboundclasnt^3} \right) \\
    &\leq
    \frac{1}{\tsopt^2}  \left( 1 - \frac{2}{3}\frac{1}{\tsopt^2} + O \left( \frac{\epsilon_n}{\tsopt^3} \right) \right)+ O\left( \frac{\tsopt^2}{n} \right) 
    \label{eq:alpha_ols_bound_nu_loneboundclasn}
\end{align}
where we used definition of $\loneboundclasnt$ from Proposition~\ref{prop:localization_noiseless_ssparse}.

From Section~\ref{subsubsec:prop_gamma_alpha} we have that $\norm{\gamma(\alpha)}_2^2$ is a convex function and it decreases over $[1,\alpha_{d+1/2}]$. 
Hence in order to lower bound $\norm{\gamma(\alpha)}_2^2$, it is sufficient to find a point $\alphaols$ such that $\alphaols \geq \alpha_m$ for which Equation~\eqref{eq:alpha_ols_bound_nu_loneboundclasn} does not hold, i.e. for $\olm$ for which we have:
\begin{align}
    \frac{1}{\tolm^2} \left( 1 - \frac{4}{\tolm^2} + O \left( \frac{1}{\tolm^4} \right)\right) 
    >
    \frac{1}{\tsopt^2} \left( 1 - \frac{2}{3}\frac{1}{\tsopt^2} + O \left( \frac{\epsilon_n}{\tsopt^3} \right) \right)
\end{align}
We can choose $\olm = \lambda \sopt$ for some constant $\lambda>1$ since 
\begin{align}
    \frac{\tsopt^2}{\tolm^2} = 1 + \frac{2\log\lambda}{\tsopt^2} + O \left( \frac{1}{\tsopt^4} \right)
\end{align}
Thus we finally obtain:
\begin{align}
    \eta^2  
    \gtrsim
    \frac{n}{\loneboundclasnt} \frac{\norm{\gamma(\alphaols)}_2^2}{\norm{H}_{\infty}^2}
    \gtrsim
    (n \tsopt)^{2/3} \frac{1}{\olm \tolm^2}
    \gtrsim
    \frac{1}{\tsopt^2}
\end{align}
\subsubsection*{Bound 4: Tight bounds on $\nu$ and $\eta = \Theta(\frac{1}{\tsopt})$}
Now we can apply Proposition~\ref{prop:fnoiselessquadratictighter} and use approximation:
\begin{align}
    \fnclasn(\nu,\eta, \varsigma) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    \kappa_4 \frac{\eta^2}{\nu} - \epstight
\end{align}
with $\epstight \asymp \frac{\log n}{\sqrt{n}}$.
% \begin{align}
%     \fnclasn(\nu,\eta) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
%     \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} + O \left( \right)
% \end{align}
\subsubsection*{Step 4.1: Tight bounds on $\nu$}
Define the following set:
\begin{align}
    % \Gamma_1^{\alpha,L} 
    \Gamma_4^{\nu} 
    = \bigg\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    &\kappa_4 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
    - \epstight
    % + O \left( \frac{1}{n^{2/3}} \right)
    \\
    &~~\andtxt~~ 
    b\alpha + \nu \norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \nu \norm{\wgt}_1 \in [\kappa_3, 1] \loneboundclasnt
    ~~\andtxt~~ 
    \alpha \leq \alphaols
     \bigg\}.
    \label{eq:Gamma_4_nu_def}
\end{align}
First note that $\setNoiselessZero \subset \Gamma_4^{\nu} \subset \Gamma_2^{\nu}$ with high probability. Thus bound $\alpha \geq \alphauls$ shown in Step 2.2 holds in $\Gamma_4^{\nu}$ as well, which we make use of in the proof below.

For any $(\nu,b,\alpha, \varsigma)\in\Gamma_4^{\nu}$ holds that:
\begin{align}
    \loneboundclasnt - \nu\norm{\wgt}_1 \geq b\alpha \geq 
    \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}}  \frac{\sqrt{n}}{\norm{H}_{\infty}} \frac{\alpha}{\sqrt{\nu}}
\end{align}
where we used that $b^2 \geq \frac{n}{\norm{H}_{\infty}^2}\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\nu}$ since $\frac{\eta^2}{\nu} = w(\epsilon)$ ($\eta = \Omega(\frac{1}{\tsopt}),\nu = \Theta(\loneboundclasnt))$. Rearranging the terms we obtain that for any $(\nu,b,\alpha,\varsigma)\in \Gamma_4^{\nu}$ must hold that:
\begin{align}
    \nu^{3/2}\norm{\wgt}_1 - \loneboundclasnt \nu^{1/2} + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \sqrt{n} \frac{\alpha}{\norm{H}_{\infty}} \leq 0
\end{align}
Thus uniformly over all $\nu$ such that $(\nu,b,\alpha)$ we the following condition must hold:
\begin{align}
    \nu^{3/2}\norm{\wgt}_1 - \loneboundclasnt \nu^{1/2} + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \sqrt{n} \left[ \min \frac{\alpha}{\norm{H}_{\infty}} \subjto (
    \nu,b,\alpha)\in\Gamma_4^{\nu} \right]\leq 0
    \label{eq:nu_ineq_min_alpha}
\end{align}
Thus in order to upper bound $\nu$ we need to find a lower bound on $\alpha$. Note that we already have $\alpha \geq \alphauls$, but using this bound will not give tight bound on $\nu$. Now we discuss obtaining a tighter lower bound on $\alpha$.

For any $ (\nu,b,\alpha,\varsigma)\in\Gamma_4^{\nu}$ holds:
\begin{align}
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} -\epstight \leq b^2 \left( \frac{\norm{H}_{\infty}^2}{n} - \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\nu} \right) 
    \leq
    \frac{(\loneboundclasnt-\nu\norm{\wgt}_1)^2}{\alpha^2} \left( \frac{\norm{H}_{\infty}^2}{n} - \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\nu} \right)
\end{align}
and then plugging $\nu\norm{\wgt}_1 = \kappa \loneboundclasnt$ for $\kappa \in [\kappaunu,1]$ into the equation above yields:
\begin{align}
\label{eq:lower_bound_alpha_fcn_kappa}
    \sqrt{\frac{2}{\pi}} \norm{\gamma(\alpha)}_2^2 
    \leq
    \frac{\norm{H}_{\infty}^2}{n} \frac{\kappa \loneboundclasnt}{\norm{\wgt}_1} - \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\loneboundclasnt^2 (1-\kappa)^2} + O \left(  \frac{\epstight \alpha^2}{\loneboundclasnt} \right)
\end{align}
Note that only the right hand side depends on $\nu$ (and thus on $\kappa$). Hence maximizing over $\kappa$ the right hand side 
% \begin{align}
%     (1-\kappa)^3 = \frac{2\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n}{\loneboundclasnt^3}
% \end{align}
and substituting this $\kappa$ into \eqref{eq:lower_bound_alpha_fcn_kappa} we get the following inequality:
\begin{align}
    \frac{\alpha^{2/3}}{\norm{H}_{\infty}^{2/3}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{1/3} + n^{2/3} \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} \norm{\wgt}_1^{2/3}
    + O \left( \frac{\epstight n^{2/3} \alpha^2}{\norm{H}_{\infty}^2 \loneboundclasnt} \right)
    \leq
    \frac{1}{n^{1/3}} \frac{\loneboundclasnt}{\norm{\wgt}_1^{1/3}}
\end{align}
Note that until now we did not relax the constraints. Now raise to the third power the previous inequality and relax inequality while keeping the first two terms to get:
\begin{align}
    \frac{\alpha^{2}}{\norm{H}_{\infty}^2} \frac{9\sqrt{2}}{4\sqrt{\pi}}  + 3 \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}\norm{\wgt}_1^{2/3} n^{2/3} \frac{\alpha^{4/3}}{\norm{H}_{\infty}^{4/3}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{2/3}
    \leq
    \frac{1}{n} \frac{\loneboundclasnt^3}{\norm{\wgt}_1}   ( 1 + O\left(\frac{\epstight n}{\loneboundclasnt^2}\frac{\alphaols^2}{\norm{H}_{\infty}^2} \right)  )
\end{align}
We can further relax this constraint by using the previous lower bound $\alphauls$ in the second term as follows:
\begin{align}
    \frac{\alpha^{2}}{\norm{H}_{\infty}^2} \frac{9\sqrt{2}}{4\sqrt{\pi}}  + 3 \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} \norm{\wgt}_1^{2/3} n^{2/3} \frac{\alphauls^{4/3}}{\norm{H}_{\infty}^{4/3}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{2/3}
    \leq
    \frac{1}{n} \frac{\loneboundclasnt^3}{\norm{\wgt}_1}  (1+O\left(\frac{\log n}{n^{1/6}}\right))  
\end{align}
Note that the term on the left hand side is sum of two convex functions in $\alpha$ and thus is convex. Similarly, as before, we look for $\alphauuls < \alpha_m$ such that the previous inequality is not satisfied. Using concentration results, we get:
\begin{align}
    \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{1}{\tuulm^2} \left( 1 - \frac{4}{\tuulm^2} + O \left( \frac{1}{\tuulm^4} \right) \right) + 3\sqrt{\frac{2}{\pi}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{2/3} \norm{\wgt}_1^{2/3} &\frac{2 n^{2/3}}{\uulm \tuulm^2} \left(1+ O \left( \frac{1}{\tuulm^2} \right) \right) \frac{1}{\tulm^{4/3}} \left( 1- \frac{8}{3}\frac{1}{\tulm^2} + O \left( \frac{1}{\tulm^4} \right) \right) \\
    &>
    \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{1}{\tsopt^2} \left( 1- \frac{2}{\tsopt^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right)\left(1+O\left( \frac{\log n}{n^{1/6}} \right)\right)
\end{align}
and we can choose $\uulm = \lambda \sopt$ with $\lambda\in(0,1)$. This gives us a lower bound on $\alpha$ which is tight enough for obtaining bounds on $\nu$ with right multiplicative constant. 
Substituting $\alpha=\alphauuls$ into inequality~\eqref{eq:nu_ineq_min_alpha} and setting $\nu\norm{
\wgt}_1 = \kappa^2\loneboundclasnt$ with $\kappa^2 \in [\kappa_3,1]$ we obtain:
\begin{align}
    \kappa^3 - \kappa + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \frac{\sqrt{n}}{\loneboundclasnt^{3/2}} \frac{\alphauuls}{\norm{H}_{\infty}} \leq 0
\end{align}
Using concentration inequalities we obtain
\begin{align}
    \kappa^3 - \kappa + \frac{2}{3\sqrt{3}} \frac{\tsopt}{\tuulm} \left( 1-\frac{2}{\tuulm^2} + O \left( \frac{1}{\tuulm^3} \right) \right) \left( 1 + \frac{1}{\tsopt^2} + O\left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) \leq 0
\end{align}
and after substituting $\uulm = \lambda \sopt$ with $\lambda<1$ we get the following:
\begin{align}
    \kappa^3 - \kappa + \frac{2}{3\sqrt{3}} + \frac{2}{3\sqrt{3}}\frac{\log\lambda -1}{\tsopt^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \leq 0
\end{align}
Thus, we obtain $\kappa^2 \in \left[ \frac{1}{3}-\frac{\tlambda}{\tsopt^{2/3}}, \frac{1}{3}+\frac{\tlambda}{\tsopt^{2/3}} \right]$ for some positive universal constant $\tlambda$, which we can write as $\nu\norm{\wgt}_1 = \frac{\loneboundclasnt}{3} (1+O(\tsopt^{-2/3}))$.
% $\ulambda,\olambda$.

\subsubsection*{Step 4.2: Upper bound on $\eta$}
Define the following set:
\begin{align}
    % \Gamma_1^{\alpha,L} 
    \Gamma_{4}^{\eta} 
    = \bigg\{ (\nu, b, \alpha, \varsigma)
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    &\kappa_4 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
    - \epstight
    % + O \left( \frac{1}{n^{2/3}} \right)
    \\
    &~~\andtxt~~ 
    b\alpha + \nu \norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \left| \nu\norm{\wgt}_1-\frac{\loneboundclasnt}{3} \right| \leq \frac{\tlambda \loneboundclasnt}{\tsopt^{2/3}}
    ~~\andtxt~~ 
    \alpha \geq \alphauuls
     \bigg\}.
    \label{eq:Gamma_4_eta_def}
\end{align}
\begin{align}
\eta^2 
    \leq
    \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 
    \leq 
    \max_{\nu,\alpha} (\loneboundclasnt-\nu\norm{\wgt}_1)^2 \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}
    \leq
    \loneboundclasnt^2 \left( 1-\frac{1}{3} + \frac{\tlambda}{\tsopt^{2/3}} \right)^2 \frac{2}{\uulm} \left(1+O\left(\frac{1}{\tuulm^2}\right)\right)
    \lesssim \frac{1}{\tsopt^2}
\end{align}
\subsubsection*{Bound 5: Tight bounds on $\eta$}
Now we can apply Proposition~\ref{prop:uniform_conv_noiseless} and use approximation:
\begin{align}
    \left|\fnclasn(\nu,\eta)     -
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} - \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} \right|
    =
    O \left( \frac{\eta^2}{\nu^3}, \rho\eta^2, \frac{\eta^3}{\nu}\epsilon_n \right) + O \left( \frac{1}{\nu^3}, \epsilon_c \right) 
    % =: O_{\eta}(\eta,n,\rho) + O_{\nu,c}(\nu,\epsilon) 
    =: \frac{\eta^2}{\nu} \OOO_f
\end{align}
with $\OOO_f = O\left( \frac{\epsilon_n^3}{\tsopt} \right)$, $\epsilon_n \asymp \sqrt{\log\log n}$.
\begin{align}
    \Gamma_5^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    \sqrt{\frac{2}{\pi}} \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu}  (1+\OOO_f)
    ~~\andtxt~~ 
    b\alpha + \nu\norm{\wgt}_1 \leq \loneboundclasnt 
    ~~\andtxt~~ 
    \left| \nu\norm{\wgt}_1-\frac{\loneboundclasnt}{3} \right| \leq \frac{\tlambda \loneboundclasnt}{\tsopt^{2/3}}
    % \nu \in\loneboundclasnt\left[ \frac{1}{3}-\frac{\tlambda}{\tsopt^{2/3}}, \frac{1}{3}+\frac{\tlambda }{\tsopt^{2/3}} \right]
    \right\}.
    \label{eq:Gamma_5_eta_def}
\end{align}
Similarly to Equality \eqref{eq:lower_bound_alpha_fcn_kappa} we get:
\begin{align}
    \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt} (1-\kappa)^2 (1+\OOO_f) + \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3} 
    \leq
    \kappa(1-\kappa)^2 \leq \frac{4}{27}
\end{align}
and using our established bound on $\nu\norm{\wgt}_1$ we get $(1-\kappa)^2 \geq (1- \frac{1}{3}-\frac{\tlambda}{\tsopt^{2/3}})^2$ and hence we obtain:
\begin{align}
    3\sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}\frac{n\norm{\wgt}_1}{\loneboundclasnt} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} +  \OOO_f \right) +  \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3} 
    \leq 1
    \label{eq:tight_bound_noisy_alpha_ineq_tight}
\end{align}
Note that the function is convex in $\alpha$. Using concentration, we get:
\begin{align}
    2 \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n \tsopt \norm{\wgt}_1 )^{2/3}}{m \tm^2} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right)  \right) \left(1+O \left( \frac{1}{\tm^2} \right) \right) 
    +
    \frac{\tsopt^2}{\tm^2} \left( 1- \frac{2}{\tm^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    \leq 1
\end{align}
Now we claim that the $\ulmstar,\olmstar$ given in Lemma~\ref{lemma_uls_ols_exp}, respectively, with $\kappa=1/3$ do not satisfy this inequality for the well-chosen universal constant $\mu$ since
\begin{align}
    2& \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n \tsopt \norm{\wgt}_1)^{2/3}}{\ulmstar \tulmstar^2} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} +  O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    +
    \frac{\tsopt^2}{\tulmstar^2} \left( 1- \frac{2}{\tulmstar^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    \\
    &=
    1 - \frac{\mu}{\tsopt^{7/3}} \left(1-\frac{\tsopt^2}{\tulmstar^2} \right)  + \frac{2\mu^2-6\tlambda}{\tulmstar^2\tsopt^{2/3}} + O \left( \frac{(\log\log n)^{3/2}}{\tsopt^3} \right) 
    =
    1 +\frac{2\mu^2-6\tlambda}{\tsopt^{8/3}} + O \left( \frac{(\log\log n)^{3/2}}{\tsopt^3} \right) > 1
\end{align}
for $\mu > \sqrt{3\tlambda}$. Similarly, for $\olmstar$ we get:
\begin{align}
    2& \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n \tsopt \norm{\wgt}_1)^{2/3}}{\olmstar \tolmstar^2} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    +
    \frac{\tsopt^2}{\tolmstar^2} \left( 1- \frac{2}{\tolmstar^2} + O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) 
    \\
    &=
    1 + \frac{\mu}{\tsopt^{7/3}} \left(1-\frac{\tsopt^2}{\tolmstar^2} \right)  + \frac{2\mu^2-6\tlambda}{\tolmstar^2\tsopt^{2/3}} + O \left( \frac{(\log\log n)^{3/2}}{\tsopt^{3}} \right) 
    =
    1 +\frac{2\mu^2-6\tlambda}{\tsopt^{8/3}} + O \left( \frac{(\log\log n)^{3/2}}{\tsopt^{3}} \right) > 1
\end{align}
Now we can bound $\eta$ as follows:
\begin{align}
    \eta^2 
    \leq
    \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 
    &\leq 
    \max_{\nu,\alpha} (\loneboundclasnt-\nu\norm{\wgt}_1)^2 \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}
    \leq
    \loneboundclasnt^2 \left( 1-\frac{1}{3} + \frac{\tlambda}{\tsopt^{2/3}} \right)^2 \frac{2}{\ulmstar} \left(1+O\left(\frac{1}{\tulmstar^2}\right)\right)
    \\
    &\leq
    \frac{2}{3} \frac{1}{\tsopt^2} \exp \left( \frac{\mu}{2\tsopt^{1/3}} \right) \left(1+ O \left( \frac{1}{\tsopt^{2/3}} \right) \right)
    = 
    \frac{2}{3} \frac{1}{\tsopt^2} \left( 1 + \frac{\mu}{2\tsopt^{1/3}} + O \left( \frac{1}{\tsopt^{2/3}} \right) \right) =: \overline{\eta}^2
\end{align}
and
\begin{align}
    \eta^2 
    \geq
    \min_{b,\alpha} b^2\norm{\gamma(\alpha)}_2^2 
    &\geq
    \min_{\nu,\alpha} \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{n}{\nu} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{n\norm{\wgt}_1}{\loneboundclasnt \left( \frac{1}{3}+\frac{\tlambda}{\tsopt^{2/3}} \right)} \frac{2}{\olmstar\tolmstar^2} \left( 1 + O \left( \frac{1}{\tolmstar^2} \right) \right)
    \\
    &\geq
    \frac{2}{3} \frac{1}{\tsopt^2} \exp \left( -\frac{\mu}{2\tsopt^{1/3}} \right) \left(1 - O \left( \frac{1}{\tsopt^{2/3}} \right) \right)
    =
    \frac{2}{3} \frac{1}{\tsopt^2} \left( 1 - \frac{\mu}{2\tsopt^{1/3}} - O \left( \frac{1}{\tsopt^{2/3}} \right) \right) =: \underline{\eta}^2
\end{align}

\subsubsection*{Bound 5: Tight upper bound on $\norm{\varsigma}_2$}
\begin{align}
    \Gamma_6^{\varsigma} = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    \sqrt{\frac{2}{\pi}} \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} (1+\OOO_f)
    + \kappa_5 \frac{\norm{\varsigma}_2^2}{\nu} 
    ~~\andtxt~~ 
    b^2\norm{\gamma(\alpha)}_2^2 \geq ... 
    ~~\andtxt~~ 
    \nu + b\alpha \leq \loneboundclasnt
    ~~\andtxt~~ 
    \left| \nu-\frac{\loneboundclasnt}{3} \right| \leq \frac{\tlambda \loneboundclasnt}{t_m^{2/3}}
    \right\}.
    \label{eq:Gamma_6_varsigma_def}
\end{align}
Similarly to Equation~\eqref{eq:tight_bound_noisy_alpha_ineq_tight}:
\begin{align}
    \kappa_5 \norm{\varsigma}_2^2 \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3} \leq 
    1-3\sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}\frac{n\norm{\wgt}_1}{\loneboundclasnt} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} +  \OOO_f \right) -  \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3}
\end{align}
\begin{align}
    \norm{\varsigma}_2^2 
    \lesssim 
    \frac{\norm{H}_{\infty}^2}{\alpha_{\ulmstar}^2}
    \frac{\loneboundclasnt^3}{n\norm{\wgt}_1} \left[
    1-3\sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha_{\olmstar} )}_2^2}{\norm{H}_{\infty}^2}\frac{n\norm{\wgt}_1}{\loneboundclasnt} \left(1 - \frac{3\tlambda}{\tsopt^{2/3}} +  O \left( \frac{\epsilon_n^3}{\tsopt^3} \right) \right) -  \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{\alpha_{\ulmstar}^2}{\norm{H}_{\infty}^2} \frac{n\norm{\wgt}_1}{\loneboundclasnt^3} \right]
    \lesssim 
    \frac{1}{\tsopt^{7/3}}
\end{align}


==> sections/subsections_theory/noiseless/unicon_proof.tex <==
% \subsection{Proof of Uniform Convergence Proposition~\ref{prop:BoundGamma0_class_noiseless}}
% As discussed in the proof sketch, proof consists of iterative bounding and approximation steps. The structure of the proof is as follows: for every bound step we use different approximation of $\fnclasn$, and based on it we develop tighter bounds on variables of interest. Thus the statement of the proposition follows from the tightest, last bound i.e. Bound 5. We start with the following bound:
% \subsubsection*{Bound 1: \texorpdfstring{$\nu = \Omega(n^{2/15})$}{nuomega}}
% Recall the definition of the set $\setNoiselessZero$ from Equation~\eqref{eq:Gamma0_def_class_noiseless} and that by parametric path approach from Section~\ref{subsec:path_param} we have $\eta = \norm{\wtwo}_2 = b\norm{\gamma(\alpha)}_2$. In order to show the lower bound $\nu = \Omega(n^{2/15})$ we define the following set:
% \begin{align}
%     % \Gamma_0^{\nu,L}
%     \Gamma_1^{\nu}
%     = \left\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasn (\nu,b\norm{\gamma(\alpha)}_2) 
%     ~~\andtxt~~ 
%     b\alpha \leq \loneboundclasn 
%     \right\}.
%     \label{eq:Gamma_1_nu_constant_lower}
% \end{align}
% in which we relax the second constraint from definition of set $\Gamma_0$ and thus $\Gamma_0 \subset \Gamma_1^{\nu}$. The goal is to show that uniformly over all $\nu\in \Gamma_1^{\nu}$ holds that $\nu=\Omega(n^{2/15})$ implying that this lower bound holds also uniformly over $\Gamma_0$.

% Note that for $(\nu,b,\alpha)\in \Gamma_1^{\nu}$ we have:
% \begin{align}
%     \fnclasn (\nu,b\norm{\gamma(\alpha)}_2) 
%     \leq
%     \max_{b,\alpha} \frac{1}{n}b^2 \norm{H}_{\infty}^2 
%     \leq
%     \max_{\alpha} \frac{1}{n} \frac{\loneboundclasn^2}{\alpha^2} \norm{H}_{\infty}^2
%     =
%     \frac{1}{n} \loneboundclasn^2 \norm{H}_{\infty}^2
%     \lesssim
%     \frac{1}{n} \left( \frac{n}{t_m^2} \right)^{2/3} \log d 
%     \lesssim
%     \left( \frac{1}{n} \right)^{2/15}
% \end{align}
% with probability $\geq 1-\frac{1}{d}$, where we used $d\lesssim \exp(\kappa n^{1/5})$ and $\alpha\geq 1$. Also, we have:
% \begin{align}
%     \fnclasn (\nu,b\norm{\gamma(\alpha)}_2)  
%     =
%     \frac{1}{n} \sum_{i=1}^n \possq{ 1 - \nu \abs{\gausswone_i} - \eta\gausswtwo_i} 
%     \gtrsim
%     \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}}
%     \label{eq_etanu_to_nu_fnclansn}
% \end{align}
% with probability $\geq 1-\exp(-c_1 n)$ for some positive universal constant $c_1$. Now we show that $\nu = \Omega(n^{2/15})$. Assume, in contradiction, that there exists some universal constant $\kappa>0$ such that $\nu \leq \kappa n^{2/15}$ for some $\nu\in\Gamma_1^{\nu}$. From the previous two inequalities, we know that $\nu$ must satisfy with high probability that:
% \begin{align}
%     \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}} 
%     \lesssim
%     \left( \frac{1}{n} \right)^{2/15}
%     \label{eq:ineq_nu_first_bound_condition}
% \end{align}
% % According to Claim 4 in \cite{wang2021tight} $\delta(\kappa,\epsilon) n$ out of $n$ elements satisfy $\abs{\gausswone_i}\leq \frac{\epsilon}{\kappa}$ for some universal constants $1>\delta,\epsilon>0$ with probability at least $1-\exp(-c_2 n)$. Hence $1-\nu\abs{\gausswone_i}\geq 1-\epsilon>0$, and the sum in the lhs does not vanish for $n$ large enough, while the term on the rhs vanishes. Thus, the inequality cannot be satisfied for $n$ sufficiently large. We conclude that there exists no constant upper bound for $\nu$ i.e. $\nu = \Omega(1)$ with high probability.
% Define $F_n(\frac{1}{2\nu}) := \frac{1}{n}\sum_{i=1}^n \indicator{|\gausswone_i|\leq \frac{1}{2\nu}}$ and $F(\frac{1}{2\nu}) := \PP( |\Gausswone| \leq \frac{1}{2\nu} )$. Using the same reasoning as in Lemma~\ref{lemma:dkw_number_active_indicators} one can show that from the set of indicators $\{ \indicator{1-\nu\abs{\gausswone_i}}\}_{i=1}^n$ there are $k:=nF_n(\frac{1}{2\nu}) \asymp n^{1-p}$ indicators activated when $\nu=\Omega(n^p)$, $p\in(0,\frac{2}{5})$. Thus we have
% \begin{align}
%     \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}} 
%     \geq
%     \frac{n F_n(\frac{1}{2\nu})}{n} \left(\frac{1}{2} \right)^2
%     \gtrsim
%     n^{-p}
% \end{align}
% % \begin{align}
% %     \sup_\nu | F_n \left( \frac{1}{2\nu} \right) - F\left( \frac{1}{2\nu} \right) | \leq \sqrt{\frac{\log d}{2n}}
% % \end{align}
% % \begin{align}
% %     \sup_\nu | F_n \left( \frac{1}{2\nu} \right) - F\left( \frac{1}{2\nu} \right) | \leq \sqrt{\frac{\log d}{2n}}
% % \end{align}
% % Hence we obtain:
% % \begin{align}
% %     \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}} 
% %     \geq
% %     \frac{n F_n(\frac{1}{2\nu})}{n} \left(\frac{1}{2} \right)^2
% %     \geq
% %     \frac{1}{4} \left( F \left( \frac{1}{2\nu} \right) - \sqrt{\frac{\log d}{2n}} \right)
% %     =
% %     \frac{1}{4} \left( \erf \left( \frac{1}{2\sqrt{2}\nu} \right) - \sqrt{\frac{\log d}{2n}} \right)    
% % \end{align}
% % We now show that for $\nu \leq \kappa n^{2/15}$ inequality~\eqref{eq:ineq_nu_first_bound_condition} does not hold. Using Taylor expression of $\erf(\cdot)$ around zero, i.e. that $\erf(\frac{1}{2\sqrt{2}\nu}) = \frac{1}{\sqrt{2\pi}} \frac{1}{\nu} + O(\frac{1}{\nu^3})$ we get that for $\nu \leq \kappa n^{2/15}$:
% % \begin{align}
% %     \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}} 
% %     \geq
% %     \frac{1}{4\sqrt{2\pi}}\frac{1}{\kappa n^{2/15}} + O\left(\frac{1}{n^{2/5}}\right) 
% % \end{align}
% Thus for any $n\geq c_1$ and $p\leq \frac{2}{15}$ we can always choose constants such that  inequality~\eqref{eq:ineq_nu_first_bound_condition} does not hold. Hence we conclude that $\nu = \Omega(n^{2/15})$.


% \subsubsection*{Bound 2: \texorpdfstring{$\eta = O(1),\ \nu \geq \kappa_3 \loneboundclasn$}{bound1} }
% Conditioning on the fact that $\nu = \Omega(n^{2/15})$ and $\nu = O(\loneboundclasn) = o(\sqrt{n})$ we can use lower bound from Proposition~\ref{prop:fnoiselessquadratic}:
% \begin{align}
%     \fnclasn(\nu,\eta) \geq \kappa_1 \frac{1}{\nu} + \kappa_2 \frac{\eta^2}{\nu}
% \end{align}
% which holds with probability $1-\exp(-c_1 n)$ for some positive universal constants $\kappa_1,\kappa_2$.

% Define
% \begin{align}
%     % \Gamma_1^{\eta,U} =
%     \Gamma_2 =
%     \left\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq \kappa_1 \frac{1}{\nu} + \kappa_2 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
%     ~~\andtxt~~ 
%     b\alpha \leq \loneboundclasn 
%     ~~\andtxt~~ 
%     \nu \leq \loneboundclasn
%     ~~\andtxt~~ 
%     \nu = \Omega(n^{2/15})
%     \right\}.
%     \label{eq:Gamma_2_eta_def_upp}
% \end{align}
% Note that constraints in $\Gamma_2$ are relaxations of constraints in definition of $\Gamma_0$ and hence $\Gamma_0 \subset \Gamma_2$ with high probability. By finding bounds on $\nu,\eta$ from $\Gamma_2$ we obtain a valid upper bound in $\Gamma_0$ as well.

% \textbf{Step 2.1: Upper bound on $\eta$.}
% We bound $\nu$ as follows:
% \begin{align}
%     \eta^2
%     &\leq
%     \max_{\nu,b,\alpha} \left[ b^2\norm{\gamma(\alpha)}_2^2
%     \subjto
%     (\nu,b,\alpha)\in \Gamma_2 \right]\\
%     &=
%     \max_{\nu,b,\alpha} \left[ b^2\norm{\gamma(\alpha)}_2^2 
%     \subjto 
%     \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n}\nu \norm{H}_{\infty}^2
%     ~~\andtxt~~ 
%     b\alpha \leq \loneboundclasn
%     ~~\andtxt~~ 
%     \nu \leq \loneboundclasn
%     \right]\\
%     &=
%     \max_{\alpha} \left[ \loneboundclasn^2\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2} 
%     \subjto 
%     \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n} \loneboundclasn \norm{H}_{\infty}^2
%     \right]
%     \label{eq:eta_upper_bound_step21}
% \end{align}
% where we used only that $(\nu,b,\alpha)\in \Gamma_2$ satisfy appropriate constraints. As we mentioned in the Section~\ref{subsubsec:prop_gamma_alpha}, function $\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}$ is monotonically decreasing function in $\alpha$, whereas $\norm{\gamma(\alpha)}_2^2$ is a convex function. Thus, similarly as previously discussed in \cite{donhauser2022fast}, it is sufficient to find $\alphauls < \alpha_m$ such that
% \begin{align}
%      \norm{\gamma(\alphauls)}_2^2 > \frac{1}{\kappa_2 n} \loneboundclasn \norm{H}_{\infty}^2
% \end{align}
% to obtain an upper bound on $\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}$. Using concentration results from Section~\ref{subsubsec:prop_gamma_alpha} we can rewrite above inequality as follows:
% \begin{align}
%     \frac{2}{\uls \tuls^2} \left( 1+O \left( \frac{1}{\tuls^2} \right) \right) > \frac{1}{\kappa_2 n} \kappa_0 \left( \frac{n}{t_\sopt^2} \right)^{1/3} \left( 1 + O \left( \frac{1}{t_\sopt^2} \right) \right)
% \end{align}
% It is straightforward to show that we can choose $\uls = \lambda \left( \frac{n}{t_\sopt^2} \right)^{2/3}$ with sufficiently small universal constant $\lambda = \lambda(\kappa_2,\kappa_0)>0$. We finish this step by substituting this choice of $\uls$ into the upper bound from Equation~\eqref{eq:eta_upper_bound_step21} to get:
% \begin{align}
%     \eta^2 
%     \leq
%     \loneboundclasn^2 \frac{\norm{\gamma(\alphauls)}_2^2}{\alphauls^2}
%     = \kappa_0^2 \left( \frac{n}{t_\sopt^2} \right)^{2/3} \left( 1 + O \left( \frac{1}{t_\sopt^2} \right) \right) 
%     \frac{2}{\uls} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) =: \boundeta^2 = O(1) 
% \end{align}\\
% \noindent\textbf{Step 2.2: Lower bound on $\nu$}.
% Similarly to Equation~\eqref{eq:eta_upper_bound_step21}, we can bound $\nu$ on the set $\Gamma_2$ as follows:
% \begin{align}
%     \nu
%     &\geq
%     \kappa_1 n \left[ \min_{b,\alpha} \frac{1}{b^2\norm{H}_{\infty}^2}  \subjto (\nu,b,\alpha)\in \Gamma_2 \right] \\
%     &=
%     \frac{\kappa_1 n}{\loneboundclasn^2} \left[ \min_{\alpha} \frac{\alpha^2}{\norm{H}_{\infty}^2} \subjto \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n} \loneboundclasn \norm{H}_{\infty}^2 \right]
%     \label{eq:nu_lower_bound_step22}
% \end{align}
% Similarly as above, we obtain that $\alpha\geq \alphauls$ and after substitution of $\uls$ as defined above, we have:
% \begin{align}
%     \nu \geq \kappa_1 \frac{n}{\loneboundclasn^2} \frac{\alphauls^2}{\norm{H}_{\infty}^2} 
%     =
%     \frac{\kappa_1}{\kappa_0^2} \frac{(n t_m^4)^{1/3}}{\tuls^2}  (1+O \left( \frac{1}{t_m^2}, \frac{1}{\tuls^2} \right) ) 
%     \geq
%     \frac{\kappa_1}{\kappa_0^2}\left( \frac{n}{t_m^2} \right)^{1/3} (1+O \left( \frac{1}{t_m^2} \right) ) =:  \kappa_3 \loneboundclasn
% \end{align}
% Note that from definition of $\kappa_0$ and the fact that $\kappa_1$ must be smaller than constant from Taylor expansion of $\fnclasn$ i.e. $\kappa_1 \leq \frac{\sqrt{2}}{3\sqrt{\pi}}$ (see Proposition~\ref{prop:uniform_conv_noiseless}) we get that $\kappa_3$ must satisfy $0 < \kappa_3 < \frac{4}{27}(1+O \left( \frac{1}{t_m^2} \right) )$.
% \\




% % \subsubsection*{Bound 2: \texorpdfstring{$\eta = O(1),\ \nu \geq \kappa_3 \loneboundclasn$}{bound1} }
% % Conditioning on the fact that $\nu = \Omega(n^{2/15})$ and $\nu = O(\loneboundclasn) = o(\sqrt{n})$ we can use lower bound from Proposition~\ref{prop:fnoiselessquadratic}:
% % \begin{align}
% %     \fnclasn(\nu,\eta) \geq \kappa_1 \frac{1}{\nu} + \kappa_2 \frac{\eta^2}{\nu}
% % \end{align}
% % which holds with probability $1-\exp(-c_1 n)$ for some positive universal constants $\kappa_1,\kappa_2$.

% % \textbf{Step 2.1: Upper bound on $\eta$.}
% % Define
% % \begin{align}
% %     % \Gamma_1^{\eta,U} =
% %     \Gamma_2^{\eta} =
% %     \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq \kappa_2 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
% %     ~~\andtxt~~ 
% %     b\alpha \leq \loneboundclasn 
% %     ~~\andtxt~~ 
% %     \nu \leq \loneboundclasn
% %     ~~\andtxt~~ 
% %     \nu = \Omega(n^{2/15})
% %     \right\}.
% %     \label{eq:Gamma_2_eta_def_upp}
% % \end{align}
% % Note that constraints in $\Gamma_2^{\eta}$ are relaxations of constraints in definition of $\Gamma_0$ and hence $\Gamma_0 \subset \Gamma_2^{\eta}$ with high probability. By finding an upper bound on $\nu$ from $\Gamma_2^{\eta}$ we obtain a valid upper bound in $\Gamma_0$ as well. We bound $\nu$ as follows:
% % \begin{align}
% %     \eta^2
% %     &\leq
% %     \max_{\nu,b,\alpha} \left[ b^2\norm{\gamma(\alpha)}_2^2
% %     \subjto
% %     (\nu,b,\alpha)\in \Gamma_2^{\eta} \right]\\
% %     &=
% %     \max_{\nu,b,\alpha} \left[ b^2\norm{\gamma(\alpha)}_2^2 
% %     \subjto 
% %     \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n}\nu \norm{H}_{\infty}^2
% %     ~~\andtxt~~ 
% %     b\alpha \leq \loneboundclasn
% %     ~~\andtxt~~ 
% %     \nu \leq \loneboundclasn
% %     \right]\\
% %     &=
% %     \max_{\alpha} \left[ \loneboundclasn^2\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2} 
% %     \subjto 
% %     \norm{\gamma(\alpha)}_2^2 \leq \frac{1}{\kappa_2 n} \loneboundclasn \norm{H}_{\infty}^2
% %     \right]
% %     \label{eq:eta_upper_bound_step21}
% % \end{align}
% % where we used only that $(\nu,b,\alpha)\in \Gamma_2^{\eta}$ satisfy appropriate constraints. As we mentioned in the Section~\ref{subsubsec:prop_gamma_alpha}, function $\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}$ is monotonically decreasing function in $\alpha$, whereas $\norm{\gamma(\alpha)}_2^2$ is a convex function. Thus, similarly as previously discussed in \cite{donhauser2022fast}, it is sufficient to find $\alphauls < \alpha_m$ such that
% % \begin{align}
% %      \norm{\gamma(\alphauls)}_2^2 > \frac{1}{\kappa_2 n} \loneboundclasn \norm{H}_{\infty}^2
% % \end{align}
% % to obtain an upper bound on $\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}$. Using concentration results from Section~\ref{subsubsec:prop_gamma_alpha} we can rewrite above inequality as follows:
% % \begin{align}
% %     \frac{2}{\uls \tuls^2} \left( 1+O \left( \frac{1}{\tuls^2} \right) \right) > \frac{1}{\kappa_2 n} \kappa_0 \left( \frac{n}{t_\sopt^2} \right)^{1/3} \left( 1 + O \left( \frac{1}{t_\sopt^2} \right) \right)
% % \end{align}
% % It is straightforward to show that we can choose $\uls = \lambda \left( \frac{n}{t_\sopt^2} \right)^{2/3}$ with sufficiently small universal constant $\lambda = \lambda(\kappa_2,\kappa_0)>0$. We finish this step by substituting this choice of $\uls$ into the upper bound from Equation~\eqref{eq:eta_upper_bound_step21} to get:
% % \begin{align}
% %     \eta^2 
% %     \leq
% %     \loneboundclasn^2 \frac{\norm{\gamma(\alphauls)}_2^2}{\alphauls^2}
% %     = \kappa_0^2 \left( \frac{n}{t_\sopt^2} \right)^{2/3} \left( 1 + O \left( \frac{1}{t_\sopt^2} \right) \right) 
% %     \frac{2}{\uls} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) =: \boundeta^2 = O(1) 
% % \end{align}\\
% % \noindent\textbf{Step 2.2: Lower bound on $\nu$}.
% % Define the following set
% % \begin{align}
% %     % \Gamma_1^{\nu,L} 
% %     \Gamma_2^{\nu} 
% %     = \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq \kappa_1 \frac{1}{\nu} 
% %     ~~\andtxt~~ 
% %     b\alpha \leq \loneboundclasn 
% %     ~~\andtxt~~ 
% %     b^2\norm{\gamma(\alpha)}_2^2 \leq \boundeta^2
% %     ~~\andtxt~~ 
% %     \nu = \Omega(n^{2/15})
% %     \right\}.
% %     \label{eq:Gamma_2_nu_low}
% % \end{align}
% % for which holds $\Gamma_0 \subset \Gamma_2^{\eta} \cap \Gamma_2^{\nu} \subset \Gamma_2^{\nu}$ with high probability. We bound $\nu$ on the set $\Gamma_2^{\nu}$ as follows:
% % \begin{align}
% %     \nu
% %     &\geq
% %     \kappa_1 n \left[ \min_{b,\alpha} \frac{1}{b^2\norm{H}_{\infty}^2}  \subjto b\alpha \leq \loneboundclasn ~~\andtxt~~ b^2\norm{\gamma(\alpha)}_2^2 \leq \boundeta^2 \right] \\
% %     &=
% %     \frac{\kappa_1 n}{\loneboundclasn^2} \left[ \min_{\alpha} \frac{\alpha^2}{\norm{H}_{\infty}^2} \subjto \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2} \leq \frac{\boundeta^2}{\loneboundclasn^2} \right]
% %     \label{eq:nu_lower_bound_step22}
% % \end{align}
% % Now we use the fact that $\frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}$ is monotonically decreasing to lower bound $\alpha$ by $\alphauls$ such that $\alphauls\leq \alpha_m$ and:
% % \begin{align}
% %     \loneboundclasn^2 \frac{\norm{\gamma(\alphauls)}_2^2}{\alphauls^2} > \boundeta^2
% % \end{align}
% % Simple calculations show that we can choose $\uls = \lambda \left( \frac{n}{t_\sopt^2} \right)^{2/3} $ with $\lambda>0$ small enough such that the following inequality holds:
% % \begin{align}
% %     \loneboundclasn^2 \frac{\norm{\gamma(\alphauls)}_2^2}{\alphauls^2} 
% %     =
% %     \kappa_1\kappa_0^2 \left( \frac{n}{t_m^2} \right)^{2/3} (1+O \left( \frac{1}{t_m^2} \right) ) \frac{2}{\uls} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right)
% %     >
% %     \boundeta^2
% % \end{align}
% % So using this lower bound on $\alpha$, we can further lower bound $\nu$ from Equation~\eqref{eq:nu_lower_bound_step22} as follows:
% % \begin{align}
% %     \nu \geq \kappa_1 \frac{n}{\loneboundclasn^2} \frac{\alphauls^2}{\norm{H}_{\infty}^2} 
% %     =
% %     \frac{\kappa_1}{\kappa_0^2} \frac{(n t_m^4)^{1/3}}{\tuls^2}  (1+O \left( \frac{1}{t_m^2}, \frac{1}{\tuls^2} \right) ) 
% %     \geq
% %     \frac{\kappa_1}{\kappa_0^2}\left( \frac{n}{t_m^2} \right)^{1/3} (1+O \left( \frac{1}{t_m^2} \right) ) =:  \kappa_3 \loneboundclasn
% % \end{align}
% % Note that from definition of $\kappa_0$ and the fact that $\kappa_1$ must be smaller than constant from Taylor expansion of $\fnclasn$ i.e. $\kappa_1 \leq \frac{\sqrt{2}}{3\sqrt{\pi}}$ (see Proposition~\ref{prop:uniform_conv_noiseless}) we get that $\kappa_3$ must satisfy $0 < \kappa_3 < \frac{4}{27}(1+O \left( \frac{1}{t_m^2} \right) )$.
% % \\
% % \begin{align}
% %     \Gamma_2^{\eta} = \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
% %     \geq
% %     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + 
% %     \kappa \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
% %     ~~\andtxt~~ 
% %     b\alpha + \nu \leq \loneboundclasn 
% %     ~~\andtxt~~ 
% %     \nu = \Omega \left( n^{1/3} t_{n^{2/3}}^{-2/3} \right)
% %     \right\}.
% %     \label{eq:Gamma_2_eta_def}
% % \end{align}

% % \begin{align}
% %     \Gamma_2^{\eta,U} = \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
% %     \geq
% %     \frac{\kappa}{\nu}
% %     ~~\andtxt~~ 
% %     b\alpha \leq \loneboundclasn 
% %     ~~\andtxt~~ 
% %     \nu = \Omega \left( n^{1/3} t_{n^{2/3}}^{-2/3} \right) = \Omega (\loneboundclasn)
% %     \right\}.
% %     \label{eq:Gamma_2_eta_upper_def}
% % \end{align}
% % \begin{align}
% %     \eta^2
% %     &\leq
% %     \max_{\nu,b,\alpha} \left[ b^2\norm{\gamma(\alpha)}_2^2
% %     \subjto
% %     (\nu,b,\alpha)\in \Gamma_2^{\eta,U} \right]\\
% %     &=
% %     \max_{\nu,\alpha} \left[ \frac{\loneboundclasn^2}{\alpha^2}\norm{\gamma(\alpha)}_2^2 
% %     \subjto 
% %     \frac{1}{n}  \frac{\loneboundclasn^2}{\alpha^2}\norm{\Hgaussian}_{\infty}^2 \geq \frac{\kappa}{\nu}
% %     ~~\andtxt~~ 
% %     \nu = \Omega (\loneboundclasn)
% %     \right]\\
% %     &=
% %     \max_{\nu,\alpha} \left[ \frac{\loneboundclasn^2}{\alpha^2}\norm{\gamma(\alpha)}_2^2 
% %     \subjto 
% %     \alpha^2 \lesssim \frac{1}{n}  \loneboundclasn^3\norm{\Hgaussian}_{\infty}^2
% %     \right]\\
% % \end{align}
% \subsubsection*{Bound 3: \texorpdfstring{$\eta = \Omega \left( \frac{1}{t_m} \right)$}{bound2} } 
% Here we use approximation:
% \begin{align}
%     \fnclasn(\nu,\eta) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + O\left( \frac{1}{\nu^3} \right)
% \end{align}
% % \noindent\textbf{Upper bound on $\alpha$}.
% % \begin{align}
% %     \Gamma_1^{\alpha,U} = \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
% %     \geq
% %     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \right)
% %     ~~\andtxt~~ 
% %     b\alpha + \nu \leq \loneboundclasn 
% %     ~~\andtxt~~ 
% %     \nu \in [\kappa_3, 1] \loneboundclasn
% %     \right\}.
% %     \label{eq:Gamma_1_alpha_upper_def}
% % \end{align}
% % Again, we have $\Gamma_0 \subset \Gamma_1^{\alpha,U}$. Note that for $(\nu,b,\alpha)\in \Gamma_1^{\alpha,U}$ holds:
% % \begin{align}
% %     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} \leq \frac{1}{n} b^2 \norm{H}_{\infty}^2 \leq \frac{1}{n} \left( \frac{\loneboundclasn-\nu}{\alpha} \right)^2 \norm{H}_{\infty}^2
% % \end{align}
% % Thus, we can write:
% % \begin{align}
% %     \alpha^2 
% %     \leq
% %     \frac{3\sqrt{\pi}}{\sqrt{2}} \frac{1}{n} \nu (\loneboundclasn -\nu)^2 \norm{H}_{\infty}^2 
% %     \leq
% %     \frac{12\sqrt{\pi}}{27\sqrt{2}} \frac{1}{n} \loneboundclasn^3 \norm{H}_{\infty}^2
% % \end{align}
% % since given that $\nu \in [\kappa_3, 1] \loneboundclasn$ the function $\nu (\loneboundclasn -\nu)^2$ is maximized for $\nu = \loneboundclasn/3$ and $1/3\in[\kappa_3,1]$. From the definition of $\loneboundclasn$ we get:
% % \begin{align}
% %     \frac{\alpha^2}{\norm{H}_{\infty}^2} \leq \frac{12\sqrt{\pi}}{27\sqrt{2}} \frac{1}{n}  \frac{27}{\sqrt{72\pi}} \frac{n}{t_m^2} \left( 1 - \frac{2}{3}\frac{1}{t_m^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right)
% % \end{align}
% % Using the convexity of $\alpha^2$ we look for the smallest $\alphaols \geq \alpha_m$ for which holds
% % \begin{align}
% %     \frac{1}{\tols^2} \left( 1 - \frac{4}{\tols^2} + O \left( \frac{1}{\tols^4} \right)\right) 
% %     >
% %     \frac{1}{t_m^2} \left( 1 - \frac{2}{3}\frac{1}{t_m^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right)
% % \end{align}
% % thus, we can choose $\ols = \lambda m$ for some constant $\lambda>1$ since 
% % \begin{align}
% %     \frac{t_m^2}{\tols^2} = 1 + \frac{2\log\lambda}{t_m^2} + O \left( \frac{1}{t_m^4} \right)
% % \end{align}\\

% % \noindent\textbf{Lower bound on $\eta$.}
% % \begin{align}
% %     \Gamma_1^{\eta,L} = \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq \kappa_1 \frac{1}{\nu} 
% %     ~~\andtxt~~ 
% %     \nu \leq \loneboundclasn
% %     ~~\andtxt~~ 
% %     \alpha \leq \alphaols
% %     \right\}.
% %     \label{eq:Gamma_1_eta_def_low}
% % \end{align}
% % We have $\Gamma_0 \subset \Gamma_1^{\olalpha} \subset \Gamma_1^{\uleta}$.
% % \begin{align}
% %     \eta^2 \geq \min_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 
% %     \geq
% %     \kappa_1 \frac{n}{\nu} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}
% %     \geq 
% %     \kappa_1 \frac{n}{\loneboundclasn} \frac{\norm{\gamma(\alphaols)}_2^2}{\norm{H}_{\infty}^2}
% %     \gtrsim
% %     (n t_m)^{2/3} \frac{1}{\ols \tols^2}
% %     \gtrsim
% %     \frac{1}{t_m^2}
% % \end{align}
% % \noindent\textbf{Upper bound on $\alpha$}.
% % \noindent\textbf{Lower bound on $\eta$.}
% \begin{align}
%     % \Gamma_1^{\alpha,U} \textbf{o}
%     \Gamma_3^{\eta} 
%     = \left\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
%     \geq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \frac{1}{\nu^3} \right)
%     ~~\andtxt~~ 
%     b\alpha + \nu \leq \loneboundclasn 
%     ~~\andtxt~~ 
%     \nu \in [\kappa_3, 1] \loneboundclasn
%     \right\}.
%     \label{eq:Gamma_3_eta_lower_def}
% \end{align}
% Again, we have $\Gamma_0 \subset \Gamma_3^{\eta}$. Note that for $(\nu,b,\alpha)\in \Gamma_3^{\eta}$ holds:
% \begin{align}
%     \eta^2 
%     &\geq 
%     \left[ \min_{\nu, b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
%     \geq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \frac{1}{\nu^3} \right)
%     ~~\andtxt~~ 
%     b\alpha + \nu \leq \loneboundclasn 
%     ~~\andtxt~~ 
%     \nu \in [\kappa_3, 1] \loneboundclasn
%     \right]\\
%     &\gtrsim
%      n \left[ \min_{\nu,\alpha} \frac{1}{\nu} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}  \subjto
%     \frac{1}{n} \left( \frac{\loneboundclasn-\nu}{\alpha} \right)^2 \norm{H}_{\infty}^2
%     \geq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu}  + O \left( \frac{1}{\nu^3} \right)
%     % ~~\andtxt~~ 
%     % b\alpha + \nu \leq \loneboundclasn 
%     ~~\andtxt~~ 
%     \nu \in [\kappa_3, 1] \loneboundclasn
%     \right]\\
%     &\gtrsim
%     \frac{n}{\loneboundclasn} \left[
%     \min_{\nu,\alpha} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} 
%     \subjto
%     \frac{\alpha^2}{\norm{H}_{\infty}^2} \leq \frac{3\sqrt{\pi}}{\sqrt{2}}\frac{1}{n}\nu(\loneboundclasn-\nu)^2 + O \left( \frac{1}{\nu^3} \right)
%     % ~~\andtxt~~ 
%     % b\alpha + \nu \leq \loneboundclasn 
%     ~~\andtxt~~ 
%     \nu \in [\kappa_3, 1] \loneboundclasn
%     \right]
% \end{align}
% % Also note that $\alpha$ that satisfies constraints above is upper bounded
% % \begin{align}
% %     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} \leq \frac{1}{n} b^2 \norm{H}_{\infty}^2 \leq \frac{1}{n} \left( \frac{\loneboundclasn-\nu}{\alpha} \right)^2 \norm{H}_{\infty}^2
% % \end{align}
% Since given that $\nu \in [\kappa_3, 1] \loneboundclasn$ the function $\nu (\loneboundclasn -\nu)^2$ is maximized for $\nu = \loneboundclasn/3$ and $1/3\in[\kappa_3,1]$ we can upper bound $\alpha$ as follows:
% \begin{align}
%     \frac{\alpha^2}{\norm{H}_{\infty}^2} 
%     \leq
%     \frac{3\sqrt{\pi}}{\sqrt{2}} \frac{1}{n} \nu (\loneboundclasn -\nu)^2 + O\left( \frac{1}{\nu^3} \right) 
%     &\leq
%     \frac{12\sqrt{\pi}}{27\sqrt{2}} \frac{1}{n} \loneboundclasn^3 + O\left( \frac{1}{\loneboundclasn^3} \right) \\
%     &\leq
%     \frac{1}{t_m^2} \left( 1 - \frac{2}{3}\frac{1}{t_m^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right)+ O\left( \frac{t_m^2}{n} \right) 
%     \label{eq:alpha_ols_bound_nu_loneboundclasn}
% \end{align}
% where we used definition of $\loneboundclasn$ from Proposition~\ref{prop:localization_noiseless}.

% From Section~\ref{subsubsec:prop_gamma_alpha} we have that $\norm{\gamma(\alpha)}_2^2$ is a convex function and it decreases over $[1,\alpha_{d+1/2}]$. 
% Hence in order to lower bound $\norm{\gamma(\alpha)}_2^2$, it is sufficient to find a point $\alphaols$ such that $\alphaols \geq \alpha_m$ for which Equation~\eqref{eq:alpha_ols_bound_nu_loneboundclasn} does not hold, i.e. for $\ols$ for which we have:
% \begin{align}
%     \frac{1}{\tols^2} \left( 1 - \frac{4}{\tols^2} + O \left( \frac{1}{\tols^4} \right)\right) 
%     >
%     \frac{1}{t_m^2} \left( 1 - \frac{2}{3}\frac{1}{t_m^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right)
% \end{align}
% We can choose $\ols = \lambda m$ for some constant $\lambda>1$ since 
% \begin{align}
%     \frac{t_m^2}{\tols^2} = 1 + \frac{2\log\lambda}{t_m^2} + O \left( \frac{1}{t_m^4} \right)
% \end{align}
% Thus we finally obtain:
% \begin{align}
%     \eta^2  
%     \gtrsim
%     \frac{n}{\loneboundclasn} \frac{\norm{\gamma(\alphaols)}_2^2}{\norm{H}_{\infty}^2}
%     \gtrsim
%     (n t_m)^{2/3} \frac{1}{\ols \tols^2}
%     \gtrsim
%     \frac{1}{t_m^2}
% \end{align}
% \subsubsection*{Bound 4: Tight bounds on $\nu$ and $\eta = \Theta(\frac{1}{t_m})$}
% Now we can apply Proposition~\ref{prop:fnoiselessquadratictighter} and use approximation:
% \begin{align}
%     \fnclasn(\nu,\eta) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
%     \kappa_4 \frac{\eta^2}{\nu} - \epstight
% \end{align}
% with $\epstight \asymp \frac{\log n}{\sqrt{n}}$.
% % \begin{align}
% %     \fnclasn(\nu,\eta) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
% %     \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} + O \left( \right)
% % \end{align}
% \subsubsection*{Step 4.1: Tight bounds on $\nu$}
% Define the following set:
% % \begin{align}
% %     % \Gamma_1^{\alpha,L} 
% %     \Gamma_4^{\nu} 
% %     = \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
% %     \geq
% %     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
% %     \sqrt{\frac{2}{\pi}} \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} + O \left( \right)
% %     ~~\andtxt~~ 
% %     b\alpha + \nu \leq \loneboundclasn 
% %     ~~\andtxt~~ 
% %     \nu \in [\kappa_3, 1] \loneboundclasn
% %      \right\}.
% %     \label{eq:Gamma_4_nu_def}
% % \end{align}
% \begin{align}
%     % \Gamma_1^{\alpha,L} 
%     \Gamma_4^{\nu} 
%     = \bigg\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
%     \geq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
%     &\kappa_4 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
%     - \epstight
%     % + O \left( \frac{1}{n^{2/3}} \right)
%     \\
%     &~~\andtxt~~ 
%     b\alpha + \nu \leq \loneboundclasn 
%     ~~\andtxt~~ 
%     \nu \in [\kappa_3, 1] \loneboundclasn
%     ~~\andtxt~~ 
%     \alpha \leq \alphaols
%      \bigg\}.
%     \label{eq:Gamma_4_nu_def}
% \end{align}
% First note that $\Gamma_0 \subset \Gamma_4^{\nu} \subset \Gamma_2^{\nu}$ with high probability. Thus bound $\alpha \geq \alphauls$ shown in Step 2.2 holds in $\Gamma_4^{\nu}$ as well, which we make use of in the proof below.

% For any $(\nu,b,\alpha)\in\Gamma_4^{\nu}$ holds that:
% \begin{align}
%     \loneboundclasn - \nu \geq b\alpha \geq 
%     \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}}  \frac{\sqrt{n}}{\norm{H}_{\infty}} \frac{\alpha}{\sqrt{\nu}}
% \end{align}
% where we used that $b^2 \geq \frac{n}{\norm{H}_{\infty}^2}\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\nu}$ since $\frac{\eta^2}{\nu} = w(\epsilon)$ ($\eta = \Omega(\frac{1}{t_m}),\nu = \Theta(\loneboundclasn))$. Rearranging the terms we obtain that for any $(\nu,b,\alpha)\in \Gamma_4^{\nu}$ must hold that:
% \begin{align}
%     \nu^{3/2} - \loneboundclasn \nu^{1/2} + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \sqrt{n} \frac{\alpha}{\norm{H}_{\infty}} \leq 0
% \end{align}
% Thus uniformly over all $\nu$ such that $(\nu,b,\alpha)$ we the following condition must hold:
% \begin{align}
%     \nu^{3/2} - \loneboundclasn \nu^{1/2} + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \sqrt{n} \left[ \min \frac{\alpha}{\norm{H}_{\infty}} \subjto (
%     \nu,b,\alpha)\in\Gamma_4^{\nu} \right]\leq 0
%     \label{eq:nu_ineq_min_alpha}
% \end{align}
% % \begin{align}
% %     \nu 
% %     &\leq
% %     \left[ \max_{\nu,b,\alpha}
% %     \loneboundclasn - b\alpha \subjto (\nu,b,\alpha)\in\Gamma_4^{\nu} \right]
% %     \leq
% %     \loneboundclasn - \left[ \min_{\nu,b,\alpha}
% %     b\alpha \subjto (\nu,b,\alpha)\in\Gamma_4^{\nu} \right]\\
% %     &\leq
% %     \loneboundclasn - \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}}  \frac{\sqrt{n}}{\norm{H}_{\infty}} 
% %     \left[ \min_{\nu,b,\alpha} \frac{\alpha}{\sqrt{\nu}}  \subjto (\nu,b,\alpha)\in\Gamma_4^{\nu} \right]
% %     \label{eq:nu_last_tight_bound_alpha}
% % \end{align}
% % where in the last step we used that $b^2 \geq \frac{n}{\norm{H}_{\infty}^2}\frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\nu}$. 
% Thus in order to upper bound $\nu$ we need to find a lower bound on $\alpha$. Note that we already have $\alpha \geq \alphauls$, but using this bound will not give tight bound on $\nu$. Now we discuss obtaining a tighter lower bound on $\alpha$.

% For any $ (\nu,b,\alpha)\in\Gamma_4^{\nu}$ holds:
% \begin{align}
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} -\epstight \leq b^2 \left( \frac{\norm{H}_{\infty}^2}{n} - \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\nu} \right) 
%     \leq
%     \frac{(\loneboundclasn-\nu)^2}{\alpha^2} \left( \frac{\norm{H}_{\infty}^2}{n} - \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\nu} \right)
% \end{align}
% and then plugging $\nu = \kappa \loneboundclasn$ for $\kappa \in [\kappaunu,1]$ into the equation above yields:
% \begin{align}
% \label{eq:lower_bound_alpha_fcn_kappa}
%     \sqrt{\frac{2}{\pi}} \norm{\gamma(\alpha)}_2^2 
%     \leq
%     \frac{\norm{H}_{\infty}^2}{n} \kappa \loneboundclasn - \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\loneboundclasn^2 (1-\kappa)^2} + O \left(  \frac{\epstight \alpha^2}{\loneboundclasn} \right)
% \end{align}
% Note that only the right hand side depends on $\nu$ (and thus on $\kappa$). Hence maximizing over $\kappa$ the right hand side 
% % \begin{align}
% %     (1-\kappa)^3 = \frac{2\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n}{\loneboundclasn^3}
% % \end{align}
% and substituting this $\kappa$ into \eqref{eq:lower_bound_alpha_fcn_kappa} we get the following inequality:
% \begin{align}
%     \frac{\alpha^{2/3}}{\norm{H}_{\infty}^{2/3}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{1/3} + n^{2/3} \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} 
%     + O \left( \frac{\epstight n^{2/3} \alpha^2}{\norm{H}_{\infty}^2 \loneboundclasn} \right)
%     \leq
%     \frac{1}{n^{1/3}} \loneboundclasn
% \end{align}
% Note that until now we did not relax the constraints. Now raise to the third power the previous inequality and relax inequality while keeping the first two terms to get:
% \begin{align}
%     \frac{\alpha^{2}}{\norm{H}_{\infty}^2} \frac{9\sqrt{2}}{4\sqrt{\pi}}  + 3 \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} n^{2/3} \frac{\alpha^{4/3}}{\norm{H}_{\infty}^{4/3}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{2/3}
%     \leq
%     \frac{1}{n} \loneboundclasn^3   ( 1 + O\left(\frac{\epstight n}{\loneboundclasn^2}\frac{\alphaols^2}{\norm{H}_{\infty}^2} \right)  )
% \end{align}
% We can further relax this constraint by using the previous lower bound $\alphauls$ in the second term as follows:
% \begin{align}
%     \frac{\alpha^{2}}{\norm{H}_{\infty}^2} \frac{9\sqrt{2}}{4\sqrt{\pi}}  + 3 \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} n^{2/3} \frac{\alphauls^{4/3}}{\norm{H}_{\infty}^{4/3}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{2/3}
%     \leq
%     \frac{1}{n} \loneboundclasn^3  (1+O\left(\frac{\log n}{n^{1/6}}\right))  
% \end{align}
% Note that the term on the left hand side is sum of two convex functions in $\alpha$ and thus is convex. Similarly, as before, we look for $\alphauuls < \alpha_m$ such that the previous inequality is not satisfied. Using concentration results, we get:
% \begin{align}
%     \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{1}{\tuuls^2} \left( 1 - \frac{4}{\tuuls^2} + O \left( \frac{1}{\tuuls^4} \right) \right) + 3\sqrt{\frac{2}{\pi}} \left( \frac{9\sqrt{2}}{4\sqrt{\pi}} \right)^{2/3} &\frac{2 n^{2/3}}{\uuls \tuuls^2} \left(1+ O \left( \frac{1}{\tuuls^2} \right) \right) \frac{1}{\tuls^{4/3}} \left( 1- \frac{8}{3}\frac{1}{\tuls^2} + O \left( \frac{1}{\tuls^4} \right) \right) \\
%     &>
%     \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{1}{t_\sopt^2} \left( 1- \frac{2}{t_\sopt^2} + O \left( \frac{\epsilon_n^3}{t_\sopt^3} \right) \right)\left(1+O\left( \frac{\log n}{n^{1/6}} \right)\right)
% \end{align}
% and we can choose $\uuls = \lambda m$ with $\lambda\in(0,1)$. This gives us a lower bound on $\alpha$ which is tight enough for obtaining bounds on $\nu$ with right multiplicative constant. 
% % Coming back to inequality \eqref{eq:nu_last_tight_bound_alpha} we get the following bound:
% % \begin{align}
% %     \Gamma_4^{\nu} = \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
% %     \geq
% %     \frac{\sqrt{2}}{3\sqrt{\pi}}  \frac{1}{\nu}  
% %     ~~\andtxt~~ 
% %     b\alpha + \nu  \leq \loneboundclasn 
% %     ~~\andtxt~~ 
% %     \nu \in [\kappa_3,1]\loneboundclasn
% %     ~~\andtxt~~ 
% %     \alpha \geq \alphauuls
% %     \right\}.
% %     \label{eq:Gamma_4_nu_def}
% % \end{align}
% % \begin{align}
% %     \nu 
% %     \leq
% %     \loneboundclasn - \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}}  \frac{\sqrt{n}}{\norm{H}_{\infty}} 
% %     \left[ \min_{\nu,b,\alpha} \frac{\alpha}{\sqrt{\nu}}  \subjto (\nu,b,\alpha)\in\Gamma_4^{\nu} \right]
% %     \leq
% %     \loneboundclasn - \left[ \min_{\nu\in [\kappa_3,1]\loneboundclasn} \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}}  \frac{\sqrt{n}}{\norm{H}_{\infty}} \frac{\alphauuls}{\sqrt{\nu}}  \right]
% % \end{align}
% % Thus under assumption that 
% % \begin{align}
% %     \nu^{3/2} - \loneboundclasn \nu^{1/2} + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \sqrt{n} \frac{\alphauuls}{\norm{H}_{\infty}} \leq 0
% % \end{align}
% Substituting $\alpha=\alphauuls$ into inequality~\eqref{eq:nu_ineq_min_alpha} and setting $\nu = \kappa^2\loneboundclasn$ with $\kappa^2 \in [\kappa_3,1]$ we obtain:
% \begin{align}
%     \kappa^3 - \kappa + \sqrt{\frac{\sqrt{2}}{3\sqrt{\pi}}} \frac{\sqrt{n}}{\loneboundclasn^{3/2}} \frac{\alphauuls}{\norm{H}_{\infty}} \leq 0
% \end{align}
% Using concentration inequalities we obtain
% \begin{align}
%     \kappa^3 - \kappa + \frac{2}{3\sqrt{3}} \frac{t_m}{\tuuls} \left( 1-\frac{2}{\tuuls^2} + O \left( \frac{1}{\tuuls^3} \right) \right) \left( 1 + \frac{1}{t_m^2} + O\left( \frac{\epsilon_n^3}{t_m^3} \right) \right) \leq 0
% \end{align}
% and after substituting $\uuls = \lambda m$ with $\lambda<1$ we get the following:
% \begin{align}
%     \kappa^3 - \kappa + \frac{2}{3\sqrt{3}} + \frac{2}{3\sqrt{3}}\frac{\log\lambda -1}{t_m^2} + O \left( \frac{\epsilon_n^3}{t_m^3} \right) \leq 0
% \end{align}
% Thus, we obtain $\kappa^2 \in \left[ \frac{1}{3}-\frac{\tlambda}{t_m^{2/3}}, \frac{1}{3}+\frac{\tlambda}{t_m^{2/3}} \right]$ for some positive universal constant $\tlambda$, which we can write as $\nu = \frac{\loneboundclasn}{3} (1+O(t_m^{-2/3}))$.
% % $\ulambda,\olambda$.

% \subsubsection*{Step 4.2: Upper bound on $\eta$}
% Define the following set:
% \begin{align}
%     % \Gamma_1^{\alpha,L} 
%     \Gamma_{4}^{\eta} 
%     = \bigg\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
%     \geq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
%     &\kappa_4 \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} 
%     - \epstight
%     % + O \left( \frac{1}{n^{2/3}} \right)
%     \\
%     &~~\andtxt~~ 
%     b\alpha + \nu \leq \loneboundclasn 
%     ~~\andtxt~~ 
%     \left| \nu-\frac{\loneboundclasn}{3} \right| \leq \frac{\tlambda \loneboundclasn}{t_m^{2/3}}
%     ~~\andtxt~~ 
%     \alpha \geq \alphauuls
%      \bigg\}.
%     \label{eq:Gamma_4_eta_def}
% \end{align}
% \begin{align}
% \eta^2 
%     \leq
%     \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 
%     \leq 
%     \max_{\nu,\alpha} (\loneboundclasn-\nu)^2 \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}
%     \leq
%     \loneboundclasn^2 \left( 1-\frac{1}{3} + \frac{\tlambda}{\tnstar^{2/3}} \right)^2 \frac{2}{\uuls} \left(1+O\left(\frac{1}{\tuuls^2}\right)\right)
%     \lesssim \frac{1}{t_m^2}
% \end{align}
% \subsubsection*{Bound 5: Tight bounds on $\eta$}
% Now we can apply Proposition~\ref{prop:uniform_conv_noiseless} and use approximation:
% \begin{align}
%     \left|\fnclasn(\nu,\eta)     -
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} - \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} \right|
%     =
%     O \left( \frac{\eta^2}{\nu^3}, \rho\eta^2, \frac{\eta^3}{\nu}\epsilon_n \right) 
%     +
%     O \left( \frac{1}{\nu^3}, \epsilon_c \right) 
%     % =: O_{\eta}(\eta,n,\rho) + O_{\nu,c}(\nu,\epsilon) 
%     =: \OOO_f
% \end{align}
% with $\OOO_f = O\left( \frac{\log\log n}{t_m} \right)$.
% \begin{align}
%     \Gamma_5^{\eta} = \left\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  
%     \geq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
%     \sqrt{\frac{2}{\pi}} \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu}  + \OOO_f
%     ~~\andtxt~~ 
%     b\alpha + \nu \leq \loneboundclasn 
%     ~~\andtxt~~ 
%     \left| \nu-\frac{\loneboundclasn}{3} \right| \leq \frac{\tlambda \loneboundclasn}{t_m^{2/3}}
%     % \nu \in\loneboundclasn\left[ \frac{1}{3}-\frac{\tlambda}{t_m^{2/3}}, \frac{1}{3}+\frac{\tlambda }{t_m^{2/3}} \right]
%     \right\}.
%     \label{eq:Gamma_5_eta_def}
% \end{align}
% Similarly to Equality \eqref{eq:lower_bound_alpha_fcn_kappa} we get:
% \begin{align}
%     \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} \frac{n}{\loneboundclasn} (1-\kappa)^2 (1+\OOO_f) + \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n}{\loneboundclasn^3} 
%     \leq
%     \kappa(1-\kappa)^2 \leq \frac{4}{27}
% \end{align}
% and using our established bound on $\nu$ we get $(1-\kappa)^2 \geq (1- \frac{1}{3}-\frac{\tlambda}{t_m^{2/3}})^2$ and hence we obtain:
% \begin{align}
%     3\sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}\frac{n}{\loneboundclasn} \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \OOO_f \right) +  \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n}{\loneboundclasn^3} 
%     \leq 1
% \end{align}
% Note that the function is convex in $\alpha$. Using concentration, we get:
% \begin{align}
%     2 \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n t_m)^{2/3}}{st_s^2} \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \OOO_f \right) \left(1+O \left( \frac{1}{t_s^2} \right) \right) 
%     +
%     \frac{t_m^2}{t_s^2} \left( 1- \frac{2}{t_s^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
%     \leq 1
% \end{align}
% Now we claim that the $\ulsstar,\olsstar$ given in Lemma~\ref{lemma_uls_ols_exp}, respectively, with $\kappa=1/3$ do not satisfy this inequality for the well-chosen universal constant $\mu$ since
% \begin{align}
%     2& \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n t_m)^{2/3}}{\ulsstar \tuls^2} \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \OOO_f \right) 
%     +
%     \frac{t_m^2}{\tulsstar^2} \left( 1- \frac{2}{\tulsstar^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
%     % \\
%     % & = 
%     % \frac{2}{\tuls^2} \frac{t_m^{2/3}}{t_{n^{2/3}}^{2/3}} \exp \left( \frac{\mu}{2t_m^{1/3}} \right) \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
%     % +
%     % \left( 1 - \frac{\mu}{\tnstar^{7/3}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\mu^2}{\tnstar^{14/3}} \right) \right) \left( 1- \frac{2}{\tuls^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
%     % \\
%     % & =
%     % \frac{2}{\tuls^2} \left( 1 + \frac{\mu}{2t_m^{1/3}} + \frac{\mu^2}{t_m^{2/3}} + O\left(\frac{1}{t_m} \right) \right) \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
%     % + 
%     % 1 - \frac{\mu}{\tnstar^{7/3}} - \frac{2}{\tuls^2} + O \left( \frac{\epsilon_n}{t_m^3} \right)
%     \\
%     &=
%     1 - \frac{\mu}{\tnstar^{7/3}} \left(1-\frac{\tnstar^2}{\tulsstar^2} \right)  + \frac{2\mu^2-6\tlambda}{\tulsstar^2\tnstar^{2/3}} + O \left( \frac{\log\log n}{t_m^3} \right) 
%     =
%     1 +\frac{2\mu^2-6\tlambda}{\tnstar^{8/3}} + O \left( \frac{\log\log n}{t_m^3} \right) > 1
% \end{align}
% for $\mu > \sqrt{3\tlambda}$. Similarly, for $\olsstar$ we get:
% \begin{align}
%     2& \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n t_m)^{2/3}}{\olsstar \tolsstar^2} \left(1 - \frac{3\tlambda}{t_m^{2/3}} + \OOO_f \right) 
%     +
%     \frac{t_m^2}{\tolsstar^2} \left( 1- \frac{2}{\tolsstar^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
%     \\
%     % & =     
%     % \frac{2}{\tols^2} \frac{t_m^{2/3}}{t_{n^{2/3}}^{2/3}} \exp \left( -\frac{\mu}{2t_m^{1/3}} \right) \left(1 - \frac{3\tlambda}{t_m^{2/3}} + \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
%     % +
%     % \left( 1 + \frac{\mu}{\tnstar^{7/3}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\mu^2}{\tnstar^{14/3}} \right) \right) \left( 1- \frac{2}{\tols^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
%     % \\
%     % & =
%     % \frac{2}{\tols^2} \left( 1 - \frac{\mu}{2t_m^{1/3}} + \frac{\mu^2}{t_m^{2/3}} + O\left(\frac{1}{t_m} \right) \right) \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
%     % + 
%     % 1 + \frac{\mu}{\tnstar^{7/3}} - \frac{2}{\tols^2} + O \left( \frac{\epsilon_n}{t_m^3} \right)
%     % \\
%     &=
%     1 + \frac{\mu}{\tnstar^{7/3}} \left(1-\frac{\tnstar^2}{\tolsstar^2} \right)  + \frac{2\mu^2-6\tlambda}{\tolsstar^2\tnstar^{2/3}} + O \left( \frac{\log\log n}{t_m^{3}} \right) 
%     =
%     1 +\frac{2\mu^2-6\tlambda}{\tnstar^{8/3}} + O \left( \frac{\log\log n}{t_m^{3}} \right) > 1
% \end{align}
% Now we can bound $\eta$ as follows:
% \begin{align}
%     \eta^2 
%     \leq
%     \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 
%     &\leq 
%     \max_{\nu,\alpha} (\loneboundclasn-\nu)^2 \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}
%     \leq
%     \loneboundclasn^2 \left( 1-\frac{1}{3} + \frac{\tlambda}{\tnstar^{2/3}} \right)^2 \frac{2}{\ulsstar} \left(1+O\left(\frac{1}{\tulsstar^2}\right)\right)
%     \\
%     &\leq
%     \frac{2}{3} \frac{1}{\tnstar^2} \exp \left( \frac{\mu}{2\tnstar^{1/3}} \right) \left(1+ O \left( \frac{1}{\tnstar^{2/3}} \right) \right)
%     = 
%     \frac{2}{3} \frac{1}{\tnstar^2} \left( 1 + \frac{\mu}{2\tnstar^{1/3}} + O \left( \frac{1}{\tnstar^{2/3}} \right) \right)
% \end{align}
% and
% \begin{align}
%     \eta^2 
%     \geq
%     \min_{b,\alpha} b^2\norm{\gamma(\alpha)}_2^2 
%     &\geq
%     \min_{\nu,\alpha} \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{n}{\nu} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}
%     \geq
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{n}{\loneboundclasn \left( \frac{1}{3}+\frac{\tlambda}{\tnstar^{2/3}} \right)} \frac{2}{\olsstar\tolsstar^2} \left( 1 + O \left( \frac{1}{\tolsstar^2} \right) \right)
%     \\
%     &\geq
%     \frac{2}{3} \frac{1}{\tnstar^2} \exp \left( -\frac{\mu}{2\tnstar^{1/3}} \right) \left(1 - O \left( \frac{1}{\tnstar^{2/3}} \right) \right)
%     =
%     \frac{2}{3} \frac{1}{\tnstar^2} \left( 1 - \frac{\mu}{2\tnstar^{1/3}} - O \left( \frac{1}{\tnstar^{2/3}} \right) \right)
% \end{align}
% Thus setting $\tsetNoiselessZero:=\Gamma_5^{\eta}$ finishes the proof of Proposition~\ref{prop:BoundGamma0_class_noiseless}.

% % Similarly to Equality \eqref{eq:lower_bound_alpha_fcn_kappa} we get:
% % \begin{align}
% %     \sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2} \frac{n}{\loneboundclasn} (1-\kappa)^2 (1+\OOO_f) + \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n}{\loneboundclasn^3} 
% %     \leq
% %     \kappa(1-\kappa)^2 \leq \frac{4}{27}
% % \end{align}
% % and using our established bound on $\nu$ we get $(1-\kappa)^2 \geq (1- \frac{1}{3}-\frac{\tlambda}{t_m^{2/3}})^2$ and hence we obtain:
% % \begin{align}
% %     3\sqrt{\frac{2}{\pi}} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}\frac{n}{\loneboundclasn} \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) +  \frac{9\sqrt{2}}{4\sqrt{\pi}} \frac{\alpha^2}{\norm{H}_{\infty}^2} \frac{n}{\loneboundclasn^3} 
% %     \leq 1
% % \end{align}
% % Note that the function is convex in $\alpha$. Using concentration, we get:
% % \begin{align}
% %     2 \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n t_m)^{2/3}}{st_s^2} \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) \left(1+O \left( \frac{1}{t_s^2} \right) \right) 
% %     +
% %     \frac{t_m^2}{t_s^2} \left( 1- \frac{2}{t_s^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
% %     \leq 1
% % \end{align}
% % Now we claim that the $\ulsstar,\olsstar$ given in Lemma~\ref{lemma_uls_ols_exp}, respectively, with $\kappa=1/3$ do not satisfy this inequality for the well-chosen universal constant $\mu$ since
% % \begin{align}
% %     2& \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n t_m)^{2/3}}{\ulsstar \tuls^2} \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
% %     +
% %     \frac{t_m^2}{\tulsstar^2} \left( 1- \frac{2}{\tulsstar^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
% %     % \\
% %     % & = 
% %     % \frac{2}{\tuls^2} \frac{t_m^{2/3}}{t_{n^{2/3}}^{2/3}} \exp \left( \frac{\mu}{2t_m^{1/3}} \right) \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
% %     % +
% %     % \left( 1 - \frac{\mu}{\tnstar^{7/3}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\mu^2}{\tnstar^{14/3}} \right) \right) \left( 1- \frac{2}{\tuls^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
% %     % \\
% %     % & =
% %     % \frac{2}{\tuls^2} \left( 1 + \frac{\mu}{2t_m^{1/3}} + \frac{\mu^2}{t_m^{2/3}} + O\left(\frac{1}{t_m} \right) \right) \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
% %     % + 
% %     % 1 - \frac{\mu}{\tnstar^{7/3}} - \frac{2}{\tuls^2} + O \left( \frac{\epsilon_n}{t_m^3} \right)
% %     \\
% %     &=
% %     1 - \frac{\mu}{\tnstar^{7/3}} \left(1-\frac{\tnstar^2}{\tulsstar^2} \right)  + \frac{2\mu^2-6\tlambda}{\tulsstar^2\tnstar^{2/3}} + O \left( \frac{\epsilon_n}{t_m^3} \right) 
% %     =
% %     1 +\frac{2\mu^2-6\tlambda}{\tnstar^{8/3}} + O \left( \frac{\epsilon_n}{t_m^3} \right) > 1
% % \end{align}
% % for $\mu > \sqrt{3\tlambda}$. Similarly, for $\olsstar$ we get:
% % \begin{align}
% %     2& \frac{2\left(\frac{3}{\pi}\right)^{1/3}(n t_m)^{2/3}}{\olsstar \tolsstar^2} \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
% %     +
% %     \frac{t_m^2}{\tolsstar^2} \left( 1- \frac{2}{\tolsstar^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
% %     \\
% %     % & =     
% %     % \frac{2}{\tols^2} \frac{t_m^{2/3}}{t_{n^{2/3}}^{2/3}} \exp \left( -\frac{\mu}{2t_m^{1/3}} \right) \left(1 - \frac{3\tlambda}{t_m^{2/3}} + \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
% %     % +
% %     % \left( 1 + \frac{\mu}{\tnstar^{7/3}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\mu^2}{\tnstar^{14/3}} \right) \right) \left( 1- \frac{2}{\tols^2} + O \left( \frac{\epsilon_n}{t_m^3} \right) \right) 
% %     % \\
% %     % & =
% %     % \frac{2}{\tols^2} \left( 1 - \frac{\mu}{2t_m^{1/3}} + \frac{\mu^2}{t_m^{2/3}} + O\left(\frac{1}{t_m} \right) \right) \left(1 - \frac{3\tlambda}{t_m^{2/3}} +  \frac{9\tlambda^2}{4t_m^{4/3}} \right) 
% %     % + 
% %     % 1 + \frac{\mu}{\tnstar^{7/3}} - \frac{2}{\tols^2} + O \left( \frac{\epsilon_n}{t_m^3} \right)
% %     % \\
% %     &=
% %     1 + \frac{\mu}{\tnstar^{7/3}} \left(1-\frac{\tnstar^2}{\tolsstar^2} \right)  + \frac{2\mu^2-6\tlambda}{\tolsstar^2\tnstar^{2/3}} + O \left( \frac{\epsilon_n}{t_m^{3}} \right) 
% %     =
% %     1 +\frac{2\mu^2-6\tlambda}{\tnstar^{8/3}} + O \left( \frac{\epsilon_n}{t_m^{3}} \right) > 1
% % \end{align}
% % Now we can bound $\eta$ as follows:
% % \begin{align}
% %     \eta^2 
% %     \leq
% %     \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 
% %     &\leq 
% %     \max_{\nu,\alpha} (\loneboundclasn-\nu)^2 \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2}
% %     \leq
% %     \loneboundclasn^2 \left( 1-\frac{1}{3} + \frac{\tlambda}{\tnstar^{2/3}} \right)^2 \frac{2}{\ulsstar} \left(1+O\left(\frac{1}{\tulsstar^2}\right)\right)
% %     \\
% %     &\leq
% %     \frac{2}{3} \frac{1}{\tnstar^2} \exp \left( \frac{\mu}{2\tnstar^{1/3}} \right) \left(1+ O \left( \frac{1}{\tnstar^{2/3}} \right) \right)
% %     = 
% %     \frac{2}{3} \frac{1}{\tnstar^2} \left( 1 + \frac{\mu}{2\tnstar^{1/3}} + O \left( \frac{1}{\tnstar^{2/3}} \right) \right)
% % \end{align}
% % and
% % \begin{align}
% %     \eta^2 
% %     \geq
% %     \min_{b,\alpha} b^2\norm{\gamma(\alpha)}_2^2 
% %     &\geq
% %     \min_{\nu,\alpha} \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{n}{\nu} \frac{\norm{\gamma(\alpha)}_2^2}{\norm{H}_{\infty}^2}
% %     \geq
% %     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{n}{\loneboundclasn \left( \frac{1}{3}+\frac{\tlambda}{\tnstar^{2/3}} \right)} \frac{2}{\olsstar\tolsstar^2} \left( 1 + O \left( \frac{1}{\tolsstar^2} \right) \right)
% %     \\
% %     &\geq
% %     \frac{2}{3} \frac{1}{\tnstar^2} \exp \left( -\frac{\mu}{2\tnstar^{1/3}} \right) \left(1 - O \left( \frac{1}{\tnstar^{2/3}} \right) \right)
% %     =
% %     \frac{2}{3} \frac{1}{\tnstar^2} \left( 1 - \frac{\mu}{2\tnstar^{1/3}} - O \left( \frac{1}{\tnstar^{2/3}} \right) \right)
% % \end{align}


==> sections/subsections_theory/noiseless/unicon_sketch.tex <==
\subsubsection*{Proof sketch of Uniform Convergence Proposition~\ref{prop:BoundGamma0_class_noiseless}}
\label{subsubsec:proof_sketch_unicon_noiseless}

\red{TO BE ADDED}


==> sections/subsections_theory/noisy/loc_sketch.tex <==
\subsubsection{Proof sketch of Localization Proposition~\ref{prop:Rbound_noisy}}
\label{subsubsec:proof_sketch_loc_noisy}
We now give a proof sketch for deriving an upper bound on $\PhiCdn$. For this, it is sufficient to find a feasible point satisfying the constraint in the optimisation problem defining $\PhiCdn$. Namely, let $(\tnu,\tb,\talpha,\tvarsigma)$ be a point which satisfies constraint from definition of $\PhiCdn$ in Proposition~\ref{prop:parametrization_class_noisy} i.e. assume that $\frac{ \tb^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fnclas \left( \tnu, \tb \norm{ \gamma \left( \talpha \right) }_2, \tvarsigma \right)$. Then by definition of $\PhiCdn$ we have:
\begin{align}
    \PhiCdn &\leq  \vert \tnu \vert \sqrt{s}  + \tb \talpha + \norm{\tvarsigma}_1
\end{align}

We will a choose point with $\tvarsigma = 0$ so we can recast $\PhiCdn$ as an optimization problem over three variables $(\tnu,\tb,\talpha)$. The rest of the proof considers choosing these three variables.

First recall that we defined $\fclas = \EE [ \fnclas]$. Now using the concentration of Lipschitz continuous function (see e.g., \cite{Ledoux1992AHS}), it is straight forward to show:
\begin{lemma}
\label{lemma_point_conv}
For any $\nu,\eta>0$ holds that:
    \begin{align}
        \prob \left( \abs{ \fnclas \left( \nu, \eta, 0 \right) -  \fclas \left( \nu, \eta, 0 \right)  }  \geq \epsilon \right) \leq \exp \left( - c \frac{ n \epsilon^2 }{ \nu^2 + \eta^2 } \right)
    \end{align}
where $c>0$ is a positive universal constant. 
\end{lemma} 
The goal is now to use Lemma~\ref{lemma_point_conv} to relax the constraints in the optimization problem $\PhiCdn$ i.e. it is sufficient to show that $(\tnu,\tb,\talpha,0)$ satisfies 
\begin{align}
    \frac{\tb^2 \norm{H}_{\infty}^2}{n} \geq \fclas(\tnu,\tb\norm{\gamma(\talpha)}_2,0) + \epsilon
    \label{eq:proof_sketch_loc_noisy_balpha}
\end{align}
The function $\fclas(\tnu,\tb\norm{\gamma(\talpha)}_2,0)$ achieves minimum for $\tnu=\nubar$ and $\tb\norm{\gamma(\talpha)}_2=0$. Thus in order for inequality~\eqref{eq:proof_sketch_loc_noisy_balpha} to hold for widest range of $\tb,\talpha$ we choose $\tnu=\nubar=const$. Now we use Taylor approximation of $\fclas$ around point $(\nubar,0,0)$ to rewrite constraint \eqref{eq:proof_sketch_loc_noisy_balpha} as:
\begin{align}
    \frac{ \tb^2 \norm{\Hgaussian}_{\infty}^2 }{n}   
    \geq
    \fstar + \frac{1}{2}\feestar \tb^2 \norm{ \gamma \left( \talpha \right) }_2^2 + O \left( \tb^3 \norm{ \gamma \left( \talpha \right) }_2^3 \right) + \epsilon
\end{align}
Rearranging this inequality a bit we get the following constraint:
\begin{equation}
    (\tb \talpha)^2 \geq \frac{ n \talpha^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar +\epsilon }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \talpha \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \tb^3 \norm{ \gamma \left( \talpha \right) }_2^3 \right)  }
    \label{eq:proof_sketch_loc_noisy_balpha_final}
\end{equation}
Since we want $\tb\talpha$ to be as small as possible to obtain a tight bound on $\PhiCdn$ we set $\tb\talpha$ to be equal to the right hand side of Equation~\eqref{eq:proof_sketch_loc_noisy_balpha_final}. Furthermore, we can minimize right hand side over $\talpha$ to obtain $\talpha=\alpha_s$ with $s=m$, and $m$ given in the statement of the proposition.

==> sections/subsections_theory/noisy/unicon_proof_old.tex <==
\subsection{Proof of Uniform Convergence Proposition~\ref{prop:BoundGamma0_class_noisy}}
\label{subsec:proof_unicon_noisy}
\begin{align}
    \setNoisyZero = \left\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2, \varsigma) ~~\andtxt~~  b\norm{\gamma(\alpha)}_1 \leq \loneboundclas \right\}.
    \label{eq:Gamma0_def_class_noisy}
\end{align}
$\setNoisyZero$ is a relaxation of the set $\setZeroUni$. \red{add here a bit}

% \subsection{Proof of Proposition~\ref{prop:BoundGamma0_class_noisy}}
The proof of the proposition follows from several steps where in each step we approximate $\fnclas$ using the bounds on $(\nu, \eta, \varsigma)$ from the previous steps to obtain a tighter bound on $(\nu, \eta, \varsigma)$ using the tools developed in \cite{wang2021tight}.  
The probability statement in Proposition~\ref{prop:BoundGamma0_class_noisy} follows when taking the union bound over all equations which we condition on throughout the proof. 
Furthermore, we note that $\Gamma_0$ is not empty as it clearly the choice $\alpha=\alpha_{\sopt}$ leads with high probability to a feasible point due to the choice of $\loneboundclas$ in Proposition~\ref{prop:Rbound_noisy}. 




\subsubsection*{Bound 1: \texorpdfstring{$\nu^2,\eta^2, \norm{\varsigma}_2^2 = O(1)$}{}}
\label{sec:l1class_nueta_const_bound}

In order to apply Lemma~\ref{lemma_quadratic_plus_fstar_bound} in the next step,  which gives tight bounds for $\fnclas$, we first need to show that with high probability, $\nu^2,\eta^2, \norm{\varsigma}_2 = O(1)$. This is the goal of this first step. More specifically, 
the goal of this first step is to show that there exist universal constants $\boundnuone, \boundetaone, \boundvarsigmaone > 0$ such that for any element $(\nu, b, \alpha, \varsigma)$ of $\Gamma_0$ we have that $ \nu \leq B_{\nu,1} $, $ \eta = b\norm{ \gamma(\alpha)}_2 \leq B_{\eta,1}$ and $\norm{\varsigma}_2 \leq \boundvarsigmaone$ with high probability over the draws of $\Hgaussian,\Ggaussian$ and $\Xs, \xi$. 

For this first step, we use the fact that in the presence of label noise, $\fnclas$ is lower bounded by a quadratic function as stated in Lemma ~\ref{quadratic_bound_fn}. 
As a result, we can relax the first constraint in Definition \eqref{eq:Gamma0_def_class_noisy} of $\Gamma_0$ to 
\begin{equation}
    \frac{1}{n} b^2\norm{\Hgaussian}_{\infty}^2  \geq  \constnu \nu^2  + \consteta  b^2 \norm{\gamma(\alpha)}_2^2  + \constvarsigma \norm{\varsigma}_2^2.
\end{equation} 
 
% \red{say more about the intuition, then we can show:}
This approximation leads to an optimization problem similar to the ones discussed in Lemma 1 in \cite{wang2021tight}. After further relaxations we obtain exactly the same form of the inequality, and hence we can use the arguments from \cite{wang2021tight}. 


Let's first consider bounding of $\eta$ and then we use the obtained result to bound $\nu$ and $\norm{\varsigma}_2$.
\paragraph{Step 1.1: Upper bound on $\eta$.}
For this part of the proof we further relax both constraints from Definition \eqref{eq:Gamma0_def_class_noisy} of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_1^{\eta} &= \left\{ (\nu, b, \alpha, \varsigma) \subjto \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \loneboundclas  \right\} \\
    &= \left\{ (\nu, b, \alpha, \varsigma) \subjto \frac{1}{n} \norm{H}_{\infty}^2 \geq \consteta  \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \loneboundclas  \right\} \label{eq:lpstep1set}
\end{align}
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ do not depend on $\nu$ and hence we will now consider only variables $b$ and $\alpha$ and bound $ \eta $ as:
\begin{align}
    &\eta^2 \leq \left[\max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto (b,\alpha) \in \Gamma_1^{\eta} \right]
    =  \left[
    \max_{1\leq \alpha \leq \alpham} \loneboundclas^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 } 
    \subjto
    %B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
    \left( \frac{\loneboundclas}{\alpha}, \alpha \right) \in \Gamma_1^{\eta} \right]
    \label{eq:l1proofstep1bound}
\end{align}

Now note that as discussed in Section~\ref{subsubsec:prop_gamma_alpha} $\norm{\gamma(\alpha)}_2^2$ is convex. Therefore, the set of feasible $\alpha$ in the Set $\Gamma_1^{\eta}$ is an non-empty interval. Indeed, to see that the interval is non empty, recall that we defined $ \loneboundclas $ in such way that $ (b,\alpha_{\soptn}) \in \Gamma_0 $ with high probability for $b \alpha_{\soptn}\leq \loneboundclas$. As $ \Gamma_0 \subset \Gamma_1^{\eta}$, with high probability there exists some $ b > 0 $ such that $ (b, \alpha_{\soptn} ) \in \Gamma_1^{\eta} $ proving that $\Gamma_1^{\eta} \neq \emptyset$. Furthermore,  since $\frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 }$ is monotonically decreasing, to upper bound Equation~\eqref{eq:l1proofstep1bound} it is sufficient to find $\ulalpha < \alpha_{\soptn}$ such that
\begin{align}
\label{eq:s_condition_one}
    \norm{\gamma(\ulalpha)}_2^2 > \frac{1}{\consteta n} \norm{H}_{\infty}^2. 
\end{align}

It is sufficient to only consider the discretized version of $\alpha$, i.e., $\alpha_s$, for which we have access to tight concentration inequalities from Proposition~\ref{prop:concentration_gammas}. We now  claim that $\alpha_{\ulm}$ with $\ulm =\lambda_{\ulm} \frac{ n }{ \log (d/n) }$ satisfies the inequality Equation~\eqref{eq:s_condition_one} for some positive universal constant $ \lambda_{\ulm} >0  $. Using the characterization $\tm^2 = 2\log (d/m) + O (\log \log (d/m) ) $ from Section~\ref{subsubsec:prop_gamma_alpha} we get:
\begin{align}
    \frac{ 2 }{ \ulm \tulm^2 } \left( 1 - O \left( \frac{ 1 }{ \tulm^2 } \right) \right)
    & >
    \frac{ 1 }{ n \lambda_{\ulm} } \left( 1 - O \left( \frac{\log\log (d/n) }{\log (d/n) } \right) \right) > \frac{1}{\consteta n}
\end{align}
where last inequality holds for $d/n$ sufficiently large and $\lambda_{\ulm}$ small enough.

Therefore, from Equation~\eqref{eq:l1proofstep1bound} and the concentration inequality from Proposition \ref{prop:concentration_gammas}, we get:
\begin{align}
    \eta^2 \leq \frac{ n \fstar }{ \tsoptn^2 } \frac{2}{\ulm}\left( 1 + O \left( \frac{1}{\tulm^2} \right) \right) %\leq \boundeta' \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
    =: B_{\eta,1}^2,
\end{align}
with $B_{\eta,1}= \Theta (1)$, as desired. 

\paragraph{Step 1.2: Upper bound on $\nu$.} Now we derive an upper bound for $\nu$. Using the result from the previous sub-step, we consider the following set:
\begin{align}
    \Gamma_1^{\nu} = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
    %\frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
\end{align}
Clearly, we have again  $\Gamma_0 \subset \Gamma_1^{\nu}$ with high probability. Hence we can upper bound $\nu$ as follows:
\begin{align} \label{eq:nu_opt_first_reduction}
    \nu^2 &\leq \frac{ 1 }{ n \constnu } \left[\max_{b,\alpha} b^2 \norm{H}_{\infty}^2
    \subjto 
    b^2 \leq \frac{\loneboundclas^2}{\alpha^2}
    \andtxts 
    b^2 \leq \frac{B_{\eta,1}^2}{\norm{ \gamma(\alpha)  }_2^2}\right]
    \\
    &= \frac{ 1 }{ n \constnu }  \norm{H}_{\infty}^2 ~\max_{\alpha}\min\left(\frac{\loneboundclas^2}{\alpha^2}, \frac{B_{\eta,1}^2}{\norm{\gamma(\alpha)}_2^2}\right)
\end{align}
Now recall that $\norm{\gamma(\alpha)}_2$ is convex with global minimum at $\alpha_{d+1/2} = \frac{\norm{H}_1 \norm{H}_{\infty}}{\norm{H}_2^2}$ (see Lemma 4 in \cite{wang2021tight}). Thus, the optimal $\alphaopt$ is obtained for $\alphaopt < \alpha_{d+1/2}$ with 
\begin{equation}
    \frac{\loneboundclas^2}{\alphaopt^2} =  \frac{B_{\eta,1}^2 }{\norm{\gamma(\alphaopt)}_2^2}.
\end{equation}
We now show that we can upper and lower bound by $\alpha_{\ulm} <\alphaopt < \alpha_{\olm}$ with high probability with $\ulm =  \lambda_{\ulm} \frac{ \soptn}{ \log (d/\soptn)} $ and $\olm =  \lambda_{\olm} \frac{ \soptn }{ \log (d/\soptn) }$ and $0<\lambda_{\ulm}<1< \lambda_{\olm}$ universal constants. For this, we need to show that with high probability, 
\begin{align}
        \frac{\norm{\gamma(\alphaols)}_2^2}{\alphaols^2} <  \frac{B_{\eta,1}^2 }{\loneboundclas^2} < \frac{\norm{\gamma(\alphauls)}_2^2}{\alphauls^2}.
\end{align}
However,  similarly to bounding $\eta$ in the previous sub-step, we can straight forwardly verify that this statement holds with high probability when using Proposition~\ref{prop:concentration_gammas} and the characterization $\tm^2 = 2\log (d/m) + O (\log \log (d/m) ) $ from Section~\ref{subsubsec:prop_gamma_alpha}. 
Therefore, as a result, we obtain the desired upper bound
\begin{align}%\label{eq:nu_opt_first_reduction}
    \nu^2 &\leq  \frac{ 1 }{ n \constnu }  \norm{H}_{\infty}^2 ~\min\left(\frac{\loneboundclas^2}{\alphauls^2}, \frac{B_{\eta,1}^2}{\norm{\gamma(\alphaols)}_2^2}\right) \leq \frac{ 1 }{ n \constnu }  \norm{H}_{\infty}^2 ~\frac{\loneboundclas^2}{\alphauls^2}
    =: B_{\nu,1}^2,
\end{align}
and in particular, we have again that $B_{\nu,1} = \Theta(1)$. 
\paragraph{Step 1.3: Upper bound on $\norm{\varsigma}_2$.}
Applying exactly the same procedure as in the section above for the set:
\begin{align}
    \Gamma_1^{\varsigma} = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constvarsigma \norm{\varsigma}_2^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
    %\frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
\end{align}
we get that $\norm{\varsigma}_2 \leq \boundvarsigmaone$ with $\boundvarsigmaone = \Theta(1)$, which completes the first step of the proof.








\subsubsection*{Bound 2: \texorpdfstring{$\deltanu^2,\eta^2,\norm{\varsigma}_2^2 = O\left(\frac{1}{\log(d/n)}\right)$}{}}

Recall that $\nubar := \arg\min \fclas(\nu, 0, 0)$ and define $\deltanu = \nu -\nubar$. Conditioning on the event where the bounds form the first step hold for $\nu,\eta,\norm{\varsigma}_2$, the goal of this second step is to show that for any element $(\nu, b, \alpha, \sigma)$ of $\Gamma_0$ we have that $\deltanu^2 = O \left( \frac{1}{ \log \left( d/n \right) }  \right) $, $ \eta^2 = b^2 \norm{\gamma(\alpha)}_2^2 = O \left( \frac{1}{ \log \left( d/n \right) } \right)$ and $\norm{\varsigma}_2^2 = O \left( \frac{1}{ \log \left( d/n \right) } \right) $ with high probability over the draws of $\Hgaussian, \Ggaussian, \Xs$ and $\xi$. 

From the previous step, we know that with high probability, $ \nu \leq \boundnuone $, $ \eta \leq \boundetaone $ and $\norm{\varsigma}_2 \leq \boundvarsigmaone$. Hence we can use Lemma~\ref{lemma_quadratic_plus_fstar_bound} to obtain a tight lower bound for $\fnclas$, which is based on uniform convergence of $\fnclas$ to its expectation in Proposition \ref{prop:unifConv}, and relax the constraint from definition of the set $\Gamma_0$ as follows:
\begin{align}
\label{eq:second_iteration_relaxed_constraint_f}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 
    \geq
    \fnclas (\nu, b\norm{\gamma(\alpha)}_2,\varsigma) 
    &\geq
    f ( \nu, b\norm{\gamma(\alpha)}_2,\varsigma) - \constconc \\
    &\geq
    \fstar  + \tconstnu \deltanu^2 + \tconsteta b^2\norm{\gamma(\alpha)}_2^2 + \tconstvarsigma \norm{\varsigma}_2^2 - \constconc, 
\end{align}
where we choose $\constconc =  O \left( \frac{1}{\tsoptn^3} \right)$ and hence it holds with probability at least $1 - \exp \left( -c_2  \frac{n}{\tsoptn^6}  \right) -  \exp \left( -c_3 \frac{ n  }{\tsoptn^3 s \log (ns)} \right)$. 
Again we first consider the bounding of $\eta$ and then use the obtained result to bound $\deltanu$ and $\norm{\varsigma}_2$.

\paragraph{Step 2.1: Upper bound on $\eta$.} 
We similarily to the previous step, we consider the set:
\begin{align}
    \Gamma_2^{\eta} = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta b^2 \norm{\gamma(\alpha)}_2^2 - \constconc
    \andtxts
    b\alpha \leq \loneboundclas
    \right\} 
\end{align}

Again, we have that with high probability $\Gamma_0 \subset \Gamma_2^{\eta} $.
Clearly, to upper bound $\eta = b \norm{\gamma(\alpha)}_2$, we can again set $ b = \frac{\loneboundclas}{\alpha} $ and thus obtain:
\begin{align}
    \eta^2 &\leq \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto \left(\frac{M}{\alpha},\alpha \right) \in \Gamma_2^{\eta}  \\
    &= \max_{\alpha} \frac{M^2}{\alpha^2} \norm{\gamma(\alpha)}_2^2 \subjto \frac{ 1 }{ n } \frac{M^2}{\alpha^2} \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta \frac{M^2}{\alpha^2} \norm{\gamma(\alpha)}_2^2 - \constconc.
    \label{eq:l1proofstep2eta}
\end{align}
Multiplying the constraint on both sides with $\alpha^2$ and using the fact that $\norm{\gamma(\alpha)}_2^2$ is convex shows that the set of feasible $\alpha$ is again a (non-empty) interval. 
Thus, by the monotonicity of $ \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2} $ the problem reduces again to finding $\alphauls < \alpha_{\soptn}$ (where we use again that $\alpha_{\soptn}$ satisfies the constraints with high probability) such that $\alphauls$ violates the constraint in Equation~\eqref{eq:l1proofstep2eta}, i.e., 
\begin{align}
\label{eq:l1proofstep2eta2}
    \left( \fstar - \constconc \right) \frac{ n \alphauls^2 }{  \loneboundclas^2 \norm{H}_{\infty}^2 } + \tconsteta n \frac{ \norm{ \gamma(\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } > 1
\end{align}

We now show that we can choose $ \ulm = \lambda_{\ulm} \soptn$ with universal constant $\lambda_{\ulm} \in (0,1)$. Indeed, applying  Proposition \ref{prop:concentration_gammas} and using the characterization $t_s =   2 \log(d/s) - \log \log (d/s) -\log(\pi) +\frac{\log\log(d/s)}{2\log(d/s)} + O\left(\frac{1}{\log(d/s)}\right)$ from Section~\ref{subsubsec:prop_gamma_alpha} we get:
\begin{align}
 \left( \fstar - \constconc \right) \frac{ n \alphauls^2 }{  \loneboundclas^2 \norm{H}_{\infty}^2} &= 1 + \frac{\log(\lambda_{\ulm})-2}{\tsoptn^2} + O\left(\frac{1}{\tsoptn^3}\right) \\
 \mathrm{and}~~\tconsteta n \frac{ \norm{ \gamma(\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } &= 
\frac{1}{\tsoptn^2}\frac{4\tconsteta}{\lambda_{\ulm}}  +  O \left( \frac{1}{ \tsoptn^3} \right)
\end{align}
where $O(.)$ has hidden dependencies on $\lambda_{\ulm}$. Hence, it is straight forward to see that for any $d \geq c n$ with universal constant $c>0$ (and thus $\tsoptn$ lower bounded), we can find a universal constant $\lambda_{\ulm}$ such that Equation~\eqref{eq:l1proofstep2eta2} holds. 

Hence, we can upper bound $\eta^2$ in Equation \eqref{eq:l1proofstep2eta} as follows:
\begin{align} \label{eq:eta_bound_second_reduction}
    \eta^2 
    \leq
    \loneboundclas^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \alpha_{\ulm}^2 } 
    \leq
    \frac{ n \fstar }{ \tsoptn^2 } \frac{2}{\ulm}\left( 1 + O \left( \frac{1}{\tulm^2} \right) \right) 
    \leq
    % \frac{c_{\eta,2}}{\log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
    \frac{2\fstar}{\feestar \lambda_{\ulm} \log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
    =:
    \frac{B_{\eta,2}^2}{\tsoptn^2}
\end{align}
with $B_{\eta,2}^2 = \Theta(1)$.


\paragraph{Step 2.2: Upper bound on $\deltanu$.}
We now again bound $\nu$ using the previous upper bound on $\eta^2 = O(\log^{-1}(d/n))$. More specifically, we bound $\deltanu$ with $\nu = \nubar +\deltanu$ and thus obtain both an upper and lower bound for $\nu$. 
 First, we again define
\begin{align}
    \Gamma_2^{\nu} = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}b^2\norm{H}_{\infty}^2 \geq \fstar - \constconc + \tconstnu \deltanu^2
    \andtxts
    b\alpha \leq \loneboundclas 
    \andtxts
    b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,2}}{\tsoptn}  \right\}
\end{align}
as in the previous step. 

Clearly, we have again  $\Gamma_0 \subset \Gamma_2^{\nu}$ with high probability. Hence we can upper bound $\deltanu$ by:
\begin{align} %\label{eq:nu_opt_first_reduction}
    \deltanu^2 &\leq \frac{1}{\tconstnu}\left(\frac{ 1 }{ n } \norm{H}_{\infty}^2 \max_{\alpha}\min\left(\frac{\loneboundclas^2}{\alpha^2}, \frac{B_{\eta,2}^2}{\tsoptn^2 \norm{\gamma(\alpha)}_2^2}\right) - \fstar + \constconc \right)
\end{align}
In particular, we obtain again an upper bound for $\deltanu$ (as for $\nu$ in the previous step) when bounding finding $\alpha_{\ulm} < \alphaopt < \alpha_{\olm}$ where $\alphaopt \leq \alpha_{d+1/2}$ is the $\alpha$ such that the two terms in the $\min$ match. However, we can verify from a similar argument as for the upper bound for $\eta^2$ in the previous sub-step that we can choose $ \ulm = \lambda_{\ulm} \soptn$ with universal constant $\lambda_{\ulm} \in (0,1)$ and $\olm =\lambda_{\olm} \soptn$ with universal constant $\lambda_{\olm} >1$. Hence, we obtain the upper bound

\begin{align}
    \deltanu^2 
    &\leq
    \frac{\norm{H}_{\infty}^2}{ n \tconstnu }  \frac{ \loneboundclas^2}{\alphauls^2}
    \leq 
    \frac{ \fstar t_{\ulm}^2}{\tsoptn^2 \tconstnu } \left( 1 + \frac{2}{\tsoptn^2}  \right)
    - \frac{\fstar}{\tconstnu} + O \left( \frac{1}{\tsoptn^3} \right)\\
    & = \frac{\fstar(2 -2\log(\lambda_{\ulm})) }{\tconstnu 2\log(d/n)}\left( 1 + O \left( \frac{1}{\sqrt{\log(d/n)}} \right) \right)
    =: 
    \frac{B_{\deltanu,2}^2}{\tsoptn^2} 
\end{align}
Similarly we get:
\paragraph{Step 2.3: Upper bound on $\norm{\varsigma}_2$.}
Using the same procedure as for $\deltanu$ we get that $\norm{\varsigma}_2^2 \leq \frac{\boundvarsigmatwo^2}{\tsoptn^2}$ which concludes the proof.
\begin{align}
    \Gamma_2^{\varsigma} = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto
    \frac{1}{n}b^2\norm{H}_{\infty}^2 \geq \fstar - \constconc + \tconstvarsigma \norm{\varsigma}_2^2
    \andtxts
    b\alpha \leq \loneboundclas 
    \andtxts
    b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,2}}{\tsoptn}  \right\}
\end{align}







% \subsubsection{Bound 3: Proof of the proposition (1-sparse case, tight bounds). }
% In order to get tight bounds up to multiplicative constant, we need to restrict analysis to $1$-sparse ground truth $\wgt$ i.e. assume $\wgt=(1,0,\dots,0)$. Note that in this case we have $\norm{\varsigma}_2=0$. We already know that $\nu$ concentrates around $\nubar$. However, in order to get a tight expression for the risk and also a valid lower bound, we need to get tighter bounds for $\eta^2$ conditioning on the bounds on $\eta^2,\deltanu^2$ from the previous step,  leading to Proposition~\ref{prop:BoundGamma0_class_noisy}.


% % In this part of the proof we use Taylor series approximation of function $f$ up to quadratic terms as shown in equation \eqref{eq:f_taylor_approx}. Using similar arguments as in previous two bounding steps, we obtain Proposition \ref{prop:BoundOmegal1}.
% % \begin{lemma}
% %     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% % \end{lemma}
% % \begin{proof}
% % Conditioning on the event where the bounds for $\nu,\eta$ from the previous second step hold, we now derive the tight bounds
% In this part of the proof we use Taylor series approximation of the function $\fclas$ where we use the result form the last step to bound the  higher order terms involving $\eta$. Similarly as in equation \eqref{eq:second_iteration_relaxed_constraint_f}, we obtain form Proposition~\ref{prop:unifConv} and the second order Taylor series approximation of $\fclas$ around the point $(\nubar, 0)$ that with high probability,
% \begin{align}
%     \label{eq:f_taylor_approx_onesparse}
%     \frac{1}{n} b^2 \norm{H}_{\infty}^2 
%     \geq 
%     % f ( \nu, \eta ) =
%     \fstar + \frac{1}{2}\feestar b^2 \norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnnstar \deltanu^2 - \constconc - \OOOc
%     % \underbrace{O \left( \frac{1}{ \log (d/n)^{3/2} } \right)}_{\OOOc}
% \end{align}
% with $\OOO_f = O(\deltanu^3 + \eta^3) =  O \left( \frac{1}{\tsoptn^3} \right)$ and $\OOOc = O \left( \frac{1}{\tsoptn^3} \right)$. 
% % \end{proof}

% \paragraph{Upper and lower bound on $\eta$.}
% We proceed in the same manner as in the previous two steps. We relax the constraint in definition of $\Gamma_0$ and define the following set:
% \begin{align}
%     \Gamma_3^{\eta} = \left\{ (\nu, b, \alpha) 
%     \subjto 
%     \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2  -\constconc - \OOOc
%     \andtxts
%     b\alpha \leq \loneboundclas
%     \right\}
% \end{align}
% Clearly, we have again with high probability that $\Gamma_0 \subset \Gamma_3^{\eta}$. The only difference between $\Gamma_3^{\eta}$ and $\Gamma_2^{\eta}$ lies in the constant $\tconsteta$ which is replaced by the tighter constant $\feestar/2$. However, this makes a big difference, as this allows us to choose $\ulm < \soptn <\olm$ much tighter. Similar to Equation~\eqref{eq:l1proofstep2eta2} we again require that $s=\ulm,\olm$ satisfies
% \begin{align}
% \label{eq:l1thirdeta_onesparse}
%     \left( \fstar - \constconc - \OOOc \right) \frac{ \alpha_s^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
%     +
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     > 1.
% \end{align}
% However, this expression allows us to choose $\ulm$ and $\olm$ as in Claims~\ref{claim:approxt_ulalpha_vgw} and \ref{claim:approxt_olalpha_vgw} respectively, with $\kappa = 1/2$. We only show it for $\ulm$ as the same argument holds for $\olm$. Applying Proposition~\ref{prop:concentration_gammas}, the LHS from Equation~\eqref{eq:l1thirdeta_onesparse} can be bounded by

% \begin{align}
%     \left( \fstar - \constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
%     &= \frac{\tsoptn^2}{t_{\ulm}^2}\left(1 -\frac{4}{t_{\ulm}^2}+\frac{2}{\tsoptn^2} + O\left(\frac{1}{\tsoptn^3}\right)\right)  = 1- \frac{\lambda}{\tsoptn^{5/2}} -\frac{2}{\tsoptn^2} + O\left(\frac{1}{\tsoptn^3}\right) + O\left(\frac{1}{\tsoptn^2 \soptn}\right)
%     \\
%     ~~\mathrm{and}\:\: \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } &= 
%     \frac{2}{\tsoptn^2} + \frac{\lambda}{\tsoptn^{5/2}} + \frac{\lambda^2}{2\tsoptn^3} + O \left( \frac{1}{\tsoptn^3} \right) + O \left( \frac{1}{\tsoptn^2 \soptn} \right)
% \end{align}
% with $O(.)$ having hidden dependencies on $\lambda$. In particular, as a result, we see that we can choose $\lambda$ such that Equation~\eqref{eq:l1thirdeta_onesparse} hold for any $d >c n$ with universal constant $c>0$. 
% Hence we can bound $\eta^2$ as follows:
% \begin{align} \label{eq:eta_bound_third_reduction_onesparse}
%     \eta^2 
%     \leq
%     \loneboundclas^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
%     & \leq
%     \frac{ n \fstar }{ \tsoptn^2 } \frac{2}{\ulm}\left( 1 + O\left( \frac{1}{\tsoptn^2} \right) \right)
%     \leq
%     % \frac{4\fstar}{\feestar} \frac{1}{\tsoptn^2}  \exp \left( \frac{\lambda}{2\sqrt{\tsoptn}} \right) \left( 1 + O\left( \frac{1}{\tsoptn^2} \right) \right) \\
%     % & \leq
%     \frac{4\fstar}{\feestar} \frac{1}{\tsoptn^2} \left( 1 + \frac{\lambda}{2\sqrt{\tsoptn}} + O \left( \frac{1}{\tsoptn} \right) \right) %=: B_{\eta,3}^2
% \end{align}
% Furthermore, we also obtain a lower bound for $\eta^2$. Similar as in Lemma~5/6 \cite{wang2021tight}, we can lower bound (using again the monotonicity of $\frac{\norm{\gamma(\alpha)}_2}{\alpha}$ and the fact that any feasible $\alpha \leq \alphaols$)
% \begin{align}
%     \eta^2 &\geq \left[\min_b b^2 \norm{\gamma(\alpha_{\olm})}_2^2 \subjto b^2   
%     \geq \frac{\fstar   -\constconc - \OOOc}{\frac{  \norm{H}_{\infty}^2}{ n } -\frac{1}{2}\feestar  \norm{\gamma(\alpha_{\olm})}_2^2} \right] =\frac{\fstar  -\constconc - \OOOc}{\frac{  \norm{H}_{\infty}^2}{ n } -\frac{1}{2}\feestar  \norm{\gamma(\alpha_{\olm})}_2^2} \norm{\gamma(\alpha_{\olm})}_2^2 \\
%     &\geq  \frac{4\fstar}{\feestar} \frac{1}{\tsoptn^2} \left( 1 - \frac{\lambda}{2\sqrt{\tsoptn}} + O \left( \frac{1}{\tsoptn} \right) \right) 
% \end{align}
% Hence we can conclude the proof. 


\subsubsection*{Bound 3: Proof of the proposition} %($s$-sparse case, loose bounds). }
We already know that $\nu$ concentrates around $\nubar$. However, in order to get a tight expression for the risk and also a valid lower bound, we need to get tighter bounds for $\eta^2$ conditioning on the bounds on $\eta^2,\deltanu^2$ from the previous step,  leading to Proposition~\ref{prop:BoundGamma0_class_noisy}.


% In this part of the proof we use Taylor series approximation of function $f$ up to quadratic terms as shown in equation \eqref{eq:f_taylor_approx}. Using similar arguments as in previous two bounding steps, we obtain Proposition \ref{prop:BoundOmegal1}.
% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}
% \begin{proof}
% Conditioning on the event where the bounds for $\nu,\eta$ from the previous second step hold, we now derive the tight bounds
In this part of the proof we use Taylor series approximation of the function $\fclas$ where we use the result form the last step to bound the  higher order terms involving $\eta$. Similarly as in equation \eqref{eq:second_iteration_relaxed_constraint_f}, we obtain form Proposition~\ref{prop:unifConv} and the second order Taylor series approximation of $\fclas$ around the point $(\nubar, 0, 0)$ that with high probability,
\begin{align}
    \label{eq:f_taylor_approx_ssparse}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 
    \geq 
    % f ( \nu, \eta ) =
    \fstar + \frac{1}{2}\feestar b^2 \norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnnstar \deltanu^2 + \frac{1}{2}\fssstar \norm{\varsigma}_2^2 - \constconc - \otaylor
    % \underbrace{O \left( \frac{1}{ \log (d/n)^{3/2} } \right)}_{\OOOc}
\end{align}
with $\otaylor = O(\deltanu^3 + \eta^3 + \norm{\varsigma}_2^3) =  O \left( \frac{1}{\tsoptn^3} \right)$ and $\constconc = O \left( \frac{1}{\tsoptn^3} \right)$. 
% \end{proof}

\paragraph{Step 3.1: Upper and lower bound on $\eta$.}
We proceed in the same manner as in the previous two steps. We relax the constraint in definition of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_3^{\eta} = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2  -\constconc - \otaylor
    \andtxts
    b\alpha \leq \loneboundclas
    \right\}
\end{align}
Clearly, we have again with high probability that $\Gamma_0 \subset \Gamma_3^{\eta}$. The only difference between $\Gamma_3^{\eta}$ and $\Gamma_2^{\eta}$ lies in the constant $\tconsteta$ which is replaced by the tighter constant $\feestar/2$. However, this makes a big difference, as this allows us to choose $\ulm < \soptn <\olm$ much tighter. Similar to Equation~\eqref{eq:l1proofstep2eta2} we again require that $s=\ulm,\olm$ satisfies
\begin{align}
\label{eq:l1thirdeta_ssparse}
    \left( \fstar - \constconc - \otaylor \right) \frac{ \alpha_s^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
    +
    \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } 
    > 1.
\end{align}
However, this expression allows us to choose $\ulm$ and $\olm$ as in Lemma~\ref{lemma_uls_ols_exp}, with $\kappa = 1/2$ and $m$ instead of $n$. We only show it for $\ulm$ as the same argument holds for $\olm$. Applying Proposition~\ref{prop:concentration_gammas}, the LHS from Equation~\eqref{eq:l1thirdeta_ssparse} can be bounded by

\begin{align}
    \left( \fstar - \constconc - \otaylor \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
    &= \frac{\tsoptn^2}{t_{\ulm}^2}\left(1 -\frac{4}{t_{\ulm}^2}+\frac{2}{\tsoptn^2} + O\left(\frac{1}{\tsoptn^3}\right)\right)  = 1- \frac{\lambda}{\tsoptn^{5/2}} -\frac{2}{\tsoptn^2} + O\left(\frac{1}{\tsoptn^3}\right) + O\left(\frac{1}{\tsoptn^2 \soptn}\right)
    \\
    ~~\mathrm{and}\:\: \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } &= 
    \frac{2}{\tsoptn^2} + \frac{\lambda}{\tsoptn^{5/2}} + \frac{\lambda^2}{2\tsoptn^3} + O \left( \frac{1}{\tsoptn^3} \right) + O \left( \frac{1}{\tsoptn^2 \soptn} \right)
\end{align}
with $O(.)$ having hidden dependencies on $\lambda$. In particular, as a result, we see that we can choose $\lambda$ such that Equation~\eqref{eq:l1thirdeta_ssparse} hold for any $d >c n$ with universal constant $c>0$. 
Hence we can bound $\eta^2$ as follows:
\begin{align} \label{eq:eta_bound_third_reduction_ssparse}
    \eta^2 
    \leq
    \loneboundclas^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
    & \leq
    \frac{ n \fstar }{ \tsoptn^2 } \frac{2}{\ulm}\left( 1 + O\left( \frac{1}{\tsoptn^2} \right) \right)
    \leq
    % \frac{4\fstar}{\feestar} \frac{1}{\tsoptn^2}  \exp \left( \frac{\lambda}{2\sqrt{\tsoptn}} \right) \left( 1 + O\left( \frac{1}{\tsoptn^2} \right) \right) \\
    % & \leq
    \frac{4\fstar}{\feestar} \frac{1}{\tsoptn^2} \left( 1 + \frac{\lambda}{2\sqrt{\tsoptn}} + O \left( \frac{1}{\tsoptn} \right) \right) %=: B_{\eta,3}^2
\end{align}
Furthermore, we also obtain a lower bound for $\eta^2$. Similar as in Lemma~5/6 \cite{wang2021tight}, we can lower bound (using again the monotonicity of $\frac{\norm{\gamma(\alpha)}_2}{\alpha}$ and the fact that any feasible $\alpha \leq \alphaols$)
\begin{align}
    \eta^2 &\geq \left[\min_b b^2 \norm{\gamma(\alpha_{\olm})}_2^2 \subjto b^2   
    \geq \frac{\fstar   -\constconc - \otaylor}{\frac{  \norm{H}_{\infty}^2}{ n } -\frac{1}{2}\feestar  \norm{\gamma(\alpha_{\olm})}_2^2} \right] =\frac{\fstar  -\constconc - \otaylor}{\frac{  \norm{H}_{\infty}^2}{ n } -\frac{1}{2}\feestar  \norm{\gamma(\alpha_{\olm})}_2^2} \norm{\gamma(\alpha_{\olm})}_2^2 \\
    &\geq  \frac{4\fstar}{\feestar} \frac{1}{\tsoptn^2} \left( 1 - \frac{\lambda}{2\sqrt{\tsoptn}} + O \left( \frac{1}{\tsoptn} \right) \right) 
\end{align}
\paragraph{Step 3.2: Upper bound on $\norm{\varsigma}_2$.}
Note that $\fssstar = \feestar$
\begin{align}
    \Gamma_3^{\varsigma} = \left\{ (\nu, b, \alpha, \varsigma) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2 + \frac{1}{2} \fssstar \norm{\varsigma}_2^2 -\constconc - \otaylor
    \andtxts
    b\alpha \leq \loneboundclas
    \right\}
\end{align}
Note that $\Gamma_3^{\varsigma} \subset \Gamma_3^{\eta}$ and thus we can use bounds $\ulm,\olm$ from the previous part. Hence we obtain:
\begin{align}
    \norm{\varsigma}_2^2 &\leq \frac{2}{\fssstar} \left( \frac{\loneboundclas^2}{n} \left( \frac{\norm{H}_{\infty}^2}{\alphauls^2} - \frac{1}{2}\feestar n \frac{\norm{\gamma(\alphaols)}_2^2}{\alphaols^2} \right)  - \fstar + \constconc + \otaylor \right)\\
    &=
    \frac{2\fstar}{\feestar} \left( \frac{1}{\tsoptn^2} \left(1-\frac{2}{\tsoptn^2} + \frac{c_1}{\tsoptn^3} \right) \left( \tulm^2 \left(1+\frac{4}{\tulm^2} + \frac{c_2}{\tulm^4} \right) -  \frac{2m}{\olm} \left( 1+\frac{c_3}{\tolm^2} \right) \right) - 1  + \constconc + \otaylor  \right) 
    \lesssim
    \frac{1}{\tsoptn^{5/2}}
\end{align}
Hence we can conclude the proof. 


==> sections/subsections_theory/noisy/unicon_sketch.tex <==
\subsubsection*{Proof sketch of Uniform Convergence Proposition~\ref{prop:BoundGamma0_class_noisy}}
\label{subsubsec:proof_sketch_unicon_noisy}


\red{TO BE ADDED}

==> sections/subsections_theory/step_CGMT.tex <==
% First, let $X = \{x_i\}_{i=1}^n$ be the matrix of features. We split $X$ and $w$ as follows: let $\matXpar = \{(\xpar)_i\}_{i=1}^n$ and $(\xpar)_i, \wpar$ be the projections of vectors onto $\wgt$ and let \red{define other w's}.

% Now, since $\RiskC(\what) = 2 -2\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$, in order to obtain a valid bounds for $\RiskC(\what)$ it is sufficient to bound $\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$. 

% The proof consists of two major parts: 
% \begin{enumerate}
%     \item \emph{Localization.}
%     We derive a  high-probability upper bound on the norm $\loneboundclasg$, which only depends on $\xi$ and $\matXpar$, of the max-$\ell_1$-margin interpolator $\what$ ,
%     by finding $\loneboundclasg>0$ such that
%     \begin{equation} \label{eq:PhiCN} \tag{$P_{\CCC,N}$}
%         \min_{ \forall i:\:y_i \langle \xui, w \rangle \geq 1}  \norm{w}_1
%         ~ =: \PhiCNuni
%         ~ \leq \loneboundclasg.
%     \end{equation}

%     \item \emph{Uniform convergence.}
%     Conditioning on $\xi$ and $\matXpar$, 
%     we derive high-probability uniform bounds on the classification error for all interpolators $w$ with  $\norm{w}_1 \leq \loneboundclasg$.
%     Namely, we find a high-probability lower and upper bound, respectively, for
%     \begin{align} \label{eq:PhiCm} \tag{$P_{\CCC,-}$} 
%         \PhiCmuni:&=\min_{\substack{
%             % \norm{w}_p^p \leq \gennormbound \\ % CONVENTION 1
%             \norm{w}_1 \leq \loneboundclasg \\ % CONVENTION 2
%              \forall i:\:y_i \langle \xui, w \rangle \geq 1
%         }}  \frac{\langle w, \wgt\rangle}{\norm{w}_2}
%         ,\\
%      \label{eq:PhiCp} \tag{$P_{\CCC,+}$} 
%          \PhiCpuni:&=\max_{\substack{
%             % \norm{w}_p^p \leq \gennormbound \\ % CONVENTION 1
%             \norm{w}_1 \leq \loneboundclasg \\ % CONVENTION 2
%              \forall i:\:y_i \langle \xui, w \rangle \geq 1
%         }} \frac{\langle w, \wgt \rangle}{\norm{w}_2} 
%     \end{align}
%     which in turn then gives us a high probability bounds for the classification error using that $\RiskC(\what) = 2 -2\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$. 
% \end{enumerate}

We begin with the application of the Gaussian comparison, the Gaussian minmax-theorem (GMT) \cite{gordon_1988} and its convex variant the Convex gaussian minmax-theorem (C)GMT \cite{thrampoulidis_2015}. In a second step, we then simplify the corresponding auxiliary optimization problems. 


\paragraph{Preliminary step 1: application of the (C)GMT}
% \subsection{Preliminary Step 1: Simplification via CGMT}
By following a standard argument relying on the Lagrange multiplier, we can bring $\PhiCNuni, \PhiCmuni, \PhiCpuni$ in a suitable form to apply the (C)GMT (see e.g. \cite{deng21} for a similar application). Define the function $\fnclasuni : \RR^{d} \to \RR_+$, 
\ifaistats
\begin{align}
    % \fnclas(\wone,\norm{\wtwo}_2) 
    \fnclasuni(w)=
    \frac{1}{n} \sumin \possq{1-\xi_i\sgn(\langle &(\xpar)_i, \wgtp \rangle) \langle (\xpar)_i, \wpar \rangle \\
    &-\Ggaussian_i \normk{\wperp}_2}
    \label{eq:fnclas_def}
    % &=
    % \frac{1}{n} \sum_{i=1}^n \left( 1 - \xi_i  \innerprod{\wone}{\wgtp} | \innerprod{\wgtp}{x'_i} | -  \innerprod{\woneper}{x'_i} - G_i \norm{\wtwo}_2  \right)_+^2,
\end{align}
\else
\begin{align}\label{eq:fnclas_def}
    % \fnclas(\wone,\norm{\wtwo}_2) 
    \fnclasuni(\wone, \wtwo)
    &=
    \frac{1}{n} \sumin \possq{1-\xi_i\sgn(\langle  \xsui,\wgtp \rangle) \langle \xsui, \wone\rangle -\Ggaussian_i \norm{\wtwo}_2}
    % &=
    % \frac{1}{n} \sum_{i=1}^n \left( 1 - \xi_i  \innerprod{\wone}{\wgtp} | \innerprod{\wgtp}{x'_i} | -  \innerprod{\woneper}{x'_i} - G_i \norm{\wtwo}_2  \right)_+^2,
\end{align}
\fi
with  $\Ggaussian \sim \NNN(0,I_n)$ and $(x)_+ = x\indicator{x\geq 0}$. Simple application of (C)GMT yields:

\begin{proposition}
\label{prop:CGMT_application_classification}
    Assume that $\wgt$ is s-sparse and let $H_1 \sim \NNN(0,I_s), \tH_2 \sim |\NNN(0,I_{d-s})| $. Define the stochastic auxiliary optimization problems 
    % \eqref{eq:phiCdn_CGMT},\eqref{eq:phiCdp_CGMT},\eqref{eq:phiCdm_CGMT} 
    as following:\footnote{We define $\PhiCNuni,\PhiCmuni,\PhiCdnuni,\PhiCdmuni = \infty$ and $\PhiCpuni,\PhiCdpuni = -\infty$ if the corresponding optimization problems have no feasible solution.}
        \ifaistats
        \begin{align}
         % \tag{$A_{\CCC,N}$} \label{eq:phiCdn_CGMT}
            \PhiCdnuni &= \min_{w} \|\wpar+\wperps\|_1+ \|\wperpsc\|_1
            \\
            & \hphantom{{} =   }\subjto \frac{1}{n} (\langle\wperps,H_1\rangle + \langle\wperpsc,\tH_2\rangle)^2 \geq  \fnclasuni(w) \\
        % \tag{$A_{\CCC,+}$} \label{eq:phiCdp_CGMT}
            \PhiCdpuni &= \max_{w} \frac{\langle \wpar, \wgtp \rangle }{\sqrt{\|\wpar\|_2^2+\|\wperps\|_2^2+\|\wperpsc\|_2^2}} 
            \subjto w\in \Gamma \\
        % \tag{$A_{\CCC,-}$}\label{eq:phiCdm_CGMT}
            \PhiCdmuni &= \min_{w} \frac{\langle \wpar, \wgtp \rangle }{\sqrt{\|\wpar\|_2^2+\|\wperps\|_2^2+\|\wperpsc\|_2^2}}
            \subjto w\in\Gamma
        \end{align}
        with 
        \begin{align}
        \Gamma:= \Big\{ w &\subjto \frac{1}{n} (\langle\wperps,H_1\rangle + \langle\wperpsc,\tH_2\rangle)^2 \geq  \fnclasuni(w) \\
        &~~\andtxt~~ \normk{\wpar+\wperps}_1+\normk{\wperpsc}_1 \leq \loneboundclasuni \\
        &~~\andtxt~~ \langle\wperps,H_1\rangle + \langle\wperpsc,\tH_2\rangle  \geq 0
        \Big\}
        \end{align}
        \else
        \begin{align}
         \tag{$A_{\CCC,N}$} \label{eq:phiCdn_CGMT}
            \PhiCdnuni &= \min_{(\wone,\wtwo)} \norm{\wone}_1+\norm{\wtwo}_1
            \subjto \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclasuni(\wone, \wtwo) \\
        \tag{$A_{\CCC,+}$} \label{eq:phiCdp_CGMT}
            \PhiCdpuni &= \max_{(\wone,\wtwo)} \frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}} 
            \subjto \begin{cases}
                \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclasuni(\wone, \wtwo)\\
              \norm{\wone}_1+\norm{\wtwo}_1 \leq \loneboundclasuni
            \end{cases}\\
        \tag{$A_{\CCC,-}$}\label{eq:phiCdm_CGMT}
            \PhiCdmuni &= \min_{(\wone,\wtwo)} \frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}}  
            \subjto \begin{cases}
               \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclasuni(\wone, \wtwo) \\
               \norm{\wone}_1+\norm{\wtwo}_1  \leq \loneboundclasuni
            \end{cases}
        \end{align}
        \fi
    where $\loneboundclasuni>0$ is a constant possibly depending on $\xi$ and $\matXpar$. Then for any $t \in \RR$ we have:
        \begin{align}
            \PP( \PhiCNuni > t \vert \xi, \matXpar) &\leq 2\PP( \PhiCdnuni \geq t \vert \xi, \matXpar)
             \\
            \PP( \PhiCpuni > t \vert \xi, \matXpar) &\leq 2\PP( \PhiCdpuni \geq t \vert \xi, \matXpar) 
             \\
            \PP( \PhiCmuni < t \vert \xi, \matXpar) &\leq 2\PP( \PhiCdmuni \leq t \vert \xi, \matXpar) ,
        \end{align}
        where the probabilities on the LHS and RHS are over the draws of $\matXperp$ and of $\Ggaussian,H_1,\tH_2$, respectively.
\end{proposition}   
Proof of the proposition is deferred to Section~\ref{sub:proof_CGMT_technical}.





\paragraph{Preliminary step 2: simplification of $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$}

% \red{PUT FULL PATH APPROAXH HERE}
\label{subsec:path_param}

\red{Restructure the full section}


As noted in \cite{wang2021tight} for the related min $\ell_1$-norm interpolator (basis pursuit), the relaxation $\|H\|_{\infty} \|w\|_1 \geq \langle w, H\rangle$ in the constraint sets defining $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in Proposition ~\ref{prop:CGMT_application_classification} leads to non-tight bounds. Following the work in \cite{wang2021tight} we can recast the optimization problems defining $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in Proposition~\ref{prop:CGMT_application_classification} as optimization problems in effectively four scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ and $\alpham = (d-s)\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_1}$.  Define the following function $\alpha  \mapsto \gamma(\alpha) \in \RR^{d-s}$ by: \red{go from H to $\tH$ everywhere}
\begin{equation}
\label{eq:def_gamma_alpha}
    \gamma(\alpha) = \argmin_{w} \norm{w}_2^2
    \subjto \begin{cases}
                \innerprodk{w}{\vert H \vert } \geq \normk{H}_{\infty}\\
                w\geq 0\\
                \transp{\onevec} w = \norm{w}_1 = \alpha
            \end{cases}
\end{equation}
\red{change this} We modify the setting from Proposition~\ref{prop:CGMT_application_classification} by proving the result assuming that $\wgt, x_i \in \RR^{d+s}$, which implies that  $H \in \RR^{d}$. This modification does not affect the expression for the bounds in Theorems~\ref{thm:mainl1_class_noisy},\ref{thm:mainl1_class_noiseless}.

Define $\nu:= \innerprod{\wpar}{\wgtp}$, $\etasc := \normk{\wperpsc}_2$, $\etas := \normk{\wperps}_2$ and $\eta :=\normk{\wperp}_2 = \sqrt{\etasc^2+\etas^2}$. With slight abuse of notation, we can rewrite function $\fnclasg$ as follows:
\begin{align}\label{eq:fnclas_def_noisy_par}
     \fnclasg(\nu,\eta) = \frac{1}{n} \sum_{i=1}^n ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta )_+^2
\end{align}
for $\gausswone,\gausswtwo \sim \NNN(0,1)$. 
Now we can reduce Proposition~\ref{prop:CGMT_application_classification} to the following proposition with optimization over the proposed path:

\begin{proposition}
\label{prop:parametrization_class_general}
% The optimization problems $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in
% Proposition~\ref{prop:CGMT_application_classification} are given by optimization problems \eqref{eq:phiCdn_par_uni}, \eqref{eq:phiCdp_par_uni}, \eqref{eq:phiCdm_par_uni} respectively, defined by:
Let $H\sim \NNN(0,I_{d-s})$, $\smax= \Theta(n^{2/3(1-7p)})$ in the noiseless, and $\smax = \Theta(n/\log^{3/2}(d/n))$ in the noisy setting. Then for any $s$-sparse $\wgt$ with $s\leq \smax$ the optimization problems $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in
Proposition~\ref{prop:CGMT_application_classification} satisfy the following:
    \ifaistats
    \begin{align}
        % \tag{$A_{\CCC,N}'$}\label{eq:phiCdn_par_uni}
            &\PhiCdnuni \leq 
            \Big[ \min_{\nu, b, \alpha, \etas} \vert \nu \vert \|\wgtp\|_1 + \sqrt{s}\etas + b \norm{\gamma(\alpha)}_1 \subjto\\
            &\frac{1}{n}  (2\sqrt{\smax}\etas + b\normk{H}_{\infty})^2  \geq  \fnclasg(\nu, \sqrt{b^2\|\gamma(\alpha)\|_2^2+\etas^2} ) \Big]\\
        % \tag{$A_{\CCC,+}'$} \label{eq:phiCdp_par_uni}
            &\PhiCdpuni   \leq \max_{(\nu, b, \alpha, \etas) \in \setZeroUni}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \etas^2}}
            % \subjto 
            % (\nu, b, \alpha, \etas) \in \setZeroUni
            \\
        % \tag{$A_{\CCC,-}'$} \label{eq:phiCdm_par_uni}
            &\PhiCdmuni   \geq \min_{(\nu, b, \alpha, \etas) \in \setZeroUni} \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \etas^2}}
            % \subjto
            % (\nu, b, \alpha, \etas) \in \setZeroUni
    \end{align}
    \else
    \begin{align}
        \tag{$A_{\CCC,N}'$}\label{eq:phiCdn_par_uni}
            \PhiCdnuni &\leq \min_{\nu, b, \alpha, \etas} \vert \nu \vert \|\wgtp\|_1 + \norm{\etas}_1 +  b \norm{\gamma(\alpha)}_1 
            \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu, b\|\gamma(\alpha)\|_2, \etas ).
            \\
        \tag{$A_{\CCC,+}'$} \label{eq:phiCdp_par_uni}
            \PhiCdpuni &\leq \max_{\nu, b, \alpha, \etas}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\etas}_2^2}}
            \subjto 
            (\nu, b, \alpha, \etas) \in \setZeroUni
            \\
        \tag{$A_{\CCC,-}'$} \label{eq:phiCdm_par_uni}
            \PhiCdmuni &\geq \min_{\nu, b, \alpha, \etas} \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\etas}_2^2}}
            \subjto
            (\nu, b, \alpha, \etas) \in \setZeroUni
    \end{align}
    \fi
with probability at least $1-2\exp(-c_1 \smax)$, for some scalars $\nu, b,\etas>0, \alpha\in[1,\alpham]$ and set $\setZeroUni$ is a set of all $(\nu, b, \alpha, \etas)$ that satisfy:
\ifaistats
\begin{gather}
    % &\setZeroUni 
    % =
    % \Big\{ (\nu, b, \alpha, \etas) 
    % \subjto
    \frac{1}{n}  (2\sqrt{\smax}\etas + b\normk{H}_{\infty})^2  \geq  \fnclasg(\nu,\sqrt{b^2\|\gamma(\alpha)\|_2^2+\etas^2}) 
    \\
    % ~~\andtxt~~ 
    % \max\left\{ |\nu| \|\wgtp\|_1 - \sqrt{s}\etas , \etas- |\nu| \|\wgtp\|_1 \right\} 
    \max\left\{ |\nu| \|\wgtp\|_1 - \sqrt{s}\etas , 0 \right\} 
    + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasg 
    % \Big\}.
    \label{eq:Gamma0_def_class_uni}
\end{gather}
% \begin{align}
%     \setZeroUni 
%     =
%     \Big\{ (\nu, b, \alpha, \etas) 
%     &\subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu,b\|\gamma(\alpha)\|_2, \etas) 
%     \\
%     &~~\andtxt~~ \Big| |\nu| \|\wgtp\|_1 - \norm{\etas}_1 \Big| + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasg \Big\}.
%     \label{eq:Gamma0_def_class_uni}
% \end{align}
\else
\begin{align}
    \setZeroUni = \left\{ (\nu, b, \alpha, \etas) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu,b\|\gamma(\alpha)\|_2, \etas) ~~\andtxt~~  |\|\wgtp\|_1 - \norm{\etas}_1 | + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasg \right\}.
    \label{eq:Gamma0_def_class_uni}
\end{align}
\fi
\end{proposition} 
\begin{proof}
Since $\normk{\wgtp}_2=1$ we have that $\|\wpar\|_2 = | \innerprod{\wpar}{\wgtp} | = |\nu|$ and $\|\wpar\|_1 = |\innerprod{\wpar}{\wgtp}| \normk{\wgt}_1 = |\nu| \normk{\wgtp}_1$. Furthermore, note that $\normk{\wperps}_1 \leq \sqrt{s} \normk{\wperps}_2 = \sqrt{s}\etas$. According to triangle inequality holds that $\normk{\wpar}_1+\normk{\wperps}_1 \geq \normk{\wpar+\wperps}_1 \geq | \normk{\wpar}_1 - \normk{\wperps}_1|$. 

The proof of the proposition follows straightforwardly after substituting $b\gamma(\alpha)$ for $\wperpsc$ and using observations we made above.
\end{proof}
% Following exactly the same arguments as in Lemma 1 in \cite{wang2021tight} we obtain: 

% \begin{proposition}
% % \begin{proposition} 
% \label{prop:parametrization_class_noisy}
% The optimization problems $\PhiCdn,\PhiCdp$ and $\PhiCdm$ in
% Proposition~\ref{prop:CGMT_application_classification} are given by optimization problems \eqref{eq:phiCdn_par}, \eqref{eq:phiCdp_par}, \eqref{eq:phiCdm_par} respectively, defined by:
%     \begin{align}
%         \tag{$A_{\CCC_\sigma,N}'$}\label{eq:phiCdn_par}
%             \PhiCdn &\leq \min_{\nu, b, \alpha, \etas} \vert \nu \vert \sqrt{s}  + b \norm{\gamma(\alpha)}_1 + \norm{\etas}_1
%             \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu, b\|\gamma(\alpha)\|_2, \etas ).
%             \\
%         \tag{$A_{\CCC_\sigma,+}'$} \label{eq:phiCdp_par}
%             \PhiCdp &= \max_{\nu, b, \alpha, \etas}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\etas}_2^2}}
%             \subjto 
%             (\nu, b, \alpha, \etas) \in \setNoisyZero
%             \\
%         \tag{$A_{\CCC_\sigma,-}'$} \label{eq:phiCdm_par}
%             % \PhiCdm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             % \subjto \begin{cases}
%             %   \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\wone,b\|\gamma(\alpha)\|_2)\\
%             %     \nu+b \leq \loneboundclas
%             % \end{cases}
%             \PhiCdm &= \min_{\nu, b, \alpha, \etas} \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\etas}_2^2}}
%             \subjto
%             (\nu, b, \alpha, \etas) \in \setNoisyZero
%     \end{align}
% for some scalars $\nu, b>0, \alpha\in[1,\alpham]$ and set $\setNoisyZero$ given by:
% % \begin{align}
% %     \Gamma_0 = \left\{ (\nu, b, \alpha, \etas) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2, \etas) ~~\andtxt~~  \nu \sqrt{s} + b\norm{\gamma(\alpha)}_1 - \norm{\etas}_1 \leq \loneboundclas \right\}.
% %     \label{eq:Gamma0_def_class_noisy}
% % \end{align}
% % \end{proposition}  
% % Note that in the proposition we make use of the triangle inequalities $\norm{\wone}_1 \leq \norm{\woneper}_1 + \norm{\wonepar}_1$ and $\norm{\wone}_1 \geq | \norm{\wonepar}_1 - \norm{\woneper}_1|$.
% \begin{align}
%     \setNoisyZero = \left\{ (\nu, b, \alpha, \etas) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2, \etas) ~~\andtxt~~  b\norm{\gamma(\alpha)}_1 \leq \loneboundclas \right\}.
%     \label{eq:Gamma0_def_class_noisy}
% \end{align}
% \end{proposition}  
% Note that in the proposition we make use of the triangle inequality $\norm{\wone}_1 \leq \norm{\woneper}_1 + \norm{\wonepar}_1$ and $\norm{\wtwo}_1 \leq \norm{\wone}_1 + \norm{\wtwo}_1 \leq \loneboundclas$.





==> sections/subsections_theory/step_CGMT_old_.tex <==
First, let $X = \{x\}_{i=1}^n$ be the matrix of features. We split $X$ and $w$ as follows: let $\Xs = \{\xsui\}_{i=1}^n$ and $\xsui, \wone$ be the vectors containing the support of $\wgt$ and let $\wtwo$ contain the other entries.

Now, since $\RiskC(\what) = 2 -2\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$, in order to obtain a valid bounds for $\RiskC(\what)$ it is sufficient to bound $\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$. 

The proof consists of two major parts: 

\begin{enumerate}
    \item \emph{Localization.}
    We derive a  high-probability upper bound on the norm $\loneboundclasg$, which only depends on $\xi$ and $\Xs$, of the max-$\ell_1$-margin interpolator $\what$ ,
    by finding $\loneboundclasg>0$ such that
    \begin{equation} \label{eq:PhiCN} \tag{$P_{\CCC,N}$}
        \min_{ \forall i:\:y_i \langle \xui, w \rangle \geq 1}  \norm{w}_1
        ~ =: \PhiCNuni
        ~ \leq \loneboundclasg.
    \end{equation}

    \item \emph{Uniform convergence.}
    Conditioning on $\xi$ and $\Xs$, 
    we derive high-probability uniform bounds on the classification error for all interpolators $w$ with  $\norm{w}_1 \leq \loneboundclasg$.
    Namely, we find a high-probability lower and upper bound, respectively, for
    \begin{align} \label{eq:PhiCm} \tag{$P_{\CCC,-}$} 
        \PhiCmuni:&=\min_{\substack{
            % \norm{w}_p^p \leq \gennormbound \\ % CONVENTION 1
            \norm{w}_1 \leq \loneboundclasg \\ % CONVENTION 2
             \forall i:\:y_i \langle \xui, w \rangle \geq 1
        }}  \frac{\langle w, \wgt\rangle}{\norm{w}_2}
        ,\\
     \label{eq:PhiCp} \tag{$P_{\CCC,+}$} 
         \PhiCpuni:&=\max_{\substack{
            % \norm{w}_p^p \leq \gennormbound \\ % CONVENTION 1
            \norm{w}_1 \leq \loneboundclasg \\ % CONVENTION 2
             \forall i:\:y_i \langle \xui, w \rangle \geq 1
        }} \frac{\langle w, \wgt \rangle}{\norm{w}_2} 
    \end{align}
    which in turn then gives us a high probability bounds for the classification error using that $\RiskC(\what) = 2 -2\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$. 
\end{enumerate}


\paragraph{Preliminary step 1: application of the (C)GMT}
% \subsection{Preliminary Step 1: Simplification via CGMT}
By following a standard argument relying on the Lagrange multiplier, we can bring \eqref{eq:PhiCN}, \eqref{eq:PhiCm},\eqref{eq:PhiCp} in a suitable form to apply the (C)GMT (see e.g. \cite{deng21} for a similar application). Define the function $\fnclasuni : \RR^{s}\times\RR^{d-s} \to \RR_+$, 
\ifaistats
\begin{align}
    % \fnclas(\wone,\norm{\wtwo}_2) 
    \fnclasuni(\wone, \wtwo)=
    \frac{1}{n} \sumin (1-\xi_i\sgn(\langle  &\xsui,\wgtp \rangle) \langle \xsui, \wone\rangle 
    \\
    &-\Ggaussian_i \norm{\wtwo}_2)_+^2
    \label{eq:fnclas_def}
    % &=
    % \frac{1}{n} \sum_{i=1}^n \left( 1 - \xi_i  \innerprod{\wone}{\wgtp} | \innerprod{\wgtp}{x'_i} | -  \innerprod{\woneper}{x'_i} - G_i \norm{\wtwo}_2  \right)_+^2,
\end{align}
\else
\begin{align}\label{eq:fnclas_def}
    % \fnclas(\wone,\norm{\wtwo}_2) 
    \fnclasuni(\wone, \wtwo)
    &=
    \frac{1}{n} \sumin \possq{1-\xi_i\sgn(\langle  \xsui,\wgtp \rangle) \langle \xsui, \wone\rangle -\Ggaussian_i \norm{\wtwo}_2}
    % &=
    % \frac{1}{n} \sum_{i=1}^n \left( 1 - \xi_i  \innerprod{\wone}{\wgtp} | \innerprod{\wgtp}{x'_i} | -  \innerprod{\woneper}{x'_i} - G_i \norm{\wtwo}_2  \right)_+^2,
\end{align}
\fi
with  $\Ggaussian \sim \NNN(0,I_n)$. Simple application of (C)GMT yields:

\begin{proposition}
\label{prop:CGMT_application_classification}
    Assume that $\wgt$ is s-sparse and let $\Hgaussian \sim \NNN(0,I_{d-s})$. Define the stochastic auxiliary optimization problems 
    % \eqref{eq:phiCdn_CGMT},\eqref{eq:phiCdp_CGMT},\eqref{eq:phiCdm_CGMT} 
    as following:\footnote{We define $\PhiCNuni,\PhiCmuni,\PhiCdnuni,\PhiCdmuni = \infty$ and $\PhiCpuni,\PhiCdpuni = -\infty$ if the corresponding optimization problems have no feasible solution.}
        \ifaistats
        \begin{align}
         % \tag{$A_{\CCC,N}$} \label{eq:phiCdn_CGMT}
            \PhiCdnuni &= \min_{(\wone,\wtwo)} \norm{\wone}_1+ \norm{\wtwo}_1
            \\
            & \hphantom{{} = \min_{(\wone,\wtwo)} \norm{\wone}_1+ }\subjto \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclasuni(\wone, \wtwo) \\
        % \tag{$A_{\CCC,+}$} \label{eq:phiCdp_CGMT}
            \PhiCdpuni &= \max_{(\wone,\wtwo)} \frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}} 
            \subjto w\in \Gamma \\
        % \tag{$A_{\CCC,-}$}\label{eq:phiCdm_CGMT}
            \PhiCdmuni &= \min_{(\wone,\wtwo)} \frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}}  
            \subjto w\in\Gamma
        \end{align}
        with 
        \begin{align}
        \Gamma:= \Big\{ (\wone,\wtwo) &\subjto \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclasuni(\wone, \wtwo) \\
        &~~\andtxt~~ \norm{\wone}_1+\norm{\wtwo}_1 \leq \loneboundclasuni \Big\}
        \end{align}
        \else
        \begin{align}
         \tag{$A_{\CCC,N}$} \label{eq:phiCdn_CGMT}
            \PhiCdnuni &= \min_{(\wone,\wtwo)} \norm{\wone}_1+\norm{\wtwo}_1
            \subjto \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclasuni(\wone, \wtwo) \\
        \tag{$A_{\CCC,+}$} \label{eq:phiCdp_CGMT}
            \PhiCdpuni &= \max_{(\wone,\wtwo)} \frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}} 
            \subjto \begin{cases}
                \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclasuni(\wone, \wtwo)\\
              \norm{\wone}_1+\norm{\wtwo}_1 \leq \loneboundclasuni
            \end{cases}\\
        \tag{$A_{\CCC,-}$}\label{eq:phiCdm_CGMT}
            \PhiCdmuni &= \min_{(\wone,\wtwo)} \frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}}  
            \subjto \begin{cases}
               \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclasuni(\wone, \wtwo) \\
               \norm{\wone}_1+\norm{\wtwo}_1  \leq \loneboundclasuni
            \end{cases}
        \end{align}
        \fi
    where $\loneboundclasuni>0$ is a constant possibly depending on $\xi$ and $\Xs$. Then for any $t \in \RR$ we have:
        \begin{align}
            \PP( \PhiCNuni > t \vert \xi, \Xs) &\leq 2\PP( \PhiCdnuni \geq t \vert \xi, \Xs)
             \\
            \PP( \PhiCpuni > t \vert \xi, \Xs) &\leq 2\PP( \PhiCdpuni \geq t \vert \xi, \Xs) 
             \\
            \PP( \PhiCmuni < t \vert \xi, \Xs) &\leq 2\PP( \PhiCdmuni \leq t \vert \xi, \Xs) ,
        \end{align}
        where the probabilities on the LHS and RHS are over the draws of $X''$ and of $\Ggaussian,\Hgaussian$, respectively.
\end{proposition}   
Proof of the proposition is deferred to Section~\ref{sub:proof_CGMT_technical}.





\paragraph{Preliminary Step 2: simplification of $\PhiCmuni,\PhiCpuni,\PhiCmuni$}
% \red{PUT FULL PATH APPROAXH HERE}
\label{subsec:path_param}


As noted in \cite{wang2021tight} for the related min $\ell_1$-norm interpolator (basis pursuit), the relaxation $\|H\|_{\infty} \|w\|_1 \geq \langle w, H\rangle$ in the constraint sets defining $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in Proposition ~\ref{prop:CGMT_application_classification} leads to non-tight bounds. Following the work in \cite{wang2021tight} we can recast the optimization problems defining $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in Proposition~\ref{prop:CGMT_application_classification} as optimization problems in effectively four scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ and $\alpham = d\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_1}$.  Define the following function $\alpha  \mapsto \gamma(\alpha) \in \RR^{d}$ by:
\begin{equation}
\label{eq:def_gamma_alpha}
    \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
    \subjto \begin{cases}
                \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
                \wtwo\geq 0\\
                \transp{\onevec} \wtwo = \norm{\wtwo}_1 = \alpha
            \end{cases}
\end{equation}
We modify the setting from Proposition~\ref{prop:CGMT_application_classification} by proving the result assuming that $\wgt, x_i \in \RR^{d+s}$, which implies that  $H \in \RR^{d}$. This modification does not affect the expression for the bounds in Theorems~\ref{thm:mainl1_class_noisy},\ref{thm:mainl1_class_noiseless}.

Define $\nu:= \innerprod{\wone}{\wgtp}$, $\eta := \norm{\wtwo}_2$, and let $\varsigma \in \RR^{s-1}$ be the last $s-1$ entries of $O\woneper$ with orthogonal matrix $O$ mapping $\wgt$ into standard unit vector $e_1$. With slight abuse of notation, we can rewrite function $\fnclasg$ as follows:
\begin{align}\label{eq:fnclas_def_noisy_par}
     \fnclasg(\nu,\eta,\varsigma) = \frac{1}{n} \sum_{i=1}^n ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )_+^2
\end{align}
for $z_i^{(j)} \sim \NNN(0,1)$ for $i=1,\dots,m$, $j=0,\dots,s$. 
Now we can reduce Proposition~\ref{prop:CGMT_application_classification} to the following proposition with optimization over the proposed path:

\begin{proposition}
\label{prop:parametrization_class_general}
% The optimization problems $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in
% Proposition~\ref{prop:CGMT_application_classification} are given by optimization problems \eqref{eq:phiCdn_par_uni}, \eqref{eq:phiCdp_par_uni}, \eqref{eq:phiCdm_par_uni} respectively, defined by:
The optimization problems $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in
Proposition~\ref{prop:CGMT_application_classification} satisfy the following:
    \ifaistats
    \begin{align}
        % \tag{$A_{\CCC,N}'$}\label{eq:phiCdn_par_uni}
            \PhiCdnuni &\leq 
            \min_{\nu, b, \alpha, \varsigma} \vert \nu \vert \|\wgtp\|_1 + \sqrt{s}\norm{\varsigma}_2 + b \norm{\gamma(\alpha)}_1 \\
            & \hphantom{{} \leq 
            \min_{\nu, b, \alpha, \varsigma} \vert \nu \vert \|\wgtp\|_1 +} \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu, b\|\gamma(\alpha)\|_2, \varsigma )\\
        % \tag{$A_{\CCC,+}'$} \label{eq:phiCdp_par_uni}
            \PhiCdpuni &  \leq \max_{\nu, b, \alpha, \varsigma}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
            \subjto 
            (\nu, b, \alpha, \varsigma) \in \setZeroUni
            \\
        % \tag{$A_{\CCC,-}'$} \label{eq:phiCdm_par_uni}
            \PhiCdmuni &  \geq \min_{\nu, b, \alpha, \varsigma} \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
            \subjto
            (\nu, b, \alpha, \varsigma) \in \setZeroUni
    \end{align}
    \else
    \begin{align}
        \tag{$A_{\CCC,N}'$}\label{eq:phiCdn_par_uni}
            \PhiCdnuni &\leq \min_{\nu, b, \alpha, \varsigma} \vert \nu \vert \|\wgtp\|_1 + \norm{\varsigma}_1 +  b \norm{\gamma(\alpha)}_1 
            \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu, b\|\gamma(\alpha)\|_2, \varsigma ).
            \\
        \tag{$A_{\CCC,+}'$} \label{eq:phiCdp_par_uni}
            \PhiCdpuni &\leq \max_{\nu, b, \alpha, \varsigma}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
            \subjto 
            (\nu, b, \alpha, \varsigma) \in \setZeroUni
            \\
        \tag{$A_{\CCC,-}'$} \label{eq:phiCdm_par_uni}
            \PhiCdmuni &\geq \min_{\nu, b, \alpha, \varsigma} \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
            \subjto
            (\nu, b, \alpha, \varsigma) \in \setZeroUni
    \end{align}
    \fi
for some scalars $\nu, b>0, \alpha\in[1,\alpham]$ and set $\setZeroUni$ given by:
\ifaistats
\begin{align}
    \setZeroUni 
    =
    \Big\{ &(\nu, b, \alpha, \varsigma) 
    \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu,b\|\gamma(\alpha)\|_2, \varsigma) 
    \\
    &~~\andtxt~~ \max\left\{ |\nu| \|\wgtp\|_1 - \sqrt{s}\norm{\varsigma}_2 , 0\right\} + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasg \Big\}.
    \label{eq:Gamma0_def_class_uni}
\end{align}
% \begin{align}
%     \setZeroUni 
%     =
%     \Big\{ (\nu, b, \alpha, \varsigma) 
%     &\subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu,b\|\gamma(\alpha)\|_2, \varsigma) 
%     \\
%     &~~\andtxt~~ \Big| |\nu| \|\wgtp\|_1 - \norm{\varsigma}_1 \Big| + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasg \Big\}.
%     \label{eq:Gamma0_def_class_uni}
% \end{align}
\else
\begin{align}
    \setZeroUni = \left\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu,b\|\gamma(\alpha)\|_2, \varsigma) ~~\andtxt~~  |\|\wgtp\|_1 - \norm{\varsigma}_1 | + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasg \right\}.
    \label{eq:Gamma0_def_class_uni}
\end{align}
\fi
\end{proposition} 
\begin{proof}
Since $\norm{\wgtp}_2=1$ we have that $\|\wonepar\|_2 = | \innerprod{\wone}{\wgtp} | = |\nu|$ and $\|\wonepar\|_1 = |\innerprod{\wone}{\wgtp}| \norm{\wgt}_1 = |\nu| \norm{\wgtp}_1$. Furthermore, note that $\norm{\woneper}_1 \leq \sqrt{s} \norm{\woneper}_2 = \sqrt{s}\norm{\varsigma}_2$. According to triangle inequality holds that $\norm{\woneper}_1+\norm{\wonepar}_1 \geq \norm{\wone}_1 \geq | \norm{\wonepar}_1 - \norm{\woneper}_1|$. 

The proof of the proposition follows straightforwardly after substituting $b\gamma(\alpha)$ for $\wtwo$ and using observations we made above.
\end{proof}
% Following exactly the same arguments as in Lemma 1 in \cite{wang2021tight} we obtain: 

% \begin{proposition}
% % \begin{proposition} 
% \label{prop:parametrization_class_noisy}
% The optimization problems $\PhiCdn,\PhiCdp$ and $\PhiCdm$ in
% Proposition~\ref{prop:CGMT_application_classification} are given by optimization problems \eqref{eq:phiCdn_par}, \eqref{eq:phiCdp_par}, \eqref{eq:phiCdm_par} respectively, defined by:
%     \begin{align}
%         \tag{$A_{\CCC_\sigma,N}'$}\label{eq:phiCdn_par}
%             \PhiCdn &\leq \min_{\nu, b, \alpha, \varsigma} \vert \nu \vert \sqrt{s}  + b \norm{\gamma(\alpha)}_1 + \norm{\varsigma}_1
%             \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu, b\|\gamma(\alpha)\|_2, \varsigma ).
%             \\
%         \tag{$A_{\CCC_\sigma,+}'$} \label{eq:phiCdp_par}
%             \PhiCdp &= \max_{\nu, b, \alpha, \varsigma}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
%             \subjto 
%             (\nu, b, \alpha, \varsigma) \in \setNoisyZero
%             \\
%         \tag{$A_{\CCC_\sigma,-}'$} \label{eq:phiCdm_par}
%             % \PhiCdm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             % \subjto \begin{cases}
%             %   \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\wone,b\|\gamma(\alpha)\|_2)\\
%             %     \nu+b \leq \loneboundclas
%             % \end{cases}
%             \PhiCdm &= \min_{\nu, b, \alpha, \varsigma} \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
%             \subjto
%             (\nu, b, \alpha, \varsigma) \in \setNoisyZero
%     \end{align}
% for some scalars $\nu, b>0, \alpha\in[1,\alpham]$ and set $\setNoisyZero$ given by:
% % \begin{align}
% %     \Gamma_0 = \left\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2, \varsigma) ~~\andtxt~~  \nu \sqrt{s} + b\norm{\gamma(\alpha)}_1 - \norm{\varsigma}_1 \leq \loneboundclas \right\}.
% %     \label{eq:Gamma0_def_class_noisy}
% % \end{align}
% % \end{proposition}  
% % Note that in the proposition we make use of the triangle inequalities $\norm{\wone}_1 \leq \norm{\woneper}_1 + \norm{\wonepar}_1$ and $\norm{\wone}_1 \geq | \norm{\wonepar}_1 - \norm{\woneper}_1|$.
% \begin{align}
%     \setNoisyZero = \left\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2, \varsigma) ~~\andtxt~~  b\norm{\gamma(\alpha)}_1 \leq \loneboundclas \right\}.
%     \label{eq:Gamma0_def_class_noisy}
% \end{align}
% \end{proposition}  
% Note that in the proposition we make use of the triangle inequality $\norm{\wone}_1 \leq \norm{\woneper}_1 + \norm{\wonepar}_1$ and $\norm{\wtwo}_1 \leq \norm{\wone}_1 + \norm{\wtwo}_1 \leq \loneboundclas$.





==> sections/subsections_theory/step_path.tex <==

\paragraph{Step 1: Simplification to a low dimensional optimization problem}
% \red{PUT FULL PATH APPROAXH HERE}
\label{subsec:path_param}


As noted in \cite{wang2021tight} for the related min $\ell_1$-norm interpolator (basis pursuit), the relaxation $\|H\|_{\infty} \|w\|_1 \geq \langle w, H\rangle$ in the constraint sets defining $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in Proposition ~\ref{prop:CGMT_application_classification} leads to non-tight bounds. Following the work in \cite{wang2021tight} we can recast the optimization problems defining $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in Proposition~\ref{prop:CGMT_application_classification} as optimization problems in five scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ and $\alpham = d\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_1}$.  We define the parametric path $\alpha  \mapsto \gamma(\alpha) \in \RR^{d}$ by:
\begin{equation}
\label{eq:def_gamma_alpha}
    \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
    \subjto \begin{cases}
                \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
                \wtwo\geq 0\\
                \transp{\onevec} \wtwo = \norm{\wtwo}_1 = \alpha
            \end{cases}
\end{equation}
We modify the setting from Proposition~\ref{prop:CGMT_application_classification} by proving the result assuming that $\wgt, x_i \in \RR^{d+s}$, which implies that  $H \in \RR^{d}$. This modification does not affect the expression for the bounds in Theorems~\ref{thm:mainl1_class_noisy},\ref{thm:mainl1_class_noiseless}.

Define $\nu:= \innerprod{\wone}{\wgtp}$, $\eta := \norm{\wtwo}_2$, $\varsigma: = \woneper \in \RR^{s-1}$. With slight abuse of notation, we can rewrite function $\fnclasg$ as follows:
\begin{align}\label{eq:fnclas_def_noisy_par}
     \fnclasg(\nu,\eta,\varsigma) = \frac{1}{n} \sum_{i=1}^n ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )_+^2
\end{align}
for $z_i^{(j)} \sim \NNN(0,1)$ for $i=1,\dots,m$, $j=0,\dots,s$. Since $\norm{\wgtp}_2=1$ we have that $\|\wonepar\|_2 = | \innerprod{\wone}{\wgtp} | = |\nu|$ and $\|\wonepar\|_1 = |\innerprod{\wone}{\wgtp}| \norm{\wgt}_1 = |\nu| \norm{\wgtp}_1$. Now we can reduce Proposition~\ref{prop:CGMT_application_classification} to the following proposition with optimization over the proposed path:

\begin{proposition}
\label{prop:parametrization_class_general}
% The optimization problems $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in
% Proposition~\ref{prop:CGMT_application_classification} are given by optimization problems \eqref{eq:phiCdn_par_uni}, \eqref{eq:phiCdp_par_uni}, \eqref{eq:phiCdm_par_uni} respectively, defined by:
The optimization problems $\PhiCdnuni,\PhiCdpuni$ and $\PhiCdmuni$ in
Proposition~\ref{prop:CGMT_application_classification} satisfy the following:
    \ifaistats
    \begin{align}
        % \tag{$A_{\CCC,N}'$}\label{eq:phiCdn_par_uni}
            \PhiCdnuni \leq 
            \min_{\nu, b, \alpha, \varsigma} \vert \nu \vert \|\wgtp\|_1 &+ \norm{\varsigma}_1 + b \norm{\gamma(\alpha)}_1 \\
            &\subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu, b\|\gamma(\alpha)\|_2, \varsigma )
    \end{align}
    \begin{align}
        % \tag{$A_{\CCC,+}'$} \label{eq:phiCdp_par_uni}
            \PhiCdpuni &  \leq \max_{\nu, b, \alpha, \varsigma}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
            \subjto 
            (\nu, b, \alpha, \varsigma) \in \setZeroUni
            \\
        % \tag{$A_{\CCC,-}'$} \label{eq:phiCdm_par_uni}
            \PhiCdmuni &  \geq \min_{\nu, b, \alpha, \varsigma} \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
            \subjto
            (\nu, b, \alpha, \varsigma) \in \setZeroUni
    \end{align}
    \else
    \begin{align}
        \tag{$A_{\CCC,N}'$}\label{eq:phiCdn_par_uni}
            \PhiCdnuni &\leq \min_{\nu, b, \alpha, \varsigma} \vert \nu \vert \|\wgtp\|_1 + \norm{\varsigma}_1 +  b \norm{\gamma(\alpha)}_1 
            \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu, b\|\gamma(\alpha)\|_2, \varsigma ).
            \\
        \tag{$A_{\CCC,+}'$} \label{eq:phiCdp_par_uni}
            \PhiCdpuni &\leq \max_{\nu, b, \alpha, \varsigma}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
            \subjto 
            (\nu, b, \alpha, \varsigma) \in \setZeroUni
            \\
        \tag{$A_{\CCC,-}'$} \label{eq:phiCdm_par_uni}
            \PhiCdmuni &\geq \min_{\nu, b, \alpha, \varsigma} \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
            \subjto
            (\nu, b, \alpha, \varsigma) \in \setZeroUni
    \end{align}
    \fi
for some scalars $\nu, b>0, \alpha\in[1,\alpham]$ and set $\setZeroUni$ given by:
\ifaistats
\begin{align}
    \setZeroUni 
    =
    \Big\{ (\nu, b, \alpha, \varsigma) 
    &\subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu,b\|\gamma(\alpha)\|_2, \varsigma) 
    \\
    &~~\andtxt~~ \Big|\|\wgtp\|_1 - \norm{\varsigma}_1 \Big| + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasg \Big\}.
    \label{eq:Gamma0_def_class_uni}
\end{align}
\else
\begin{align}
    \setZeroUni = \left\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclasg(\nu,b\|\gamma(\alpha)\|_2, \varsigma) ~~\andtxt~~  |\|\wgtp\|_1 - \norm{\varsigma}_1 | + b\norm{\gamma(\alpha)}_1 \leq \loneboundclasg \right\}.
    \label{eq:Gamma0_def_class_uni}
\end{align}
\fi
\end{proposition}  

% Following exactly the same arguments as in Lemma 1 in \cite{wang2021tight} we obtain: 

% \begin{proposition}
% % \begin{proposition} 
% \label{prop:parametrization_class_noisy}
% The optimization problems $\PhiCdn,\PhiCdp$ and $\PhiCdm$ in
% Proposition~\ref{prop:CGMT_application_classification} are given by optimization problems \eqref{eq:phiCdn_par}, \eqref{eq:phiCdp_par}, \eqref{eq:phiCdm_par} respectively, defined by:
%     \begin{align}
%         \tag{$A_{\CCC_\sigma,N}'$}\label{eq:phiCdn_par}
%             \PhiCdn &\leq \min_{\nu, b, \alpha, \varsigma} \vert \nu \vert \sqrt{s}  + b \norm{\gamma(\alpha)}_1 + \norm{\varsigma}_1
%             \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu, b\|\gamma(\alpha)\|_2, \varsigma ).
%             \\
%         \tag{$A_{\CCC_\sigma,+}'$} \label{eq:phiCdp_par}
%             \PhiCdp &= \max_{\nu, b, \alpha, \varsigma}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
%             \subjto 
%             (\nu, b, \alpha, \varsigma) \in \setNoisyZero
%             \\
%         \tag{$A_{\CCC_\sigma,-}'$} \label{eq:phiCdm_par}
%             % \PhiCdm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             % \subjto \begin{cases}
%             %   \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\wone,b\|\gamma(\alpha)\|_2)\\
%             %     \nu+b \leq \loneboundclas
%             % \end{cases}
%             \PhiCdm &= \min_{\nu, b, \alpha, \varsigma} \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2 + \norm{\varsigma}_2^2}}
%             \subjto
%             (\nu, b, \alpha, \varsigma) \in \setNoisyZero
%     \end{align}
% for some scalars $\nu, b>0, \alpha\in[1,\alpham]$ and set $\setNoisyZero$ given by:
% % \begin{align}
% %     \Gamma_0 = \left\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2, \varsigma) ~~\andtxt~~  \nu \sqrt{s} + b\norm{\gamma(\alpha)}_1 - \norm{\varsigma}_1 \leq \loneboundclas \right\}.
% %     \label{eq:Gamma0_def_class_noisy}
% % \end{align}
% % \end{proposition}  
% % Note that in the proposition we make use of the triangle inequalities $\norm{\wone}_1 \leq \norm{\woneper}_1 + \norm{\wonepar}_1$ and $\norm{\wone}_1 \geq | \norm{\wonepar}_1 - \norm{\woneper}_1|$.
% \begin{align}
%     \setNoisyZero = \left\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2, \varsigma) ~~\andtxt~~  b\norm{\gamma(\alpha)}_1 \leq \loneboundclas \right\}.
%     \label{eq:Gamma0_def_class_noisy}
% \end{align}
% \end{proposition}  
% Note that in the proposition we make use of the triangle inequality $\norm{\wone}_1 \leq \norm{\woneper}_1 + \norm{\wonepar}_1$ and $\norm{\wtwo}_1 \leq \norm{\wone}_1 + \norm{\wtwo}_1 \leq \loneboundclas$.












==> sections/technical_lemmas.tex <==
\section{Technical Lemmas}
\input{sections/technical_lemmas/TL0_CGMT.tex}
\input{sections/technical_lemmas/TL4_noiseless}
\input{sections/technical_lemmas/TL1_quadratic_bound_fn}
\input{sections/technical_lemmas/TL2_quadratic_plus_fstar_bound}
\input{sections/technical_lemmas/TL3_uniform_convergence_fn}
\input{sections/technical_lemmas/TL5_additional_technical_lemmas}



==> sections/technical_lemmas/TL1_quadratic_bound_fn_old.tex <==

% % \onecolumn



% \subsection{Lower bounding \texorpdfstring{$\fnclas$}{fn} by a quadratic form}
% \label{apx:subsec:quadratic_bound_fn}
% Recall that we have defined $\fnclas (\nu, \eta, \varsigma) := \frac{1}{n} \sum_{i=1}^n ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )_+^2$ and  
% \begin{equation}
% \label{eq:defoff}
%     \fclas(\nu,\eta, \varsigma) = \EE [ \fnclas \left( \nu, \eta, \varsigma \right) ] = \EE_{\{Z^{(j)}\}_{j=0}^s \sim \NNN(0,I_{s+1})} \EE_{\xi \sim \prob(\cdot\vert Z^{(0)})} ( 1- \xi \nu \vert Z^{(0)} \vert -  Z^{(1)}\eta - \sum_{j=2}^s Z^{(j)}\varsigma_j )_+^2 .
% \end{equation}
% We show the following lemma.
% \begin{lemma} \label{quadratic_bound_fn}
%     There exist universal positive constants $\constnu, \consteta, \constvarsigma$ only depending on $\probsigma$ and $c$ such that for any $\nu,\eta,\varsigma$ we have that: 
%         \begin{align}
%         \label{eq:quadratic_bound_fn}
%             \fnclas(\nu,\eta,\varsigma) \geq \constnu \nu^2  + \consteta \eta^2 + \constvarsigma \norm{\varsigma}_2^2
%         \end{align}
%     with probability at least $1 - \exp \left( -cn \right)$ over the draws of $\{z^{(j)}\}_{j=0}^s,\xi$.
% \end{lemma}

% \begin{proof}
%  We can assume that $\nu ,\eta, \varsigma \geq 0$ as the other cases follow from exactly the same argument. 
%  First we show an auxiliary statement which we use later in the proof. Namely, we claim that there exists some positive constant $c_1$ such that for all $z \in [z_1,z_2]$,  $\probsigma \left( \xi = -1; z \right) > c_1$ for some $z_1, z_2 \in \RR$ and $z_1\neq z_2$. Let's prove this statement by contradiction and assume that there exists no $z \in [z_1,z_2]$ which satisfy the previous equation. Then, for almost any $z \sim \NNN(0,1)$, we have $\probsigma (\xi; z) = +1$ and hence the minimum of the function $\fclas(\nu, \eta, \varsigma) = \EE \fnclas (\nu, \eta, \varsigma)$ is obtained for $\nu = \infty$. However, this is in contradiction with the assumption on $\probsigma$ in Section \ref{subsec:clasetting}. Hence there exists some $z$ for which $\prob \left( \xi = -1;  z \right) > c_1$. By the assumption on $\probsigma$ in Section \ref{subsec:clasetting} we assume piece-wise continuity of $z \to \probsigma(\xi=-1;z)$ and hence there exists some interval $[z-\delta, z+\delta] =: [z_1,z_2]$ in which the given probability is bounded away from zero. 

% We can assume without loss of generality that this interval does not contain zero, since in that case we can always define a new interval of the form $[\epsilon, z_2]$ or $[z_1, -\epsilon]$ for $\epsilon>0$ small enough, which does not contain zero. Let's define $\tilde{z} = \max \{ \abs{z_1}, \abs{z_2} \}$.

%  We can now bound $\fnclas(\nu,\eta, \varsigma)$ as follows:
% \begin{align}
%     \fnclas(\nu,\eta,\varsigma) 
%     & =
%     \frac{1}{n} \sum_{i=1}^n ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )_+^2\\
%     % \frac{1}{n} \sumin \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \eta \gausswtwo_i }
%     &\geq
%     \frac{1}{n}\sumin \idvec [ \xi_i = -1, {z_i}^{(0)} \in [z_1,z_2], {z_i}^{(1)} < - c_2, \sum_{j=2}^s z_i^j \varsigma_j \leq 0  ] ( 1 - \xi_i \nu |{z_i}^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )_+^2
%     \\
%     & \geq \left( 1 + \tilde{z} \abs{\nu} + c_2 \eta + c_3 \norm{\varsigma}_2 \right)^2 \frac{1}{n}\sumin \idvec [ \xi_i = -1, {z_i}^{(0)} \in [z_1,z_2], {z_i}^{(1)} < - c_2, \sum_{j=2}^s z_i^{(j)} \varsigma_j \leq 0  ]
% \end{align}
% where in the last step we used concentration of sub-exponential random variables i.e. that $|\sum_{j=2}^s z_i^{(j)} \varsigma_j | \gtrsim \norm{\varsigma}_2$ holds with probability at least $1-\exp(-cn)$.
% From Section~\ref{subsec:path_param} we have that $z^{(j)}$ for $j=1,\dots,s$ are mutually independent and independent of $\xi$ and $z^{(0)}$. Hence:
% \begin{align}
%     \prob ( \xi = -1, & z^{(0)} \in [z_1,z_2], z^{(1)} < - c_2, \sum_{j=2}^s z_i^{(j)} \varsigma_j \leq 0 ) \\
%     &=
%     \prob ( \xi = -1 \vert \gausswone \in [z_1,z_2] ) \prob ( \gausswone \in [z_1,z_2] ) \prob ( \gausswtwo < - c_2 ) \prob ( \sum_{j=2}^s z^{(j)} \varsigma_j \leq 0 )
%     \\
%     &\geq
%     c_1 \left( \Phic(z_1) - \Phic(z_2) \right) \Phic(c_2) 
%     \geq
%     c
% \end{align}
% for some positive universal constant $c$. Now using concentration of i.i.d. Bernoulli random variables we obtain:
% \begin{align}
%     \fnclas (\nu,\eta) \geq \left( 1 + \tilde{z}\abs{\nu} + c_2 \eta + c_3 \norm{\varsigma}_2 \right)^2 \frac{c}{2} 
%     \gtrsim
%     \nu^2 + \eta^2 + \norm{\varsigma}_2^2
%     % \prob \left( \xi = \sign (\nu), \gausswone \in [z_1,z_2], \gausswtwo > \kappa_2 \right) 
% \end{align}
% with probability at least $1 - \exp \left( - cn \right)$.
% \end{proof}


% \onecolumn



\subsection{Lower bounding \texorpdfstring{$\fnclas$}{fn} by a quadratic form}
\label{apx:subsec:quadratic_bound_fn}
Recall that we have defined $\fnclas (\nu, \eta, \varsigma) := \frac{1}{n} \sum_{i=1}^n ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )_+^2$ and  
\begin{equation}
\label{eq:defoff}
    \fclas(\nu,\eta, \varsigma) = \EE [ \fnclas \left( \nu, \eta, \varsigma \right) ] = \EE_{\{Z^{(j)}\}_{j=0}^s \sim \NNN(0,I_{s+1})} \EE_{\xi \sim \prob(\cdot\vert Z^{(0)})} ( 1- \xi \nu \vert Z^{(0)} \vert -  Z^{(1)}\eta - \sum_{j=2}^s Z^{(j)}\varsigma_j )_+^2 .
\end{equation}
We show the following lemma.
\begin{lemma} \label{quadratic_bound_fn}
    There exist universal positive constants $\constnu, \consteta, \constvarsigma$ only depending on $\probsigma$ and $c$ such that for any $\nu,\eta,\varsigma$ we have that: 
        \begin{align}
        \label{eq:quadratic_bound_fn}
            \fnclas(\nu,\eta,\varsigma) \geq \constnu \nu^2  + \consteta \eta^2 + \constvarsigma \norm{\varsigma}_2^2
        \end{align}
    with probability at least $1 - \exp \left( -cn \right)$ over the draws of $\{z^{(j)}\}_{j=0}^s,\xi$.
\end{lemma}

\begin{proof}
 We can assume that $\nu ,\eta, \varsigma \geq 0$ as the other cases follow from exactly the same argument. 
 First we show an auxiliary statement which we use later in the proof. Namely, we claim that there exists some positive constant $c_1$ such that for all $z \in [z_1,z_2]$,  $\probsigma \left( \xi = -1; z \right) > c_1$ for some $z_1, z_2 \in \RR$ and $z_1\neq z_2$. Let's prove this statement by contradiction and assume that there exists no $z \in [z_1,z_2]$ which satisfy the previous equation. Then, for almost any $z \sim \NNN(0,1)$, we have $\probsigma (\xi; z) = +1$ and hence the minimum of the function $\fclas(\nu, \eta, \varsigma) = \EE \fnclas (\nu, \eta, \varsigma)$ is obtained for $\nu = \infty$. However, this is in contradiction with the assumption on $\probsigma$ in Section \ref{subsec:clasetting}. Hence there exists some $z$ for which $\prob \left( \xi = -1;  z \right) > c_1$. By the assumption on $\probsigma$ in Section \ref{subsec:clasetting} we assume piece-wise continuity of $z \to \probsigma(\xi=-1;z)$ and hence there exists some interval $[z-\delta, z+\delta] =: [z_1,z_2]$ in which the given probability is bounded away from zero. 

We can assume without loss of generality that this interval does not contain zero, since in that case we can always define a new interval of the form $[\epsilon, z_2]$ or $[z_1, -\epsilon]$ for $\epsilon>0$ small enough, which does not contain zero. Let's define $\tilde{z} = \max \{ \abs{z_1}, \abs{z_2} \}$.

 We can now bound $\fnclas(\nu,\eta, \varsigma)$ as follows:
\begin{align}
    \fnclas(\nu,\eta,\varsigma) 
    & =
    \frac{1}{n} \sum_{i=1}^n ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )_+^2\\
    % \frac{1}{n} \sumin \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \eta \gausswtwo_i }
    &\geq
    \frac{1}{n}\sumin \indicator{ \xi_i = -1, \gausswone_i \in [z_1,z_2], \gausswtwo_i < - c_2 } \indicator{ -\sum_{j=2}^s \gausswj_i \varsigma_j \geq c_3\norm{\varsigma}_2} ( 1 - \xi_i \nu |\gausswone_i| - \gausswtwo_i \eta - \sum_{j=2}^s \gausswj_i \varsigma_j )_+^2
    \\
    & \geq \left( 1 + \tilde{z} \abs{\nu} + c_2 \eta + c_3 \norm{\varsigma}_2 \right)^2 \frac{1}{n} \sum_{i=1}^k \idvec [ \xi_i = -1, {z_i}^{(0)} \in [z_1,z_2], {z_i}^{(1)} < - c_2 ]
\end{align}
with $k:= n \inf_{\norm{\varsigma}_2=1} \frac{1}{n} \sum_{i=1}^n \indicator{\sum_{j=2}^s \gausswj_i \varsigma_j \geq c_3} =n\inf_{\norm{\varsigma}_2=1} P_n g_{\varsigma}$ with $g_{\varsigma}:= \indicator{\sum_{j=2}^s \gausswj_i \varsigma_j \geq c_3}$.
\begin{lemma}
Assume that $G:=\{g_{\varsigma}:\norm{\varsigma}_2=1\}$ is bounded class of functions i.e. $\norm{g_{\varsigma}}_{\infty}\leq b$ $\forall \varsigma$ with $\norm{\varsigma}_2=1$. Then
\begin{align}
    \PP \left( \norm{P_n-P}_G  \geq 2\RRR_n(G) + t \right) \leq 2\exp\left(-\frac{nt^2}{2b^2} \right)
\end{align}
for all $n$ and $t>0$.
\end{lemma}
\begin{align}
    \RRR_n(G) = \EE \left[ \sup_{\norm{\varsigma}_2=1} \left| \frac{1}{n}\sum_{i=1}^n \epsilon_i \indicator{\sum_{j=2}^s \gausswj_i \varsigma_j \geq c_3} \right|\right] 
    \lesssim
    \frac{1}{c_3^2} \EE \left[ \sup_{\norm{\varsigma}_2=1} \left| \frac{1}{n}\sum_{i=1}^n \epsilon_i (\sum_{j=2}^s \gausswj_i \varsigma_j)^2  \right| \right]
    \lesssim
    \sqrt{\frac{s}{n}}
\end{align}
from Corollary~\ref{corr:sup_sphere_inner_prod_gauss}. Also note that $b=1$. Thus:
\begin{align}
    \PP \left( \norm{P_n-P}_G  \gtrsim \sqrt{\frac{s}{n}} \right) \leq 2\exp\left(-c_1 s \right)
\end{align}
% Now using that $\sum_{j=2}^s \gausswj_i \frac{\varsigma_j}{\norm{\varsigma}_2}$ for $i=1,\dots,n$ are i.i.d. samples of $\NNN(0,1)$ random variable, and applying the Dvoretzky-Kiefer-Wolfowitz inequality \cite{massart} we have:
% \begin{align}
%     k &= \inf_{\norm{\varsigma}_2=1} \sum_{i=1}^n \indicator{\sum_{j=2}^s \gausswj_i \varsigma_j \geq c_3} 
%     \geq
%     n( \inf_{\norm{\varsigma}_2=1} \PP (\sum_{j=2}^s \gausswj \varsigma_j \geq c_3)  - \sup_{\norm{\varsigma}_2=1} \left| \frac{1}{n}\sum_{i=1}^n \indicator{\sum_{j=2}^s \gausswj_i \varsigma_j \geq c_3} -  \PP (\sum_{j=2}^s \gausswj \varsigma_j \geq c_3) \right| )\\
%     &\geq
%     n(\inf_{\norm{\varsigma}_2=1}  \Phic(c_3) - \sup_{\norm{\varsigma}_2=1} \left| \Phic_n(c_3) - \Phic(c_3) \right|) \geq \frac{1}{2} \Phic(c_3) n
% \end{align}
% with probability at least $1-$, and where $\Phic_n(x):= \frac{1}{n} \indicator{z_i \geq x}$ for $z_i\sim \NNN(0,1)$.
From Section~\ref{subsec:path_param} we have that $z^{(j)}$ for $j=1,\dots,s$ are mutually independent and independent of $\xi$ and $z^{(0)}$. Hence:
\begin{align}
    \prob ( \xi = -1,  z^{(0)} \in [z_1,z_2], z^{(1)} < - c_2 ) 
    &=
    \prob ( \xi = -1 \vert \gausswone \in [z_1,z_2] ) \prob ( \gausswone \in [z_1,z_2] ) \prob ( \gausswtwo < - c_2 )
    \\
    &\geq
    c_1 \left( \Phic(z_1) - \Phic(z_2) \right) \Phic(c_2) 
    \geq
    c
\end{align}
for some positive universal constant $c$. Now using concentration of i.i.d. Bernoulli random variables we obtain:
\begin{align}
    \fnclas (\nu,\eta) \geq \left( 1 + \tilde{z}\abs{\nu} + c_2 \eta + c_3 \norm{\varsigma}_2 \right)^2 \frac{c}{2} 
    \gtrsim
    \nu^2 + \eta^2 + \norm{\varsigma}_2^2
    % \prob \left( \xi = \sign (\nu), \gausswone \in [z_1,z_2], \gausswtwo > \kappa_2 \right) 
\end{align}
with probability at least $1 - \exp \left( - cn \right)$.
\end{proof}


==> sections/technical_lemmas/TL2_quadratic_plus_fstar_bound_old.tex <==


% \onecolumn

\subsection{Lower bounding \texorpdfstring{$\fnclas$}{fn} by a quadratic form with constant}
\label{apx:subsec:quadratic_plus_fstar_bound}
Recall that $\deltanu = \nu -\nubar$. We show the following lemma. 
\begin{lemma} \label{lemma_quadratic_plus_fstar_bound}
    Let $\boundnu, \boundeta, \boundvarsigma >0$ be universal positive constants. Then, there exist positive constants $\tconstnu,\tconsteta, \tconstvarsigma >0$ and $c_1, c_2,c_3 >0$ only depending on $\probsigma$, such that for any $\epsilon \geq  c_1 \sqrt{\frac{s}{n}}$ and any $\nu \leq \boundnuone, \eta \leq \boundetaone, \norm{\varsigma}_2 \leq \boundvarsigma$ we have that: 
        \begin{align}
        \label{eq:quadratic_plus_fstar_bound}
            \fnclas(\nu,\eta) \geq \fstar + \tconstnu \left( \deltanu \right)^2  + \tconsteta \eta^2  + \tconstvarsigma \norm{\varsigma}_2^2 - \epsilon
        \end{align}
    with probability at least $1 - \exp \left( -c_2  n \epsilon^2  \right) -  \exp \left( -c_3 \frac{ n \epsilon }{s\log (ns)} \right)$ over the draws of $z^{(j)},\xi$ for $j=0,\dots,s$.
\end{lemma}
\begin{proof}
First note that from the uniform convergence result in Proposition \ref{prop:unifConv} we have that $\fclas(\nu,\eta,\varsigma) \geq \fnclas(\nu,\eta,\varsigma) - \epsilon$, with $\fclas$ from Equation~\eqref{eq:defoff}, with high probability. Thus, it is sufficient to study $\fclas$.  Clearly, by the convexity of $\fclas$ we have that $\fclas \geq \fstar$ with $\fstar = \fclas(\nubar, 0, 0)$ where we use the simple fact that $(\nubar, 0)$ is the global minimizer of $\fclas$, which follows from the  assumption on $\probsigma$ in Section \ref{subsec:clasetting}. 
Furthermore, it is not difficult to check that for for any $\nu,\eta,\varsigma$, $\nabla^2 \fclas(\nu,\eta,\varsigma) \succ 0$ and therefore, $\fclas$ is strictly convex on every compact set. Hence, the proof follows. 
\end{proof}


==> sections/technical_lemmas/TL3_uniform_convergence_fn_old.tex <==
\subsection{Uniform convergence of \texorpdfstring{$\fnclas$}{fnclas} to \texorpdfstring{$\fclas$}{fclas}}
\label{apx:subsec:unif_conv}
Denote with $Z^{(j)} \sim \Normal(0,1)$, $j=0,\dots,s$, independent Gaussian random variables and let $\xirv \vert Z^{(0)} \sim \probsigma(.; Z^{(0)})$. 

% Let $P$ be the distribution of $(\{Z^{(j)}\}_{j=0}^s,\xirv)$ and let $P_n = \frac{1}{n} \sumin \delta_{\gausswone_i,\gausswtwo_i,\xi_i}$. Define $\gnueta(Z,\xi) = \possq{1-\xirv \abs{\Gausswone}\nu - \eta\Gausswtwo}$ with $Z = (\Gausswone, \Gausswtwo)$. Note that using this notation, we have $P\gnueta = \EE \gnueta(Z,\xi) = \fclas (\nu,\eta)$, with $f$ from Equation~\eqref{eq:defoff}, and $P_n \gnueta = \fnclas(\nu,\eta)$. Let $\GB = \left\{ \gnueta\ |\ \nu \leq \boundnuone, \eta \leq \boundetaone \right\}$ with positive constants $\boundetaone$ and $\boundnuone$. Moreover define:
Let $P$ be the distribution of $(\{Z^{(j)}\}_{j=0}^s,\xirv)$ and let $P_n = \frac{1}{n} \sumin \delta_{\{ z_i^{(j)}\}_{j=0}^s,\xi_i}$. Define $\gnuetasigma(Z,\xi) = \possq{1-\xirv |Z^{(0)}|\nu - \eta Z^{(1)} - \sum_{j=2}^s Z^{(j)}\varsigma_j}$ with $Z = \{Z^{(j)}\}_{j=0}^s$. Note that using this notation, we have $P\gnuetasigma = \EE \gnuetasigma(Z,\xi) = \fclas (\nu,\eta,\varsigma)$, with $\fclas$ from Equation~\eqref{eq:defoff}, and $P_n \gnuetasigma = \fnclas(\nu,\eta,\varsigma)$. Let $\GB = \left\{ \gnuetasigma\ |\ \nu \leq \boundnuone, \eta \leq \boundetaone, \norm{\varsigma}_2 \leq \boundvarsigma \right\}$ with positive constants $\boundetaone$,$\boundnuone$ and $\boundvarsigma$. Moreover define:
\begin{align}
    \norm{ P_n - P }_{\GB} := \sup_{\gnuetasigma \in \GB} \abs{(P_n - P)\gnuetasigma}
\end{align}
and $P_n^{\epsilon} g = \frac{1}{n}\sum_{i=1}^n \epsilon_i g(Z_i)$ and $ \norm{P_n^{\epsilon}}_\GGG = \sup_{g\in \GGG} \abs{P_n^{\epsilon}g}$.
\red{where to introduce this notation?}

We then obtain from an application of Theorem 4 in \cite{adamczak2008tail} the following uniform convergence result
\begin{proposition}
\label{prop:unifConv}
There exist positive universal constants $c_1,c_2,c_3>0$ such that
    \begin{align}
        \prob \left( \norm{ P_n - P }_{\GB} \leq c_1 \frac{\sqrt{s}}{\sqrt{n}} + \epsilon \right) 
        \geq
        1 - \exp \left( -c_2  n \epsilon^2  \right) -  \exp \left( -c_3 \frac{ n \epsilon }{s\log (ns)} \right)
    \end{align}
\end{proposition}

\begin{proof}

The proof follows from an application of the tail-bound result from Theorem 4 in \cite{adamczak2008tail}. More precisely, 


We choose $\alpha = 1$ and explicitly show that condition from Theorem 4 in \cite{adamczak2008tail} requiring finite Orlicz norms is indeed satisfied for this choice of $\alpha$.
We separate the proof into two steps, where in a first step we bound the $ \psi_{\GB}$ and then apply Theorem~\ref{thm:unifconvmain}. 

\paragraph{Step 1: Bounding $\psi_{\GB}$}

By the definition of Orlicz norms, $\psi_{\GB}$ is given by:
% \begin{align}\label{eq_psi_GB_def}
%     \psi_{\GB} 
%      =&
%     \orlicznorm{ \max_{1 \leq i \leq n} \sup_{\nu,\eta,\varsigma} \frac{1}{n} | ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )_+^2 - \EE [ ( 1 - \xi \nu |z^{(0)}| - z^{(1)} \eta - \sum_{j=2}^s z^{(j)} \varsigma_j )_+^2 ] | } 
%     \\ 
%     =& \inf \{ \lambda>0:\ \EE [ \exp ( \frac{1}{\lambda} \max_i \sup_{\nu,\eta,\varsigma} \frac{1}{n}
%     | ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )_+^2 \\
%     & - \EE [ ( 1 - \xi \nu |z^{(0)}| - z^{(1)} \eta - \sum_{j=2}^s z^{(j)} \varsigma_j )_+^2 ] | ) - 1 ] \leq 1 \}
% \end{align}
\begin{align}\label{eq_psi_GB_def}
    \psi_{\GB} 
    = \inf \{ \lambda>0:\ \EE [ \exp ( \frac{1}{\lambda} \max_i \sup_{\nu,\eta,\varsigma} \frac{1}{n}
    | \gnuetasigma(z_i,\xi_i) - \EE [\gnuetasigma] | - 1 ]) \leq 1 \}
\end{align}
Applying the triangle inequality and using that $\nu,\eta,\norm{\varsigma}_2$ are bounded by constants, we can bound the expectation from the expression above as:
\begin{align}
    \EE \bigg[ \exp \Big( \frac{1}{\lambda} \max_i& \sup_{\nu,\eta,\varsigma} \frac{1}{n}
    \Big| (1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j)_+^2 - \EE [ (1 - \xi \nu |z^{(0)}| - z^{(1)} \eta - \sum_{j=2}^s z^{(j)} \varsigma_j)_+^2 ] \Big| \Big) \bigg]
    \\
     \leq 
    % \EE \left[ \exp \left(  \frac{1}{n\lambda} \max_i \sup_{\nu,\eta} 
    % \possq{ 1 - \xi_i \abs{\gausswone_i} \nu -  \gausswtwo_i \eta} + \frac{1}{n\lambda}\sup_{\nu,\eta} \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right]  \right) \right]
    % \\
    % & = 
    \EE \bigg[ \exp \Big(  \frac{1}{n\lambda} &\max_i \sup_{\nu,\eta,\varsigma} 
    (1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j)_+^2 \Big) \bigg]\\
    & \cdot
    \exp \Big( \frac{1}{n\lambda}\sup_{\nu,\eta,\varsigma} \EE [ (1 - \xi \nu |z^{(0)}| - z^{(1)} \eta - \sum_{j=2}^s z^{(j)} \varsigma_j)_+^2 ] \Big) 
    \leq
    \EE \left[ \exp \left(  c_1\frac{s}{n\lambda}\norm{z}_{\infty}^2 \right) \right] \exp \left( \frac{c_2}{n\lambda} \right)  
\end{align}
for some positive universal constants $c_1,c_2$ that may depend on $\boundnu,\boundeta,\boundvarsigma$ and recall that $z = \{z_i^{(j)}\}_{i,j}$. Now we split the expectation from the above inequality into two terms:
\begin{align}
   \EE \left[\onevec \Big[\norm{z}_\infty < \sqrt{2 \log (ns)} \Big] \exp \left(  c_1\frac{s}{n\lambda}\norm{z}_{\infty}^2  \right) \right]
%   &= \int_{-\sqrt{2\log n}}^{\sqrt{2\log n}}\cdots\int_{-\sqrt{2\log n}}^{\sqrt{2\log n}} \exp \left( \frac{B}{n\lambda}  \zmax^2 \right) \prod_{i=1}^{2n} \frac{ \exp \left( -\frac{1}{2} z_i^2 \right) }{\sqrt{2\pi}}dz_i
   \leq
   \exp \left( c_4 \frac{\log (ns)}{n\lambda} \right)
\end{align}
and
\begin{align}
    \EE & \left[\onevec \Big[\norm{z}_{\infty} \geq \sqrt{2 \log (ns)} \Big] \exp \left(  c_1\frac{s}{n\lambda}\norm{z}_{\infty}^2  \right) \right]
    \lesssim
    ns \int_{\sqrt{2 \log (ns)}}^{\infty} \int_{-z_1}^{z_1} \cdots \int_{-z_1}^{z_1} \exp \left( c_1 \frac{s}{n\lambda}  z_1^2 \right) \prod_{i=1}^{n(s+1)} \frac{\exp(-\frac{1}{2}z_i^2)}{\sqrt{2\pi}} dz_i
    \\
    &\lesssim
    ns \int_{\sqrt{2 \log (ns)}}^{\infty} \exp \left( - z_1^2 (\frac{1}{2} - c_1\frac{s}{n\lambda}) \right) dz_1 
    \lesssim
    \frac{(ns)^{\frac{2c_1 s}{n\lambda}}}{\sqrt{\log (ns) }(1- \frac{2c_1s}{n\lambda})}
\end{align}
where we assumed that $\lambda > 2c_1\frac{s}{n}$. Now choosing $\lambda = c_{\lambda} \frac{s \log (ns)}{n}$ with a positive constant $c_{\lambda}$ sufficiently large, we find that the condition in Equality \eqref{eq_psi_GB_def} is satisfied for this $\lambda$, which implies that $\psi_{\GB} \leq c_{\lambda}\frac{s\log (ns)}{n}$.

\paragraph{Step 2: Proof of the statement}
To apply Theorem~\ref{thm:unifconvmain}, we also need to bound the variance $\sigma_{\GB}^2$ and use that $\EE \norm{P_n-P}_{\GB} \leq 2 \rademacher(\GB)$  where $ \rademacher(\GB)$ is the Rademacher complexity given by $\rademacher(\GB) = \EE \left[ \sup_{\gnuetasigma\in \GB} \left|\frac{1}{n}\sumin \epsilon_i \gnuetasigma(z_i,\xi_i) \right| \right]$. 
% The bound on the variance follows from a straightforward calculation:
% \begin{align}
%     \sigma_{\GB}^2
%   % & =  \sup_{ \gnueta \in \GB } \frac{1}{n}\left( \EE \left[ \gnueta^2 \right] - \left( \EE \left[ \gnueta \right] \right)^2 \right)
%     \leq 
%     \frac{1}{n} \sup_{ \gnuetasigma \in \GB } \EE \left[ \gnuetasigma^2 \right]
%     % \leq
%     % \frac{1}{n} \EE \left[ 1 + \boundnuone \nu + \boundetaone \eta \right]^4 
%     % \leq
%     % \frac{1}{n} c_{\sigma_{\GB}} \left( 1 + \boundnuone^4 + \boundetaone^4 \right)
% \end{align}

To make notation less cumbersome, let $g_+ := \gnuetasigma, g_-:= ( 1- \xirv |Z^{(0)}| \nu - \eta Z^{(1)} - \sum_{j=2}^s \varsigma_j Z^{(j)})_-^2 $ and $g_{+,-} := g_- + g_+$. First, note that:
\begin{align}
\EE g_{+,-} \lesssim 1 + \nu^2 + \eta^2 + \norm{\varsigma}_2^2 = \OOO(1)    
\end{align}
Since $g_+,g_-\geq 0$ inequality above implies that $\EE g_+ = \OOO(1)$ and $\EE g_- = \OOO(1)$. Also note that $\EE \left[ g_+ g_- \right] = 0$ and thus $\mathrm{Cov}(g_+,g_-) \leq 0$. But then we use that:
\begin{align}
    \var(g_+) 
    =
    \var(g_{+,-}) - \var(g_-) + 2\EE g_+ \EE g_- 
    \leq
    \var(g_{+,-}) + c_1
\end{align}
for some universal constant $c_1>0$. Thus for some positive universal constant $c_{\sigma_{\GB}}$ we can upper bound variance of $g_+$ i.e. $\sigma_{\GB}^2$ as follows:
% \begin{align}
%     \EE \left[ g_+^2 \right] - \left( \EE \left[ g_+ \right] \right)^2 
%     \leq
%     \EE \left[g_{+,-}^2 \right] - \left( \EE \left[g_{+,-} \right] \right)^2 + c_1
% \end{align}
% and substituting the last inequality in the definition \eqref{eq:def_var_orlicz_proof} we obtain for
\begin{align}
    \sigma_{\GB}^2 \leq \frac{1}{n} \sup_{\nu\leq \boundnu, \eta \leq \boundeta, \norm{\varsigma}_2 \leq \boundvarsigma} ( \EE [  ( 1- &\xirv | Z^{(0)} | \nu - \eta Z^{(1)} - \sum_{j=2}^s \varsigma_j Z^{(j)} )^4 ] \\
    -& \EE [  ( 1- \xirv | Z^{(0)} | \nu - \eta Z^{(1)} - \sum_{j=2}^s \varsigma_j Z^{(j)} )^2 ]^2 ) + \frac{c_1}{n} \leq \frac{c_{\sigma_{\GB}}}{n}
\end{align}
% \begin{align}
%     \sigma_{\GB}^2
%     \leq 
%     \frac{1}{n} \sup_{ \gnuetazeta \in \GB } \EE \left[ \gnuetazeta^2 \right]
%     \leq
%     \frac{1}{n} \kappa_{\sigma_{\GB}} \left( 1 + \boundnuone^4 + \boundetaone^4 \right)
% \end{align}
where in the last step we used expressions for moments of Gaussian random variables.

Next, note that we can upper bound the Rademacher complexity using the triangle inequality and the fact that $(\cdot)_+$ is $1$-Lipschitz:
% \begin{align}
%      \rademacher(\GB) &\leq 
%     \EE \left[\sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i (1-\xi_i \abs{\gausswone_i}\nu - \eta\gausswtwo_i)^2\right| \right] 
%     \\ 
%     &\lesssim \EE \left[ \sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i\right| \right] +  \EE \left[ \sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i (\xi_i \abs{\gausswone_i}\nu)^2\right| \right] \\
%     &+  \EE \left[ \sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i ( \eta\gausswtwo_i)^2\right| \right] 
%     \lesssim \frac{1}{\sqrt{n}}
% \end{align}
\begin{align}
     \rademacher(\GB) &\leq 
    \EE \left[\sup_{\nu\leq \boundnu,\eta\leq \boundeta, \norm{\varsigma}_2 \leq \boundvarsigma }\left| \frac{1}{n}\sumin \epsilon_i ( 1 - \xi_i \nu |z_i^{(0)}| - z_i^{(1)} \eta - \sum_{j=2}^s z_i^{(j)} \varsigma_j )^2 \right| \right] 
    \\ 
    &\lesssim \EE \left[ \left| \frac{1}{n}\sumin \epsilon_i\right| \right] +  \EE \left[ \sup_{\nu\leq \boundnu}\left| \frac{1}{n}\sumin \epsilon_i (\xi_i \abs{\gausswone_i}\nu)^2\right| \right] \\
    &+  \EE \left[ \sup_{\eta\leq \boundeta}\left| \frac{1}{n}\sumin \epsilon_i ( \eta\gausswtwo_i)^2\right| \right] 
    +  \EE \left[ \sup_{\norm{\varsigma}_2 \leq \boundvarsigma}\left| \frac{1}{n}\sumin \epsilon_i ( \sum_{j=2}^s z_i^{(j)} \varsigma_j )^2 \right| \right] 
    \lesssim \frac{\sqrt{s}}{\sqrt{n}}
\end{align}
where the last line follows from applying the standard concentration results and Corollary~\ref{corr:sup_sphere_inner_prod_gauss}. Thus, we obtain:
    \begin{align}
        % \prob \left( \norm{ P_n - P }_{\GB} \geq \kappa_1 \sqrt{\frac{\log(n)}{n}} + t \right) 
        \prob \left( \norm{ P_n - P }_{\GB} \geq 2(1+t) \mathcal{R}_{\GB} + \epsilon \right) 
        \leq
        \exp \left( - c_2 n \epsilon^2 \right) + 3\exp \left( -c_3 \frac{ n \epsilon }{s\log (ns)} \right)
    \end{align}
with $c_2^{-1} = 2(1+\delta)c_{\sigma_{\GB}}$ and $c_3^{-1} = C c_{\lambda}$, which concludes the proof. 

%Recalling result from Lemma \ref{lm:rademacher} concludes the proof.
\end{proof}


==> sections/technical_lemmas/TL4_noiseless_old.tex <==
\subsection{Lower bounding \texorpdfstring{$\fnclasn$}{fnn}}
\begin{proposition}
\label{prop:fnoiselessquadraticvarsigma}
There exist positive universal constants $\kappa_1,\kappa_2,\kappa_3, \kappa_4, c_1$ such that for any $\nu,\eta>0$ with $\nu = \Omega(1)$, inequality
% \begin{align}
%     \fnclasn (\nu,b\norm{\gamma(\alpha)}_2) \geq \max \{ \kappa_1 \frac{1}{\nu}, \kappa_2 \frac{\eta^2}{\nu} \}
% \end{align}
\begin{align}
    \fnclasn (\nu,\eta,\varsigma) \geq  \kappa_3 \frac{\norm{\varsigma}_2^2}{\nu} - \kappa_4 \frac{s}{\sqrt{n}}
\end{align}
holds with probability at least $1-s\exp(-c_1 n)$ over the draws of $\{z_i^{(0)},z_i^{(1)}\}_{i=1}^n$.
\end{proposition}


\begin{proposition}
\label{prop:fnoiselessquadratic}
There exist positive universal constants $\kappa_1,\kappa_2,\kappa_3, \kappa_4, c_1$ such that for any $\nu,\eta>0$ with $\nu = \Omega(1)$, inequality
% \begin{align}
%     \fnclasn (\nu,b\norm{\gamma(\alpha)}_2) \geq \max \{ \kappa_1 \frac{1}{\nu}, \kappa_2 \frac{\eta^2}{\nu} \}
% \end{align}
\begin{align}
    \fnclasn (\nu,\eta,\varsigma) \geq \kappa_1 \frac{1}{\nu} + \kappa_2 \frac{\eta^2}{\nu} + \kappa_3 \frac{\norm{\varsigma}_2^2}{\nu} - \kappa_4 \frac{\norm{\varsigma}_2^2 \log(ns)}{\sqrt{n}}
\end{align}
holds with probability at least $1-c_1/(n s)$ over the draws of $\{z_i^{(0)},z_i^{(1)}\}_{i=1}^n$.
\end{proposition}
\begin{proof}
We can use the same reasoning as in Lemma~\ref{lemma_uniform_conv_semiindic_noiseless} to show the following inequalities:
\begin{align}
    \left|\frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu |\gausswone_i|} 
    -
    \EE \left[ \possq{1-\nu|\Gausswone|} \right] \right|
    \lesssim
    \frac{1}{\sqrt{n}}
    \label{eq:sup_uniform_conv_nu_only}
\end{align}
\begin{align}
    \left|\frac{1}{n} \sum_{i=1}^{n} (\gausswj_i)^2 \indicator{ 1 - \nu |\gausswone_i|} 
    -
    \EE \left[ (\Gausswj)^2 \indicator{ 1 - \nu |\Gausswone|} \right]  \right|
    \lesssim
    \frac{1}{\sqrt{n}},\quad j=1,2,\dots,s
    \label{eq:sup_uniform_conv_indicators_nu_only}
\end{align}
hold simultaneously with probability $\geq 1-s\exp(-c_1 n)$. Since $\{\{z_i^{(j)}\}_{i=1}^n\}_{j=1}^s$ are i.i.d. $\NNN(0,1)$ random variables, we have $\PP(-\eta \gausswtwo_i - \sum_{j=2}^s \gausswj_i \varsigma_j \geq 0) = \frac{1}{2}$ and thus, the inequality:
\begin{align}
    \fnclasn(\nu,\eta,\varsigma) 
    =
    \frac{1}{n}\sum_{i=1}^n ( 1 - \nu |\gausswone_i| - \eta \gausswtwo_i - \sum_{j=2}^s \gausswj_i \varsigma_j )_+^2
    \gtrsim
    \frac{1}{n} \sum_{i=1}^{n} \possq{ 1 - \nu \abs{\gausswone_i}}
    \label{eq:fn_first_bound_nu_lower}
\end{align}
holds with probability $\geq 1-\exp(-c_2 n)$ for some positive universal constant $c_2$.

From proof of Lemma~\ref{lemma:exp_semi_indicator_noiseless} i.e. Equality~\eqref{eq_exp_partial_nu_fnclasn} and $\nu=\Omega(1)$ we have $\EE \possq{1-\nu\abs{\Gausswone}} = \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + O \left( \frac{1}{\nu^3} \right) \geq 2\kappa_1\frac{1}{\nu}$ for some universal constant $\kappa_1 >0$. From inequalities~\eqref{eq:sup_uniform_conv_nu_only} and \eqref{eq:fn_first_bound_nu_lower} we obtain that $ \fnclasn (\nu,\eta) \geq \kappa_1 \frac{1}{\nu} - \kappa_4\frac{1}{\sqrt{n}}$  with high probability.

Similarly to the above, we have:
\begin{align}
    \fnclasn (\nu,\eta, \varsigma)  
    =
    \frac{1}{n}\sum_{i=1}^n ( 1 - \nu |\gausswone_i| - \eta \gausswtwo_i - \sum_{j=2}^s \gausswj_i \varsigma_j )_+^2
    &\gtrsim
    \frac{1}{n} \sum_{i=1}^n ( 1-\nu\abs{\gausswone_i} + \eta \abs{\gausswtwo_i} )^2 \indicator{1-\nu\abs{\gausswone_i}}\\
    &\gtrsim
    \frac{1}{n} \eta^2 \sum_{i=1}^n (\gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}}
    \label{eq:fn_first_bound_eta_lower}
\end{align}
where in the first step we used that $cn$ out of $n$ Gaussian random variables are positive with high probability for some universal constant $c>0$, and in the second that $1-\nu\abs{\gausswone_i}\geq 0$. From the exactly same reasoning we conclude that $\fnclasn(\nu,\eta,\varsigma) \gtrsim \frac{1}{n} \varsigma_j^2 \sum_{i=1}^n (\gausswj_i)^2 \indicator{1-\nu\abs{\gausswone_i}}$ for every $j=2,\dots,s$.


In the proof of Lemma~\ref{lemma:exp_semi_indicator_noiseless} we show that $\EE [ (\Gausswtwo)^2 \indicator{ 1 - \nu |\Gausswone|} ] = \sqrt{\frac{2}{\pi}} \frac{1}{\nu} + O(\frac{1}{\nu^3}) \geq 2\kappa_2 \frac{1}{\nu}$ for $\nu = \Omega(1)$. Now from inequalities~\eqref{eq:sup_uniform_conv_indicators_nu_only},~\eqref{eq:fn_first_bound_eta_lower}, we get that there exists a universal constant $\kappa_2>0$ such that inequality $\fnclasn (\nu,\eta, \varsigma) \geq \kappa_2 \frac{\eta^2}{\nu} - \kappa_4 \frac{1}{\sqrt{n}}$ holds with high probability. Similarly we have that $\fnclasn (\nu,\eta, \varsigma) \geq \kappa_3 \frac{\varsigma_j^2}{\nu} - \kappa_4 \frac{1}{\sqrt{n}}$ and thus $\fnclasn (\nu,\eta, \varsigma) \geq \kappa_2 \frac{\norm{\varsigma}_2^2}{\nu} - \kappa_4 \frac{1}{\sqrt{n}}$. Taking the intersection of all $s+1$ high probability events concludes the proof.
\end{proof}


\subsection{Tighter lower bounding \texorpdfstring{$\fnclasn$}{fnntighter}}
\begin{proposition}
\label{prop:fnoiselessquadratictighter}
% There exist positive universal constants $\kappa_4,c_1$ such that for any $\nu,\eta>0$ with $\nu = \Omega(n^p)$, $p\in(0,\frac{2}{5})$, $\eta=O(1)$ and $\epsilon \asymp \max\{ \frac{\log n}{n^{(1+p)/2}},\frac{1}{n^{3p}}\}$, inequality
% \begin{align}
%     \fnclasn (\nu,\eta) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + \kappa_4 \frac{\eta^2}{\nu} - \epsilon
% \end{align}
% holds with probability at least $1-\exp(-c_1 n^{1-p})$ over the draws of $\{z_i^{(0)},z_i^{(1)}\}_{i=1}^n$.
% \end{proposition}
There exist positive universal constants $\kappa_4,c_1$ such that for any $\nu,\eta>0$ with $\nu = \Omega(n^p)$, $p\in(0,\frac{2}{5})$, $\eta=O(1)$ and $\epsilon \asymp \max\{ \frac{\log n}{\sqrt{n}},\frac{1}{n^{3p}}\}$, inequality
\begin{align}
    \fnclasn (\nu,\eta) \geq \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + \kappa_4 \frac{\eta^2}{\nu} - \epsilon
\end{align}
holds with probability at least $1-c_1n^{-1}$ over the draws of $\{z_i^{(0)},z_i^{(1)}\}_{i=1}^n$.
\end{proposition}
\begin{proof}
% Setting $\eta=0$ into Proposition~\ref{prop:uniform_conv_noiseless} and recalling that $\epsilon_c \asymp n^{-(1+p)/2}$ we have:
% \begin{align}
%     \sup_{\nu = \Omega(n^p)} \left|\fnclasn(\nu,0) 
%     -
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} \right|
%     =
%     O \left( \frac{1}{\nu^3}, \epsilon_c \right) 
% \end{align}
% with probability at least $1-\exp(-c_1 n^{1-p})-c_2d^{-1}$.

Similarly to Lemma~\ref{lemma_uniform_conv_semiindic_noiseless} we can show that
% \begin{align}
%    \PP \left(\norm{ P_n - P }_{\mathcal{G}''} \leq c_3 \frac{\log n}{n^{(1+p)/2}} \right) \geq 1-c_1 \exp (-c_2 n^{1-p})
% \end{align}
\begin{align}
   \PP \left(\norm{ P_n - P }_{\mathcal{G}''} \leq c_3 \frac{\log n}{\sqrt{n}} \right) \geq 1-c_1 n^{-1}
\end{align}
with $\mathcal{G}'':=\{ (\Gausswone,\Gausswtwo)\mapsto (1-\nu \abs{\Gausswone} - \eta \Gausswtwo)_+^2 \ |\nu = \Omega(n^p), \eta = O(1) \}$. 

Recall that $\fclasn(\nu,\eta) = \EE [\fnclasn(\nu,\eta)]$. It is straightforward to check that $\fclasn$ is a continuous function and that it is monotonically non-decreasing function in $\eta$. Furthermore we have that $\frac{\partial^2}{\partial\eta^2}\fclasn(\nu,\eta)\vert_{\eta=0} = \frac{2c_1}{\nu}$ for some universal positive constant $c_1$. 

By continuity of $\fclasn$ there exists some neighborhood of zero i.e. $[0,\delta)$ in which holds that $\fclasn(\nu,\eta) \geq \fclasn(\nu,0) + \eta^2\frac{c_1}{\nu}$ for $\eta \in [0,\delta)$ and any $\nu$. Now using the fact that $\fclasn$ is monotonically non-decreasing there exists some positive universal constant $\kappa_4$ such that $\fclasn(\nu,\eta) \geq \fclasn(\nu,0) + \eta^2\frac{\kappa_4}{\nu}$ for $\eta \in [0,B_{\eta}]$, with $B_{\eta}=O(1)$ and any $\nu$.

From Equality~\eqref{eq_exp_partial_nu_fnclasn} we have that $\fclasn(\nu,0) = \EE \possq{1-\nu\abs{\Gausswone}} = \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + O \left( \frac{1}{\nu^3} \right)$. Combining all results we obtain:
% \begin{align}
%     \fnclasn(\nu,\eta) \geq \fclasn(\nu,\eta) - c_3 \frac{\log n}{n^{(1+p)/2}} \geq \frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\nu} + \kappa_4 \frac{\eta^2}{\nu} + O\left(\frac{\log n}{n^{(1+p)/2}},\frac{1}{n^{3p}}\right)
% \end{align}
\begin{align}
    \fnclasn(\nu,\eta) \geq \fclasn(\nu,\eta) - c_3 \frac{\log n}{\sqrt{n}} \geq \frac{\sqrt{2}}{3\sqrt{\pi}}\frac{1}{\nu} + \kappa_4 \frac{\eta^2}{\nu} + O\left(\frac{\log n}{\sqrt{n}},\frac{1}{n^{3p}}\right)
\end{align}
which is what we wanted to prove.
\end{proof}

\red{TO DO: THIS NEEDS TO BE FINISHED}
\begin{proposition}
\begin{align}
    \fnclasn(\nu,\eta,\varsigma)
    \geq
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} +
    \sqrt{\frac{2}{\pi}} \frac{b^2\norm{\gamma(\alpha)}_2^2}{\nu} (1+\OOO_f)
    + \kappa_5 \frac{\norm{\varsigma}_2^2}{\nu} 
\end{align}
\end{proposition}
\begin{proof}
Follows from proof of Proposition~\ref{prop:fnoiselessquadratictighter} and Proposition~\ref{prop:uniform_conv_noiseless}.
\end{proof}

\subsection{Uniform convergence of \texorpdfstring{$\fnclasn$}{fnclasn} to \texorpdfstring{$\fclasn$}{fclasn}: Proof of Proposition~\ref{prop:uniform_conv_noiseless}}
\label{sec:uniform_conv_noiseless}

% \begin{proposition}
% \label{prop:uniform_conv_noiseless}
% For any $p\in(0,1)$, $\rho \asymp \sqrt{\frac{\log d}{n}}$, $\epsilon_n \asymp \sqrt{\log\log n}$ and $\epsilon_c \asymp n^{-(1+p)/2} $ the following inequality holds with probability at least $1-\exp(-c_1 n^{1-p})-\exp(-c_2 \sqrt{n\log d}) -c_3d^{-1}$:
% \begin{align}
%     \sup_{\substack{\nu = \Omega(n^p)\\ \eta = \OOO(1)}} \left|\fnclasn(\nu,\eta) 
%     -
%     \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} - \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} \right|
%     =
%     \OOO \left( \frac{\eta^2}{\nu^3}, \rho\eta^2, \frac{\eta^3}{\nu}\epsilon_n \right) 
%     +
%     \OOO \left( \frac{1}{\nu^3}, \epsilon_c \right) 
%     % =: \OOO_{\eta}(\eta,n,\rho) + \OOO_{\nu,c}(\nu,\epsilon) 
%     % =: \OOO_{\eta} + \OOO_c
% \end{align}
% \end{proposition}
Recall that $\fnclasn(\nu,\eta):= \frac{1}{n} \sum_{i=1}^n  (1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i)_+^2$. Proposition follows straightforwardly from using triangle inequality as follows:
\begin{align}
    \bigg| \fnclasn(\nu,\eta) &- \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} - \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} \bigg|
    \leq
    \left\vert \frac{1}{n} \sum_{i=1}^n \left( \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} \right) \left(1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i\right)^2 \right\vert\\
    &+
    \left| \frac{1}{n} \sum_{i=1}^n \indicator{1-\nu\abs{\gausswone_i}} \left(1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i\right)^2 - \EE \Big[ (1-\nu \abs{\Gausswone} - \eta \Gausswtwo  )^2 \indicator{1-\nu\abs{\Gausswone}} \Big]\right|\\
    &+
    \left| \EE [ (1-\nu \abs{\Gausswone} - \eta \Gausswtwo  )^2 \indicator{1-\nu\abs{\Gausswone}} ] - \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} - \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} \right|
\end{align}
and then using the results from Lemmas~\ref{lemma_uniform_bound_diff_indicators}, \ref{lemma_uniform_conv_semiindic_noiseless} and \ref{lemma:exp_semi_indicator_noiseless} to bound each of the three terms, respectively.

% % ------------------ old lemma (before 31/08)----------------------------
% \begin{lemma}
% \label{lemma_uniform_bound_diff_indicators}
% Let $\{\gausswone_i,\gausswtwo_i\}_{i=1}^n$ be i.i.d. $\sim\NNN(0,1)$ random variables, let $\rho \asymp \sqrt{\frac{\log d}{n}}$ and let $c_1,c_2,c_3,c_4$ be some positive universal constants.% and $\gamma_m = \sqrt{\log n}$.
%  Assuming that $\nu = \Omega(1,\eta\sqrt{\log\log n})>0$ and $\eta>0$, the inequality
% \begin{align}
%     \sup_{\nu,\eta}
%     \left\vert \frac{1}{n} \sum_{i=1}^n \left( \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} \right) \left(1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i\right)^2 \right\vert
%     \lesssim
%     (\rho + \frac{\eta}{\nu}\log\log n )\eta^2
% \end{align}
% holds with probability at least $1-\exp \left( -c_1 n (\rho+\frac{\eta}{\nu}\sqrt{\log\log n}) \right) - \exp \left( -c_3\frac{n}{(\log n)^{c_2}} \right) -c_4d^{-1}$ over the draws of $\{\gausswone_i,\gausswtwo_i\}_{i=1}^n$.
% \end{lemma}
% \begin{proof}

% First consider the case $\indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i}=0$ and $\indicator{1-\nu\abs{\gausswone_i}} = 1$ indexed by some set $\III_1\subseteq [n]$. For $i\in\III_1$ we have $0\leq 1-\nu\abs{\gausswone_i} < \eta\gausswtwo_i$ implying that $\frac{1}{n} \sum_{i\in \III_1} (1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i)^2 \lesssim \frac{1}{n}\sum_{i\in \III_1} (\eta\gausswtwo_i)^2$.

% Now consider the case $\indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i}=1$ and $\indicator{1-\nu\abs{\gausswone_i}} = 0$ indexed by some set $\III_2\subseteq [n]$. Here, for $i\in\III_2$ we have $\eta\gausswtwo_i \leq 1-\nu\abs{\gausswone_i} < 0$ and using the same reasoning as above, we have $\sum_{i\in \III_2} (1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i)^2 \lesssim \sum_{i\in \III_2} (\eta \gausswtwo_i)^2$. 
% % \lesssim \frac{\card{\III_2}}{n}\eta^2$.
% Note that
% \begin{align}
%     \frac{\card{\III_1}+\card{\III_2}}{n}
%     =
%     \frac{1}{n}\sum_{i=1}^n & \left\vert \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} \right\vert,
%     \label{eq:sum_indicators_sets_proof_lemma}
% \end{align}
% so we can upper-bound the expression as follows:
% \begin{align}
%     \sup_{\nu,\eta} &
%     \left\vert \frac{1}{n} \sum_{i=1}^n \left( \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i}  -  \indicator{1-\nu\abs{\gausswone_i}} \right) \left(1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i\right)^2 \right\vert \\
%     &\leq 
%     \frac{1}{n}\sum_{i\in \III_1 \cup \III_2}  \left(1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i\right)^2
%     \lesssim
%     \frac{1}{n}\sum_{i\in \III_1 \cup \III_2} \left( \eta \gausswtwo_i \right)^2
%     % \leq
%     % \frac{\card{\III_1}+\card{\III_2}}{n} \frac{1}{\card{\III_1}+\card{\III_2}} \sum_{i\in \III_1 \cup \III_2} \left( \eta \gausswtwo_i \right)^2 
%     \leq
%     \frac{\card{\III_1}+\card{\III_2}}{n} \eta^2
%     \label{eq:diff_indicators_card_sets}
% \end{align}
% % with probability at least $1-c_1\exp(-c_2\min \{ \eta^2,\eta^4 \} (\card{\III_1}+\card{\III_2}))$.
% with probability at least $1-\exp(-c_1 (\card{\III_1}+\card{\III_2}))$.

% To bound $\card{\III_1}+\card{\III_2}$ we follow the same reasoning as in Lemma 10 in \cite{donhauser2022fast} and define $F_n(x) = \frac{1}{n}\sum_{i=1}^n \indicator{\abs{\gausswone_i}\leq x}$, $F(x) = \PP ( \abs{\Gausswone}\leq x )$. Recall that we defined $\rho \asymp \sqrt{\frac{\log d}{n}}$ and divide the sum from Equation \eqref{eq:sum_indicators_sets_proof_lemma} into two parts which we bound as follows:
% \begin{align}
%     \frac{1}{n}\sum_{i\in[n]: \abs{\gausswtwo_i}\leq \sqrt{\log\log n}} & \left\vert \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} \right\vert
%     \leq
%     F_n \left( \frac{1}{\nu}(1+\eta \sqrt{\log\log n}) \right) - F_n \left( \frac{1}{\nu} \right) \\
%     &\lesssim
%     \rho + F \left( \frac{1}{\nu}(1+\eta\sqrt{\log\log n}) \right) - F \left( \frac{1}{\nu} \right)
%     \lesssim
%     \rho + \frac{\eta}{\nu}\sqrt{\log\log n}
% \end{align}
% with probability at least $1-c_3 d^{-1}$. On the other hand, using similar reasoning as above, we get:
% \begin{align}
%     \frac{1}{n}\sum_{i\in[n]: \abs{\gausswtwo_i}\geq \sqrt{\log\log n}}  \vert &\indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} \vert \\
%     &\lesssim 
%     \frac{\card{\{i\in[n]: \abs{\gausswtwo_i}\geq \sqrt{\log\log n} \}}}{n}  \left( \rho + \frac{\eta}{\nu}\right)\sqrt{\log n} 
%     \lesssim 
%     \left(\rho + \frac{\eta}{\nu}\right)\frac{1}{\sqrt{\log n}}
% \end{align}
% where we used Claim 4 from \cite{wang2021tight} to show that $\card{\{i\in[n]: \abs{\gausswtwo_i}\geq \sqrt{\log\log n}\}} \lesssim \frac{n}{\log n}$ with probability $\geq 1 - \exp(-c_1 n/(\log n)^{c_2})$ for some universal positive constants $c_1,c_2>0$. Summing the last two obtained expressions we get an upper bound on $\card{\III_1}+\card{\III_2}$ which after substitution into Equation \eqref{eq:diff_indicators_card_sets} finishes the proof.
% \end{proof}
% % ----------------------------------------------------------------------------

\begin{lemma}
\label{lemma_uniform_bound_diff_indicators}
Let $\{\gausswone_i,\gausswtwo_i\}_{i=1}^n$ be i.i.d. $\sim\NNN(0,1)$ random variables, let $\rho \asymp \sqrt{\frac{\log d}{n}}, \epsilon_n\asymp \sqrt{\log\log n}$ and let $c_1$ be a positive universal constant.% and $\gamma_m = \sqrt{\log n}$.
Assuming that $\nu = \Omega(1,\eta\epsilon_n)>0$ and $\eta>0$, the inequality
\begin{align}
    \sup_{\nu,\eta}
    \left\vert \frac{1}{n} \sum_{i=1}^n \left( \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} \right) \left(1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i\right)^2 \right\vert
    \lesssim
    (\rho + \frac{\eta}{\nu}\epsilon_n )\epsilon_n^2 \eta^2
\end{align}
% holds with probability at least $1-\exp \left( -c_1 n (\rho+\frac{\eta}{\nu}\sqrt{\log\log n}) \right) - \exp \left( -c_3\frac{n}{(\log n)^{c_2}} \right) -c_4d^{-1}$ over the draws of $\{\gausswone_i,\gausswtwo_i\}_{i=1}^n$.
holds with probability at least $1-c_1n^{-1}$.
\end{lemma}
\begin{proof}

First consider the case $\indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i}=0$ and $\indicator{1-\nu\abs{\gausswone_i}} = 1$ indexed by some set $\III_1\subseteq [n]$. For $i\in\III_1$ we have $0\leq 1-\nu\abs{\gausswone_i} \leq \eta\gausswtwo_i$ implying that $\frac{1}{n} \sum_{i\in \III_1} (1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i)^2 \lesssim \frac{1}{n}\sum_{i\in \III_1} (\eta\gausswtwo_i)^2$.

Now consider the case $\indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i}=1$ and $\indicator{1-\nu\abs{\gausswone_i}} = 0$ indexed by some set $\III_2\subseteq [n]$. Here, for $i\in\III_2$ we have $\eta\gausswtwo_i \leq 1-\nu\abs{\gausswone_i} \leq 0$ and using the same reasoning as above, we have $\sum_{i\in \III_2} (1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i)^2 \lesssim \sum_{i\in \III_2} (\eta \gausswtwo_i)^2$. 
% \lesssim \frac{\card{\III_2}}{n}\eta^2$.
% Note that
% \begin{align}
%     \frac{\card{\III_1}+\card{\III_2}}{n}
%     =
%     \frac{1}{n}\sum_{i=1}^n & \left\vert \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} \right\vert,
%     \label{eq:sum_indicators_sets_proof_lemma}
% \end{align}
Thus we have the following upper-bound:
\begin{align}
    \sup_{\nu,\eta} 
    \bigg| \frac{1}{n} \sum_{i=1}^n ( \indicator{1-\nu\abs{\gausswone_i}-& \eta\gausswtwo_i}  -  \indicator{1-\nu\abs{\gausswone_i}} ) \left(1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i\right)^2 \bigg| \\
    &\leq 
    \sup_{\nu,\eta} \eta^2
     \frac{1}{n} \sum_{i=1}^n (\gausswtwo_i)^2 \left\vert \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i}  -  \indicator{1-\nu\abs{\gausswone_i}} \right\vert
    \label{eq:diff_indicators_card_sets}
\end{align}
% with probability at least $1-c_1\exp(-c_2\min \{ \eta^2,\eta^4 \} (\card{\III_1}+\card{\III_2}))$.

To bound the term above we follow the same reasoning as in Lemma 10 in \cite{donhauser2022fast} and define $F_n(x) = \frac{1}{n}\sum_{i=1}^n \indicator{\abs{\gausswone_i}\leq x}$, $F(x) = \PP ( \abs{\Gausswone}\leq x )$. Recall that we defined $\rho \asymp \sqrt{\frac{\log d}{n}}$, $\epsilon_n\asymp \sqrt{\log\log n}$ and let $c>0$ be an arbitrary universal constant. Now divide the sum from Equation \eqref{eq:diff_indicators_card_sets} into two parts which we bound using Dvoretzky-Kiefer-Wolfowitz inequality \cite{massart} i.e. inequality~\eqref{eq:dkw_ineq}. The first part we bound as follows:
% \begin{align}
%     \frac{1}{n}\sum_{i\in[n]: \abs{\gausswtwo_i}\leq c\sqrt{\log\log n}} & (\gausswtwo_i)^2 \vert \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} \vert\\
%     &\lesssim
%     \log\log n ( F_n \left( \frac{1}{\nu}(1+\eta \sqrt{\log\log n}) \right) - F_n \left( \frac{1}{\nu} \right) )\\
%     &\lesssim
%     \log\log n(\rho + F \left( \frac{1}{\nu}(1+\eta\sqrt{\log\log n}) \right) - F \left( \frac{1}{\nu} \right))
%     \lesssim
%     (\rho + \frac{\eta}{\nu}\sqrt{\log\log n})\log\log n
% \end{align}
\begin{align}
    \frac{1}{n}\sum_{i\in[n]: \abs{\gausswtwo_i}\leq c\epsilon_n} (\eta \gausswtwo_i)^2 \vert &\indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} \vert
    \lesssim
    \epsilon_n^2 \eta^2 ( F_n \left( \frac{1}{\nu}(1+\eta \epsilon_n) \right) - F_n \left( \frac{1}{\nu} \right) )\\
    &\lesssim
    \epsilon_n^2 \eta^2(\rho + F \left( \frac{1}{\nu}(1+\eta\epsilon_n) \right) - F \left( \frac{1}{\nu} \right))
    \lesssim
    (\rho + \frac{\eta}{\nu}\epsilon_n)\epsilon_n^2\eta^2
    \label{eq:proof_unicon_first_term_DKW}
\end{align}
with probability at least $1-c_3 d^{-1}$. Define $n':=|\{i\in[n]: \abs{\gausswtwo_i}\geq c\epsilon_n \} |$ and $\rho' \asymp \sqrt{\frac{\log d}{n'}}$. We bound the second term as follows:
% \begin{align}
%     \frac{1}{n}\sum_{i\in[n]: \abs{\gausswtwo_i}\geq c\sqrt{\log\log n}}  (\gausswtwo_i)^2 | &\indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} | \\
%     &\lesssim 
%     \frac{\card{\{i\in[n]: \abs{\gausswtwo_i}\geq c\sqrt{\log\log n} \}}}{n}  \left( \rho + \frac{\eta}{\nu}\right)(\log n)^{3/2} 
%     \lesssim 
%     \left(\rho + \frac{\eta}{\nu}\right)\frac{1}{\sqrt{\log n}}
% \end{align}
\begin{align}
    \frac{1}{n}&\sum_{i\in[n]: \abs{\gausswtwo_i}\geq c\epsilon_n}  (\eta \gausswtwo_i)^2 | \indicator{1-\nu\abs{\gausswone_i}-\eta\gausswtwo_i} - \indicator{1-\nu\abs{\gausswone_i}} | \\
    &\lesssim 
    \eta^2\frac{\log n}{n} \sum_{i=1}^{n'} | \indicator{1-\nu\abs{\gausswone_i}+\eta c_2\sqrt{\log n}} - \indicator{1-\nu\abs{\gausswone_i}} | 
    \lesssim
    \eta^2\frac{ n'\log n}{n}(\rho' + \frac{\eta}{\nu}\sqrt{\log n})
    % \\
    % &\lesssim 
    % \frac{n'}{n}  \left( \rho + \frac{\eta}{\nu}\right)(\log n)^{3/2} 
    % \lesssim 
    % \left(\rho + \frac{\eta}{\nu}\right)\frac{1}{\sqrt{\log n}}
    \label{eq:proof_lemma_unicon_second_term}
\end{align}
where in the first inequality we used that $|\gausswtwo_i|\lesssim \sqrt{\log n}$ with probability $\geq 1-c_1n^{-1}$ and the second inequality follows from the same steps as in inequality~\eqref{eq:proof_unicon_first_term_DKW}. Using the same reasoning as in the proof of Lemma~\ref{lemma:dkw_number_active_indicators} one can show that $n' \lesssim \frac{n}{(\log n)^2}$ with probability $\geq 1 -c_1 d^{-1} $. Substituting this expression for $n'$ into \eqref{eq:proof_lemma_unicon_second_term} we get that the second term is bounded by $\lesssim (\rho + \frac{\eta}{\nu}\frac{1}{\sqrt{\log n}})\eta^2$.

Summing two obtained expressions we get upper bound as claimed in the lemma.
\end{proof}

Similarly as in Section~\ref{apx:subsec:unif_conv} define a set of functions $\mathcal{G}'= \{ (\Gausswone,\Gausswtwo)\mapsto (1-\nu \abs{\Gausswone} - \eta \Gausswtwo)^2 \indicator{1-\nu\abs{\Gausswone}}\ |\nu = \Omega(n^p), \eta = O(1) \}$ and using the same notation as in the beginning of Section~\ref{apx:subsec:unif_conv} we have the following lemma:
\begin{lemma}
\label{lemma_uniform_conv_semiindic_noiseless}
Let $p, c_1,c_2$ be some universal positive constants with $p\in(0,\frac{2}{5})$. Then
% \begin{align}
%     \sup_{\substack{\nu = \Omega(n^p)\\ \eta = O(1)}}
%     \left|
%     \frac{1}{n}\sum_{i=1}^n (1-\nu \abs{\gausswone_i} - \eta \gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}}
%     -
%     \EE \left[ \left(1-\nu \abs{\Gausswone} - \eta \Gausswtwo \right )^2 \indicator{1-\nu\abs{\Gausswone}} \right] 
%     \right| \leq c_3 n^{-(1+p)/2}
% \end{align}
\begin{align}
   \PP \left(\norm{ P_n - P }_{\mathcal{G}'} \leq c_1 n^{-(1+p)/2} \right) \geq 1-c_2d^{-1}
\end{align}
% holds with probability at least $1-c_1 \exp (-c_2 n^{1-p})$.
\end{lemma}
\begin{proof}
% Define a set of functions $\mathcal{G}= \{ (\Gausswone,\Gausswtwo)\mapsto (1-\nu \abs{\Gausswone} - \eta \Gausswtwo)^2 \indicator{1-\nu\abs{\Gausswone}}\ |\nu = \Omega(n^p), \eta = O(1) \}$. 
According to symmetrization lemma (Lemma~\ref{lemma_emp_rademacher}), it is sufficient to show that the probability of the event
\begin{align}
    \norm{P_n^{\epsilon}}_{\GGG'} = \sup_{\substack{\nu = \Omega(n^p)\\ \eta = O(1)}}
    \left| \frac{1}{n}\sum_{i=1}^n \epsilon_i(1-\nu \abs{\gausswone_i} - \eta \gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}} \right|
    >
    \frac{c_1}{4} n^{-(1+p)/2}
    \label{eq:rademacher_prob_proof_lema_unicon}
\end{align}
is decaying appropriately for some constant $c_1$. We first apply triangle inequality as follows:
\begin{align}
&\left|\frac{1}{n}\sum_{i=1}^n \epsilon_i(1-\nu \abs{\gausswone_i} - \eta \gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}} \right| \\
\leq &
\left|\frac{1}{n}\sum_{i=1}^n \epsilon_i \possq{1-\nu\abs{\gausswone_i}} \right|
+ \left| \frac{1}{n}\sum_{i=1}^n 2\eta \epsilon_i (1-\nu\abs{\gausswone_i})_+ \gausswtwo_i \right|
+ \left| \frac{1}{n}\sum_{i=1}^n \eta^2 \epsilon_i (\gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}} \right|
\end{align}
and note that $0\leq \possq{1-\nu\abs{\gausswone_i}}\leq (1-\nu\abs{\gausswone_i})_+\leq 1$ for any $\nu$. Now assume that there are exactly $k$ indicators functions that are active. According to Lemma~\ref{lemma:dkw_number_active_indicators} we have $k\lesssim n^{1-p}$ with  probability $\geq 1-c_2d^{-1}$. Therefore, using the concentration of subexponential random variables and independence of $\epsilon_i,\gausswtwo_i$'s from $\gausswone_i$'s, we have:
\begin{align}
    \sup_{\substack{\nu = \Omega(n^p)\\ \eta = O(1)}}
    \left|\frac{1}{n}\sum_{i=1}^n \epsilon_i(1-\nu \abs{\gausswone_i} - \eta \gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}} \right|
    \lesssim
    \frac{\sqrt{k}}{n} \max_{\eta=O(1)} (\eta^2,1)  
    \lesssim
    n^{-(1+p)/2}
\end{align}
with probability at least $1-c_2 \exp (-c_3 n^{1-p})$ for some constants $c_1,c_2>0$. The statement of the lemma follows from the Lemma~\ref{lemma_emp_rademacher} by noting that probability of the event from Equation~\eqref{eq:rademacher_prob_proof_lema_unicon} is $\leq c_2d^{-1}$.
\end{proof}
% \begin{proof}
% Define a set of functions $\mathcal{G}= \{ (\nu,\eta)\mapsto (1-\nu \abs{\gausswone} - \eta \gausswtwo)^2 \indicator{1-\nu\abs{\gausswone}}\ |\nu = \Omega(n^p), \eta = O(1) \}$. According to symmetrization lemma (Lemma~\ref{lemma_emp_rademacher}), it is sufficient to show that the probability of the following event is decaying appropriately:
% \begin{align}
%     \sup_{\substack{\nu = \Omega(n^p)\\ \eta = O(1)}}
%     \left| \frac{1}{n}\sum_{i=1}^n \epsilon_i(1-\nu \abs{\gausswone_i} - \eta \gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}} \right|
%     >
%     \frac{c_3}{4} \frac{\log n}{n^{(1+p)/2}}
% \end{align}
% for some constant $c_3$. But now for any $\nu,\eta$ with $\nu = \Omega(n^p), \eta = O(1)$  we have:
% \begin{align}
% &\left|\frac{1}{n}\sum_{i=1}^n \epsilon_i(1-\nu \abs{\gausswone_i} - \eta \gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}} \right| \\
% \leq &
% \left|\frac{1}{n}\sum_{i=1}^n \epsilon_i \possq{1-\nu\abs{\gausswone_i}} \right|
% + \left| \frac{1}{n}\sum_{i=1}^n 2\eta \epsilon_i (1-\nu\abs{\gausswone_i})_+ \gausswtwo_i \right|
% + \left| \frac{1}{n}\sum_{i=1}^n \eta^2 \epsilon_i (\gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}} \right|
% \end{align}
% Note that $0\leq \possq{1-\nu\abs{\gausswone_i}}\leq (1-\nu\abs{\gausswone_i})_+\leq 1$. Now assume that there are exactly $k$ indicators functions that are active (note that $\epsilon_i,\gausswtwo_i$'s are independent of $\gausswone_i$'s). According to Corollary \ref{cor:cor_k_indicators} we have $k\lesssim n^{1-p} \log^2(n)$ with high probability. Therefore, using the concentration of subexponential random variables, we have:
% \begin{align}
%     \sup_{\substack{\nu = \Omega(n^p)\\ \eta = O(1)}}
%     \left|\frac{1}{n}\sum_{i=1}^n \epsilon_i(1-\nu \abs{\gausswone_i} - \eta \gausswtwo_i)^2 \indicator{1-\nu\abs{\gausswone_i}} \right|
%     \lesssim
%     \frac{\sqrt{k}}{n} \max_{\eta=O(1)} (\eta^2,1)  
%     =:
%     \frac{c_3}{4}\frac{\log n}{n^{(1+p)/2}}
% \end{align}
% with probability at least $1-\frac{c_1}{4} \exp (-c_2 n^{1-p})$ for some constants $c_1,c_2>0$. The statement of the lemma follows from the symmetrization argument as mentioned previously.
% \end{proof}

% Following the same argument as in Claim 7 and Claim 9 in \cite{wang2021tight}, we can prove the following lemma:
% \begin{lemma}
% \label{lemma_uls_ols_exp}
%     Let any fixed constant $ 0 < \mu \leq  (\log c)^{1/6} $ where by assumption $d\geq m c$ and let $\uls$ be the largest integer $s$ such that $t_s^2 \geq \tnstar^2 + \frac{\mu}{\tnstar^{1/3}}$. Then
%     \begin{align}
%         \uls = \nstar \exp \left( -\frac{ \mu }{ 2 \tnstar^{1/3}} \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
%         \andtxts
%         \left| \tuls^2 - \left( \tnstar^2 + \frac{\mu}{\tnstar^{1/3}} \right) \right| \leq O \left( \frac{1}{m} \right)
%     \end{align}
%     Moreover, let $\ols$ be the smallest integer $s$ such that $t_s^2 \leq \tnstar^2 - \frac{\mu}{\tnstar^{1/3}}$. Then,
%     \begin{align}
%         \ols = \nstar \exp \left( \frac{ \mu }{ 2 \tnstar^{1/3} } \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
%         \andtxts
%         \left| \tols^2 - \left( \tnstar^2 - \frac{\mu}{\tnstar^{1/3}} \right) \right| \leq O \left( \frac{1}{m} \right)
%     \end{align}
% \end{lemma}
%  Furthermore, analogously to the proof of Claim 8 in \cite{wang2021tight} we get:
% \begin{align}
%     \frac{\tnstar^2}{\tuls^2} 
%     =
%     \frac{1}{1 + \frac{\mu}{\tnstar^{7/3}} + O \left( \frac{1}{\tnstar^2 \nstar} \right)}
%     =
%     1 - \frac{\mu}{\tnstar^{7/3}}  + O \left( \frac{\mu^2}{\tnstar^{14/3}} \right) + O \left( \frac{1}{\tnstar^2 \nstar} \right)
% \end{align}
% Similar result holds for $\tols$.

\begin{lemma}\label{lemma:exp_semi_indicator_noiseless}
Let $\Gausswone,\Gausswtwo\sim\NNN(0,1)$ be independent, $\eta,\nu>0$ and $\nu = \Omega(1)$. Then:
\begin{align}
    \EE [ (1-\nu \abs{\Gausswone} - \eta \Gausswtwo  )^2 \indicator{1-\nu\abs{\Gausswone}} ] 
    =
    \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + \sqrt{\frac{2}{\pi}} \frac{\eta^2}{\nu} + O \left( \frac{1}{\nu^3} \right) + O \left( \frac{\eta^2}{\nu^3} \right)
\end{align}
\end{lemma}
\begin{proof}
Using the independence of $\Gausswone,\Gausswtwo$ and the fact that they have zero mean, we obtain the following:
\begin{align}
    \EE [ (1-\nu \abs{\Gausswone} - \eta \Gausswtwo  )^2 &\indicator{1-\nu\abs{\Gausswone}} ] 
    = 
    % \EE \possq{1-\nu\abs{\Gausswone}} - 2 \eta \EE [ ( 1- \nu\abs{\Gausswone} )_+ ] \EE \Gausswtwo + 
    % \\ 
    % &+ \eta^2 \EE [ \indicator{1-\nu\abs{\Gausswone}} ] \EE (\Gausswtwo)^2 
     % = 
    \eta^2 \PP ( \abs{\Gausswone} \leq \frac{1}{\nu} ) + \EE \possq{1-\nu\abs{\Gausswone}} 
    \label{eq:expect_split_nu_eta_proof}
\end{align}
% Now we can determine the last term as follows:
% \begin{align}
%     \PP \left( \abs{\Gausswone} \leq \frac{1}{\nu} \right) = 2\int_{0}^{1/\nu} \frac{1}{\sqrt{2\pi}} \exp \left( -\frac{z^2}{2} \right) dz = \frac{2}{\sqrt{\pi}} \int_{0}^{1/(\sqrt{2}\nu)} \exp \left( -t^2\right)dt = \erf \left( \frac{1}{\sqrt{2}\nu} \right)
% \end{align}
Now we consider the first term. From the definition of error function we have $\PP ( \abs{\Gausswone} \leq \frac{1}{\nu} )=\erf(\frac{1}{\sqrt{2}\nu})$. Also recall that the Taylor series approximation of the error function around zero is given by $\erf ( \frac{1}{\sqrt{2}\nu} ) =  \sqrt{\frac{2}{\pi}}\frac{1}{\nu} - \frac{1}{3\sqrt{2\pi}}\frac{1}{\nu^3} + O(\frac{1}{\nu^5})$. Thus the first term is equal to $\sqrt{\frac{2}{\pi}}\frac{\eta^2}{\nu} + O (\frac{\eta^2}{\nu^3})$.

Applying standard integration results and Taylor expansion of error function, for the second term from Equation~\eqref{eq:expect_split_nu_eta_proof}, we obtain:
\begin{align}
    \EE \possq{1-\nu\abs{\Gausswone}} 
    &=
    \frac{2}{\sqrt{2\pi}} \int_{0}^{1/\nu} (1-\nu z)^2 \exp \left( -\frac{z^2}{2} \right) dz \\
    &=
    (\nu^2+1)\erf \left( \frac{1}{\sqrt{2}\nu} \right) + \sqrt{\frac{2}{\pi}} \nu \left( \exp \left( -\frac{1}{2\nu^2} \right) -2 \right) \\
    &=
    (\nu^2+1)\frac{2}{\sqrt{\pi}} \left( \frac{1}{\sqrt{2}\nu} - \frac{1}{6\sqrt{2}\nu^3} + O \left( \frac{1}{\nu^5} \right) \right) - \sqrt{\frac{2}{\pi}}\nu \left( 1+\frac{1}{2\nu^2} + O \left( \frac{1}{\nu^4} \right) \right) \\
    &= \frac{\sqrt{2}}{3\sqrt{\pi}} \frac{1}{\nu} + O \left( \frac{1}{\nu^3} \right)
    \label{eq_exp_partial_nu_fnclasn}
\end{align}
The statement of the lemma follows after adding the obtained expressions.
\end{proof}


% \subsubsection{Auxiliary lemmas}
% % \begin{lemma}[Lemma 9 in \cite{gordon2006minimum}]
% % \label{lemma_mink_gaussian}
% % Let $z_1,\dots,z_n$ be i.i.d. $\sim \NNN(0,1)$ and assume that they are ordered such that $\abs{z_1}\leq \abs{z_2}\leq \cdots\leq \abs{z_n}$. Fix $1\leq k\leq n$ and let $a = \sqrt{\frac{2}{\pi}}e \frac{n}{k}$. Then, for every $0<t<1/a$, one has
% % \begin{align}
% %     \PP \left[ \abs{z_k} \leq t \right] \leq \frac{1}{\sqrt{2\pi k}}\frac{(at)^k}{1-at}
% % \end{align}
% % \end{lemma}

% % % \begin{corollary}
% % % \label{cor:cor_k_indicators}
% % % Let $\nu = \Omega(n^p)$ for $p\in(0,1)$ and let $\epsilon>0$ be some constant. Then $k \lesssim n^{1-p} (\log n)^{\epsilon}$ of the $n$ indicators $\indicator{1-\nu\abs{\gausswone_i}}$ are activated with probability at least $ 1 - n^{-0.5(1-p)}(\frac{1}{c_1}\log n)^{- \epsilon n^{1-p}}\geq 1 - c_3\exp(-c_4 n^{1-p})$ for any $n\geq c_2 $ with some $c_1,c_2,c_3,c_4>0$ constants.
% % % \end{corollary}
% % \begin{corollary}
% % \label{cor:cor_k_indicators}
% % Let $\nu = \Omega(n^p)$ for $p\in(0,1)$. Then $k \lesssim n^{1-p}$ of the $n$ indicators $\indicator{1-\nu\abs{\gausswone_i}}$ are activated with probability at least %$ 1 - n^{-0.5(1-p)}(\frac{1}{c_1}\log n)^{- \epsilon n^{1-p}}\geq 
% % $1 - c_2\exp(-c_3 n^{1-p})$ for any $n\geq c_1 $ with some $c_1,c_2,c_3>0$ constants.
% % \end{corollary}

% \begin{lemma}
% Let $\nu=\Omega(n^p)$ for any universal constant $p\in(0,\frac{2}{5})$. Let $k\in[0,n]$ be the the number of indicators $\indicator{1-\nu\abs{\gausswone_i}}$ which are activated. Then, under assumptions on $n,d$ from Section~\ref{}, we have:
% \begin{align}
%     k \asymp n^{1-p} 
% \end{align}
% with probability at least $1-c_1 d^{-1}$.

% \end{lemma}
% \begin{proof}
% Define $F_n(\frac{1}{\nu}) := \frac{1}{n}\sum_{i=1}^n \indicator{|\gausswone_i|\leq \frac{1}{\nu}}$ and $F(\frac{1}{\nu}) := \EE[F_n(\frac{1}{\nu})] = \PP( |\Gausswone| \leq \frac{1}{\nu} )$. Note that $k= \sum_{i=1}^n \indicator{|\gausswone_i|\leq \frac{1}{\nu}} = n F_n(\frac{1}{\nu})$. According to the Dvoretzky-Kiefer-Wolfowitz inequality \cite{massart} we have with probability at least $1-\frac{2}{d}$ that
% \begin{align}
%     \sup_\nu \left| F_n \left( \frac{1}{\nu} \right) - F\left( \frac{1}{\nu} \right) \right| \leq \sqrt{\frac{\log d}{2n}}
%     \label{eq:dkw_ineq}
% \end{align}
% For Gaussian random variables holds that $F(\frac{1}{\nu})=\erf(\frac{1}{\sqrt{2}\nu})$ by definition of error function. Using the fact $\nu = \Omega(n^p)$ and Taylor approximation of error function around zero we have that $F(\frac{1}{\nu}) \asymp \frac{1}{\nu}$. Furthermore, we have that $\sqrt{\frac{\log d}{n}} = O(n^{-2/5})$ by assumption on $d$. Thus combining this result with inequality~\eqref{eq:dkw_ineq} we obtain:
% \begin{align}
%     k = nF_n \left( \frac{1}{\nu} \right) \asymp \frac{n}{\nu} + O (n^{3/5}) \asymp n^{1-p}
% \end{align}
% \end{proof}


% % Now recall the following symmetrization lemma with probabilities:
% \begin{lemma}[Lemma 5.3.1, Empirical Process Theory]
% \label{lemma_emp_rademacher}
% Let $Z \in \ZZZ$ be a random variable and $\GGG$ a set of functions defined on $\ZZZ$. Furthermore, let $z_i$ be i.i.d. samples of $Z$ and $\epsilon_i$ be i.i.d. Rademacher random variables for $i=1,\dots,n$. Let $\delta>0$ and suppose that for all $g\in \GGG$,
% \begin{align}
%     \PP \left( \left| (P_n-P)g \right| > \frac{\delta}{2} \right) \leq \frac{1}{2}
% \end{align}
% Then
% \begin{align}
%     \PP \left( \norm{P_n-P}_{\GGG} > \delta \right) 
%     \leq
%     4\PP \left( \norm{P_n^{\epsilon}}_\GGG > \frac{\delta}{4} \right)
% \end{align}
% \end{lemma}



==> sections/theory_max_l1_classifiers.tex <==
% \section{Theory of Maximum-\texorpdfstring{$\ell_1$}{l1}-margin interpolators for classification} 
\section{Main Results}

\input{sections/subsections_theory/intro_theory}
\input{sections/subsections_theory/setting}
\input{sections/subsections_theory/main_theorems}

==> sectionsAISTATS/proof1_sketch.tex <==
% %\documentclass[main.tex]{subfiles}
% %\begin{document}

% %%%%%%%%%%%%%%%%%%%%

% \ifaistats
% \section{Proof of Theorem~\ref{thm:mainl1_class_noisy}} 
% \else
% \subsection{Proof of Theorem~\ref{thm:mainl1_class_noisy}} 
% \fi
% \label{subsec:proof_sketch_noisy_main}
% % \subfile{../sections/subsections_theory/step_path}
% In this section we present the proof of  Theorem~\ref{thm:mainl1_class_noisy}. We begin with some definitions:  $\fclas(\nu,\eta) = \EE  \fnclas \left( \nu, \eta \right)  = 
% % \EE_{\{Z^{(j)}\}_{j=0}^s \sim \NNN(0,I_{s+1})} \EE_{\xi \sim \prob(\cdot\vert Z^{(0)})}
% \EE \left( 1- \xi \nu \vert \Gausswone \vert -  \Gausswtwo \eta \right)_+^2 $ and $\nubar := \arg\min \fclas(\nu, 0)$. Further, define  
% $\fstar = \fclas(\nubar, 0)$, ${\feestar = \frac{d^2}{d^2 \eta}\vert_{(\nubar, 0)} \fclas(\nu,\eta)}$, ${\fnnstar = \frac{d^2}{d^2 \nu}\vert_{(\nubar, 0)} \fclas(\nu,\eta)}$. 
% which are all non-zero positive constants.  
% We define the constant $\kappanoise$ in Theorem~\ref{thm:mainl1_class_noisy} by:
% % \kd{stefan, we need ot check this once more}
% \begin{equation}
% \label{eq:kappanoise}
%   \kappanoise = \frac{ 2 \fstar }{\feestar \nubar^2}.
% \end{equation}
% In a first localization step, we bound $\PhiCNuni$. By proposition~\ref{prop:CGMT_application_classification}, it suffices to upper bound $\PhiCdn$, which by Proposition~\ref{prop:parametrization_class_general} can be reduced to a low dimensional stochastic optimization problem. We show:
% \begin{proposition}
% \label{prop:Rbound_noisy}
%      Let the assumptions of Theorem~\ref{thm:mainl1_class_noisy} hold.
%      Let $\tsoptn$ be given by $2\Phic(\tsoptn) = \soptn/d$ with $\soptn = n\feestar/2$. There exist universal positive constants $c_1,c_2,c_3>0$ such that
%     \begin{align} \label{PhiCdn_bound}
%         (\PhiCdn)^2 
%         \leq
%         \frac{ n \fstar }{ \tsoptn^2 } \left( 1 - \frac{ 2 }{ \tsoptn^2 } + \frac{c_1}{ \tsoptn^3 } \right) =:\loneboundclas^2
%     \end{align}
% with probability at least $ 1 - c_2 \exp \left( -c_3\frac{n}{\log^5(d/n)} \right)$
% % $ 1 - 2 \exp \left( -\frac{ c_4 n }{ \tsoptn^6 } \right) - 6 \exp \left( -\frac{\soptn}{\log^5(d/\soptn)} \right) $
% over the draws of $\Hgaussian$, $\Ggaussian$, $\matXpar$ and $\xi$.
% \end{proposition}  
% The proof of the proposition is is deferred to Appendix~\ref{subsec:proof_loc_noisy}. As described in Section~\ref{subsec:proof_sketch}, in a second uniform convergence step, we bound the constraint set $\setZeroUni$ in Equation~\eqref{eq:Gamma0_def_class_uni}:

% \begin{proposition}
% \label{prop:BoundGamma0_class_noisy}
% Let the assumptions of Theorem~\ref{thm:mainl1_class_noisy} hold and let $\setNoisyZero$ be as in Equation~\eqref{eq:Gamma0_def_class_uni} with $M$ from Proposition~\ref{prop:BoundGamma0_class_noisy}. 
% Define a set $\tsetNoisyZero$ as a set of all $(\nu,b,\alpha,\etas)$ that satisfy:
% \begin{gather} 
%     \abs{ \nu-\nubar }^2 \lesssim \frac{1}{ \log(d/\soptn)}, ~\etas^2 \lesssim  \frac{1}{\log^{5/4}(d/\soptn)} ,\\
%     % ~~\andtxt~~ 
%     \left| b^2\norm{\gamma(\alpha)}_2^2 - \frac{2\fstar}{\feestar \log(d/\soptn) } \right| \lesssim   \frac{1}{\log^{5/4}(d/\soptn)}  
%     % &~~\andtxt~~ 
% \end{gather}
% with $\soptn = n \feestar/2$.
% % Under the same conditions on $n,d$ as in Theorem~\ref{thm:mainl1_class_noisy},
% There exist universal constants $ c_1, c_2, c_3,c_4 > 0 $ such that
% % , if $ n\geq c_1 $ and $ c_2 n \leq d \leq \exp \left( c_3 n^{1/5} \right) $ then 
% $\setNoisyZero \subset \tsetNoiselessZero$
% with probability at least $1 - c_1\exp \left( -c_2  \frac{n}{\log^5(d/n)}  \right) -  c_3\exp \left( -c_4 \frac{ n }{\log n \log^{3/2}(d/n)} \right)$ over the draws of $\Hgaussian$, $\Ggaussian$, $\matXpar$ and $\xi$.
% \end{proposition}  
% The proof of the proposition is deferred to Appendix~\ref{subsec:proof_unicon_noisy} in the appendix and a proof sketch for the proposition is given below.  As a consequence, when applying Proposition~\ref{prop:parametrization_class_general} we can upper and lower bound $\PhiCdp$ and $\PhiCdm$:
% \ifaistats
% \begin{align}
%     %\max_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     \PhiCdp
%     & \leq \left[1 + \frac{\min\limits_{(b,\alpha) \in \tsetNoisyZero} ~b^2\norm{\gamma(\alpha)}_2^2 + \min\limits_{\etas \in \tsetNoisyZero} ~\etas^2}{\max\limits_{\nu \in \tsetNoisyZero}~ \nu^2}  \right]^{-1/2}\\
%     % & \leq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 -O\left( \frac{1}{\log(d/\soptn)^{1/4}} \right)\right) 
%     & \leq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 - \frac{c}{\log(d/\soptn)^{1/4}} \right) 
%     % \\
%     % & \leq 1 -  \frac{\kappanoise}{2 \log(d/ \soptn)} \left( 1 - O\left(\frac{1}{\log(d/\soptn)^{1/4}}\right) \right) \\
% \end{align}
% \else
% \begin{align}
%     \PhiCdp
%     \leq \left[1 + \frac{\min\limits_{(b,\alpha) \in \tsetNoisyZero} ~b^2\norm{\gamma(\alpha)}_2^2 + \min\limits_{\etas \in \tsetNoisyZero} ~\etas^2}{\max\limits_{\nu \in \tsetNoisyZero}~ \nu^2}  \right]^{-1/2}
%     % & \leq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 -O\left( \frac{1}{\log(d/\soptn)^{1/4}} \right)\right) 
%     \leq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 - \frac{c}{\log(d/\soptn)^{1/4}} \right) 
% \end{align}
% \fi
% % and
% \ifaistats
% \begin{align}
%     %\min_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     \PhiCdm &\geq \left[1 + \frac{\max\limits_{(b,\alpha) \in \tsetNoisyZero} ~b^2\norm{\gamma(\alpha)}_2^2 + \max\limits_{\etas \in \tsetNoisyZero} ~\etas^2}{\min\limits_{\nu \in \tsetNoisyZero}~ \nu^2}  \right]^{-1/2}\\
%      &\geq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 + \frac{c}{\log(d/\soptn)^{1/4}}\right) 
%     %  \\
%     % & \geq 1 -  \frac{ \kappanoise}{2 \log(d/ \soptn)} \left( 1 + O\left(\frac{1}{\log(d/\soptn)^{1/4}}\right) \right)
% \end{align}
% \else
% \begin{align}
%     %\min_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     \PhiCdm \geq \left[1 + \frac{\max\limits_{(b,\alpha) \in \tsetNoisyZero} ~b^2\norm{\gamma(\alpha)}_2^2 + \max\limits_{\etas \in \tsetNoisyZero} ~\etas^2}{\min\limits_{\nu \in \tsetNoisyZero}~ \nu^2}  \right]^{-1/2}
%      \geq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 + \frac{c}{\log(d/\soptn)^{1/4}}\right) 
% \end{align}
% \fi
% Where we slightly abuse the notation by writing $(b,\alpha) \in \tsetNoisyZero$ and similar for $\nu \in \tsetNoisyZero$ and $\etas \in \tsetNoisyZero$. 

% Finally the proof follows when applying Proposition~\ref{prop:CGMT_application_classification}. \qed

% \paragraph{Proof sketch for Proposition~\ref{prop:BoundGamma0_class_noisy}}
% The proof consists of three iterations where in each iteration we use a different relaxation for $\fnclas(\nu,\eta)$ in Equation~\ref{eq:Gamma0_def_class_uni} (relying on the previous steps), to obtain a tighter bound for $\Gamma$. 



% % $\tsetNoisyZero$, where each characterized by different relaxation of the first constraint of $\setZeroUni$ i.e. by approximation of the lower bound of function 




% % We now give a proof sketch for Proposition~\ref{prop:BoundGamma0_class_noisy}. 
% % The proof consists of three iterations of bounding $\tsetNoisyZero$, where each characterized by different relaxation of the first constraint of $\setZeroUni$ i.e. by approximation of the lower bound of function $\fnclas(\nu,\eta)$. By bounding variables of interest, $\nu^2,\eta^2$, we obtain tighter bounds for $\fnclas$, which in turn can be used to tighten the bounds on the variables. Moreover, we relax the second constraint 
% % % $| |\nu| \|\wgtp\|_1 - \norm{\etas}_1 | + b\norm{\gamma(\alpha)}_1 \leq \loneboundclas$
% % from definition of $\setZeroUni$ in Proposition~\ref{prop:parametrization_class_general} to $b\norm{\gamma(\alpha)}_1 \leq \loneboundclas$.

% % Now, let us give a sketch of three rounds of bounding:
% % \\
% \textbf{Bound 1:} In a first step we show that with high probability
% \begin{equation}
%     \setNoisyZero \subset \{ (\nu,b,\alpha,\etas) 
%     ~\text{s.t.}~\nu^2\lor b^2\|\gamma(\alpha)\|_2^2\lor \etas^2 = O(1) \}
% \end{equation}

% The key idea is to make use of the following uniform lower bound from   Lemma~\ref{quadratic_bound_fn} in Appendix~\ref{subsec:appendix_lower_bounds_fnclas}:
% \begin{equation}
%     \fnclas (\nu, \sqrt{b^2\norm{\gamma(\alpha)}_2^2+\etas^2}) 
%     \geq  \constnu \nu^2  + \consteta  b^2 \norm{\gamma(\alpha)}_2^2  + \consteta \etas^2.
% \end{equation} 
% We divide the first step into three substeps, where we first upper bound $b \|\gamma(\alpha)\|_2$ by relaxing  the constraints in $\setNoisyZero$ to:
% \begin{align}
%     \mathrm{on}\  \Gamma_1^{\etasc}: 
%     \begin{cases}
%     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \\ 
%     b \alpha \leq \loneboundclas  
%     \end{cases}
% \end{align}
% Because $\setNoisyZero$ is with high probability contained in $\Gamma_1^{\etasc}$,  we have
%  $\max_{(b,\alpha) \in\Gamma_1^{\etasc}} b \|\gamma(\alpha)\|_2 \geq \max_{(b,\alpha) \in\Gamma} b \|\gamma(\alpha)\|_2  $. We can bound:
% \begin{align}
%     \etasc^2 &\leq \max_{ (b,\alpha) \in \Gamma_1^{\eta} } b^2 \norm{\gamma(\alpha)}_2^2 \\
%     &\leq 
%     \max_{\alpha} \loneboundclas^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 } 
%     \subjto
%     %B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
%     \left( \frac{\loneboundclas}{\alpha}, \alpha \right) \in \Gamma_1^{\etasc} 
% \end{align}
% and note that the constraints of $\Gamma_1^{\etasc}$ are satisfied for $\frac{1}{n}\norm{H}_{\infty}^2 \geq c_{\eta} \norm{\gamma(\alpha)}_2^2$. We leverage two properties of function $\gamma(\alpha)$ - that $\alpha\mapsto \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 } $ is monotonically decreasing function and that the mentioned constraint is convex constraint in $\alpha$. Also note that by definition of $\soptn$, we know that $\alpha_{\soptn}$ satisfies given constraint. Thus we can upper bound expression above by substituting a point $\alpha\geq \alpha_{\soptn}$ which does not satisfy the given constraint.

% Using this newly established bound on $\etasc = b\norm{\gamma(\alpha)}_2$, we can similarly bound $\nu$ on the following set $\Gamma_1^{\nu}\supset \setNoisyZero$:
% \begin{align}
%     \mathrm{on}\ \Gamma_1^{\nu}:\
%     \begin{cases}
%     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 \\ b\alpha \leq \loneboundclas \\
%     b\norm{\gamma(\alpha)}_2 \leq B_{\etasc,1} 
%     \end{cases}
% \end{align}
% Using these three constraints we have:
% \begin{align} 
%     \nu^2 &\leq \frac{ \norm{H}_{\infty}^2 }{ n \constnu } \left[\max_{b,\alpha} b^2 
%     \subjto 
%     (b,\alpha)\in \Gamma_1^{\nu} \right]
%     \\
%     &= \frac{ \norm{H}_{\infty}^2 }{ n \constnu }  \left[ ~\max_{\alpha}\min\{\frac{\loneboundclas^2}{\alpha^2}, \frac{B_{\etasc,1}^2}{\norm{\gamma(\alpha)}_2^2}\} \right]
% \end{align}
% % \begin{align}
% %     \Gamma_1^{\nu} = \left\{ (\nu, b, \alpha, \etas) 
% %     \subjto
% %     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
% % \end{align}
% which then can be upper bounded by using mentioned properties of $\gamma(\alpha)$.

% Bound $\etas = O(1)$ follows exactly the same steps as the bound $\nu^2=O(1)$ above.
% % \begin{align}
% %     \mathrm{on}\ \Gamma_1^{\etas}:\ 
% %     \begin{cases}
% %     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constvarsigma \etas^2 \\
% %     b\alpha \leq \loneboundclas \\
% %     b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1}
% %     \end{cases}
% % \end{align}
% % \begin{align}
% %     \Gamma_1^{\etas} = \left\{ (\nu, b, \alpha, \etas) 
% %     \subjto
% %     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constvarsigma \etas^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
% % \end{align}

% \textbf{Bound 2:} Here we show that $\deltanu^2,\etasc^2,\etas^2 = O\left(\frac{1}{\log(d/n)}\right)$ where $\deltanu = \nu - \nubar$. Based on bounds established in the previous step, we can lower bound $\fnclas$ more tightly as shown in Lemma~\ref{lemma_quadratic_plus_fstar_bound}. Namely, we use that:
% \begin{align}
%     &\fnclas (\nu, \sqrt{b^2\norm{\gamma(\alpha)}_2^2 + \etas^2}) 
%     \geq
%     \fstar  + \tconstnu \deltanu^2 \\
%     &\hphantom{{}\fnclas (\nu, \sqrt{b^2\norm{\gamma(\alpha)}_2^2}}
%     + \tconsteta b^2\norm{\gamma(\alpha)}_2^2 
%     + \tconstvarsigma \etas^2 - \constconc, 
% \end{align}
% for a small concentration term $\constconc$. Reasoning behind the following steps is the same as in the previous bound with a few technical differences. We can find constant $B_{\etasc,2}$ such that $\eta \leq \frac{B_{\etasc,2}}{t_{\soptn}}$ on a set $\Gamma_2^{\etasc}\supset \setNoisyZero$ such that:
% \begin{align}
%     \mathrm{on}\ \Gamma_2^{\etasc}:\
%     \begin{cases}
%     \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta b^2 \norm{\gamma(\alpha)}_2^2 - \constconc\\
%     b\alpha \leq \loneboundclas
%     \end{cases}
% \end{align}
% The approach is exactly the as in the previous bound, since the obtained constraint is still convex in $\alpha$. For bounding $\deltanu$ we define a set $\Gamma_2^{\nu}\supset \setNoisyZero$ such that:
% % \begin{align}
% %     \Gamma_2^{\eta} = \left\{ (\nu, b, \alpha, \etas) 
% %     \subjto 
% %     \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta b^2 \norm{\gamma(\alpha)}_2^2 - \constconc
% %     \andtxts
% %     b\alpha \leq \loneboundclas
% %     \right\} 
% % \end{align}
% \begin{align}
%     \mathrm{on}\ \Gamma_2^{\nu}:
%     \begin{cases}
%     \frac{1}{n}b^2\norm{H}_{\infty}^2 \geq \fstar - \constconc + \tconstnu \deltanu^2\\
%     b\alpha \leq \loneboundclas \\
%     b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,2}}{\tsoptn}  
%     \end{cases}
% \end{align}
% Once again, the approach is the same as in the previous step for $\nu$, and similarly, the bound $\etas = O(\frac{1}{\log(d/n)})$ can be obtained.
% % \begin{align}
% %     \Gamma_2^{\nu} = \left\{ (\nu, b, \alpha, \etas) 
% %     \subjto
% %     \frac{1}{n}b^2\norm{H}_{\infty}^2 \geq \fstar - \constconc + \tconstnu \deltanu^2
% %     \andtxts
% %     b\alpha \leq \loneboundclas 
% %     \andtxts
% %     b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,2}}{\tsoptn}  \right\}
% % \end{align}

% \textbf{Bound 3:} Here we prove the tight bounds from the proposition. We make use of the lower bound of $\fnclas$ from
% Proposition~\ref{prop:unifConv} and claim that the following inequality holds with high probability:
% \begin{align}
%     &\fnclas (\nu, \sqrt{b^2\norm{\gamma(\alpha)}_2^2  +\etas^2}) 
%     \geq 
%     \fstar + \frac{1}{2}\feestar b^2 \norm{\gamma(\alpha)}_2^2 \\
%     &\hphantom{{}    \fnclas (\nu, \sqrt{b^2\norm{\gamma(\alpha)}_2^2}}
%     + \frac{1}{2}\fnnstar \deltanu^2 
%     + \frac{1}{2}\fssstar \etas^2 - \constconc - \otaylor
% \end{align}
% for a small concentration term $\constconc$, and a small Taylor approximation term $\otaylor$. We bound $\etasc=b\norm{\gamma(\alpha)}_2$ on a set $\Gamma_3^{\etasc}\supset \setNoisyZero$ such that:
% \begin{align}
%     \mathrm{on}\ \Gamma_3^{\etasc}:\  
%     \begin{cases}
%     \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2  -\constconc - \otaylor
%     \\
%     b\alpha \leq \loneboundclas
%     \end{cases}
% \end{align}
% The upper bound on $\etasc^2$ is obtained as described in the previous steps, while the lower bound is analogously obtained by searching for $\alpha\leq \alpha_{\soptn}$ which does not satisfy the given constraint.

% Bounding of $\etas^2$ is done on the set $\Gamma_3^{\etas}\supset \setNoisyZero$ such that: 
% \begin{align}
%     \mathrm{on}\ \Gamma_3^{\etas}:\ 
%     \begin{cases}
%     \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2 \\
%     \hspace{3cm} + \frac{1}{2} \fssstar \etas^2 -\constconc - \otaylor
%     \\
%     b\alpha \leq \loneboundclas
%     \end{cases}
% \end{align}
% Then, the bounds on $\etas^2$ follow straightforwardly from using the lower and upper bound on $\alpha$, obtained in the bounding of $\etasc^2$.














% %\end{document}

==> sectionsAISTATS/proof1_sketch_old.tex <==
% %\documentclass[main.tex]{subfiles}
% %\begin{document}

% %%%%%%%%%%%%%%%%%%%%

% \ifarx
% \subsection{Proof of Theorem~\ref{thm:mainl1_class_noisy}} 
% \else
% \subsection{Proof of Theorem~\ref{thm:mainl1_class_noisy}} 
% \fi
% \label{subsec:proof_sketch_noisy_main}
% % \subfile{../sections/subsections_theory/step_path}
% In this section we present rest of the proof of Theorem~\ref{thm:mainl1_class_noisy}. Before considering the two main steps, localization and uniform convergence, let us introduce notation specific for noisy setting.

% Define  $\fclas(\nu,\eta, \varsigma) = \EE \left[ \fnclas \left( \nu, \eta, \varsigma \right) \right] = 
% % \EE_{\{Z^{(j)}\}_{j=0}^s \sim \NNN(0,I_{s+1})} \EE_{\xi \sim \prob(\cdot\vert Z^{(0)})}
% \EE \left( 1- \xi \nu \vert Z^{(0)} \vert -  Z^{(1)}\eta - \sum_{j=2}^s Z^{(j)}\varsigma_j \right)_+^2 $ and $\nubar := \arg\min \fclas(\nu, 0, 0)$. Further, define the quantities 
% $\fstar = \fclas(\nubar, 0, 0),\feestar = \frac{d^2}{d^2 \eta}\vert_{(\nu, \eta) = (\nubar, 0, 0)} \fclas(\nu,\eta, \varsigma),\fnnstar = \frac{d^2}{d^2 \nu}\vert_{(\nu, \eta) = (\nubar, 0, 0)} \fclas(\nu,\eta, \varsigma)$.
% % \ifaistats
% % \begin{gather}
% %     \fstar = \fclas(\nubar, 0, 0),\quad
% %     \feestar = \frac{d^2}{d^2 \eta}\vert_{(\nu, \eta) = (\nubar, 0, 0)} \fclas(\nu,\eta, \varsigma),
% %     \\
% %     \fnnstar = \frac{d^2}{d^2 \nu}\vert_{(\nu, \eta) = (\nubar, 0, 0)} \fclas(\nu,\eta, \varsigma)
% % \end{gather}
% % \else
% % \begin{align}
% %     {\fstar = \fclas(\nubar, 0, 0)},\quad
% %     {\feestar = \frac{d^2}{d^2 \eta}\vert_{(\nu, \eta) = (\nubar, 0, 0)} \fclas(\nu,\eta, \varsigma)},\quad
% %     {\fnnstar = \frac{d^2}{d^2 \nu}\vert_{(\nu, \eta) = (\nubar, 0, 0)} \fclas(\nu,\eta, \varsigma)} 
% % \end{align}
% % \fi
% which are all non-zero positive constants.  
% % We now show the proof of Theorem~\ref{thm:mainl1_class_noisy} with  
% Furthermore, the constant $\kappanoise$ from statement of Theorem~\ref{thm:mainl1_class_noisy} is defined by:
% % \kd{stefan, we need ot check this once more}
% \begin{equation}
% \label{eq:kappanoise}
%   \kappanoise = \frac{ 2 \fstar }{\feestar \nubar^2}.
% \end{equation}


% \paragraph{Step 1: Localization}
% \begin{proposition}
% \label{prop:Rbound_noisy}
%      Let the assumptions of Theorem~\ref{thm:mainl1_class_noisy} hold.
%      Let $\tsoptn$ be given by $2\Phic(\tsoptn) = \soptn/d$ with $\soptn = n\feestar/2$. There exist universal positive constants $c_1,c_2>0$ such that
%     \begin{align} \label{PhiCdn_bound}
%         (\PhiCdn)^2 
%         \leq
%         \frac{ n \fstar }{ \tsoptn^2 } \left( 1 - \frac{ 2 }{ \tsoptn^2 } + \frac{c_1}{ \tsoptn^3 } \right) =:\loneboundclas^2
%     \end{align}
% with probability at least $ 1 - c_2 \exp \left( -\frac{n}{\log^5(d/n)} \right) $
% % $ 1 - 2 \exp \left( -\frac{ c_4 n }{ \tsoptn^6 } \right) - 6 \exp \left( -\frac{\soptn}{\log^5(d/\soptn)} \right) $
% over the draws of $\Hgaussian$, $\Ggaussian$, $\Xs$ and $\xi$.
% \end{proposition}  
% % \begin{proposition}
% % \label{prop:Rbound_noisy}
% %      % Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$. Furthermore assume that $\wgt$ is $s$-sparse with $s\lesssim n/\log^{5/2}(d/n)$. 
% %      Let the assumptions of Theorem~\ref{thm:mainl1_class_noisy} hold.
% %      Let $\tsoptn$ be given by $2\Phic(\tsoptn) = \soptn/d$ with $\soptn = n\feestar/2$. There exist universal positive constants $c_1,c_2,c_3,c_4,c_5>0$ such that, if $n\geq c_1$ and $c_2 n\leq d\leq \exp(c_3 n^{1/5})$ then
% %     \begin{align} \label{PhiCdn_bound}
% %         (\PhiCdn)^2 
% %         \leq
% %         \frac{ n \fstar }{ \tsoptn^2 } \left( 1 - \frac{ 2 }{ \tsoptn^2 } + \frac{c_4}{ \tsoptn^3 } \right) =:\loneboundclas^2
% %     \end{align}
% % with probability at least $ 1 - c_5 \exp \left( -\frac{n}{\log^5(d/n)} \right) $
% % % $ 1 - 2 \exp \left( -\frac{ c_4 n }{ \tsoptn^6 } \right) - 6 \exp \left( -\frac{\soptn}{\log^5(d/\soptn)} \right) $
% % over the draws of $\Hgaussian$, $\Ggaussian$, $\Xs$ and $\xi$.
% % \end{proposition}  
% Proof of the proposition is deferred to Section~\ref{subsec:proof_loc_noisy} in the appendix.

% % For the sake of clarity we recall once again definition of $\setNoisyZero$ from Equation~\eqref{eq:Gamma0_def_class_noisy}:
% % \ifaistats
% % \begin{align}
% %     \setNoisyZero = \Big\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  &b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2, \varsigma) 
% %     \\ &~~\andtxt~~  b\norm{\gamma(\alpha)}_1 \leq \loneboundclas \Big\}.
% % \end{align}
% % \else
% % \begin{align}
% %     \setNoisyZero = \left\{ (\nu, b, \alpha, \varsigma) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2, \varsigma) ~~\andtxt~~  b\norm{\gamma(\alpha)}_1 \leq \loneboundclas \right\}.
% % \end{align}
% % \fi






% \paragraph{Step 2: Uniform Convergence}



% We can bound uniformly all elements of this set as we show in the following result:
% % \begin{proposition}
% % \label{prop:BoundGamma0_class_noisy}
% %     Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
% % Under the same conditions on $n,d$ as in Theorem~\ref{thm:mainl1_class_noisy},
% % there exist universal constants $ c_1, c_2, c_3, c_4 > 0 $ such that, if $ n\geq c_1 $ and $ c_2 n \leq d \leq \exp \left( c_3 n^{1/5} \right) $, then
% % \begin{align}
% %     \setNoisyZero 
% %     \subset
% %     \bigg\{ (\nu, b, \alpha, \varsigma) &\subjto  
% %     \left| \eta^2 - \frac{2\fstar}{\feestar \log(d/\soptn) } \right| =   O \left( \frac{1}{\log^{5/4}(d/\soptn)} \right) \\
% %     &~~\andtxt~~ 
% %     \deltanu^2 = \abs{ \nu-\nubar }^2 = O \left( \frac{1}{ \log(d/\soptn)} \right) 
% %     ~~\andtxt~~ 
% %     \norm{\varsigma}_2^2 = O \left( \frac{1}{\log^{5/4}(d/\soptn)} \right)
% %     \bigg\} =: \tilde{\Gamma}
% %     % \frac{2 \fstar \lambda}{\fnstar}\frac{1}{\log(d/n)^{5/4}} \left( 1 + O \left( \frac{1}{\log(d/n)^{1/4}} \right) \right) \} %
% % \end{align}
% \begin{proposition}
% \label{prop:BoundGamma0_class_noisy}
% Let the assumptions of Theorem~\ref{thm:mainl1_class_noisy} hold.
% % Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
% Define a set $\tilde{\Gamma}$ as a set of all $(\nu,b,\alpha,\varsigma)$ that satisfy:
% \begin{gather} 
%     \left| \eta^2 - \frac{2\fstar}{\feestar \log(d/\soptn) } \right| =   O \left( \frac{1}{\log^{5/4}(d/\soptn)} \right) \\
%     % &~~\andtxt~~ 
%     \deltanu^2 = \abs{ \nu-\nubar }^2 = O \left( \frac{1}{ \log(d/\soptn)} \right) \\
%     % ~~\andtxt~~ 
%     \norm{\varsigma}_2^2 = O \left( \frac{1}{\log^{5/4}(d/\soptn)} \right)
% \end{gather}
% with $\soptn = n \feestar/2$.
% % Under the same conditions on $n,d$ as in Theorem~\ref{thm:mainl1_class_noisy},
% There exist universal constants $ c_1, c_2 > 0 $ such that
% % , if $ n\geq c_1 $ and $ c_2 n \leq d \leq \exp \left( c_3 n^{1/5} \right) $ then 
% $\setNoisyZero \subset \tilde{\Gamma}$
% with probability at least $1 - \exp \left( -c_1  \frac{n}{\log^6(d/n)}  \right) -  \exp \left( -c_2 \frac{ n }{s\log (ns) \log^3(d/n)} \right)$ over the draws of $\Hgaussian$, $\Ggaussian$, $\Xs$ and $\xi$.
% \end{proposition}  
% Proof sketch of this proposition is given next, while the proof is deferred to Section~\ref{subsec:proof_unicon_noisy} in the appendix. 

% From the Propositions \ref{prop:parametrization_class_general}, \ref{prop:BoundGamma0_class_noisy} and using trivial bound $\norm{\varsigma}_2\geq 0$, we get the following high probability bounds on $\PhiCdp$ and $\PhiCdm$:
% \ifaistats
% \begin{align}
%     %\max_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     \PhiCdp
%     & \leq \left(1 + \frac{\min_{\eta \in \tilde{\Gamma}} ~\eta^2 + \min_{\varsigma \in \tilde{\Gamma}} ~\norm{\varsigma}_2^2}{\max_{\nu \in \tilde{\Gamma}}~ \nu^2}  \right)^{-1/2}\\
%     % & \leq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 -O\left( \frac{1}{\log(d/\soptn)^{1/4}} \right)\right) 
%     & \leq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 - \frac{c_1}{\log(d/\soptn)^{1/4}} )\right) 
%     % \\
%     % & \leq 1 -  \frac{\kappanoise}{2 \log(d/ \soptn)} \left( 1 - O\left(\frac{1}{\log(d/\soptn)^{1/4}}\right) \right) \\
% \end{align}
% \else
% \begin{align}
%     %\max_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     \PhiCdp
%     & \leq \left(1 + \frac{\min_{\eta \in \tilde{\Gamma}} ~\eta^2 + \min_{\varsigma \in \tilde{\Gamma}} ~\norm{\varsigma}_2^2}{\max_{\nu \in \tilde{\Gamma}}~ \nu^2}  \right)^{-1/2}
%      \leq 1 - \frac{ \fstar }{ \feestar (\nubar)^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 -O\left( \frac{1}{\log(d/\soptn)^{1/4}} \right)\right) \\
%     % & \leq 1 -  \frac{\kappanoise}{2 \log(d/ \soptn)} \left( 1 - O\left(\frac{1}{\log(d/\soptn)^{1/4}}\right) \right) 
%     & \leq 1 -  \frac{\kappanoise}{2 \log(d/ \soptn)} \left( 1 - \frac{c_1}{\log(d/\soptn)^{1/4}} \right) 
% \end{align}
% \fi
% % and
% \ifaistats
% \begin{align}
%     %\min_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     \PhiCdm &\geq \left(1 + \frac{\max_{\eta \in \tilde{\Gamma}} ~\eta^2 + \max_{\varsigma \in \tilde{\Gamma}} ~\norm{\varsigma}_2^2 }{\min_{\nu \in \tilde{\Gamma}}~ \nu^2}  \right)^{-1/2}\\
%      &\geq 1 - \frac{ \fstar }{ \feestar (\nubar)^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 + \frac{c_1}{\log(d/\soptn)^{1/4}}\right) 
%     %  \\
%     % & \geq 1 -  \frac{ \kappanoise}{2 \log(d/ \soptn)} \left( 1 + O\left(\frac{1}{\log(d/\soptn)^{1/4}}\right) \right)
% \end{align}
% \else
% \begin{align}
%     %\min_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     \PhiCdm &\geq \left(1 + \frac{\max_{\eta \in \tilde{\Gamma}} ~\eta^2 + \max_{\varsigma \in \tilde{\Gamma}} ~\norm{\varsigma}_2^2 }{\min_{\nu \in \tilde{\Gamma}}~ \nu^2}  \right)^{-1/2}
%      \geq 1 - \frac{ \fstar }{ \feestar (\nubar)^2 } \frac{1}{ \log(d/ \soptn)} \left( 1 +O\left( \frac{1}{\log(d/\soptn)^{1/4}}\right) \right)\\
%     & \geq 1 -  \frac{ \kappanoise}{2 \log(d/ \soptn)} \left( 1 + O\left(\frac{1}{\log(d/\soptn)^{1/4}}\right) \right)
% \end{align}
% \fi
% \begin{proof}[Proof sketch for Proposition~\ref{prop:BoundGamma0_class_noisy}]
% The proof consists of three iterations of bounding, each characterized by different relaxation of the first constraint of $\setZeroUni$ i.e. by approximation of the lower bound of function $\fnclas(\nu,b\norm{\gamma(\alpha)}_2,\varsigma)$. By bounding variables of interest, $\nu^2,\eta^2,\norm{\varsigma}_2^2$, we obtain tighter bounds for $\fnclas$, which in turn can be used to tighten the bounds on the variables. Moreover, we relax the second constraint 
% % $| |\nu| \|\wgtp\|_1 - \norm{\varsigma}_1 | + b\norm{\gamma(\alpha)}_1 \leq \loneboundclas$
% from definition of $\setZeroUni$ in Proposition~\ref{prop:parametrization_class_general} to $b\norm{\gamma(\alpha)}_1 \leq \loneboundclas$.

% Now, let us give a sketch of three rounds of bounding:
% \\
% \textbf{Bound 1:} In this step we show that $\nu^2,\eta^2, \norm{\varsigma}_2^2 = O(1)$ with high probability for $(\nu,b,\alpha,\varsigma)\in\setNoisyZero$. We show these bounds using the following lower bound of $\fnclas$ from Lemma~\ref{quadratic_bound_fn}:
% \begin{equation}
%     \fnclas (\nu, b\norm{\gamma(\alpha)}_2,\varsigma) 
%     \geq  \constnu \nu^2  + \consteta  b^2 \norm{\gamma(\alpha)}_2^2  + \constvarsigma \norm{\varsigma}_2^2.
% \end{equation} 
% First we obtain bound $\eta^2=O(1)$, more precisely we show that $\eta \leq B_{\eta,1}$ for some universal positive constant $B_{\eta,1}$. Using proposed lower bound for $\fnclas$ we can relax constraints from $\setNoisyZero$ and define a set $\Gamma_1^{\eta}\supset \setNoisyZero$ such that:
% \begin{align}
%     \mathrm{on}\  \Gamma_1^{\eta}: 
%     \begin{cases}
%     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \\ 
%     b \alpha \leq \loneboundclas  
%     \end{cases}
% \end{align}
% % \begin{align}
% %     \Gamma_1^{\eta}= \{ (\nu, b, \alpha, \varsigma) \subjto
% %     \begin{cases}
% %     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \\ 
% %     b \alpha \leq \loneboundclas  
% %     \end{cases}
% %     \}
% % \end{align}
% Because of the inclusion of $\setNoisyZero$ inside of $\Gamma_1^{\eta}$ showing upper bound on $\Gamma_1^{\eta}$ gives a valid upper bound on $\setNoisyZero$ as well. Now we bound $\eta^2$ by:
% \begin{align}
%     \eta^2 &\leq \left[\max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto (b,\alpha) \in \Gamma_1^{\eta} \right]
%     \\&=  \left[
%     \max_{\alpha} \loneboundclas^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 } 
%     \subjto
%     %B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
%     \left( \frac{\loneboundclas}{\alpha}, \alpha \right) \in \Gamma_1^{\eta} \right]
% \end{align}
% and note that the constraints of $\Gamma_1^n$ are satisfied for $\frac{1}{n}\norm{H}_{\infty}^2 \geq c_{\eta} \norm{\gamma(\alpha)}_2^2$. We leverage two properties of function $\gamma(\alpha)$ - that $\alpha\mapsto \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 } $ is monotonically decreasing function and that the mentioned constraint is convex constraint in $\alpha$. Also note that by definition of $\soptn$, we know that $\alpha_{\soptn}$ satisfies given constraint. Thus we can upper bound expression above by substituting a point $\alpha\geq \alpha_{\soptn}$ which does not satisfy the given constraint.

% Using this newly established bound on $\eta$, we can similarly bound $\nu$ on the following set $\Gamma_1^{\nu}\supset \setNoisyZero$:
% \begin{align}
%     \mathrm{on}\ \Gamma_1^{\nu}:\
%     \begin{cases}
%     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 \\ b\alpha \leq \loneboundclas \\
%     b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} 
%     \end{cases}
% \end{align}
% Using these three constraints we have:
% \begin{align} 
%     \nu^2 &\leq \frac{ \norm{H}_{\infty}^2 }{ n \constnu } \left[\max_{b,\alpha} b^2 
%     \subjto 
%     (b,\alpha)\in \Gamma_1^{\nu} \right]
%     \\
%     &= \frac{ \norm{H}_{\infty}^2 }{ n \constnu }  \left[ ~\max_{\alpha}\min\{\frac{\loneboundclas^2}{\alpha^2}, \frac{B_{\eta,1}^2}{\norm{\gamma(\alpha)}_2^2}\} \right]
% \end{align}
% % \begin{align}
% %     \Gamma_1^{\nu} = \left\{ (\nu, b, \alpha, \varsigma) 
% %     \subjto
% %     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
% % \end{align}
% which then can be upper bounded by using mentioned properties of $\gamma(\alpha)$.

% Bound $\norm{\varsigma}_2 = O(1)$ follows exactly the same steps as the bound $\nu^2=O(1)$ above.
% % \begin{align}
% %     \mathrm{on}\ \Gamma_1^{\varsigma}:\ 
% %     \begin{cases}
% %     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constvarsigma \norm{\varsigma}_2^2 \\
% %     b\alpha \leq \loneboundclas \\
% %     b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1}
% %     \end{cases}
% % \end{align}
% % \begin{align}
% %     \Gamma_1^{\varsigma} = \left\{ (\nu, b, \alpha, \varsigma) 
% %     \subjto
% %     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constvarsigma \norm{\varsigma}_2^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
% % \end{align}

% \textbf{Bound 2:} Here we show that $\deltanu^2,\eta^2,\norm{\varsigma}_2^2 = O\left(\frac{1}{\log(d/n)}\right)$ where $\deltanu = |\nu - \nubar|$. Based on bounds established in the previous step, we can lower bound $\fnclas$ more tightly as shown in Lemma~\ref{lemma_quadratic_plus_fstar_bound}. Namely, we use that:
% \begin{align}
%     \fnclas (\nu, b\norm{\gamma(\alpha)}_2,\varsigma) 
%     \geq
%     \fstar  &+ \tconstnu \deltanu^2 + \tconsteta b^2\norm{\gamma(\alpha)}_2^2 \\
%     &+ \tconstvarsigma \norm{\varsigma}_2^2 - \constconc, 
% \end{align}
% for a small concentration term $\constconc$. Reasoning behind the following steps is the same as in the previous bound with a few technical differences. We can find constant $B_{\eta,2}$ such that $\eta \leq \frac{B_{\eta,2}}{t_{\soptn}}$ on a set $\Gamma_2^{\eta}\supset \setNoisyZero$ such that:
% \begin{align}
%     \mathrm{on}\ \Gamma_2^{\eta}:\
%     \begin{cases}
%     \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta b^2 \norm{\gamma(\alpha)}_2^2 - \constconc\\
%     b\alpha \leq \loneboundclas
%     \end{cases}
% \end{align}
% The approach is exactly the as in the previous bound, since the obtained constraint is still convex in $\alpha$. For bounding $\deltanu$ we define a set $\Gamma_2^{\nu}\supset \setNoisyZero$ such that:
% % \begin{align}
% %     \Gamma_2^{\eta} = \left\{ (\nu, b, \alpha, \varsigma) 
% %     \subjto 
% %     \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta b^2 \norm{\gamma(\alpha)}_2^2 - \constconc
% %     \andtxts
% %     b\alpha \leq \loneboundclas
% %     \right\} 
% % \end{align}
% \begin{align}
%     \mathrm{on}\ \Gamma_2^{\nu}:
%     \begin{cases}
%     \frac{1}{n}b^2\norm{H}_{\infty}^2 \geq \fstar - \constconc + \tconstnu \deltanu^2\\
%     b\alpha \leq \loneboundclas \\
%     b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,2}}{\tsoptn}  
%     \end{cases}
% \end{align}
% Once again, the approach is the same as in the previous step for $\nu$, and similarly, the bound $\norm{\varsigma}_2 = O(\frac{1}{\log(d/n)})$ can be obtained.
% % \begin{align}
% %     \Gamma_2^{\nu} = \left\{ (\nu, b, \alpha, \varsigma) 
% %     \subjto
% %     \frac{1}{n}b^2\norm{H}_{\infty}^2 \geq \fstar - \constconc + \tconstnu \deltanu^2
% %     \andtxts
% %     b\alpha \leq \loneboundclas 
% %     \andtxts
% %     b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,2}}{\tsoptn}  \right\}
% % \end{align}

% \textbf{Bound 3:} Here we prove the tight bounds from the proposition. We make use of the lower bound of $\fnclas$ from
% Proposition~\ref{prop:unifConv} and claim that the following inequality holds with high probability:
% \begin{align}
%     \fnclas (\nu, b\norm{\gamma(\alpha)}_2,\varsigma) 
%     \geq 
%     \fstar &+ \frac{1}{2}\feestar b^2 \norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnnstar \deltanu^2 \\
%     &+ \frac{1}{2}\fssstar \norm{\varsigma}_2^2 - \constconc - \otaylor
% \end{align}
% for a small concentration term $\constconc$, and a small Taylor approximation term $\otaylor$. We bound $\eta$ on a set $\Gamma_3^{\eta}\supset \setNoisyZero$ such that:
% \begin{align}
%     \mathrm{on}\ \Gamma_3^{\eta}:\  
%     \begin{cases}
%     \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2  -\constconc - \otaylor
%     \\
%     b\alpha \leq \loneboundclas
%     \end{cases}
% \end{align}
% The upper bound on $\eta^2$ is obtained as described in the previous steps, while the lower bound is analogously obtained by searching for $\alpha\leq \alpha_{\soptn}$ which does not satisfy the given constraint.

% Bounding of $\norm{\varsigma}_2^2$ is done on the set $\Gamma_3^{\varsigma}\supset \setNoisyZero$ such that: 
% \begin{align}
%     \mathrm{on}\ \Gamma_3^{\varsigma}:\ 
%     \begin{cases}
%     \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2 \\
%     \hspace{3cm} + \frac{1}{2} \fssstar \norm{\varsigma}_2^2 -\constconc - \otaylor
%     \\
%     b\alpha \leq \loneboundclas
%     \end{cases}
% \end{align}
% Then, the bounds on $\norm{\varsigma}_2^2$ follow straightforwardly from using the lower and upper bound on $\alpha$, obtained in the bounding of $\eta^2$.

% \end{proof}














% %\end{document}

==> sectionsAISTATS/proof2_sketch_old.tex <==
\subsection{Proof of Theorem~\ref{thm:mainl1_class_noiseless}} 
\label{subsec:proof_sketch_noiseless_main}

Similarly to Equation~\eqref{eq:fnclas_def_noisy_par} we define function $\fnclasn:\RR\times\RR_+\times\RR^s \to \RR_+$ as follows:
\begin{align}
    \fnclasn(\nu,\eta,\varsigma):= \frac{1}{n}\sum_{i=1}^n ( 1 - \nu |\gausswone_i| - \eta \gausswtwo_i - \sum_{j=2}^s \gausswj_i \varsigma_j )_+^2
\end{align}

\paragraph{Step 1: Localization}
\begin{proposition}
\label{prop:localization_noiseless_ssparse}
Let the assumptions of Theorem~\ref{thm:mainl1_class_noiseless} hold.
Let $\sopt := 2(\frac{3}{\pi})^{1/3} \norm{\wgt}_1^{2/3}  (n t_{n^{2/3}})^{2/3}$, $\kappam = 3(72\pi)^{-1/6}$ and $\epsilon_n \asymp \sqrt{\log\log n}$. There exists universal positive constants $c_1,c_2$ such that
\begin{align}
\label{eq_loneboundclasn_def}
    \PhiCndn 
    \leq
    \kappam
    \Big( &\frac{n}{\tsopt^2} \norm{\wgt}_1 \Big)^{1/3}\\
    & \cdot \left( 1 - \frac{2}{3}\frac{1}{\tsopt^2} + c_2 \frac{\epsilon_n^3}{\tsopt^3} \right)
    =:
    \loneboundclasn 
\end{align}
holds with probability at least $1-c_1 n^{-1}$ over the draws of $\Hgaussian$, $\Ggaussian$ and $\Xs$. 
\end{proposition}
Proof of the proposition is deferred to Section~\ref{sec:proof_loc_noiseless} in the appendix.

\paragraph{Step 2: Uniform Convergence}
\begin{proposition}
\label{prop:BoundGamma0_class_noiseless}
Let the assumptions of Theorem~\ref{thm:mainl1_class_noiseless} hold. Let $\tsetNoiselessZero$ be a set of all $(\nu,b,\alpha,\varsigma)$ that satisfy:
% Let the data distribution be as described in Section~\ref{subsec:clasetting}. Under the same conditions on $n,d$ as in Theorem~\ref{thm:mainl1_class_noiseless}, there exist universal constants $ c_1, c_2, c_3, c_4 > 0 $ such that, if $ n\geq c_1 $ and $ c_2 n \leq d \leq \exp \left( c_3 n^{1/5} \right) $, then
% \begin{align}
%     \setNoiselessZero 
%     \subset
%     \Bigg\{ (\nu, b, \alpha, \varsigma) \subjto  
%     &\left| \eta^2 - \frac{1}{3}\frac{1}{\log(d/\sopt)} \right| =   O \left( \frac{1}{\log^{7/6}(d/\sopt)} \right)  
%     ~~\andtxt~~ 
%     \norm{\varsigma}_2^2 = O \left( \frac{1}{\log^{7/6}(d/\sopt)} \right) \\ 
%     &~~\andtxt~~ 
%     % \left| \nu^2- \left( \frac{1}{12\sqrt{2\pi}} \frac{n}{\norm{\wgt}_1^2 \log(d/\sopt)} \right)^{2/3} \right|  
%     \left| \nu^2-  \frac{1}{(288\pi)^{1/3}} \frac{n^{2/3}}{\norm{\wgt}_1^{4/3} \log^{2/3}(d/\sopt)}  \right| 
%     = O \left( \frac{n^{2/3}}{ \norm{\wgt}_1^{4/3} \log(d/\sopt)} \right) \Bigg\} =: \tsetNoiselessZero
% \end{align}
\begin{gather}
    \left| \eta^2 - \frac{1}{3}\frac{1}{\log(d/\sopt)} \right| =   O \left( \frac{1}{\log^{7/6}(d/\sopt)} \right)  \\
    \norm{\varsigma}_2^2 = O \left( \frac{1}{\log^{7/6}(d/\sopt)} \right) \\ 
    % \left| \nu^2-  \frac{1}{(288\pi)^{1/3}} \frac{n^{2/3}}{\norm{\wgt}_1^{4/3} \log^{2/3}(d/\sopt)}  \right| 
    % = O \left( \frac{n^{2/3}}{ \norm{\wgt}_1^{4/3} \log(d/\sopt)} \right) 
    \left| \nu^2-   \frac{(288\pi)^{-1/3} n^{2/3}  } {\norm{\wgt}_1^{4/3} \log^{2/3}(d/\sopt)}  \right| 
    = O \left( \frac{n^{2/3}}{ \norm{\wgt}_1^{4/3} \log(d/\sopt)} \right) 
\end{gather}
with $\sopt = 2(\frac{3}{\pi})^{1/3} \norm{\wgt}_1^{2/3} (n t_{n^{2/3}})^{2/3}$. Then there exists positive universal constant $c_1$ such that $\setNoiselessZero\subset \tsetNoiselessZero$ with probability at least $ 1 -  c_1n^{-1}$ over the draws of $\Hgaussian$, $\Ggaussian$ and $\Xs$.
\end{proposition}  
Proof sketch of this proposition is given next, while the proof is deferred to Section~\ref{sec:proof_unicon_noiseless} in the appendix. 

From the Propositions \ref{prop:parametrization_class_general} and \ref{prop:BoundGamma0_class_noiseless} and using that $\norm{\varsigma}_2^2 \geq 0$, we get the following bounds on $\PhiCndp$ and $\PhiCndm$:
\ifaistats
\begin{align}
    \PhiCndp
    &\leq
    \left(1 + \frac{\min_{\eta \in \tsetNoiselessZero} ~\eta^2 + \min_{\varsigma \in \tsetNoiselessZero} ~\norm{\varsigma}_2^2}{\max_{\nu \in \tsetNoiselessZero}~ \nu^2}  \right)^{-1/2}\\
    &\leq
    1 - \frac{4\norm{\wgt}_1^2}{\sopt}\left( 1 - O \left( \frac{1}{\log^{1/6}(d/\sopt)} \right) \right)
\end{align}
\else
\begin{align}
    \PhiCndp
    &\leq
    \left(1 + \frac{\min_{\eta \in \tsetNoiselessZero} ~\eta^2 + \min_{\varsigma \in \tsetNoiselessZero} ~\norm{\varsigma}_2^2}{\max_{\nu \in \tsetNoiselessZero}~ \nu^2}  \right)^{-1/2}
    \leq
    1 - \frac{4\norm{\wgt}_1^2}{\sopt}\left( 1 - O \left( \frac{1}{\log^{1/6}(d/\sopt)} \right) \right)
\end{align}
\fi

\ifaistats
\begin{align}
    \PhiCndm 
    &\geq
    \left(1 + \frac{\max_{\eta \in \tsetNoiselessZero} ~\eta^2 + \max_{\varsigma \in \tsetNoiselessZero} ~\norm{\varsigma}_2^2}{\min_{\nu \in \tsetNoiselessZero}~ \nu^2}  \right)^{-1/2}\\
    &\geq
    1 - \frac{4\norm{\wgt}_1^2}{\sopt}\left( 1 + O \left( \frac{1}{\log^{1/6}(d/\sopt)} \right) \right)
\end{align}
\else
\begin{align}
    \PhiCndm &\geq \left(1 + \frac{\max_{\eta \in \tsetNoiselessZero} ~\eta^2 + \max_{\varsigma \in \tsetNoiselessZero} ~\norm{\varsigma}_2^2}{\min_{\nu \in \tsetNoiselessZero}~ \nu^2}  \right)^{-1/2}
    \geq
    1 - \frac{4\norm{\wgt}_1^2}{\sopt}\left( 1 + O \left( \frac{1}{\log^{1/6}(d/\sopt)} \right) \right)
\end{align}
\fi

% \input{../sections/subsections_theory/noiseless/unicon_sketch.tex}

\begin{proof}[Proof sketch for Proposition~\ref{prop:BoundGamma0_class_noiseless}]


\end{proof}
